Resource Usage Analysis for the Pi-Calculus

We propose a type-based resource usage analysis for the &#960;-calculus extended with resource creation/access primitives. The goal of the resource usage analysis is to statically check that a program accesses resources such as files and memory in a valid manner. Our type system is an extension of previous behavioral type systems for the &#960;-calculus, and can guarantee the safety property that no invalid access is performed, as well as the property that necessary accesses (such as the close operation for a file) are eventually performed unless the program diverges. A sound type inference algorithm for the type system is also developed to free the programmer from the burden of writing complex type annotations. Based on the algorithm, we have implemented a prototype resource usage analyzer for the &#960;-calculus. To the authors' knowledge, ours is the first type-based resource usage analysis that deals with an expressive concurrent language like the pi-calculus.

==> Abstract.tex <==
\begin{abstract}

We propose a type-based resource usage analysis for the
\(\pi\)-calculus extended with resource creation/access primitives.
The goal of the resource usage analysis is to statically check that a
program accesses resources such as files and memory in a valid manner.
Our type system is an extension of previous behavioral type systems
for the \(\pi\)-calculus. It can guarantee the safety property that no
invalid access is performed, as well as the property that necessary
accesses (such as the close operation for a file) are eventually
performed unless the program diverges.  A sound type inference
algorithm for the type system is also developed to free the programmer
from the burden of writing complex type annotations.  Based on our
algorithm, we have implemented a prototype resource usage analyzer for
the $\pi$-calculus.  To the authors' knowledge, this is the first
type-based resource usage analysis that deals with an expressive
concurrent language like the $\pi$-calculus.
\end{abstract}


==> Ack.tex <==
\subsection*{Acknowledgments}
We would like to thank Andrew Gordon, Jakob Rehof, Atsushi Igarashi
and Eijiro Sumii for useful discussions and comments.
We would also like to thank
anonymous referees for useful comments and suggestions.
%%%, and anonymous referees of POPL 2001 


==> AlgorithmPT.tex <==
\section{The Algorithm PT}
\label{sec:PT}
The typing rules presented in Section~\ref{sec:typing} can be transformed to
the syntax-directed typing rules shown in Figure~\ref{fig:sd-typing}.
In the figure, \(\Gamma_1\TEcup \Gamma_2\) is the type environment obtained by merging
both bindings, and defined only if
\(\Gamma_1(x)=\Gamma_2(x)\) for every \(x\in\dom(\Gamma_1)\cap \dom(\Gamma_2)\).
Type equality here is syntactic equality up to $\alpha$-renaming.
And \(\WF(\Gamma_1\cup \Gamma_2)\) means that \(\Gamma_1\cup \Gamma_2\) is well-defined.
The two sets of typing rules are equivalent in the following sense:
If \(\tjudge{\Gamma}{P}{A}\) is derivable,
then there exists \(A'\) such that \(A'\newsubtype A\) holds
and \(\sdtjudge{\Gamma}{P}{A'}\) is derivable. Conversely,
 if \(\sdtjudge{\Gamma}{P}{A}\) is derivable, so is \(\tjudge{\Gamma}{P}{A}\).
%Actually, this step 1 is fairly standard so that I even wonder if
%we should Theorem 4.1 as a theorem. If we run out of the space,
%some or most of the material here could be moved to Appendix.

\input{SyntaxDirectedTyping}

Based on the syntax-directed rules, we obtain the algorithm in
Figure~\ref{fig:algorithm-PT}, which takes a process \(P\) and outputs a triple
consisting of a type environment \(\Gamma\), a behavioral type \(A\), and
a set \(C\) of constraints.
In the figure, \(\Gamma_1\Tcup \cdots \Tcup \Gamma_n\) is defined to be
\((\Gamma, C)\) where \(\Gamma\) and \(C\) are given by:
\[
\begin{array}{l}
\dom(\Gamma) = \dom(\Gamma_1)\cup \cdots \cup \dom(\Gamma_n)\\
\Gamma(x) = \Gamma_i(x) \mbox{ where $x\in \dom(\Gamma_i)\setdif
   (\dom(\Gamma_1)\cup \cdots\cup \dom(\Gamma_{i-1}))$}\\
C = \set{\Gamma_i(x)=\Gamma_j(x) \mid x\in \dom(\Gamma_i)\cap \dom(\Gamma_j)}
\end{array}
\]

\iftwocol
\begin{figure}[tbp]
\else
\begin{figure}[tbp]
\fi
\begin{center}
\fbox{
\begin{minipage}{\figwidth}
\begin{tabbing}
\(\PTv(x) = \) \= \((x\COL\Tvvar, \Tvvar)\) (where $\Tvvar$ fresh)\\
\(\PTv(b) = \) \> \((\emptyset, \Tbool)\) \mbox{ if $b\in \set{\TRUE,\FALSE}$}\\
\rulesp{}\\
\( \PT(\zeroexp) = \)\= \((\emptyset, \Tzero, \emptyset) \)  \\
\( \PT(\outexp{x}{\seq{v}}{}P_0) = \) \\ \>
\(    \PLET\)\= \((\Gamma_i, \mvtype_i) = \PTv(v_i) \) \\ \> \>
                \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
\(    (\Gamma, C) = \Gamma_0 \Tcup (x\COL\Tchan{(\seq{y}\COL{}\seq{\mvtype})\Tbvar})\Tcup
    \Gamma_1\Tcup \cdots \Tcup \Gamma_n\) \\ \>
\(\PIN (\Gamma, \Tout{x}(\Tsubst{\Tbvar}{\seq{y}}{\seq{v}}\PAR A_0), C)\)
 (where $\Tbvar$ fresh)\\
\( \PT(\inexp{x}{\seq{y}}{}P_0) = \) \\ \>
\(    \PLET\)\= \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
  \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tchan{(\seq{y}\COL{}\seq{\Tvvar})\Tbvar})
            \Tcup (\seq{y}\COL\seq{\Tvvar})\)\\ \>
\(\PIN (\Gamma\setdif{\seq{y}}, \Tin{x}{\exclude{A_0}{\set{\seq{y}}}},
        C_0\cup C_1 \cup \set{\Tbvar\subtype \project{A_0}{\set{\seq{y}}}})\)\\ \> \>
  (where $\Tbvar$, $\seq{\Tvvar}$ fresh)\\
\( \PT(P_0\PAR P_1) = \) \\ \>
\(    \PLET\)\= \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
   \((\Gamma_1,A_1,C_1) = \PT(P_1)\)\\\>\>
  \((\Gamma_2, C_2) = \Gamma_0\Tcup \Gamma_1\)\\ \>
\(\PIN (\Gamma_2, A_0\TPAR A_1, C_0\cup C_1\cup C_2)\)\\
\( PT(\ifexp{v}{P_0}{P_1}) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
   \((\Gamma_1,A_1,C_1) = \PT(P_1)\)\\\>\>
   \((\Gamma_2, \mvtype) = \PTv(v)\)\\ \>\>
   \((\Gamma, C_2) = \Gamma_0\Tcup \Gamma_1\Tcup \Gamma_2\)\\\>
\(    \PIN (\Gamma, A_0\TOR A_1, C_0\cup C_1 \cup C_2\cup \set{\mvtype=\Tbool}) \)\\
\( PT(\nuexp{x}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
\( C_1 = \PIF x\in \dom(\Gamma_0)\PTHEN
   \set{\isTchan(\Gamma_0(x))} \PELSE \emptyset\)\\ \>
\(    \PIN (\Gamma_0\restrictTE{\set{x}}, \Thiding{x}{A_0}, C_0\cup C_1) \)\\
\( PT(\repexp P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \>
\(    \PIN (\Gamma_0, \Trep{A_0}, C_0) \)\\
\( PT(\accexp{\acclab}{x}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
    \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tres)\)\\ \>
\(    \PIN (\Gamma_1, \Tacc{\acclab}{x}{A_0}, C_0\cup C_1) \)\\
\( PT(\nurexp{x}{\spec}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
    \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tres)\)\\ \>
\(    \PIN (\Gamma_1\restrictTE{\set{x}}, \exclude{A_0}{\set{x}},
   C_0\cup C_1\cup \set{\traces{x}{A_0}\subseteq \spec}) \)
\end{tabbing}
\end{minipage}
}
\caption{A Type Inference Algorithm}
\label{fig:algorithm-PT}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi


==> Application.tex <==
\sect{Applications}
\label{sec:application}

We show that a variety of type systems ---
those for arity-mismatch check, race detection, 
static garbage-channel collection, and deadlock detection, --- can indeed be
obtained as instances of the generic type system.
Thanks to the common properties shown in
Section~\ref{subsec:common-properties}, only a small amount of extra
work is necessary to define each instance and prove its correctness.

Table~\ref{tab:prop-processes} shows the invariant properties of
processes that should be guaranteed by those type systems.  The
condition \(p_1(P)\) means that no arity-mismatch error occurs
immediately.  (So, if \(p_1\) is an invariant condition, no
arity-mismatch error occurs during reduction of \(P\).)  \(p_2(P)\)
means that \(P\) is not in a race condition on any output actions
annotated with \(\ev\).  \(p_3(P)\) means that it is not the case that
an input process labeled with \(\ev\) can be reduced and the same
channel is used for input or output after that.  The invariance of
that property means that  after a channel has been used for an input
action annotated with \(\ev\), the channel is no longer used. So, it
is safe to deallocate the channel after the action annotated with
\(\ev\). For example, the process
\(\nuexp{x}(\outnilatom{x}{\ev_1}\PAR \outnilatom{x}{\ev_2}
\PAR \innil{x}{\ev_3}{\innilatom{x}{\ev}})\) satisfies this
property.
\(p_4(P)\) means that \(P\) is not deadlocked on any actions annotated with \(\ev\)
in the sense that whenever \(P\) is  trying to perform an action
annotated with \(\ev\), \(P\) can be reduced further.

\begin{table}
\begin{tabular}{|l|l|}
\hline
\(p_1(P)\) & \(P\SPCONG \nuexpseq{w}P'\) implies
\(P' \models {\neg\exists x.\exists \ev_1,\ev_2.\exists \ivar_1,\ivar_2\COL\set{\ivar_1\neq \ivar_2}.
  (\PLout{x}{\ev_1}{\ivar_1}\PAR \PLin{x}{\ev_2}{\ivar_2})}\)\\
\hline
\(p_2(P)\) & \(P\SPCONG \nuexpseq{w}P'\) implies
  \(P' \models \neg\exists x.\exists \ev_1.\exists \ivar_1,\ivar_2.
  (\PLout{x}{\ev}{\ivar_1}\PAR \PLout{x}{\ev_1}{\ivar_2})\)\\
\hline
\(p_3(P)\) & \(P\SPCONG \nuexpseq{w}P'\) implies
\(P' \models \neg \exists x.\exists \ev_1,\ev_2.\exists \ivar.
\PLsometr{\labcom{x}{\ev_1}{\ev}}\eventual(\PLout{x}{\ev_2}{\ivar}\lor \PLin{x}{\ev_2}{\ivar})\)\\
\hline
\(p_4(P)\) & \(P\SPCONG \nuexpseq{w}P'\) implies
\(P' \models \neg\exists x,\exists\ivar.((\PLout{x}{\ev}{\ivar}\lor \PLin{x}{\ev}{\ivar})
                  \land \neg \exists y.\exists \ev_1,\ev_2.(
                   \PLsometr{\labcom{y}{\ev_1}{\ev_2}}{\PLTRUE}\lor 
                   \PLsometr{\labcom{\epsilon}{\ev_1}{\ev_2}}{\PLTRUE}))\)\\
\hline
\end{tabular}
\caption{Properties of Processes}
\label{tab:prop-processes}
\end{table}



Table~\ref{tab:consistency-conditions} shows the consistency condition
for each type system. \(\reliable_2(\Gamma)\) means that no race
occurs on output actions annotated with \(\ev\) during reduction of
the abstract process \(\Gamma\).   \(\reliable_3(\Gamma)\) means that,
after \(\Gamma\) has been reduced on an action involving a channel
\(x\) and the event \(\ev\), the reduced process type no longer
performs an input or output action on the same channel.
\(\reliable_4(\Gamma)\) means that
whenever \(\Gamma\) is reduced to a process type trying to perform
an action annotated with an event \(\ev_1\) less than or equal to
\(\ev\), \(\Gamma\) can be further reduced on some channel or on an
event \(\ev_2\) less than \(\ev_1\). 
Here, we assume that \(\EOrd\) is some
well-founded relation on events, and \(\ev_1\EOrdeq\ev_2\)
means \(\ev_1\EOrd\ev_2\) or \(\ev_1=\ev_2\). We added new formulas 
\(\ev_1\EOrdeq \ev_2\), \(\ev_1\EOrd\ev_2\),
 and \(\PLsometr{\ev}{A}\) to express properties of
process types; their semantics is defined by:
\begin{eqnarray*}
\semTF{\ev_1\EOrd\ev_2} &=& 
    \left\{\begin{array}{ll}
       \TSET & \mbox{if $\ev_1\EOrd\ev_2$}\\
       \emptyset & \mbox{otherwise}
       \end{array}
   \right.\\
\semTF{\ev_1\EOrdeq\ev_2} &=& 
    \left\{\begin{array}{ll}
       \TSET & \mbox{if $\ev_1\EOrdeq\ev_2$}\\
       \emptyset & \mbox{otherwise}
       \end{array}
   \right.\\
\semTF{\PLsometr{\ev}{A}} &=&
    \set{\Gamma \mid \Gamma\TEredwith{{\ev}}\Gamma' \land \Gamma'\in \semTF{A}}
\end{eqnarray*}


\begin{table}
\begin{tabular}{|l|l|}
\hline
\(\reliable_1(\Gamma)\) & \(\wf(\Gamma)\) \\
\hline
\(\reliable_2(\Gamma)\) & \(\conTE(\Gamma)\) and 
\(\Gamma \models \neg\eventual({\exists x.\exists \ev_1.\exists \ivar_1,\ivar_2:\set{\ivar_1\neq \ivar_2}.
  (\PLout{x}{\ev}{\ivar_1}\PAR \PLout{x}{\ev_1}{\ivar_2})})\)\\
\hline
\(\reliable_3(\Gamma)\) & 
\(\conTE(\Gamma)\) and 
\(\Gamma \models \neg\eventual(\exists x.\exists \ev_1,\ev_2.\exists \ivar.
\PLsometr{\labcom{x}{\ev_1}{\ev}}\eventual(\PLout{x}{\ev_2}{\ivar}\lor \PLin{x}{\ev_2}{\ivar}))\)\\
\hline
\(\reliable_4(\Gamma)\) & \begin{minipage}{15cm}
\(\wf(\Gamma)\) and \\
\(\Gamma \models \neg \eventual(\exists \ev'.\exists x.\exists\ivar.
  (\ev'\EOrdeq \ev \land 
  (\PLout{x}{\ev'}{\ivar}\lor \PLin{x}{\ev'}{\ivar})\\
 \myquad\myquad  \land \neg \exists y.\exists \ev_1,\ev_2.(\PLsometr{\labcom{y}{\ev_1}{\ev_2}}{\PLTRUE}
     \lor (\PLsometr{\ev_1}{\PLTRUE}\land \ev_1\EOrd \ev'))))\).
\end{minipage}\\
\hline
\end{tabular}
\caption{Consistency Conditions}
\label{tab:consistency-conditions}
\end{table}

Soundness of the first three type systems follows immediately from
Corollary~\ref{cor:general-soundness}.
\begin{theorem}
\label{thm:correctness-of-app}
Let \(\reliable\) be \(\reliable_i\) ($i\in\{1,2,3\}$).
If \(\Gamma\p P\) and \(\reliable(\Gamma)\), then \(p_i(Q)\) holds for every
\(Q\) such that \(P\red^*\SPCONG Q\).
\end{theorem}
\begin{proof}
\begin{itemize}
\item Case for \(i=1\):
Suppose that \(\Gamma\p P\), \(\reliable(\Gamma)\), and 
\(P\red^* \SPCONG Q\).
Let \(A\) be:
 \[\neg\eventual(\exists x.\exists \ev_1,\ev_2.
     \exists \ivar_1,\ivar_2\COL\set{\ivar_1\neq \ivar_2}.
  (\PLout{x}{\ev_1}{\ivar_1}\PAR \PLin{x}{\ev_2}{\ivar_2})).\]
To show \(p_1(Q)\), it is sufficient to show that
\(Q\SPCONG \nuexpseq{w}\nuexp{\seq u}Q'\) implies \(\nuexpseq{w}Q'\models A\).
Since \(\reliable_1(\Gamma)\) implies \(\Gamma\models A\) and \(A\) is a negative formula,
Corollary~\ref{cor:general-soundness} implies the sufficient condition.
\item Case for \(i=2\):
Since \(\reliable_2\) is an invariant condition,
 \(\reliable_2\) is a proper consistency predicate.
Suppose that \(\Gamma\p P\), \(\reliable(\Gamma)\), and 
\(P\red^* \SPCONG Q\).
Let \(A\) be:
 \[
\neg\eventual({\neg\exists x.\exists \ev_1.\exists \ivar_1,\ivar_2:\set{\ivar_1\neq \ivar_2}.
  (\PLout{x}{\ev}{\ivar_1}\PAR \PLout{x}{\ev_1}{\ivar_2})}).\]
To show \(p_2(Q)\), it is sufficient to show that
\(Q\SPCONG \nuexpseq{w}\nuexp{\seq u}Q'\) implies \(\nuexpseq{w}Q'\models A\).
Since \(\reliable_2(\Gamma)\) implies \(\Gamma\models A\) and
\(A\) is a negative formula, 
Corollary~\ref{cor:general-soundness} implies the sufficient condition.
\item Case for \(i=3\): Similar to the case for \(i=2\).
\end{itemize}
\end{proof}

In the theorem above, \(\subtype\) can be any proper subtyping relation.
Choosing an appropriate subtyping relation for each type system would 
simplify type-checking or type-reconstruction. For example,
%%in the above type systems,
we can identify \(\evty{\ev}\PrTy\) with \(\PrTy\) by 
the rule \(\evty{\ev}\PrTy\TEcong \PrTy\), 
except for the case \(i=4\). 
For a naive arity-mismatch check~\cite{Gay93,Vasco93CONCUR}, we can ignore the order of
communications by introducing rules like 
\(\InTE{x}{\tau}{\ev}\PrTy
\TEcong \InTEatom{x}{\tau}{\ev}\TPAR \PrTy\).

For the type system for deadlock-freedom (\(\reliable = \reliable_4\)), 
we need to choose a particular subtyping relation.  Let
\(\leq_1\) be the least proper subtyping relation and
\(\leq_2\) be the least subtyping relation closed under 
the rules in Figure~\ref{fig:subtyping} with \rn{Sub-Divide}.
Then, deadlock-freedom holds for both relations:
\begin{theorem}
\label{thm:correctness-of-deadlock}
Let \(\reliable\) be \(\reliable_4\) and \(\subtype\) be
\(\leq_i\) (\(i \in \set{1, 2}\)).  If \(\Gamma\p P\) and
\(\reliable(\Gamma)\), then \(p_4(Q)\) holds for every \(Q\) such that
\(P\red^*\SPCONG Q\).
\end{theorem}
We cannot use Corollary~\ref{cor:general-soundness} 
to prove the theorem above, because 
\(p_4(P)\) is described using a non-negative formula.
Using more basic theorems shown in Section~\ref{subsec:common-properties}, however,
we can easily prove the above theorem.
By Theorem~\ref{thm:type-soundness}, it suffices to show
that \(\Gamma\p P\) and
\(\reliable_4(\Gamma)\) imply \(p_4(P)\), by using 
Theorems~\ref{thm:normal-derivation}--\ref{lem:property-of-normal-derivation}: See
Appendix~\ref{sec:proof-of-sec4} for a proof.

%%\iffull
%%%\else
%%%To prove this, it suffices to show
%%% that \(\Gamma\p P\) and
%%%\(\reliable_i(\Gamma)\) imply \(p_i(P)\) for each \(i\), by using 
%%%Theorems~\ref{thm:normal-derivation}--\ref{lem:property-of-normal-derivation}
%%%(see the full version~\cite{Kobayashi00TR:Unifying} for details). 
%%%The above theorem then follows from
%%%Theorem~\ref{thm:type-soundness}.
%%%\fi


The following examples indicate that our framework not only has 
many of the existing type systems as instances but also can express
more expressive type systems than them (see also Section~\ref{sec:object}).
\begin{example}
The process \(\inexp{x}{y}{}\innilatom{x}{} \PAR 
 \outexp{x}{w}{}\outnilatom{x}{\,}{}\) is well typed 
in the first ($i=1$) type system. 
So, unlike in earlier type systems
for arity-mismatch check~\cite{Gay93,Vasco93CONCUR}, 
the same channel can be used for communicating
values of different types.\footnote{Yoshida's type system~\cite{Yoshida96FST} 
also allows such use of channels.}
\end{example}

\begin{example}
The second type system guarantees that the process
\iffull
\[
\else
\(
\fi
\nuexp{l,x}(\outnilatom{l}{\ev_0}\PAR 
 \repexp\innil{l}{\ev_1}\outnil{x}{\ev}
 \outnilatom{l}{\ev_3}\PAR
%%  \PAR\inexp{l}{\,}{\ev_1}\inexp{x}{\,}{\ev_2}\outatom{l}{\,}{\ev_3}\PAR
  \innilatom{x}{\ev_4})
\iffull
\]
\else
\)
\fi
is race-free on the channel \(x\). So, 
\iffull unlike the linear type 
system~\cite{KobayashiTOPLAS:LinearPi} for the \(\pi\)-calculus,
\else
 unlike the linear \(\pi\)-calculus~\cite{KobayashiTOPLAS:LinearPi},
\fi
our type system can guarantee lack of race conditions even on 
channels that are used more than once.%
\footnote{Flanagan and Abadi's type system~\cite{Flanagan99CONCUR} also
gives such a guarantee. Since their target calculus has locks as
primitives, the problem is a little simpler.}
\end{example}

\begin{example}
The fourth type system \iffull (for deadlock-freedom) \fi rejects 
the process 
\iffull
\[
\else
\(
\fi
P = \nuexp{x}\nuexp{y}(\innil{x}{\ev}\outnilatom{y}{\ev_1}
\PAR \innil{y}{\ev_2}\outnilatom{x}{\ev_3}).
\iffull
\]
\else
\)
\fi
The type of the sub-process \(\innil{x}{\ev}\outnilatom{y}{\ev_1}
\PAR \innil{y}{\ev_2}\outnilatom{x}{\ev_3}\) is
 \(\InTEnil{x}{\ev}\OutTEnilatom{y}{\ev_1}
\PAR\InTEnil{y}{\ev_2}\OutTEnilatom{x}{\ev_3}\).
So, in order for \(P\) to be well-typed, the following constraints
must be satisfied:
\[
\begin{array}{l}
\reliable_4(\InTEnil{x}{\ev}\evTEatom{\ev_1}
\PAR\evTE{\ev_2}\OutTEnilatom{x}{\ev_3})\\
\reliable_4(\evTE{\ev}\OutTEnilatom{y}{\ev_1}
\PAR\InTEnil{y}{\ev_2}\evTEatom{\ev_3})
\end{array}
\]
The former constraint requires that \(\ev_2\EOrd \ev\)
(because the input from \(x\) succeeds only after 
the event \(\ev_2\) succeeds), while
the latter requires that \(\ev\EOrd \ev_2\), hence a contradiction.
\end{example}

%%%\iffull
%%%We think that we can also obtain type systems for
%%%livelock-freedom~\cite{Kobayashi00TCS} and information 
%%%flow~\cite{Hennessy00ICALP,Honda00ESOP} in a similar manner.
%%%\fi


\begin{remark}
A type environment in a usual type system
corresponds to the equivalence class of a process type
with respect to the relation \(\TEcong\) derived from 
an appropriate subtyping relation. (Recall that
\(\PrTy_1\TEcong \PrTy_2\) means
\(\PrTy_1\subTE\PrTy_2\land \PrTy_2\subTE \PrTy_1\).)
For example, the type environment
\[x\COL\CHAN{\CHAN{\,}{O}}{(O|I)}, z\COL\CHAN{\,}{(O | I.I)}\]
given in Section~\ref{sec:intro} corresponds to the equivalence class
of a process type
\[\OutTEatom{x}{\typ{y}{\OutTEnilatom{y}{\ev}}}{\ev}\TEPAR 
   \InTEatom{x}{\typ{y}{\OutTEnilatom{y}{\ev}}}{\ev}
  \TEPAR \OutTEnilatom{z}{\ev}\TEPAR \InTEnil{z}{\ev}\InTEnilatom{z}{\ev},\]
with respect to \(\TEcong\) that satisfy the rules
\(\OutTE{x}{\tau}{\ev}{\Gamma}\TEcong\OutTE{x}{\tau}{\ev'}{\Gamma}\),
\(\InTE{x}{\tau}{\ev}{\Gamma}\TEcong\InTE{x}{\tau}{\ev'}{\Gamma}\),
\(\evTE{\ev}{\Gamma}\TEcong \Gamma\), and
\((\project{\PrTy}{S}\TEPAR\exclude{\PrTy}{S}) \TEcong \PrTy\).
The last rule removes information about the order of communications 
between different channels.
A type environment of the linear 
\(\pi\)-calculus~\cite{KobayashiTOPLAS:LinearPi} is obtained by 
further removing information about channel usage,
by adding the rules \(\OutTE{x}{\tau}{\ev}{\Gamma}\TEcong
\OutTEatom{x}{\tau}{\ev}\PAR {\Gamma}\), 
\(\InTE{x}{\tau}{\ev}{\Gamma}\TEcong
\InTEatom{x}{\tau}{\ev}\PAR {\Gamma}\), and 
\(\Gamma\TEPAR \Gamma \TEcong \TEREP{\Gamma}\). 
A type environment of the input-only/output-only channel type 
system~\cite{Pierce96MSCS} is obtained by further adding the rule
\(\TEREP{\Gamma}\TEcong \Gamma\).
%%%\fi
\end{remark}


==> Basis.tex <==

\section{Computing a Basis of Behavioral Type}
\label{sec:basis-of-behavioral-type}
\def\excludeaux#1#2#3#4{{#3}\uparrow_{#4}^{#1,#2}}

This section is an appendix for Section~\ref{sec:petrinet-construction}.
Let \(A\) be a behavioral type of the form
\(\nuexp{\seq{y}}B\), where \(B\) does not contain any \(\nu\)-prefix.
Such \(A\) can be obtained by pushing all the \(\nu\)-prefixes out to the top-level,
as described in Section~\ref{sec:petrinet-construction}.
We show how to compute a basis of \(A\) below.

\def\elimup#1#2#3#4{\textit{ElimUp}^{#3,#4}(#1,#2)}
The constructor \(\exclude{\cdot}{S}\) can be eliminated by running
 the algorithm \(\elimup{B}{\emptyset}{\emptyset}{\emptyset}\) below.
%%with the empty function as the initial values of \(F\) and \(D\).
%%The algorithm for eliminating  from \(B\) is given as follows.
%%%(The procedure below can be applied even if the type contains \(\nu\)-prefixes.
\[
\begin{array}{l}
\elimup{\Tzero}{S}{F}{D} = \Tzero\\
\elimup{\Tbvar}{S}{F}{D} = \\
\myquad  \left\{
   \begin{array}{ll}
       A & \mbox{if $F(\Tbvar,S) = A$}\\
       \Trec{\beta}{\elimup{D(\Tbvar)}{S}{F\set{(\Tbvar,S)\mapsto \beta}}{D}}
        & \mbox{if $(\Tbvar,S)\not\in \dom(F)$}
   \end{array}\right.\\
\elimup{\Tact{\act}{A}}{S}{F}{D} = \Tact{(\act\backslash{S})}{\elimup{{A}}{S}{F}{D}}\\
\elimup{A_1\TPAR A_2}{S}{F}{D} =
  \elimup{A_1}{S}{F}{D}\TPAR \elimup{A_2}{S}{F}{D}\\
\elimup{A_1\TOR A_2}{S}{F}{D} =\\
\myquad  \elimup{A_1}{S}{F}{D}\TOR \elimup{A_2}{S}{F}{D}\\
\elimup{\Trep{A}}{S}{F}{D} = \Trep\elimup{A}{S}{F}{D}\\
\elimup{\csubst{\seq{x}}{\seq{y}}A}{S}{F}{D} =
  \elimup{A}{\set{z \mid [\seq{y}/\seq{x}]z\in S}}{F}{D}\\
%%%\elimup{\Thiding{x}{A}}{S}{F}{D} =
%%%   \Thiding{x}{\elimup{A}{S\setdif\set{x}}{F}{D}}\\
%%%\myquad \mbox{ (we assume that $x$ does not ocur free in $D,F,S$)}\\
\elimup{\Trec{\Tbvar}{A}}{S}{F}{D} =
  \Trec{\Tbvar}{\elimup{{A}}{S}{F\set{(\Tbvar,S)\mapsto \Tbvar}}{D\set{\Tbvar\mapsto A}}}\\
\elimup{\exclude{A}{S_1}}{S}{F}{D} =
   \elimup{A}{S\cup S_1}{F}{D}\\
\elimup{\project{A}{S_1}}{S}{F}{D} =
   \project{\elimup{A}{S}{F}{D}}{S_1}
\end{array}
\]
Here, \(\act\backslash{S}\) is \(\tau\) if \(\acctarget{l}\subseteq S\)
and \(\act\) otherwise.
\(D\) keeps recursive definitions and \(F\) is a cache for avoiding repeated computation.
If \(A\) does not contain \(\nu\)-prefixes, \(\elimup{B}{\emptyset}{\emptyset}{\emptyset}\) always
terminates since \(S\) can range over a finite set (which is the powerset of \(\FV(B)\)).
%%%[*** How can we show that \(\exclude{A}{S}\) given above is well-defined?
%%% --- probably because \(S\) can contain only free variables, so that
%%% \(F\) ranges over a finite set ***]
The constructor \(\project{\cdot}{S}\) can be removed in the same manner.

We can further eliminate the renaming constructor \(\csubst{\seq{x}}{\seq{y}}\)
by using the following algorithm.
\def\elimrename#1#2#3#4{\textit{ElimRen}^{#3, #4}(#1, #2)}
\[
\begin{array}{l}
\elimrename{\Tzero}{\theta}{F}{D} = \Tzero\\
\elimrename{\Tbvar}{\theta}{F}{D} = \\
\myquad
  \left\{
   \begin{array}{ll}
       A & \mbox{if $F(\Tbvar,\theta) = A$}\\
       \Trec{\beta}{\elimrename{D(\Tbvar)}{\theta}{F\set{(\Tbvar,\theta)\mapsto \beta}}{D}}
        & \mbox{if $(\Tbvar,\theta)\not\in \dom(F)$}
   \end{array}\right.\\
\elimrename{\Tact{\act}A}{\theta}{F}{D} =
     \Tact{\theta \act}\elimrename{A}{\theta}{F}{D}\\
\elimrename{A_1\PAR A_2}{\theta}{F}{D} =
 \elimrename{A_1}{\theta}{F}{D}\PAR \elimrename{A_2}{\theta}{F}{D}\\
\elimrename{A_1\TOR A_2}{\theta}{F}{D} =\\
\myquad \elimrename{A_1}{\theta}{F}{D}\TOR \elimrename{A_2}{\theta}{F}{D}\\
\elimrename{\Trep{A}}{\theta}{F}{D} =
 \Trep{\elimrename{A}{\theta}{F}{D}}\\
\elimrename{\csubst{\seq{x}}{\seq{y}}A}{\theta}{F}{D} =
  \elimrename{A}{\theta\comp\subst{\seq{x}}{\seq{y}}}{F}{D}\\
\elimrename{\Trec{\Tbvar}{A}}{\theta}{F}{D} =
  \Trec{\Tbvar}{\elimrename{A}{\theta}{F\set{(\Tbvar,\theta)\mapsto \Tbvar}}{D\set{\Tbvar\mapsto A}}}
\end{array}
\]
%%%\begin{remark}
%%%It is not trivial to remove \([y/x]\Trec{\Tbvar}{A}\) as well.
%%%Consider
%%%\[ [y/x]\Trec{\Tbvar}x.y.[z/x]\Tbvar\]
%%%We need a definition similar to that of \(\excludeaux{D}{F}{A}{S}\),
%%%and again we are left with the question of whether the definition is well-formed.
%%%\end{remark}


\def\SIMPLETYPE{\textbf{A}_\textbf{0}}
By applying the above algorithms to \(A = \nuexp{\seq{y}}B\),
we obtain an equivalent type \(A'=\nuexp{\seq{y}}B'\), where
\(B'\) does not contain any \(\nu\)-prefixes, 
\(\project{\cdot}{S}\), \(\exclude{\cdot}{S}\), or \(\csubst{\seq{x}}{\seq{y}}\).
So, only elements of \(\ATOMS(B')\) defined below (modulo folding/unfolding
of recursive types)
can appear in transitions of \(B\). So, \((\set{\seq{y}}, \ATOMS(B'))\) forms a basis of \(A\).
\begin{defi}
Let \(A\) be a behavioral type that does not contain any \(\nu\)-prefix,
\(\project{\cdot}{S}\), \(\exclude{\cdot}{S}\), or \(\csubst{\seq{x}}{\seq{y}}\).
The set of {\em atoms} \(\ATOMS(A)\) is the least set that satisfies the following conditions.
\[
\begin{array}{l}
\ATOMS(\Tact{\act}A) \supseteq \set{\Tact{\act}A}\cup \ATOMS(A)\\
\ATOMS(A_1\TPAR A_2) \supseteq \ATOMS(A_1)\cup \ATOMS(A_2)\\
\ATOMS(A_1\TOR A_2) \supseteq \set{A_1\TOR A_2}\cup \ATOMS(A_1)\cup \ATOMS(A_2)\\
\ATOMS(\Trep{A}) \supseteq \set{\Trep{A}}\cup \ATOMS(A)\\
\ATOMS(\Trec{\Tbvar}{A}) \supseteq \set{\Trec{\Tbvar}{A}} \cup \ATOMS(\subst{\Tbvar}{\Trec{\Tbvar}{A}}A)
\end{array}
\]
\end{defi}


%%%We show below how to construct the Petri net \(\petrinetaux{A}{x}{(, \ATOMS(A))}\).
%%%
%%%\def\AtoP{\textbf{A2P}}
%%%The mapping from behavioral types to Petri net states is given by:
%%%\[
%%%\begin{array}{l}
%%%\AtoP(A_1\TPAR A_2) = \AtoP(A_1)\PPAR \AtoP(A_2)\\
%%%\AtoP(A) = s_{A}  \mbox{ if \(A\)'s outermost constructor is not \(\TPAR\)}
%%%\end{array}
%%%\]
%%%
%%%The set of net transitions are given by:
%%%\[
%%%\begin{array}{l}
%%%\set{
%%%s_{\Tacc{\acclab}{x}B} \Predwith{\acclab} \AtoP(B)  \mid \Tacc{\acclab}{x}B\in \ATOMS(A)
%%%}\\
%%%\cup
%%%\set{
%%%s_{\Tact{\actout{z}}B_1}\PPAR s_{\Tact{\actin{z}}B_2}
%%%   \Predwith{\tau} \AtoP(B_1)\PPAR \AtoP(B_2) \mid 
%%%{\Tact{\actout{z}}B_1}, {\Tact{\actin{z}}B_2}\Tacc{\acclab}{x}B\in \ATOMS(A)
%%%}\\
%%%\cup 
%%%\set{
%%%s_{B_1\TOR B_2} \Predwith{\tau} \AtoP(B_1) \mid B_1\TOR B_2\in \ATOMS(A)
%%%}\\
%%%\cup
%%%\set{
%%%s_{B_1\TOR B_2} \Predwith{\tau} \AtoP(B_2) \mid B_1\TOR B_2\in \ATOMS(A)
%%%}\\
%%%\cup
%%%\set{
%%%s_{\Trep{B}} \Predwith{\tau} s_{\Trep{B}}\PPAR \AtoP(B) \mid \Trep{B}\in \ATOMS(A)
%%%}\\
%%%\cup
%%%\set{
%%%s_{\Trec{\Tbvar}{B}} \Predwith{\tau} \AtoP(\subst{\Tbvar}{\Trec{\Tbvar}{B}}B) 
%%%  \mid \Trec{\Tbvar}{B}\in \ATOMS(A)
%%%}
%%%\end{array}
%%%\]
%%%


==> CCS-to-Petri.tex <==

\section{Approximation of behavioral types by Petri nets}

\def\excludeaux#1#2#3#4{{#3}\uparrow_{#4}^{#1,#2}}

First, we assume that a behavioral type does not contain \(\exclude{A}{S}\).
It can be removed as follows:
\[
\begin{array}{l}
\exclude{A}{S} = \excludeaux{\emptyset}{\emptyset}{A}{S}\\
\excludeaux{D}{F}{\Tzero}{S} = \Tzero\\
\excludeaux{D}{F}{\Tact{\act}{A}}{S} = \Tact{(\act\backslash{S})}{\excludeaux{D}{F}{A}{S}}\\
\excludeaux{D}{F}{\Tbvar}{S} = 
  \left\{
   \begin{array}{ll}
       A & \mbox{if $F(\Tbvar,S) = A$}\\
       \Trec{\beta}{\excludeaux{D}{F\set{(\Tbvar,S)\mapsto \beta}}{D(\Tbvar)}{S}}
        & \mbox{if $(\Tbvar,S)\not\in \dom(F)$}
   \end{array}\right.\\
\excludeaux{D}{F}{\Trec{\Tbvar}{A}}{S} =
  \excludeaux{D\set{\Tbvar\mapsto A}}{F\set{(\Tbvar,S)\mapsto A}}{\Trec{\Tbvar}{A}}{S}\\
\excludeaux{D}{F}{[\seq{y}/\seq{x}]A}{S} =
  \excludeaux{D}{F}{A}{\set{z \mid [\seq{y}/\seq{x}]z\in S}}\\
\excludeaux{D}{F}{\Thiding{x}{A}}{S} =
   \Thiding{x}{\excludeaux{D}{F}{A}{S}} \mbox{ (we assume that $x$ does not ocur in $D,F,S$)}\\
\cdots
\end{array}
\]
Here, \(D\) keeps recursive definitions and \(F\) is a cache.

[*** How can we show that \(\exclude{A}{S}\) given above is well-defined?
 --- probably because \(S\) can contain only free variables, so that
 \(F\) ranges over a finite set ***]

We also assume that renamings are applied only to variables
\(\Tbvar\) and recursive types \(\Trec{\Tbvar}{A}\).
\def\rename#1#2{[{#2}/{#1}]}
\[
\begin{array}{l}
\rename{\seq x}{\seq y}\Tzero = \Tzero\\
\rename{\seq x}{\seq y}\Tact{\act}A =
   \Tact{\rename{\seq x}{\seq y}\act}\rename{\seq x}{\seq y}A\\
\rename{\seq x}{\seq y}(A_1\PAR A_2) =
  (\rename{\seq x}{\seq y}A_1) \PAR (\rename{\seq x}{\seq y}A_2) \\
\rename{\seq x}{\seq y}\rename{\seq x'}{\seq y'}A =
  (\rename{\seq x}{\seq y}\circ \rename{\seq x'}{\seq y'})A\\
\cdots
\end{array}
\]
\begin{remark}
It is not trivial to remove \([y/x]\Trec{\Tbvar}{A}\) as well.
Consider
\[ [y/x]\Trec{\Tbvar}x.y.[z/x]\Tbvar\]
We need a definition similar to that of \(\excludeaux{D}{F}{A}{S}\),
and again we are left with the question of whether the definition is well-formed.
\end{remark}

We also push operators \(\Thiding{x}{}\) and \(\Trep\) inside as much as possible:
\[
\begin{array}{l}
\Trep{(A_1|A_2)} = \Trep{A_1}\PAR \Trep{A_2}\\
\Thiding{x}{(A_1|A_2)} = \Thiding{x}{A_1} \PAR A_2 \mbox{ if $x$ is not free in $A_2$}\\
\Thiding{x}{A} = A \mbox{ if $x$ is not free in $A$}\\
\end{array}
\]

We call a behavioral type \(A\) {\em atomic} if 
\(A\)'s outermost operator is not \(\PAR\).
%%% and \(A\) does not contain
%%%a formula of the form \([\Trec{\Tbvar}{A}/\Tbvar]A\)
%%%(which should be folded to \(\Trec{\Tbvar}{A}\).
(We assume that the above transformation have been already applied,
so that \(A\) cannot be a type like \(\Trep{(A_1|A_2)}\).)

Let us define \(\Deriv(A)\) to be the least set satisfying the following rules.
\[
\begin{array}{l}
\Deriv{A} \supseteq \set{A} \cup \bigcup\{\Deriv{A_1},\ldots,\Deriv{A_n}
    \mid A \Tredwith{l} B\\
\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad 
 \mbox{and  $A_1\PAR A_2\PAR \cdots \PAR A_n$ is a normal form of $B$}
\}
\end{array}
\]

%%%[*** Actually, we also need to assume that unnecessary unfold has not been performed
%%%to derive \(A \Tredwith{l} A_1\PAR A_2\PAR \cdots \PAR A_n\).
%%%How can we formally state that? ***]

If \(\Deriv{A}\) is infinite,
we apply the following approximation to eliminate hiding operators.

\[
\Trec{\Tbvar}{A} \approx [\Trec{\Tbvar}{A'}/\Tbvar]A
\]
where \(A'\) is the type obtained by removing all the hiding constructors in \(A\).
The above approximation identifies all the local channels created inside recursion.
Note that \([\Trec{\Tbvar}{A'}/\Tbvar]A\subtype \Trec{\Tbvar}{A}\) holds.
It also implies \(\traces{x}{[\Trec{\Tbvar}{A'}/\Tbvar]A} \supseteq \traces{x}{\Trec{\Tbvar}{A}}\).

Having removed hiding operators, we conjecture that 
\(\Deriv{A}\) is finite.

\begin{conjecture}
If \(A\) does not contain the hiding constructor, \(\Deriv{A}\) is finite.
\end{conjecture}



==> Conc.tex <==
\section{Conclusion}
\label{sec:conclusion}

We have formalized a type system for resource usage analysis
and proved its soundness. We have also developed a sound (but incomplete
because of the last phase for deciding the trace inclusion relation
\(\traces{x}{A}\subseteq \spec\)) algorithm for it
in order to liberate programmers from the burden of writing complex type annotations.
We have also implemented a prototype resource usage analyzer based on the algorithm.

There remains much future work.
It is necessary to assess the effectiveness of our analysis, including
the design of the type system and the algorithm for deciding the trace inclusion relation
\(\traces{x}{A}\subseteq \spec\), in more detail, and refine the analysis if necessary.
It is also necessary to make the analyzer more user-friendly, by devising a method
for generating comprehensive explanation of the verification result; currently, the analyzer
gives only a yes/no answer.
Extensions of the type system to deal with
other typical synchronization primitives like join-patterns and internal choice is also
left for future work.


==> Exclude.tex <==
\def\excludeaux#1#2#3#4{{#3}\uparrow_{#4}^{#1,#2}}
\(\exclude{A}{S}\) is defined by:

\[
\begin{array}{l}
\exclude{A}{S} = \excludeaux{\emptyset}{\emptyset}{A}{S}\\
\excludeaux{D}{F}{\Tzero}{S} = \Tzero\\
\excludeaux{D}{F}{\Tbvar}{S} = 
  \left\{
   \begin{array}{ll}
       A & \mbox{if $F(\Tbvar,S) = A$}\\
       \Trec{\beta}{\excludeaux{D}{F\set{(\Tbvar,S)\mapsto \beta}}{D(\Tbvar)}{S}}
        & \mbox{if $(\Tbvar,S)\not\in \dom(F)$}
   \end{array}\right.\\
\excludeaux{D}{F}{\Trec{\Tbvar}{A}}{S} =
  \excludeaux{D\set{\Tbvar\mapsto A}}{F}{\Trec{\Tbvar}{A}}{S}\\
\excludeaux{D}{F}{[\seq{y}/\seq{x}]A}{S} =
  \excludeaux{D}{F}{A}{\set{z \mid [\seq{y}/\seq{x}]z\in S}}\\
\cdots
\end{array}
\]
Here, \(D\) keeps recursive definitions and \(F\) is a cache.


==> Ext-local-tag.tex <==
\section{Extension}
\label{sec:ext-tag}
The type system for deadlock-freedom derived in Section~\ref{sec:application}
subsumes our recent type system for deadlock-freedom~\cite{Kobayashi00CONCUR},
 but does not subsume our earlier type system~\cite{Kobayashi98TOPLAS}.
In fact, unlike the earlier type system~\cite{Kobayashi98TOPLAS},
the type system in Section~\ref{sec:application} cannot
guarantee the following process to be deadlock-free on the event \(\ev\):
\[\outatom{f}{reply}{\ev_0}\PAR \inexp{reply}{\,}{\ev}\zeroexp \PAR
 \repexp\inexp{f}{r}{\ev_1}\nuexp{r'}
        (\outexp{f}{r'}{\ev_2}
         \inexp{r'}{\,}{\ev'}\outatom{r}{\,}{\ev_3}).
          \]
The part \(\repexp\inexp{f}{r}{\ev_1}\nuexp{r'}\cdots\) 
 simulates the behavior of a recursive function:
Upon receiving a request through \(f\), the process forwards the
request to itself, waits for a reply on \(r'\), and then sends
the null tuple to \(r\).

The part \(\outexp{f}{r'}{\ev_2}
         \inexp{r'}{\,}{\ev'}\outatom{r}{\,}{\ev_3}\) is typed under
the type environment:
\[\OutTE{f}{\tau}{\ev_2}
        (\evTE{\ev_2}(\Gamma\TEPAR \evTE{\ev'}\OutTEatom{r'}{\,}{\ev_3})
       \TEPAR \InTE{r'}{\,}{\ev'}\OutTEatom{r}{\,}{\ev_3}),\]
where \(\tau = \typ{x}{\evTE{\ev_2}(\Gamma\TEPAR \evTE{\ev'}\OutTEatom{x}{\,}{\ev_3})}\)
and \(\Gamma\) is a certain type environment such that \(\nullTE(\Gamma)\).
For the whole process to be deadlock-free, it must be the case that:
\[\reliable_3(\evTE{\ev_2}(\evTE{\ev_2}
    (\Gamma\TEPAR \evTE{\ev'}\OutTEatom{r'}{\,}{\ev_3})
  \TEPAR \InTE{r'}{\,}{\ev'}\evTE{\ev_3}\zeroty)).\]
It does not hold, however, because the input from \(r'\),
which is annotated  with \(\ev'\), depends on the success of
an event of the same name
(\(\ev'\) of the part \(\evTE{\ev'}\OutTEatom{r'}{\,}{\ev_3}\)).

Intuitively, the above failure to guarantee deadlock-freedom comes from
the fact that the same event \(\ev'\) is assigned to 
inputs on all channels created by \(\nuexp{r'}\).
To overcome that problem, we can introduce a rule for renaming events,
so that some events that are identified in a global context
can be distinguished in a local context.
The resulting type system can guarantee deadlock-freedom
of processes like above, and is cleaner than the earlier type
system for deadlock-freedom~\cite{Kobayashi98TOPLAS}, which uses
ad hoc conditions to solve a similar problem.


%%%For simplicity, we consider only the specific type system for
%%%deadlock-freedom in Section~\ref{sec:application}. So, we assume
%%% \(\reliable\) to be \(\reliable_3\).
%%%Because we allow events to be renamed, we need to add an event ordering
%%%\(\EOrd\) to the assumption of a type judgment.
%%%\begin{defn}[refined type judgment]
%%%A type judgment is of the form \(\Gamma\ET \EOrd \p P\), where
%%%\(\EOrd\) is a well-founded relation on events, and
%%%every event appearing in \(\Gamma\) must also appear in \(\EOrd\).
%%%\end{defn}

To give new typing rules, we need some auxiliary definitions.
Basically, we want to introduce the following rule.
\infrule{\Gamma\p P}{\subst{\ev_1}{\ev_0}\Gamma\p \subst{\ev_1}{\ev_0}P}
This allows us to distinguish between \(\ev_1\) and \(\ev_0\) locally inside 
of \(P\) but identify them outside of \(P\).
To make this work, however, we must forbid the outside process 
to pass an event \(\ev_0\) (\(\ev_1\), resp.)
when \(P\) expects an event \(\ev_1\) (\(\ev_0\), resp.).
So, we impose the constraint that \(\ev_1\) cannot appear in
inner places of channel types (so that 
channels labelled with \(\ev_1\) cannot be passed through other channels). 
To state such a condition, we use the set \(\Iev(\Gamma)\) defined below.
It is the set of events appearing in inner places of \(\Gamma\).
%%%\begin{defn}
%%%Let \(\EOrd\) be a well-founded relation on events.
%%%\(\restrictEOrd{\EOrd}{S}\) is defined to be
%%%\(\EOrd \cap (\EVSET\setdif S)\times(\EVSET\setdif S)\).
%%%\end{defn}
%%%\begin{defn}
%%%Let \(\EOrd\) be a well-founded relation on events.
%%%The binary relation \(\eqev{\EOrd}\) is defined by:
%%%\[
%%%\begin{array}{ll}
%%%\ev_1\eqev{\EOrd}\ev_2\IFF\\
%%%\quad
%%%   ((\{\ev\in \EVSET\setdif{\ev_1,\ev_2}\mid \ev\EOrd \ev_1\}
%%%   = \{\ev\in \EVSET\setdif{\ev_1,\ev_2}\mid \ev\EOrd \ev_2\})\\
%%%\quad  \land 
%%%   (\{\ev\in \EVSET\setdif{\ev_1,\ev_2}\mid \ev_1\EOrd \ev\}
%%%   = \{\ev\in \EVSET\setdif{\ev_1,\ev_2}\mid \ev_2\EOrd \ev\})\\
%%%\quad \ev_1\EOrd \ev_2
%%%\end{array}
%%%\]
%%%\end{defn}
%%%\begin{defn}
%%%Let \(\EOrd\) be a well-founded relation on events.
%%%\(\merge{\EOrd}{\ev_1}{\ev_2}\) is defined by:
%%%\[
%%%\begin{array}{lcl}
%%%\merge{\EOrd}{\ev_1}{\ev_2} &= &
%%%  \{(\ev,\ev')\mid \ev \EOrd \ev' \land \ev_1\not\in\{\ev, \ev'\}\}\\
%%% &  &\cup \{(\ev_2,\ev)\mid \ev_1\EOrd\ev \land \ev\neq \ev_2\}\\
%%% &  &\cup \{(\ev,\ev_2)\mid \ev\EOrd\ev_1 \land \ev\neq \ev_2\}
%%%\end{array}
%%%\]
%%%\end{defn}

\begin{defn}
The set \(\Iev(\Gamma)\) of events is defined by:
\begin{eqnarray*}
\Iev(\zeroTE) &=& \emptyset\\
\Iev(\tev) &=& \emptyset\\
\Iev(\OutTE{x}{\tau}{\ev}\Gamma) &=& \Ev(\tau)\cup \Iev(\Gamma)\\
\Iev(\InTE{x}{\tau}{\ev}\Gamma) &=& \Ev(\tau)\cup \Iev(\Gamma)\\
\Iev(\evTE{\ev}\Gamma) &=& \Iev(\Gamma)\\
\Iev(\gamma_1+\cdots+\gamma_n) &=& \Iev(\gamma_1)\cup\cdots\cup \Iev(\gamma_n)\\
\Iev(\Gamma_1\TEPAR\Gamma_2) &=& \Iev(\Gamma_1)\cup \Iev(\Gamma_2)\\
\Iev(\Gamma_1\TEIOR\Gamma_2) &=& \Iev(\Gamma_1)\cup \Iev(\Gamma_2)\\
\Iev(\recTE{\tev}{\Gamma}) &=& \Iev(\Gamma)\\
\ \\
\Ev(\zeroTE) &=& \emptyset\\
\Ev(\tev) &=& \emptyset\\
\Ev(\OutTE{x}{\tau}{\ev}\Gamma) &=& \set{\ev}\cup\Ev(\tau)\cup \Ev(\Gamma)\\
\Ev(\InTE{x}{\tau}{\ev}\Gamma) &=& \set{\ev}\cup\Ev(\tau)\cup \Ev(\Gamma)\\
\Ev(\evTE{\ev}\Gamma) &=& \Ev(\Gamma)\\
\Ev(\gamma_1+\cdots+\gamma_n) &=& \Ev(\gamma_1)\cup\cdots\cup \Ev(\gamma_n)\\
\Ev(\Gamma_1\TEPAR\Gamma_2) &=& \Ev(\Gamma_1)\cup \Ev(\Gamma_2)\\
\Ev(\Gamma_1\TEIOR\Gamma_2) &=& \Ev(\Gamma_1)\cup \Ev(\Gamma_2)\\
\Ev(\recTE{\tev}{\Gamma}) &=& \Ev(\Gamma)\\
\end{eqnarray*}
\end{defn}

We allow \(\ev_2\) to be identified with \(\ev_1\) only when
the condition \(\ev_1\subEV\ev_2\) given below is met.
As explained above, the condition
\(\reliable(\Gamma) \imply \ev_2\not\in\Iev(\Gamma)\) forbids an event
\(\ev_2\) to be passed through channels.
If \(\ev_2\) is identified with \(\ev_1\) globally, 
each occurrence of \(\ev_1\) may be actually \(\ev_2\). It is taken into
account by the other condition
\(\forall \Delta.((\ev_2\not\in\Iev(\Delta)\land 
         \reliable(\subst{\ev_2}{\ev_1}\Delta))\imply \reliable(\Delta))\).

\begin{defn}
A binary relation \(\subEV\) on events is defined by:
\[
\begin{array}{l}
\ev_1\subEV \ev_2 \IFF \\
\quad (\reliable(\Gamma) \imply \ev_2\not\in\Iev(\Gamma))\land
     \forall \Delta.((\ev_2\not\in\Iev(\Delta)\land 
         \reliable(\subst{\ev_2}{\ev_1}\Delta))\imply \reliable(\Delta))
%%   \ev_1\EOrd\ev_2} 
\end{array}
\]
\end{defn}

The set of new typing rules consists of the rules in Section~\ref{sec:typing},
%%except for \rname{T-New}
%%(with \(\EOrd\) added to each type judgment), 
plus the following rule:

\infrule[T-Merge]
  {\Gamma \p P\\
   \ev_0\subEV \ev_1\subEV \ev_2\subEV \cdots \mbox{ for
    an infinite sequence $\ev_0,\ev_1,\ev_2,\ldots$}}
%%   \ev_1\not\in \Iev(\Gamma)\andalso 
%%   \forall \Delta.((\ev_1\not\in\Iev(\Delta)\land \reliable(\subst{\ev_1}{\ev_2}\Delta))\imply \reliable(\Delta))}
%%   \ev_1\EOrd\ev_2}
%%   \merge{\EOrd}{\ev_1}{\ev_2}\mbox{ is a well-founded relation}}
  {\subst{\ev_1}{\ev_0}\Gamma\p
       \subst{\ev_1}{\ev_0}P}
The reason why we require the existence of an infinite sequence
is that \(\subst{\ev_1}{\ev_0}P\) may be copied during reduction
and therefore, to type the reduced process, we need to rename
events (by \rname{T-Merge}) an arbitrary number of times.

%%%\begin{remark}
%%%To remove the condition \(\ev_1\EOrd\ev_2\), we need to 
%%%\begin{enumerate}
%%%\item parametrize judgments with \(\reliable\) as well, or
%%%\item introduce the condition \(\ev_1\EOrd\ev \IFF \ev_2\EOrd \ev\)?
%%%\end{enumerate}
%%%\end{remark}
We have not yet proved the correctness of the above rule, which is
left for future work. We conclude this section by showing
how the example given in the beginning of
this section can be typed under the extended type system.

\begin{example}
Let 
\(P = \repexp\inexp{f}{r}{\ev_1}\nuexp{r'}
        (\outexp{f}{r'}{\ev_2}
         \inexp{r'}{\,}{\ev'_0}\outatom{r}{\,}{\ev'_0})\).
Let \(\reliable\) be \(\reliable_3\) in Section~\ref{sec:application},
and let \(\EOrd\) be 
\((\{(\ev_2, \ev'_0), (\ev_3, \ev'_0)\}\cup\{(\ev'_i, \ev'_{i+1}), (\ev'_i, \ev)\mid
 i\in\{0,1,2,\ldots\}\})^*\).
Let \(\tau = 
   (x)\evty{\ev_2}(\Gamma \TPAR
    \evty{\ev'_0}\OutTEatom{x}{\,}{\ev'_0})\)
and \(\Gamma = \recty{\alpha}{(\evty{\ev_2}(\alpha\TPAR
              (\evty{\ev'_0}\evty{\ev'_0}\zeroty)))}\).

\[ \OutTE{f}{\tau}{\ev_2}
  (   \evty{\ev_2}(\Gamma\PAR 
       \evTE{\ev'_0}\OutTEatom{r'}{\,}{\ev'_0})
   \TEPAR
   \InTE{r'}{\,}{\ev'_1}\OutTEatom{r}{\,}{\ev'_0})
    \p \outexp{f}{x}{\ev_1}\inexp{r'}{\,}{\ev'_1}\outatom{r}{\,}{\ev'_0}\]
By applying \rname{T-New}, we obtain
\[ \OutTE{f}{\tau}{\ev_2}
  (   \evty{\ev_2}(\Gamma\PAR 
       \evTE{\ev'_0}\evTE{\ev'_0}\zeroty)
   \TEPAR
   \evTE{\ev'_1}\OutTEatom{r}{\,}{\ev'_0})
    \p \nuexp{r'}(\outexp{f}{x}{\ev_1}\inexp{r'}{\,}{\ev'_1}\outatom{r}{\,}{\ev'_0})\]
By applying \rname{T-Merge}, we obtain
\[ \OutTE{f}{\tau}{\ev_2}
  (  \Gamma
   \TEPAR
   \evTE{\ev'_0}\OutTEatom{r}{\,}{\ev'_0})
    \p \nuexp{r'}(\outexp{f}{x}{\ev_1}\inexp{r'}{\,}{\ev'_0}\outatom{r}{\,}{\ev'_0})\]
By applying \rname{T-In} and \rname{T-Rep}, we obtain
\[\TEREP\InTE{f}{\tau}{\ev_1} \OutTE{f}{\tau}{\ev_2}
  (  \Gamma
   \TEPAR
   \evTE{\ev'_0}\evTE{\ev'_0}\zeroTE)
    \p P\]
The type \(\tau\) indicates that if \(P\) receives a channel \(r\) on
\(f\), it replies to \(r\) after waiting for events
\(\ev_2\) and \(\ev_0'\) to occur. Because \(\ev_2\EOrd\ev_0'\EOrd\ev\) holds,
the type system guarantees that
a client process like
\(\outatom{f}{reply}{\ev_2}\PAR \inexp{reply}{\,}{\ev}\zeroexp\) does not
deadlock. (Actually, the whole process diverges in this case.)

%%%\(P = \repexp\inexp{f}{y}{}(\ifexp{b}{\outatom{y}{\,}{}}
%%%                   {\nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})})\).
%%%
%%%Let \(\tau = 
%%%   \evty{\evig}(\outtyatom{1}{\zeroty}{\ev}{0}
%%%   \TEIOR \evty{\evig}\evty{\ev}\outtyatom{1}{\zeroty}{\ev}{0})\).
%%%
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\outTEatom{x}{\zeroty}{\ev}{0}\TEIOR
%%%  \evty{\evig}\evty{\ev}\outTEatom{x}{\zeroty}{\ev}{0}) \TEPAR
%%%   \inTE{x}{\zeroty}{\ev'}{0}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev \EOrd \ev'
%%%    \p \outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{}\]
%%%
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\evTEatom{\ev}\TEIOR
%%%  \evty{\evig}\evty{\ev}\evTEatom{\ev}) \TEPAR
%%%   \evTE{\ev'}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev \EOrd \ev'
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%By using the rule \rname{T-Merge},  we obtain
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\evTEatom{\ev}\TEIOR
%%%  \evty{\evig}\evty{\ev}\evTEatom{\ev}) \TEPAR
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev 
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%By \rname{T-Sub}, we have
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0}
%%%  \ET \evig \EOrd \ev 
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%By the rule for conditionals, we have
%%%\[\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTEatom{\delta}(\outTEatom{y}{\zeroty}{\ev}{0}
%%%   \TEIOR \outTE{f}{\tau}{\evig}{1}
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0})\ET \evig\EOrd \ev \p 
%%%    \ifexp{b}{\outatom{y}{\,}{}}
%%%                   {\nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})}\]
%%%
%%%So, we have
%%%\[ \TEREP(\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \inTE{f}{\tau}{\evinf}{1}\evTE{\evig}(\evTEatom{\ev}
%%%  \TEIOR\outTEatom{f}{\tau}{\evig}{1}))
%%%  \ET \evig \EOrd \ev \p P\]

\end{example}


%%%
%%%\iffull\else
%%%$B7?IU$15,B'$r(Bevent ordering $B$K$h$C$F(Bparametrize$B$7!$(B
%%%$B%m!<%+%k$K$O0[$J$k(Bevent $B$rF10l;k$9$k$?$a$N(B\rname{T-Merge}$B$rF3F~!%(B
%%%
%%%\begin{defn}
%%%A binary relation \(\EOrd\) on events is called an event ordering
%%%if (i) \(\EOrd\cap ((\{\EVSET\}\setdif\{\evinf\})\times
%%%(\{\EVSET\}\setdif\{\evinf\}))\) is a strict partial order,
%%%(ii) \(\evig\) is the least element, and (iii)
%%%\(\forall \ev\in \dom(\EOrd)\cup\codom(\EOrd).\ev\EOrd \evinf\).
%%%\end{defn}
%%%
%%%\begin{remark}
%%%\(\EOrd\)$B$r(Bpreorder $B$H$7$F$=$3$+$iF@$i$l$kF1CM4X78$K(B
%%%$B4X$9$k(Bstrict partial order$B$r9M$($kJ}$,$-$l$$!)(B
%%%\end{remark}
%%%\begin{defn}
%%%\(\merge{\EOrd}{\ev_1}{\ev_2}\) is an event ordering defined by:
%%%\[
%%%\begin{array}{lcl}
%%%\merge{\EOrd}{\ev_1}{\ev_2} &= &
%%%  \{(\ev,\ev')\mid \ev \EOrd \ev' \land \ev_1\not\in\{\ev, \ev'\}\}\\
%%% &  &\cup \{(\ev_2,\ev)\mid \ev_1\EOrd\ev \land \ev\neq \ev_2\}\\
%%% &  &\cup \{(\ev,\ev_2)\mid \ev\EOrd\ev_1 \land \ev\neq \ev_2\}
%%%\end{array}
%%%\]
%%%\end{defn}
%%%
%%%\begin{defn}
%%%The set \(\Iev(\Gamma)\) of events is defined by:
%%%\[
%%%\begin{array}{l}
%%%\Iev(\zeroTE) = \emptyset\\
%%%\Iev(\tev) = \emptyset\\
%%%\Iev(\outTE{x}{\tau}{\ev}{n}\Gamma) = \Ev(\tau)\cup \Iev(\Gamma)\\
%%%\Iev(\inTE{x}{\tau}{\ev}{n}\Gamma) = \Ev(\tau)\cup \Iev(\Gamma)\\
%%%\Iev(\evTE{\ev}\Gamma) = \Iev(\Gamma)\\
%%%\Iev(\gamma_1+\cdots+\gamma_n) = \Iev(\gamma_1)\cup\cdots\cup \Iev(\gamma_n)\\
%%%\Iev(\Gamma_1\TEPAR\Gamma_2) = \Iev(\Gamma_1)\cup \Iev(\Gamma_2)\\
%%%\Iev(\Gamma_1\TEIOR\Gamma_2) = \Iev(\Gamma_1)\cup \Iev(\Gamma_2)\\
%%%\Iev(\recTE{\tev}{\Gamma}) = \Iev(\Gamma)\\
%%%\ \\
%%%\Ev(\zeroTE) = \emptyset\\
%%%\Ev(\tev) = \emptyset\\
%%%\Ev(\outTE{x}{\tau}{\ev}{n}\Gamma) = \set{\ev}\cup\Ev(\tau)\cup \Ev(\Gamma)\\
%%%\Ev(\inTE{x}{\tau}{\ev}{n}\Gamma) = \set{\ev}\cup\Ev(\tau)\cup \Ev(\Gamma)\\
%%%\Ev(\evTE{\ev}\Gamma) = \Ev(\Gamma)\\
%%%\Ev(\gamma_1+\cdots+\gamma_n) = \Ev(\gamma_1)\cup\cdots\cup \Ev(\gamma_n)\\
%%%\Ev(\Gamma_1\TEPAR\Gamma_2) = \Ev(\Gamma_1)\cup \Ev(\Gamma_2)\\
%%%\Ev(\Gamma_1\TEIOR\Gamma_2) = \Ev(\Gamma_1)\cup \Ev(\Gamma_2)\\
%%%\Ev(\recTE{\tev}{\Gamma}) = \Ev(\Gamma)\\
%%%\end{array}
%%%\]
%%%\end{defn}
%%%
%%%
%%%\infrule[T-Merge]
%%%  {\Gamma\ET \EOrd \p P\andalso \ev_1\not\in \Iev(\Gamma)}
%%%  {\subst{\ev_1}{\ev_2}\Gamma\ET \merge{\EOrd}{\ev_1}{\ev_2}\p 
%%%           \subst{\ev_1}{\ev_2}P}
%%%
%%%\begin{remark}
%%%\(\ev_1\not\in \Iev(\Gamma)\)$B$,@.$jN)$?$J$$>l9g!$Nc$($P(B
%%%\(\Gamma = \inTEatom{x}{\intyatom{1}{\zeroty}{\ev_1}{0}}{\ev}{1}\)$B$N$H$-$K(B
%%%$B>e$N5,B'$rE,MQ$9$k$N$O$^$:$$!%(B\(P\)$B$NCf$G$O(B\(\ev_1\)$B$H(B\(\ev_2\)$B$r6hJL$7$F$$$k$N$K(B
%%%$B30$N%W%m%;%9$,:.F1$7$F(B\(x\)$B$KBP$7$F%$%Y%s%H(B\(\ev_2\)$B$r;}$D%A%c%M%k(B
%%%$B$r8m$C$FAw$k2DG=@-$,$"$k$+$i!%F1MM$K(B
%%%\(\Gamma = \outTEatom{x}{\intyatom{1}{\zeroty}{\ev_1}{0}}{\ev}{1}\)$B$N$H$-$K(B
%%%$B>e$N5,B'$rE,MQ$9$k$H!$(B\(x\)$B$+$iAw$i$l$?%A%c%M%k(B\(y\)$B$,(B\(\ev_2\)$B$r;}$D$H(B
%%%$B8m2r$7$F(B\(P\)$B$,(B\(\ev_2\)$B$,$/$k$H2>Dj$7$F$$$k%A%c%M%k$K(B\(\ev_1\)$B$N%A%c%M%k(B\(y\)$B$r(B
%%%$BAw$C$F$7$^$&2DG=@-$,$"$k!%(B
%%%
%%%$B<B:]$K$O>e$N>r7o$r4K$a$F(B\(P\)$B$,(B\(\ev_1\)$B$N%A%c%M%k$r(Boutput$B$7$+$D(B
%%%\(\ev_2\)$B$N%A%c%M%k$r(Binput$B$9$k$+!$(B\(\ev_2\)$B$N%A%c%M%k$r(Boutput$B$7$+$D(B
%%%\(\ev_1\)$B$N%A%c%M%k$r(Binput$B$9$k$3$H$,$J$1$l$P$h$$!$$H$7$F$b$h$$$+$b$7$l$J$$!%(B
%%%\end{remark}
%%%
%%%\rname{T-Merge}$B$r;H$C$?5,B'$NNc(B
%%%
%%%\begin{example}
%%%Let \(P = \repexp\inexp{f}{y}{}(\ifexp{b}{\outatom{y}{\,}{}}
%%%                   {\nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})})\).
%%%
%%%Let \(\tau = 
%%%   \evty{\evig}(\outtyatom{1}{\zeroty}{\ev}{0}
%%%   \TEIOR \evty{\evig}\evty{\ev}\outtyatom{1}{\zeroty}{\ev}{0})\).
%%%
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\outTEatom{x}{\zeroty}{\ev}{0}\TEIOR
%%%  \evty{\evig}\evty{\ev}\outTEatom{x}{\zeroty}{\ev}{0}) \TEPAR
%%%   \inTE{x}{\zeroty}{\ev'}{0}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev \EOrd \ev'
%%%    \p \outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{}\]
%%%
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\evTEatom{\ev}\TEIOR
%%%  \evty{\evig}\evty{\ev}\evTEatom{\ev}) \TEPAR
%%%   \evTE{\ev'}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev \EOrd \ev'
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%\rname{T-Merge}$B$h$j(B
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%  ((\evTEatom{\ev}\TEIOR
%%%  \evty{\evig}\evty{\ev}\evTEatom{\ev}) \TEPAR
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0}) 
%%%  \ET \evig \EOrd \ev 
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%$B4X78$J$$(Bevent$B$r>C5n!JE,Ev$J(Bsub-type-environment relation$B$rF3F~$9$kI,MW$"$j!K(B
%%%\[ \outTE{f}{\tau}{\evig}{1}
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0}
%%%  \ET \evig \EOrd \ev 
%%%    \p \nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})\]
%%%
%%%If$B$NF3=P5,B'$h$j(B
%%%\[\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTEatom{\delta}(\outTEatom{y}{\zeroty}{\ev}{0}
%%%   \TEIOR \outTE{f}{\tau}{\evig}{1}
%%%   \evTE{\ev}\outTEatom{y}{\zeroty}{\ev}{0})\ET \evig\EOrd \ev \p 
%%%    \ifexp{b}{\outatom{y}{\,}{}}
%%%                   {\nuexp{x}(\outexp{f}{x}{}\inexp{x}{\,}{}\outatom{y}{\,}{})}\]
%%%
%%%$B$h$C$F(B
%%%\[ \TEREP(\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \inTE{f}{\tau}{\evinf}{1}\evTE{\evig}(\evTEatom{\ev}
%%%  \TEIOR\outTEatom{f}{\tau}{\evig}{1}))
%%%  \ET \evig \EOrd \ev \p P\]
%%%
%%%\end{example}
%%%
%%%\subsection{BOOL$B$N(Bencoding}
%%%
%%%\[\BOOL = \TREP \inTEatom{\cdot}{\tau_{\BOOL}}{\evinf}{2} \TPAR 
%%%   \TREP \evty{\evinf}\outTEatom{\cdot}{\tau_{\BOOL}}{\evig}{2}\]
%%%where
%%%%%\[ \tau_{\BOOL} = \evty{\evig}\outtyatom{1}{\,}{\evinf}
%%%%%   \TOR \evty{\evig}{\outtyatom{2}{\,}{\evinf}}\]
%%%\[ \tau_{\BOOL} = \outtyatom{1}{\zeroty}{\evinf}{0}
%%%   \TIOR {\outtyatom{2}{\zeroty}{\evinf}{0}}\]
%%%
%%%\[\TEREP{\intyatom{\TRUE}{\tau_{\BOOL}}{\evinf}{2}}\ET \EOrd 
%%%   \p \repexp\inexp{\TRUE}{t,f}{}\outatom{t}{\,}{}\]
%%%\[\TEREP{\intyatom{\FALSE}{\tau_{\BOOL}}{\evinf}{2}}\ET \EOrd 
%%%   \p \repexp\inexp{\FALSE}{t,f}{}\outatom{f}{\,}{}\]
%%%
%%%\[\ifexp{b}{P}{Q} = 
%%%   \nuexp{t,f}(\outatom{b}{t,f}{\caponly}\PAR 
%%%    \inexp{t}{\,}{\caponly}P+\inexp{f}{\,}{\caponly}Q)\]
%%%
%%%{\small
%%%\[
%%%  {\infers{\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTE{\evig}{\Gamma} \ET \merge{\EOrd}{\ev_1}{\evig} 
%%%    \p \ifexp{b}{P}{Q}}
%%%  {\infers{\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTE{\ev_1}{\Gamma} \ET \EOrd \p \ifexp{b}{P}{Q}}
%%%  {\infers{\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTE{\ev_1}{\Gamma} \TEPAR
%%%    \evTE{\evig}(\outTEatom{t}{\zeroty}{\evinf}{0}
%%%     \TEIOR \outTEatom{f}{\zeroty}{\evinf}{0})
%%%   \TEPAR
%%%   \outTEatom{t}{\zeroty}{\ev_1}{0}\TOR  \outTEatom{f}{\zeroty}{\ev_1}{0}
%%%     \ET \EOrd \p \outatom{b}{t,f}{\caponly}\PAR 
%%%    \inexp{t}{\zeroty}{\caponly}P+\inexp{f}{\zeroty}{\caponly}Q}
%%%  {\infers{\outTE{b}{\tau_{\BOOL}}{\evig}{2}
%%%    (\outTEatom{t}{\zeroty}{\evinf}{0}
%%%   \TEIOR \outTEatom{f}{\zeroty}{\evinf}{0})\TEPAR
%%%   \inTE{t}{\zeroty}{\ev_1}{0}{\Gamma}\TOR
%%%           \inTE{f}{\zeroty}{\ev_1}{0}{\Gamma}
%%%     \ET \EOrd \p \outatom{b}{t,f}{\caponly}\PAR 
%%%    \inexp{t}{\zeroty}{\caponly}P+\inexp{f}{\zeroty}{\caponly}Q}
%%%  {\outTE{b}{\tau_{\BOOL}}{\evig}{2}
%%%   (\outTEatom{t}{\zeroty}{\evinf}{0}
%%%   \TIOR \outTEatom{f}{\zeroty}{\evinf}{0})\ET \EOrd \p 
%%%       \outatom{b}{t,f}{\caponly}
%%%   \quad \infers{\inTE{t}{\zeroty}{\ev_1}{\Gamma}\TOR
%%%           \inTE{f}{\zeroty}{\ev_1}{0}{\Gamma}\ET \EOrd\p
%%%      \inexp{t}{\zeroty}{\caponly}P+\inexp{f}{\zeroty}{\caponly}Q}
%%%  {\infers{\inTE{t}{\zeroty}{\ev_1}{0}{\Gamma}\ET 
%%%        \EOrd \p \inexp{t}{\zeroty}{\caponly}P}
%%%     {\Gamma\ET \EOrd \p P}\quad
%%%   \infers{\inTE{f}{\zeroty}{\ev_1}{0}{\Gamma}\ET 
%%%        \EOrd \p \inexp{f}{\zeroty}{\caponly}Q}
%%%     {\Gamma\ET \EOrd \p Q}}}}}}}
%%%\]
%%%}
%%%
%%%\(\ev_1\)$B$,(Bfresh$B$J(Bevent$B$H$9$k$H(B
%%%\infrule{\Gamma\ET \EOrd\p P\andalso \Gamma\ET \EOrd \p Q}
%%%  {\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTE{\evig}{\Gamma}\ET \EOrd
%%%       \p \ifexp{b}{P}{Q}}
%%%$B$,$($i$l$k!%$5$i$K$3$N0lHL7A$H$7$F(B
%%%\infrule{\Gamma_1\ET \EOrd\p P\andalso \Gamma_2\ET \EOrd \p Q}
%%%  {\outTEatom{b}{\tau_{\BOOL}}{\evig}{2}\TEPAR
%%%   \evTE{\evig}{\Gamma_1}\TEOR \evTE{\evig}{\Gamma_2} \ET\EOrd
%%%       \p \ifexp{b}{P}{Q}}
%%%$B$bF1MM$K$($i$l$k!%(B
%%%\fi

==> Extension.tex <==
\section{Extensions}
\label{sec:extension}

The type system given so far guarantees that no invalid resource access is performed,
but not that any necessary access is performed eventually; for example,
the type system does {\em not} guarantee that a file is eventually closed.
We discuss extensions of the type system to guarantee such properties.

We are interested in type systems that satisfy either \emph{partial
liveness}\footnote{This is not a standard term; actually, the partial liveness here can be
viewed as the safety property that no `bad' state is reachable such that the necessary
accesses have not yet been performed but the system cannot make any move.} or the stronger
\emph{liveness} property:
\begin{itemize}
\item partial liveness: If \(P\reds Q\) and \(Q\not\red\), then \(Q\) does not
contain any resource to which some access {\em must} be performed.
\item liveness: In any fair reduction sequence \(P\red P_1\red P_2\red \cdots\),
\(P\) eventually performs all the necessary resource access.
(Here, a reduction sequence is fair if an input or output action that is infinitely enabled
will eventually succeed. Without the fairness assumption, no process can satisfy
the liveness property in the presence of a divergent process \(\nuexp{x}(\outatom{x}{\,}{}\PAR
\repexp{\inexp{x}{\,}{}\outatom{x}{\,}{}}\), which is too restrictive.)
\end{itemize}
Our idea is to take the resource type system from the previous sections,
and combine it with some existing system that annotates
those communications that eventually succeed. Specifically, this existing
system might be (1) deadlock-freedom~\cite{Kobayashi00CONCUR,Kobayashi05ActInf},
which guarantees that the annotated communications eventually
succeed unless the process diverges; the combination would then
guarantee partial liveness. Or the existing system
could be (2) lock-freedom~\cite{Kobayashi02IC,Kobayashi05ActInf},
which guarantees that the annotated communications eventually
succeed even in the presence of divergence (assuming a strongly
fair scheduler); the combination would
then guarantee full liveness.

To formally state which resource access {\em must} be performed, we extend the trace sets.
% $\downarrow$ is needed in the formal system, but you could avoid letting users write
%it in some way or another; for example, you could let the user declare a regular expression
%$e$ (which is not prefix-closed), and the system can assume that the actual formal specification
%is the prefix-closure of $e\downarrow$.

\begin{defi}
An {\em extended trace set} is a set of sequences of access labels, possibly ending
with a special label \(\conv\), that is closed under the prefix operation.
\end{defi}
Intuitively, the special label \(\conv\) means that no further resource access
need to be performed.
For example, the trace set \(\prefixclos{\set{C\conv, RC\conv}}\)
means that the close operation needs to be performed, while
\(\prefixclos{\set{\conv, R\conv, C\conv, RC\conv}}\) means that the close operation
need not be performed.

Now we can state the partial liveness property more formally.
We write \(\nuandnur{}\) for a (possibly empty)
sequence of \(\nu\)- and \(\NUR\)-binders.
\begin{defi}
A process \(P\) is \emph{partially live} if
\(\conv\in \spec\) whenever \(P\reds\SPCONG
\nuandnur{}\nurexp{x}{\spec}Q\not\red\).
\end{defi}
%%%The following proposition states that
%%%if a well-typed process has been fully reduced
%%%all necessary accesses to resources has been performed.
%%%\begin{prop}
%%%\label{th:deadlock-freedom}
%%%If \(P\) is well-typed (in an extended type system) and
%%%\(P\red^* \nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%%             (\nurexp{z}{\spec}Q\PAR R)\not\red\), then
%%%\(\epsilon\in \spec\).
%%%\end{prop}

%%%The above proposition does not guarantee that all the necessary
%%%resource accesses will be eventually performed
%%%(since a process may diverge).
%%%The following proposition states that
%%%all the necessary resource accesses will be eventually performed
%%%no matter whether a process diverges.
%%%\begin{prop}[type soundness (liveness)]
%%%\label{th:lock-freedom}
%%%Suppose f \(P\) is well-typed (in an extended type system) and \\
%%%\(P\red^* \nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%%             (\nurexp{z}{\spec}Q_1\PAR Q_2)\), then
%%%for any fair, full reduction sequence
%%%\(\nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%%             (\nurexp{z}{\spec}Q_1\PAR Q_2)\red R_1 \red R_2 \red \cdots\),
%%%there exists \(R_n\) such that
%%%\(
%%%\nuexp{\seq{x}'}\nurexp{\seq{y}'}{\seq{\spec}'}
%%%             (\nurexp{z}{\spec'\cup \set{\epsilon}}Q_1'\PAR Q_2')
%%%\SPCONG R_n\).
%%%\end{prop}
%%%\begin{remark}
%%%For the definition of ``full, fair reduction sequence,''
%%%refer to \cite{Kobayashi02IC}.
%%%Actually, we need to be more careful in stating the above properties
%%%because \(z\) may be renamed because of \(\alpha\)-conversion.
%%%Consult \cite{Kobayashi02IC}.
%%%\end{remark}

\subsection{A Type System for the Partial Liveness Property}

%%%Rather than fully integrating the type system presented so far with
%%%a specific type system for
%%%deadlock-freedom~\cite{Kobayashi98TOPLAS,Kobayashi00CONCUR,Kobayashi05ActInf},
%%%we assume that there is {\em some} type system that guarantees deadlock-freedom
%%%and parameterize the type system for resource usage analysis with the type system
%%%for deadlock-freedom.
%%% nb. There are some overlaps with what we have already said in the beginning of the section.
We extend the syntax of processes to
allow each input and output prefix to be annotated with information about whether the communication
is guaranteed to succeed.
\begin{defi}[(extended) processes]
The set of (extended) processes  is given by:
\[
\begin{array}{lcl}
t \mbox{ (attributes) } &::= & \capable \mid \mayfail\\
P &::= &
     \Exoutexp{x}{\dltag}{y_1,\ldots,y_n}P
\mid \Exinexp{x}{\dltag}{y_1,\ldots,y_n}P
\mid \cdots\\
\end{array}
\]
\end{defi}
The attribute \(\capable\) indicates that when the annotated input or output
operation appears at the top-level, the operation will succeed unless the whole process diverges,
while \(\mayfail\) does not give such a guarantee.
We often omit tag \(\mayfail\).

We assume that there exists a type system guaranteeing that
any well-typed process is {\em well-annotated} in the sense of Definition~\ref{def:wellannot}
below.
There are indeed such type
systems~\cite{Kobayashi98TOPLAS,Kobayashi00CONCUR,Kobayashi05ActInf}.
Moreover, the static analysis tool \texttt{TyPiCal}~\cite{TyPiCal} can
automatically infer the annotations.
\begin{defi} \label{def:wellannot}
\(P\) is {\em active}, written \(\Penabled(P)\), if\\
\(P \SPCONG \nuandnur{}
             (\Exoutexp{x}{\capable}{\seq v}Q \PAR R)\) or
        \(P \SPCONG \nuandnur{}
             (\Exinexp{x}{\capable}{\seq y}Q \PAR R)\).
Additionally, \(P\) is {\em well-annotated}, written \(\wellannot{P}\),
if for any \(P'\) such that \(P\reds P'\) and \(\Penabled(P')\),
there exists \(P''\) such that \(P'\red P''\).
\end{defi}
For example, \(\Exoutexp{x}{\capable}{\,}\zeroexp \PAR
 \Exinexp{x}{\capable}{\,}\Exoutexp{y}{\mayfail}{\,}\zeroexp\)
is well-annotated, but \\
\(\Exoutexp{x}{\capable}{\,}\zeroexp \PAR
 \Exinexp{x}{\capable}{\,}\Exoutexp{y}{\capable}{\,}\zeroexp\)
is not.
Note that \(\Exinexp{x}{\mayfail}{\,}\Exoutexp{x}{\capable}{\,}\zeroexp\) \emph{is}
well-annotated since, although the output never succeeds,
it does not appear at the top-level.

Now we introduce the type system that guarantees the partial liveness.
We extend the behavioral types by extending each input, output, or \(\tau\)-action with
an attribute to indicate whether the action is guaranteed to succeed.
\[
\begin{array}{lcl}
A &::=&
     \ExTout{x}{\dltag}A
\mid \ExTin{x}{\dltag}A
\mid \ExTtau{\dltag}A
\mid \cdots
\end{array}
\]
For example, a process having type \(\ExTout{x}{\capable}\ExTout{x}{\mayfail}\Tzero\) implies that
the process may send values on \(x\) twice, and that the first send is guaranteed to succeed
(i.e., the sent value will be received by some process), while there is no such guarantee for
the second send.

The transition semantics of behavioral types is unchanged;
The attribute \(\dltag\) is just ignored.


%%%\infax[TR-In]{\ExTin{x}{\dltag}A \Tredwith{\ExTinatom{x}{\dltag}} A}
%%%
%%%\infax[TR-Out]{\Tout{x}A \Tredwith{\ExToutatom{x}{\dltag}} A}
%%%
%%%\infrule[TR-Com]
%%%{A_1 \Tredwith{\ExTinatom{a}{\dltag_1}} A_1'  \andalso  A_2 \Tredwith{\ExToutatom{a}{\dltag_2}} A_2'}
%%%{A_1 \TPAR A_2 \Tredsilent A_1' \TPAR A_2'}

% \begin{defi}
% \(\WAITING\) is a predicate defined as follows:
% \begin{itemize}
% \item \(\waiting{\Exoutexp{x}{\capable}{v_1,\ldots,v_n}P}\)
% \item \(\waiting{\Exinexp{x}{\capable}{x_1,\ldots,x_n}P}\)
% \item If \(\waiting{P}\) then \(\waiting{P|Q}\)
% \item If \(\waiting{P}\) then \(\waiting{\nuexp{x}P}\)
% \item If \(\waiting{P}\) then \(\waiting{\nurexp{x}{\spec}P}\)
% \item If \(\waiting{P}\) and \(P \SPCONG Q\) then \(\waiting{Q}\)
% \end{itemize}
% \end{defi}

%% \begin{assumption}
%% Suppose \(P \SPCONG \nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%              (\Exoutexp{x}{\capable}{\seq v}Q \PAR R)\) or
%%         \(P \SPCONG \nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%              (\Exinexp{x}{\capable}{\seq y}Q \PAR R)\)
%% Then, there exists \(Q'\) such that \(P \red Q'\) and
%% \(Q'\) is well-annotated.
%% NB. We need to mention the definition of ``well-annotated''.
%% \end{assumption}

%% We assume that processes and types are correctly annotated
%% by using other analysis.
%% \begin{assumption}
%% Properties of \(\dltag\).
%% \end{assumption}

% \(\enabled{A}{S}\) is a binary predicate which means that

\begin{figure}
%\infrule{}{ \disabled{\Tzero}{S}}
%\rulesp
%\infrule{ \disabled{A}{S} \andalso x\not\in S}
%        {\disabled{\Tacc{\acclab}{x}A}{S}}
%\rulesp
%\infrule{\disabled{A}{S}}
%          {\disabled{\Tact{\cact_{\capable}}A}{S}}
%\rulesp
%\infrule{}
%          {\disabled{\Tact{\cact_{\mayfail}}A}{S}}
%\rulesp
%\infrule{\disabled{A}{S}}
%          {\disabled{\ExTtau{\capable}A}{S}}
%\rulesp
%\infrule{}
%          {\disabled{\ExTtau{\mayfail}A}{S}}
%\rulesp
%\infrule{ \disabled{A_1}{S}\andalso \disabled{A_2}{S}}{\disabled{A_1\TPAR A_2}{S}}
%\rulesp
%\infrule{ \disabled{A_i}{S}\andalso i\in\set{1,2}}{ \disabled{A_1\TOR A_2}{S}}
%\rulesp
%\infrule{\disabled{A}{S}}{\disabled{\Trep{A}}{S}}
%\rulesp
%\infrule{\disabled{A}{S\setdif\set{x}}}{\disabled{\Thiding{x}{A}}{S}}
%\rulesp
%\infrule{\disabled{A}{S\setdif S'}}{\disabled{\exclude{A}{S'}}{S}}
%\rulesp
%\infrule{\disabled{A}{\set{z \mid \subst{\seq x}{\seq y}z\in S}}}
%   {\disabled{\Tren{A}{\seq x}{\seq y}}{S}}
%\rulesp
%\infrule{\disabled{\subst{\Tbvar}{\Trec{\Tbvar}A}}{S}}
%   {\disabled{\Trec{\Tbvar}{A}}{S}}
\fbox{\small
\begin{minipage}{14.5 cm}
\begin{eqnarray*}
 \disabled{\Tzero}{S} \\
 \disabled{\Tacc{\acclab}{x}A}{S} & \mbox{if} & \disabled{A}{S}\ \mbox{and}\ x\not\in S \\
 \disabled{\Tact{\cact_{\capable}}A}{S} & \mbox{if} & \disabled{A}{S} \\
 \disabled{\Tact{\cact_{\mayfail}}A}{S} \\
 \disabled{\ExTtau{\capable}A}{S} & \mbox{if} & \disabled{A}{S} \\
 \disabled{\ExTtau{\mayfail}A}{S} \\
 \disabled{A_1\TPAR A_2}{S} & \mbox{if} & \disabled{A_1}{S}\ \mbox{and}\ \disabled{A_2}{S} \\
 \disabled{A_1\TOR A_2}{S} & \mbox{if} & \disabled{A_1}{S}\ \mbox{or}\ \disabled{A_2}{S} \\
 \disabled{\Trep{A}}{S} & \mbox{if} & \disabled{A}{S} \\
 \disabled{\Thiding{x}{A}}{S} & \mbox{if} & \disabled{A}{S\setdif\set{x}} \\
 \disabled{\exclude{A}{S'}}{S} & \mbox{if} & \disabled{A}{S\setdif S'} \\
 \disabled{\project{A}{S'}}{S} & \mbox{if} & \disabled{A}{S\cap S'} \\
 \disabled{\Tren{A}{\seq x}{\seq y}}{S} & \mbox{if} & \disabled{A}{\set{z \mid \subst{\seq x}{\seq y}z\in S}} \\
 \disabled{\Trec{\Tbvar}{A}}{S} & \mbox{if} & \disabled{\subst{\Tbvar}{\Trec{\Tbvar}A}A}{S}
\end{eqnarray*}
\end{minipage}
}
\caption{The definition of $\disabled{A}{S}$}
\label{fig:disabledness}
\end{figure}

We revise the definitions of the subtype relation and
the traces by using the following predicate \(\disabled{A}{S}\).
Intuitively, this means that
\(A\) describes a process that may get blocked without
accessing any resources in \(S\).
\begin{defi}
%%Let \(A\) be an (extended) behavioral type and \(S\) be a set of
%%variables.
\(\disabled{A}{S}\) is the least binary relation between extended behavioral types
and sets of variables closed under the rules in Figure~\ref{fig:disabledness}.
%%%We write \(\enabled{A}{S}\) when
%%%\(\enabledfun{\emptyset}{A}{S}=\true\), where
%%%\(\enabledfun{F}{A}{S}\) is defined by:
%%%\[
%%%\begin{array}{lcl}
%%%\enabledfun{F}{\Tzero}{S} = \false\\
%%%\enabledfun{F}{\Tbvar}{S} = F(\Tbvar)\\
%%%\enabledfun{F}{\Tacc{\acclab}{x}A}{S} = \true \mbox{ if }x \in S\\
%%%\enabledfun{F}{\Tacc{\acclab}{x}A}{S} = \enabledfun{F}{A}{S} \mbox{ if }x \not\in S\\
%%%\enabledfun{F}{\Tact{\cact_{\capable}}A}{S} = \enabledfun{F}{A}{S}\\
%%%%%\enabledfun{F}{\ExTout{x}{\capable}A}{S} = \enabledfun{F}{A}{S}\\
%%%\enabledfun{F}{\Tact{\cact_{\mayfail}}A}{S} = \false\\
%%%%%\enabledfun{F}{\ExTout{x}{\mayfail}A}{S} = \false\\
%%%\enabledfun{F}{\tau.A}{S} = \enabledfun{F}{A}{S}\\
%%%\enabledfun{F}{A \TPAR A'}{S} = \enabledfun{F}{A}{S} \lor \enabledfun{F}{A'}{S}\\
%%%\enabledfun{F}{A_1 \TOR A_2}{S} = \enabledfun{F}{A_1}{S} \land \enabledfun{F}{A_2}{S}\\
%%%\enabledfun{F}{\Trep{A}}{S} = \enabledfun{F}{A}{S}\\
%%%\enabledfun{F}{\Thiding{x}A}{S} = \enabledfun{F}{A}{S\setdif\set{x}}\\
%%%\enabledfun{F}{\exclude{A}{S}}{S'} = \enabledfun{F}{A}{S' \setdif S}\\
%%%\enabledfun{F}{\Tren{A}{\seq x}{\seq y}}{S} = \enabledfun{F}{A}{\Tren{S}{\seq x}{\seq y}}\\
%%%\enabledfun{F}{\Trec{\Tbvar}A}{S} = \gfp\lambda u.\enabledfun{F\set{\Tbvar\mapsto u}}{A}{S}
%%%\end{array}
%%%\]
%%%Here, \(\gfp\) is the greatest fixed-point operator on the order \(\false \leq \true\).
%%%The function \(F\) in \(\enabledfun{F}{A}{S}\) maps each type variable to
%%%\(\true\) or \(\false\).
\end{defi}

%%%\def\vd#1{\vdash_{#1}}
%%%\begin{figure}
%%%\infax{\Theta \vd{D} \enabled{\Tzero}{S}}
%%%\infax{\Theta, \enabled{\Tbvar}{S} \vd{D} \enabled{\Tbvar}{S}}
%%%\infrule{\Theta, \enabled{\Tbvar}{S}\vd{D} \enabled{A}{S}\andalso D(\Tbvar)=A}
%%%     {\Theta \vd{D} \enabled{\Tbvar}{S}}
%%%\infrule{x\in S}{\Theta\vd{D} \enabled{\Tacc{\acclab}{x}A}{S}}
%%%\infrule{\Theta \vd{D} \enabled{A}{S} \andalso x\not\in S}
%%%        {\Theta \vd{D} \enabled{\Tacc{\acclab}{x}A}{S}}
%%%\infrule{\Theta \vd{D} \enabled{A}{S}}
%%%          {\Theta\vd{D} \enabled{\Tact{\cact_{\capable}}A}{S}}
%%%%%%\infrule{\Theta \vd{D} \enabled{A}{S}}
%%%%%%         {\Theta \vd{D} \enabled{\tau.A}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A_i}{S}\andalso i\in\set{1,2}}{\Theta\vd{D} \enabled{A_1\TPAR A_2}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A_1}{S}\andalso \Theta\vd{D}\enabled{A_2}{S}}{\Theta\vd{D} \enabled{A_1\TOR A_2}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A}{S}}{\Theta\vd{D}\enabled{\Trep{A}}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A}{S\setdif\set{x}}}{\Theta\vd{D}\enabled{\Thiding{x}{A}}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A}{S\setdif S'}}{\Theta\vd{D} \enabled{\exclude{A}{S'}}{S}}
%%%\infrule{\Theta\vd{D} \enabled{A}{\set{z \mid \subst{\seq x}{\seq y}z\in S}}}
%%%   {\Theta \vd{D} \enabled{\Tren{A}{\seq x}{\seq y}}{S}}
%%%\infrule{\Theta, \enabled{\Tbvar}{S} \vd{D\set{\Tbvar\mapsto A}} \enabled{A}{S}}
%%%   {\Theta \vd{D} \enabled{\Trec{\Tbvar}{A}}{S}}
%%%\end{figure}
%
%%%\begin{defi}
%%%% \(\ENABLED\) is the least binary predicate which satisfies the following conditions:
%%%\(\ENABLED\) is a function defined as follows:
%%%\begin{itemize}
%%%\item \(\enabled{\Tacc{\acclab}{x}A}{S} = \true\) if \(x \in S\)
%%%\item \(\enabled{\Tacc{\acclab}{y}A}{S} = \enabled{A}{S}\) if \(y \notin S\)
%%%% \item If \(\enabled{A}{S}\), then
%%%% \begin{itemize}
%%%\item \(\enabled{\ExTin{x}{\capable}A}{S} = \enabled{A}{S}\)
%%%\item \(\enabled{\ExTout{x}{\capable}A}{S} = \enabled{A}{S}\)
%%%\item \(\enabled{A \TPAR A'}{S} = \enabled{A}{S} \vee \enabled{A'}{S}\)
%%%% \item \(\enabled{A' \TPAR A}{S} = \enabled{A}{S}\)
%%%\item \(\enabled{\Thiding{x}A}{S} = \enabled{A}{S}\)
%%%% \end{itemize}
%%%\item \(\enabled{A_1 \TOR A_2}{S} = \enabled{A_1}{S} \wedge \enabled{A_2}{S}\)
%%%\item \(\enabled{\exclude{A}{S}}{S'} = \enabled{A}{S' \setdif S}\)
%%%% \item If \(\enabled{\Tbvar}{x}\) implies \(\enabled{A}{x}\), then \(\enabled{\Trec{\Tbvar}{A}}{x}\)
%%%\item \(\enabled{\Tren{A}{\seq x}{\seq y}}{\Tren{S}{\seq x}{\seq y}} = \enabled{A}{S}\)
%%%\item \(\enabled{\Trec{\Tbvar}A}{S} =  \bigvee \set{ b | b = \enabled{\Tbvar}{S} = \enabled{A}{S}}\)\\
%%%\quad \mbox{where \(\bigvee \emptyset = \false\)}% \GFP(\lambda \Tbvar.\enabled{A}{S})\)
%%%\item \(\enabled{A}{S} = \false\) \mbox{in other cases}
%%%\end{itemize}
%%%\end{defi}
%
%%%By abuse of notations, we write \(\enabled{A}{S}\) for a predicate
%%%which holds when \(\enabled{A}{S} = \false\).
%
%% \begin{lemma}
%% Properties of \(\ENABLED\).
%% \end{lemma}
%
%The trace set \(\traces{x}{A}\) is extended as follows.
\begin{defi}
The set \(\etraces{x}{A}\) of extended traces is:
\[
\begin{array}{l}
\set{\acclab_1\cdots\acclab_n\endtrace | \exists B.
  \project{A}{\set{x}} \Tredsacc{x}{\acclab_1} \cdots \Tredsacc{x}{\acclab_n} B \wedge \converge{B}{\set{x}}} \\
\cup
\set{\acclab_1\cdots\acclab_n | \exists B.
  \project{A}{\set{x}} \Tredsacc{x}{\acclab_1} \cdots \Tredsacc{x}{\acclab_n} B}
\end{array}
\]
\end{defi}
Here,
\(\project{A}{\set{x}} \Tredsacc{x}{\acclab_1} \cdots \Tredsacc{x}{\acclab_n} B \wedge \converge{B}{\set{x}}\)
means that \(\acclab_n\) may be the last access to \(x\), so that
\(\endtrace\) is attached to the sequence \(\acclab_1\cdots\acclab_n\).
By definition, \(\etraces{x}{A}\) is prefix-closed.

%The subtyping relation is refined as follows.
\begin{defi}
\label{def:ex-subtype}
\(A_1 \newsubtype A_2\) is the largest relation on closed behavioral types
that satisfies the following properties:
\begin{itemize}
\item If \(A_1 \Tredwith{l} A_1'\) then there exists \(A_2'\) such that \(A_2 \Tredswith{l} A_2'\) and
      \(A_1' \newsubtype A_2'\).
\item \(\disabled{A_1}{S}\) implies \(\disabled{A_2}{S}\) for any set \(S\) of variables.
\end{itemize}
\end{defi}
Note that by the definition, \(A_1\newsubtype A_2\) implies \(\etraces{x}{A_1}\subseteq \etraces{x}{A_2}\).


The typing rules are the same as those in Section~\ref{sec:typing},
except for the rules shown in Figure~\ref{fig:typing-extension}.
The only changes are that attributes have been attached to
\rname{ET-Out} and \rname{ET-In}, and that
\(\traces{x}{\project{A}{\set{x}}}\) has been replaced by
\(\etraces{x}{\project{A}{\set{x}}}\) in \rname{ET-NewR}.
An important invariant maintained by the typing rules
is that the type of an input/output process is annotated with \(\capable\)
only if the process itself is annotated with \(\capable\).
For example, we cannot derive
\(\etjudge{x\COL\Tchan{}}{\Exoutatom{x}{\mayfail}{\,}{}}{\ExToutatom{x}{\capable}}\).

%nb. Naoki: if we run out of the space, we could move Figure~\ref{fig:typing-extension}
%to Appendix and summarize only the differences from the basic type system.
\iftwocol
\begin{figure}
\else
\begin{figure}
\fi
\begin{center}
\fbox{
\iftwocol
\begin{minipage}{\hfigwidth} %[t]{8cm}
\else
\begin{minipage}{14.5 cm} %{17cm}
\fi
\typicallabel{T-Zero}

%%%\infax[ET-Zero]
%%%            {\etjudge{\Gamma}{\zeroexp}{\Tzero}}
%\rulesp{}
\infrule[ET-Out]
  {\etjudge{\Gamma}{P}{A_2}\andalso
    {\Gamma} \pannot x\COL\Tchan{(\yy\COL\seq{\mvtype})A_1} \\
    \Gamma \pannot \seq{v}\COL{}\seq{\mvtype}}
  {\etjudge{\Gamma}{\Exoutexp{x}{\dltag}{\seq{v}}{}P}{
    \ExTout{x}{\dltag}(\csubst{\seq{y}}{\seq{v}}A_1\PAR A_2)}
     }
\rulesp{}

\infrule[ET-In]
   {\etjudge{\Gamma,
    \seq{y}\COL\seq{\mvtype}}{P}{A_2}\andalso \Gamma \p x\COL{}\Tchan{(\yy\COL\seq{\mvtype})A_1}\\
    \project{A_2}{\set{\seq{y}}}\newsubtype A_1
   }
   {\etjudge{\Gamma}{\Exinexp{x}{\dltag}{\seq y}{}P}{\ExTin{x}{\dltag}(\exclude{A_2}{\set{\seq{y}}})}}
\rulesp{}
%%%\infrule[ET-Par]
%%%   {\etjudge{\Gamma}{P_1}{A_1}\andalso \etjudge{\Gamma}{P_2}{A_2}}
%%%   {\etjudge{\Gamma}{P_1\PAR P_2}{ A_1\TPAR{}A_2}}
%%%%\rulesp{}
%%%\infrule[ET-Rep]
%%%   {\etjudge{\Gamma}{P}{A}}
%%%   {\etjudge{\Gamma}{\repexp{P}}{\Trep{A}}}
%%%
%%%%\rulesp{}
%%%
%%%\infrule[ET-If]
%%%  {\Gamma\pannot v\COL{}\Tbool\andalso
%%%   \etjudge{\Gamma}{P}{A} \andalso \etjudge{\Gamma}{Q}{A}}
%%%  {\etjudge{\Gamma}{\ifexp{v}{P}{Q}}{A}}
%%%%\rulesp{}
%%%

%%%% [Kohei] : I removed ET-New and added ET-NewR because the latter is more
%%%%           interesting than the former.
%% \infrule[ET-New]
%%    {\etjudge{\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}{P}{A_2}
%%     }
%%    {\etjudge{\Gamma}{\nuexp{x}P}{\Thiding{x}A_2}}
%\rulesp{}

%%%\infrule[ET-Acc]
%%%  {\etjudge{\Gamma, x\COL\Tres}{P}{A}}
%%%  {\etjudge{\Gamma, x\COL\Tres}{\accexp{\acclab}{x}P}{\Tacc{\acclab}{x}A}}
%%%
%%%%\rulesp{}
\infrule[ET-NewR]
 {\etjudge{\Gamma, x\COL\Tres}{P}{A}\andalso \etraces{x}{{A}} \subseteq {\spec}}
 {\etjudge{\Gamma}{\nurexp{x}{\spec}P}{\exclude{A}{\set{x}}}}
%%%
%%%\infrule[ET-Sub]
%%%  {\etjudge{\Gamma}{P}{A'}\andalso A'\newsubtype A}
%%%  {\etjudge{\Gamma}{P}{A}}
\end{minipage}
}
\caption{Typing Rules for Partial Liveness}
\label{fig:typing-extension}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi



The following theorem states the soundness of the extended type system.
\begin{thm}
\label{th:partial-liveness}
% If \(P\) is well-typed (in an extended type system) and
If \(\wellannot{P}\) and \(\etjudge{\emptyTE}{P}{A}\), then
 \(P\) is partially live.
%%%\(P\red^* \nuexp{\seq{x}}\nurexp{\seq{y}}{\seq{\spec}}
%%%             (\nurexp{z}{\spec}Q\PAR R)\notred\), then
%%%\(\endtrace\in \spec\).
\end{thm}
\proof
We make use of three lemmas. The first two show that typing and well-annotatedness are preserved by reduction.
The third means that the type of a process properly captures the possibility of the process being blocked.
\begin{itemize}
\item \textbf{Subject reduction.} If \(\etjudge{\Gamma}{P}{A}\) and \(P\redwith{\pact} Q\), then
there exists some \(B\) such that \(\etjudge{\Gamma}{Q}{B}\) and
\(A\Tredswith{\pact} B\). Proof:
See Appendix~\ref{sec:app:subject-reduction}.
%
\item \textbf{Well-annotatedness.} If \(\wellannot{P}\) and \(P\reds\SPCONG Q\), \\ then \(\wellannot{Q}\).
Proof: trivial by definition of\\ $\wellannot{P}$.
%
\item \textbf{Disabled.} If \(\wellannot{P}\) and \(\etjudge{\Gamma}{P}{A}\) with
\(\Tbool\not\in\codom(\Gamma)\), then
\(P\notred\) implies \(\disabled{A}{S}\) for any \(S\).
Proof: See Appendix~\ref{sec:proof-of-partial-liveness}.
\end{itemize}
Now we are ready to prove the theorem. Suppose that
\(P\reds \nuandnur{}\nurexp{x}{\spec}Q\notred\)
and \(\wellannot{P}\), \(\etjudge{\emptyTE}{P}{A}\).
We have to show \(\conv\in \spec\).
By \emph{subject-reduction}
we obtain \(\etjudge{\emptyTE}{\nuandnur{}\nurexp{x}{\spec}Q}{A'}\)
for some \(A'\).
By the inversion of the typing rules,
we get \(\etjudge{\seq{y}\COL\seq{\Tres},\seq{z}\COL\seq{\mvtype},x\COL\Tres}{Q}{B}\)
and \(\traces{x}{B}\subseteq \spec\) for some sequence \(\seq{\mvtype}\) of channel types.
%%%\(\nuexp{\seq{z}}(\exclude{B}{\set{\seq{y},x}})\newsubtype A'\).
(Here, \(\seq{y}\) and \(\seq{z}\) are the variables bound by \(\NUR\).)
%%%and \(\nu\) respectively, and \(\seq{\tau}\) is a sequence of channel types.
By \emph{well-annotatedness}
we also have \(\wellannot{\nuandnur{}\nurexp{x}{\spec}Q}\), which implies
\(\wellannot{Q}\). Thus, by \emph{Disabled},
we get \(\disabled{B}{S}\) for any \(S\),
which implies \(\disabled{\project{B}{\set{x}}}{\set{x}}\).
So, we have \(\conv\in \etraces{x}{B} \subseteq \spec\) as required.
\qed

\begin{exa}
An annotated version of Example~\ref{ex:typing-repeatread}:
%Let us consider Example~\ref{ex:typing-repeatread}. The annotated version of the program:
\[
\begin{array}{rcl}
P &=& \nuexp{s} (\repexp \Exinexp{s}{\capable}{n,x,r} P_1 \PAR \nurexp{x}{\spec} P_2)\\
P_1 &=& \IF\ n=0\ \THEN\ \Exoutatom{r}{\capable}{}\\
    & & \ELSE\ \nuexp{r'}(\Exoutexp{s}{\capable}{n-1,x,r'} \PAR \Exinexp{r'}{\capable}{} \Read(x). \Exoutatom{r}{\capable}{})\\
P_2 &=& \nuexp{r}(\Init(x). \Exoutatom{s}{\capable}{100,x,r} \PAR \Exinexp{r}{\capable}{} \Close(x))\\
\spec &=& \prefixclos{IR^*C\endtrace}
\end{array}
\]
is well-annotated.
%% Let \(A_1 = \mu\alpha.(\ExToutatom{r}{\capable} \TOR \nuexp{r'}(\csubst{r}{r'}\alpha | \ExTin{r'}{\capable}\Tacc{R}{x}\ExToutatom{r}{\capable})\) and
%% let \(\Gamma = s{:}\Tchan{(b{:}\mathbf{int},\, x{:}\Tres,\, r{:}\Tchan{})\,A_1}\). Then
Suppose
\[
\begin{array}{l}
A_1 = \mu\alpha.(\ExToutatom{r}{\capable} \TOR \nuexp{r'}(\csubst{r}{r'}\alpha | \ExTin{r'}{\capable}\Tacc{R}{x}\ExToutatom{r}{\capable})\\
\Gamma = s{:}\Tchan{(b{:}\mathbf{int},\, x{:}\Tres,\, r{:}\Tchan{})\,A_1}.
\end{array}
\]
Then
\[
\begin{array}{rcl}
 & & \tjudge{\Gamma}{P_1}{A_1}\\
 & & \tjudge{\Gamma}{\repexp\Exinexp{s}{\capable}{n,x,r} P_1}{\repexp\ExTin{s}{\capable}(\exclude{A_1}{\{n,x,r\}}) \eqtype \repexp\ExTinatom{s}{\capable}} \\
 & & \tjudge{\Gamma}{P_2}{\nuexp{r}(\Tacc{I}{x}A_1 | \ExTin{r}{\capable}\Taccatom{C}{x})}.\\
\end{array}
\]
So long as \(\etraces{x}{\Thiding{r}(\Tacc{I}{x} A_1 \TPAR \ExTin{r}{\capable} \Tacc{C}{x})} \subseteq \spec\), we obtain \(\tjudge{\emptyset}{P}{\Tzero}\).
\eoe
\end{exa}

\subsection{Type Inference}

The type inference algorithm for the extended type system is almost the same as
the algorithm for the basic type system discussed in Section~\ref{sec:inference}.
The only changes are:
\begin{itemize}
\item In the constraint generaltion algorithm \(\PT\), attribute annotations for
input and ouptut processes are propagated to types. For example, the case for
output processes becomes:
\[
\begin{array}{l}
 \PT(\outexp{x}{\seq{v}}{\dltag}P_0) = \\
\myquad  \PLET\ (\Gamma_i, \mvtype_i) = \PTv(v_i) \\
\myquad\myquad     (\Gamma_0,A_0,C_0) = \PT(P_0)\\
\myquad\myquad  (\Gamma, C) = \Gamma_0 \Tcup (x\COL\Tchan{(\seq{y}\COL{}\seq{\mvtype})\Tbvar})\Tcup
    \Gamma_1\Tcup \cdots \Tcup \Gamma_n\\
\myquad \PIN (\Gamma, \ExTout{x}{\dltag}(\Tsubst{\Tbvar}{\seq{y}}{\seq{v}}\PAR A_0), C)
 \mbox{ (where $\Tbvar$ fresh)}
\end{array}
\]
\item The constraint \(\traces{x}{A}\subseteq \spec\) is replaced by \(\etraces{x}{A}\subseteq \spec\).
\end{itemize}

The second change forces us to adjust the reduction of the constraint to the reachability problem
of Petri nets (recall step 3 of the algorithm in Section~\ref{sec:inference}).
First, we need to use \(\eptraces{\petrinet{A}{x}}\) defined below,
which corresponds to \(\etraces{x}{A}\),
instead of \(\ptraces{\petrinet{A}{x}}\) in the reduction.
\begin{defi}
\(\eptraces{\petrinet{A}{x}}\) is the set
\[ 
\set{\acclab_1 \cdots \acclab_k \mid \Marking_I \Predswith{\acclab_1} \cdots \Predswith{\acclab_k}\Marking'}\\
\cup \set{\acclab_1 \cdots \acclab_k \endtrace \mid \Marking_I \Predswith{\acclab_1} \cdots \Predswith{\acclab_k}\Marking' \wedge \pdisabled{\Marking'}{\set{x}}}
\]
where \(\Marking_I\) is the initial marking of \(\petrinet{A}{x}\).
% The predicate \(\disabled{\Marking}{\set{x}}\) is defined in the similar manner to the definition in Figure~\ref{fig:disabledness}.
\(\pdisabled{\Marking}{S}\) means that \(\disabled{A}{S}\) holds
for the behavioral type \(A\) expressed by \(\Marking\).
\end{defi}
Second, the construction of an automaton needs to be adjusted
so that it accepts extended traces.
% For example, the automaton of Step 3-2 in Section~\ref{sec:inference} is
For example, the automaton used in the explanation of Step 3-2 
in Section~\ref{sec:inference} is
replaced by the one that accepts \(IR^{*}C\endtrace\).

With these changes, the validity of a constraint \(\etraces{x}{A}\subseteq \spec\)
is reduced to the reachability problem of a Petri net \(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\)
where composition of a Petri net \(\petrinet{A}{x}\) and an automaton \(\automaton{\spec}\)
is defined in the same manner as Definition~\ref{def:composition-petrinet}.
\begin{thm}
\label{le:petrinet-reachability-extended}
\(\eptraces{\petrinet{A}{x}} \subseteq {\spec}\)
if and only if no marking \(\Marking\PPAR q\) that satisfies the following conditions is reachable:
\begin{itemize}
\item \(\pdisabled{\Marking}{\set{x}}\).
% \item \(q\) is not an accepting state.
\item \(\trans{\spec}(q, \endtrace)\) is undefined.
\end{itemize}
\end{thm}

%% \finish{Summarize the main change: redefine ptraces as petraces, adjust the construction of an 
%% automaton (so that it accepts \(\downarrow\)), and state a theorem corresonding to Theorem 4.4}


==> General-Soundness.tex <==
\subsection{General Type Soundness Theorem}
\label{sec:general-soundness}


%%%\paragraph{$BLdBjE@(B}
%%%$B<+M3JQ?t$K4X$9$k@)8B$N=|5n$K$h$j!$(B
%%%\verb|(nu x)(nu y)P| $B$H(B\verb|(nu y)(nu x)P|
%%%$B$N7?IU$1$OF1$8$G$J$/$J$C$?!%(B
%%%$B$=$N$?$a!"(BCorollary 4.2.17$B$N>ZL@$O$^$:$$!%(B
%%%
%%%\paragraph{$B2~A1J}K!(B}
%%%formula A $B$N0UL#$r!$!V$I$N%A%c%M%k$KCmL\$7$F$$$k$+!J$"$k$$$O(B
%%%$B$I$N%A%c%M%k$r<+M3$H$_$J$9$+!K$N=89g(BS$B!W$K$h$C$F(Bparameterize$B$9$k!%(B
%%%$B$=$l$KH<$$!$(B
%%%\begin{itemize}
%%%\item Def.4.2.8 and 4.2.9$B$NJQ99!J(Bx!, x?, $B$*$h$S%i%Y%k$D$-(Btransition$B!K(B
%%%\item Def.4.2.12$B$NJQ99!JG$0U$NL58B=89g(BS$B$K$D$$$F!"$H$$$&>r7o$rIU2C!K(B
%%%\item $B$=$l$KH<$&(BLem 4.2.13$B$NJQ99(B
%%%\item $BJdBj$H$7$F!"(B
%%%\begin{verbatim}
%%%-  D \in A^{S\x} and A positive => D|x \in A
%%%-  D|x \in A and A negative => D \in A^{S\x}
%%%- P \in B^{S\x} <=> (nu x)Q |= B?
%%%\end{verbatim}
%%%\end{itemize}
%%%

In Section~\ref{sec:soundness-basic}, we have shown that a
process satisfies a certain property \(p\) if its process type
satisfies the {\em corresponding} consistency condition \(\reliable\).
However, it is left to the designer of
a specific type system to find a consistency
condition that {\em corresponds to} a process property of interest and
prove that the correspondence is indeed correct.
%%%In fact, in Section~\ref{sec:application},
%%%we had to find a suitable consistency condition on process types
%%%and prove its correctness (Theorem~\ref{thm:correctness-of-app})
%%%for each type system.
There also remains a general question 
about the power of our generic type system: 
What kind of type system can be obtained as an instance?
%%what kind of property of a process can be verified by analyzing
%%%its process type? 
Clearly, not all properties can be verified in our
type system: For example, the property ``a process can create
at most \(n\) channels'' cannot be verified, because process types
does not carry information about channel creation.
This section gives a partial answer to those questions: 
For a certain class of properties of processes, there is indeed 
a systematic way for obtaining the corresponding consistency condition
\(\reliable\) on process
types, so that the instantiated type system is sound.
%%%For lack of space, details are omitted: They
%%%are found in the full paper~\cite{Kobayashi00TR:Unifying}.

We first introduce logical formulas~\cite{Stirling96,Cardelli00POPL}
 to formally state properties of processes and types.
\begin{defn}
\iffull
The set \(\FSET\) of formulas is given by the following syntax:
\else
The set \(\FSET\) of formulas is given by the following syntax
(\(i,j\) denote variables ranging over the set \(\Nat\) of
non-negative integers and \(n\) denotes a non-negative integer or 
a variable ranging over \(\Nat\)):
\fi
\[
\begin{array}{lcll}
A &::=& \PLTRUE  \mid \PLout{x}{\ev}{n}\mid  \PLin{x}{\ev}{n}
       \mid (A\PAR B)\mid \PLsometr{\redlab}A\mid \eventual(A)\\
  & &  \mid \neg A \mid A\lor B  \mid \exists x.A \mid
      \exists \ev.A \mid \exists \ivar\COL{}C.A\\
C &::=& \{m_1\neq n_1,\ldots,m_k\neq n_k\}
\end{array}
\]
\iffull
Here, the meta-variable \(\ivar\) ranges over the set \(\IVAR\) of
variables (called {\em integer variables}), 
disjoint from \(\VAR\). The meta-variables \(n, m_i,n_i\) range
over the union of the set \(\IVAR\) and the set \(\Nat\) of
non-negative integers.  We often abbreviate \(\neg (\neg A \lor \neg B)\) to
\(A \land B\).
\fi
\end{defn}

A formula \(A\) describes a property of both processes and types.
Intuitively, \(\PLout{x}{\ev}{n}\) means that some sub-process is ready to
output an \(n\)-tuple on the channel \(x\) and that the output is tagged with
\(\ev\). Similarly, \(\PLin{x}{\ev}{n}\) means that some sub-process
is ready to input an \(n\)-tuple. A formula \(A\PAR B\) means that
the process is parallel composition of a process satisfying \(A\) and
another process satisfying \(B\). A formula \(\PLsometr{\redlab}A\) means that 
the process can be reduced in one step to a process satisfying \(A\) and 
that the reduction is labeled with \(l\). A formula \(\eventual(A)\) means that
the process can be reduced to a process satisfying \(A\)
in a finite number of steps.\footnote{It is possible to introduce a general
fixed-point operator~\cite{Stirling96} instead, but we did not do so in this paper
for simplicity.}
\iffull
For example, the formula
  \[\neg \exists \ev,\ev'.\exists \ivar_1,\ivar_2\COL\emptyset.\eventual(
 \PLout{x}{\ev}{\ivar_1} \PAR \PLout{x}{\ev'}{\ivar_2})\]
means that no two processes try to output a value on \(x\) simultaneously.
\fi

\iffull
We define the formal semantics of formulas below.
As usual, \(\exists x.A\), \(\exists \ev.A\), and
\(\exists \ivar\COL{}C.A\) bind \(x\), \(\ev\), and \(\ivar\) respectively. 
We write \(\FIV(A)\) for the set of free integer variables in \(A\).
We define substitutions for variables, events, and integer variables in
a customary manner. For example, \(\subst{\ivar}{n}A\) denotes the formula
obtained from \(A\) by substituting \(n\) for all free occurrences of \(\ivar\).
We write \(\FV(A)\) for the set of free variables (in \(\VAR\)), and
\(\FIV(A)\) for the set of free integer variables (in \(\IVAR\)).
\begin{defn}
The size of a formula \(A\), written \(\size(A)\), is defined by:
\[
\begin{array}{l}
\size(\PLTRUE) = \size(\PLout{x}{\ev}{n})=\size(\PLin{x}{\ev}{n})=1\\
\size(A\PAR B)=\size(A\lor B) = \size(A)+\size(B)+1\\
\size(\PLsometr{\redlab}A)=\size(\eventual(A))=\size(\neg A)=
  \size(\exists x.A)=
      \size(\exists \ev.A)=\size(\exists \ivar\COL{}C.A)=\size(A)+1
\end{array}
\]
\end{defn}
\fi

We define the semantics \(\semPF{A}\) 
of a formula \(A\) as the set of processes satisfying \(A\).
To define it, we introduce an auxiliary function \(\semPFaux{A}{S}\),
which denotes the set of processes satisfying \(A\) provided that all channels
in \(S\) are invisible.
\begin{defn}
Let \(A\) be a formula such that \(\FIV(A)=\emptyset\), and
let \(S\) be a finite set of variables.
The sets \(\semPF{A}\) and \(\semPFaux{A}{S}\) of processes are defined by
(\(\PSET\) is the set of processes):
\begin{eqnarray*}
\semPF{A} &=& \semPFaux{A}{\emptyset}\\
\semPFaux{\PLTRUE}{S} &=& \PSET\\
\semPFaux{\PLout{x}{\ev}{n}}{S} &=& 
   \{P \mid  P\SPCONG \nuexpbseq{x}{1}{k} 
            (\cdots+\outexp{x}{\seq y}{\ev}Q+\cdots\PAR R),
              x\not\in S\cup \set{\seq{x_1},\ldots,\seq{x_k}}, \seqlen{\seq y}=n\}\\
\semPFaux{\PLin{x}{\ev}{n}}{S} &=& 
    \{P \mid 
    P\SPCONG \nuexpbseq{x}{1}{k}(\cdots+\inexp{x}{\seq y}{\ev}Q+\cdots \PAR R),
    x\not\in S\cup \set{\seq{x_1},\ldots,\seq{x_k}}, \seqlen{\seq y}=n\}\\
\semPFaux{A\PAR B}{S} &=& 
    \{P \mid P\SPCONG \nuexpbseq{x}{1}{k}(Q\PAR R), 
     Q\in\semPFaux{A}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}},
     R\in\semPFaux{B}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}}\}\\
\semPFaux{\PLsometr{\redlab}A}{S} &=& 
  \set{P \mid P\redwith{\redlab'}Q, \redlab = \restrictL{\redlab'}{S}, Q\in \semPFaux{A}{S}}\\
\semPFaux{\eventual(A)}{S} &=& \set{P \mid P\red^* Q, Q\in \semPFaux{A}{S}}\\
\semPFaux{\neg A}{S} &=& \PSET\setdif \semPFaux{A}{S}\\
\semPFaux{A\lor B}{S} &=& \semPFaux{A}{S}\cup \semPFaux{B}{S}\\
\semPFaux{\exists x.A}{S} &=& \bigcup_{y\in \VAR}\semPFaux{[y/x]A}{S}\\
\semPFaux{\exists \ev.A}{S} &=& \bigcup_{\ev'\in \EVSET}\semPFaux{[\ev'/\ev]A}{S}\\
\semPFaux{\exists \ivar\COL{}C.A}{S} &=& 
   \{P \mid P\in\semPFaux{\subst{\ivar}{n}A}{S}, n\in \Nat, \models \subst{\ivar}{n}C\}
\end{eqnarray*}
Here, \(\models C\) means that all the inequalities \(i \neq
j\) hold.   We write \(P \models A\) when \(P\in \semPF{A}\) holds.
\end{defn}
It is easy to prove that \(\semPF{A}\) and \(\semPFaux{A}{S}\) are well defined,
by induction on the size of \(A\).

We show some properties of \(\semPFaux{A}{S}\).
\begin{lemma}
\label{lem:red-normal-derivation}
If \(\nuexp{\seq x}P\redwith{l}Q\), then there exists \(Q'\) such that
\(P\redwith{l'} Q'\) with
 \(\nuexp{\seq x}Q'\SPCONG Q\) and \(\restrictL{l'}{\set{\seq x}} = l\).
\end{lemma}
\begin{proof}
This follows by straightforward induction on derivation of 
\(\nuexp{\seq x}P\redwith{l}Q\).
\end{proof}
\begin{lemma}
\label{lem:sempf-closed-under-spcong}
If \(P\SPCONG Q\), then \(P\in \semPFaux{A}{S}\) if and only if \(Q\in \semPFaux{A}{S}\).
\end{lemma}
\begin{proof}
This lemma follows by induction on the size of \(A\).
\end{proof}
\begin{lemma}
\label{lem:semPF-restriction}
Suppose that \(P\in \PSET\), \(A\in \FSET\), and \(S\cup \set{\seq x}\subseteq \VAR\).
Suppose also that \(S\cap \set{\seq x}=\emptyset\).
Then, \(\nuexp{\seq x}P \in \semPFaux{A}{S}\) holds if and only if
  \(P\in \semPFaux{A}{S\cup \set{\seq x}}\) holds.
\end{lemma}
\begin{proof}
The proof proceeds by induction on the size of \(A\).
We show only main cases; The other cases are similar or trivial.
\begin{itemize}
\item Case \(A=\PLout{x}{\ev}{n}\): the required property follows by:
\[
\begin{array}{lcl}
\nuexp{\seq x}P\in \semPFaux{A}{S} 
&\IFF &
 ( \nuexp{\seq x}P \SPCONG \nuexp{\seq x}\nuexpbseq{x}{1}{k} 
            (\cdots+\outexp{x}{\seq y}{\ev}Q+\cdots\PAR R))\\
 & & \land 
        (x\not\in S\cup \set{\seq x}\cup \set{\seq{x_1},\ldots,\seq{x_k}})\land
    \seqlen{\seq y}=n\\
&\IFF &
 ( P \SPCONG \nuexpbseq{x}{1}{k} 
            (\cdots+\outexp{x}{\seq y}{\ev}Q+\cdots\PAR R))\\
 & & \land 
        (x\not\in S\cup \set{\seq x}\cup \set{\seq{x_1},\ldots,\seq{x_k}})\land
    \seqlen{\seq y}=n\\
 &\IFF& P \in \semPFaux{A}{S\cup \set{\seq x}}\\
\end{array}
\]
\item Case \(A=A_1\PAR A_2\): the required property follows by:
\[
\begin{array}{lcl}
\nuexp{\seq x}P\in \semPFaux{A}{S} 
 &\IFF &
 \nuexp{\seq x} P \SPCONG \nuexp{\seq x}\nuexpbseq{x}{1}{k}
            (P_1\PAR P_2)\\
 & &\land
            P_1\in \semPFaux{A_1}{S\cup\set{\seq{x}}\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\land
            P_2\in \semPFaux{A_2}{S\cup\set{\seq{x}}\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\\
 &\IFF &
  P \SPCONG \nuexpbseq{x}{1}{k}
            (P_1\PAR P_2)\\
 & &\land
            P_1\in \semPFaux{A_1}{S\cup\set{\seq{x}}\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\land
            P_2\in \semPFaux{A_2}{S\cup\set{\seq{x}}\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\\
 &\IFF& P \in \semPFaux{A}{S\cup \set{\seq x}}\\
\end{array}
\]
\item Case \(A=\PLsometr{\redlab}B\): 
Suppose \(\nuexp{\seq x}P\in \semPFaux{A}{S}\). Then, there exists
 \(Q\) such that 
\(\nuexp{\seq x}P\redwith{\redlab'}Q\) with \(\restrictL{\redlab'}{S}=\redlab\) and 
\(Q\in \semPFaux{B}{S}\). By Lemma~\ref{lem:red-normal-derivation}, there exists
\(Q'\) such that \(P\redwith{\redlab''} Q'\) with \(\nuexp{\seq x}{Q'}\SPCONG Q\)
and \(\restrictL{\redlab''}{\set{\seq x}} = \redlab'\).
By Lemma~\ref{lem:sempf-closed-under-spcong} and \(Q\in \semPFaux{B}{S}\), we have 
\(\nuexp{\seq x}Q'\in \semPFaux{B}{S}\). 
By induction hypothesis, we have \(Q'\in \semPFaux{B}{S\cup \set{\seq x}}\).
Since \(\restrictL{\redlab''}{S\cup\set{\seq x}} = \restrictL{\redlab'}{S} = \redlab\),
we have \(P\in \semPFaux{A}{S\cup\set{\seq x}}\) as required.

On the other hand, suppose \(P\in \semPFaux{A}{S\cup \{\seq x\}}\), with
\(S\cap \set{\seq x}=\emptyset\).
Then, there exists \(Q\) and \(\redlab'\) such that 
\(P\redwith{\redlab'} Q\) with \(\restrictL{\redlab'}{S\cup\set{\seq x}}=\redlab\)
and \(Q\in \semPFaux{B}{S\cup \set{\seq x}}\). 
By rule \rname{R-New}, we have 
\(\nuexp{\seq x}P\redwith{\restrictL{\redlab'}{\set{\seq x}}} \nuexp{\seq x}{Q}\).
By applying the induction hypothesis to \(Q\in \semPFaux{B}{S\cup \set{\seq x}}\), 
we obtain \(\nuexp{\seq x}{Q}\in \semPFaux{B}{S}\).
Since \(\restrictL{(\restrictL{\redlab'}{\set{\seq x}})}{S} = 
\restrictL{\redlab'}{S\cup\set{\seq x}}=\redlab\), we have
\(\nuexp{\seq x}P\in \semPFaux{A}{S}\) as required.
\endofpf
\end{itemize}
\end{proof}

A formula is interpreted also as a property of process types
(\(\TSET\) is the set of process types):
\begin{defn}
Let \(A\) be a formula such that \(\FIV(A)=\emptyset\), and
The set \(\semTF{A}\) and \(\semTFaux{A}{S}\) of process types are defined by:
\begin{eqnarray*}
\semTF{\PLTRUE} &=& \TSET\\
\semTF{\PLout{x}{\ev}{n}} &=& \set{\Gamma \mid
    \Gamma\subTE \cdots+\OutTE{x}{\tau}{\ev}\Delta_1+\cdots\TEPAR \Delta_2,
    \arity{\tau}=n}\\
\semTF{\PLin{x}{\ev}{n}} &=& \set{\Gamma \mid 
    \Gamma\subTE \cdots+\InTE{x}{\tau}{\ev}\Delta_1+\cdots\TEPAR \Delta_2,
    \arity{\tau}=n}\\
\semTF{A\PAR B} &=& \set{\Gamma \mid 
   \Gamma\subTE (\Delta_1\TEPAR\Delta_2), \Delta_1\in \semTF{A}, 
   \Delta_2\in \semTF{B}}\\
\semTF{\PLsometr{\redlab}A} &=& 
   \set{\Gamma \mid \Gamma\redwith{\labPtoT{\redlab}}\Delta, 
                                    \Delta\in \semTF{A}}\\
\semTF{\eventual(A)} &=& \set{\Gamma \mid \Gamma\red^* \Delta, 
  \Delta\in \semTF{A}}\\
\semTF{\neg A} &=& \TSET\setdif \semTF{A}\\
\semTF{A\lor B} &=& \semTF{A}\cup \semTF{B}\\
\semTF{\exists x.A} &=& \bigcup_{y\in \VAR}\semTF{[y/x]A}\\
\semTF{\exists \ev.A} &=& \bigcup_{\ev'\in \EVSET}\semTF{[\ev'/\ev]A}\\
\semTF{\exists \ivar\COL{}C.A} &=& 
   \{\Gamma \mid \Gamma\in\semTF{\subst{\ivar}{n}A}, 
                     n\in \Nat, \models \subst{\ivar}{n}C\}\\
\semTFaux{A}{S} &=& \set{\Gamma \mid \exclude{\Gamma}{S}\in \semTF{A}}
\end{eqnarray*}
We write \(\Gamma \models A\) when \(\Gamma\in \semTF{A}\) holds.
\end{defn}
%%%\begin{lemma}
%%%If \(\Gamma\in \semTF{A}\) and \(S\cap \FV(A)=\emptyset\), then
%%%\(\exclude{\Gamma}{S}\in \semTF{A}\).
%%%\end{lemma}
%%%\begin{pf}
%%%THIS IS FALSE!. Consider \(\OutTEatom{x}{\,}{\ev}\in \exists x.\PLout{x}{0}{\ev}\).
%%%\end{pf}

\iffull
To formally define what property of process types {\em corresponds to} a property
of processes, we introduce two binary relations on formulas.
\begin{notation}
We write \(\GS(A)\) for the set of substitutions that map
all the free integer variables in \(A\) to non-negative integers.
\end{notation}

%%%\begin{notation}
%%%\finish{The following notation is no longer necessary?}
%%%We write \(\tjudge{\reliable}{\Gamma}{P}\) when we want to explicitly state
%%%the consistency condition used in the derivation. For example, 
%%%\(\tjudge{\wf}{\Gamma}{P}\) means that \(\Gamma\p P\) is derivable for
%%%\(\reliable=\wf\).
%%%\end{notation}
\begin{defn}
Binary relations \(\TFtoPF\) and \(\PFtoTF\) on formulas are defined by:
\begin{eqnarray*}
A \TFtoPF B &\IFF& \forall \Gamma\in\TSET, P\in\PSET, S\subseteq \VAR, 
   \theta\in \GS(A\PAR B)\\
%%%  & &\myquad   ((\typing{\wf}{\Gamma}{P} 
%%%                       \land \wf(\Gamma)\land \Gamma\in \semTF{\theta A})\imply
%%%          P\in \semPF{\theta B})\\
  & &\myquad   ((\typing{\wf}{\Gamma}{P}
                       \land \wf(\Gamma)\land \Gamma\in \semTFaux{\theta A}{S})\imply
          P\in \semPFaux{\theta B}{S})\\
A \PFtoTF B &\IFF& \forall \Gamma\in\TSET, P\in\PSET, S\subseteq \VAR, \theta\in \GS(A\PAR B).\\
  & &\myquad ((\typing{\wf}{\Gamma}{P} \land \wf(\Gamma)\land P\in \semPFaux{\theta A}{S})\imply
          \Gamma\in \semTFaux{\theta B}{S})\\
\end{eqnarray*}
\end{defn}
Intuitively, \(A\TFtoPF B\) means that if a process type satisfies the property \(A\),
every process of that type satisfies the property \(B\). 
Conversely, \(A\PFtoTF B\) means that
if a process satisfies \(A\), its type satisfies \(B\).

We obtain sound inference rules to derive the relations
\(A \TFtoPF B\) and \(A\PFtoTF B\) as shown 
in Figure~\ref{fig:property-logic}. 
We have also standard logical rules like:
\[
\begin{minipage}{7cm}
\infrule{A \TFtoPF B}{A \TFtoPF B\lor C}
\end{minipage}
\begin{minipage}{7cm}
\infrule{A \TFtoPF C\andalso B\TFtoPF C}{A\lor B \TFtoPF C}
\end{minipage}
\]

\begin{figure}
\begin{center}
\fbox{
\begin{minipage}{16cm}
\infax[F-Out]{\PLout{x}{\ev}{n} \PFtoTF \PLout{x}{\ev}{n}}
\rulesp{}
\infax[F-In]{\PLin{x}{\ev}{n} \PFtoTF \PLin{x}{\ev}{n}}
\rulesp{}
\infrule[F-Red]{A\PFtoTF B}{\PLsometr{l}A \PFtoTF \PLsometr{l}B}
\rulesp{}
\infrule[F-Ev]{A\PFtoTF B}{\eventual(A) \PFtoTF \eventual(B)}
\rulesp{}
\infrule[F-Par]{A_1 \PFtoTF B_1\andalso A_2\PFtoTF B_2}
      {A_1\PAR A_2\PFtoTF B_1\PAR B_2}
\rulesp{}
\infrule[F-Neg1]{A\TFtoPF B}{\neg B\PFtoTF \neg A}
\rulesp{}
\infrule[F-Neg2]{A\PFtoTF B}{\neg B \TFtoPF \neg A}
\end{minipage}
}
\caption{Inference Rules for Proving $A\TFtoPF B$ and $A\PFtoTF B$}
\label{fig:property-logic}
\end{center}
\end{figure}

The soundness of inference rules is proved as follows.
\begin{lemma}
\label{lem:soundness-of-logic}
The inference rules in Figure~\ref{fig:property-logic} are sound.
\end{lemma}
\begin{pf}
Without loss of generality, we can assume that formulas do not
contain free integer variables.
The soundness of the rules \rname{F-Out} and \rname{F-In}
follow immediately from Corollary~\ref{cor:normal-derivation}.

To show the soundness of \rname{F-Red}, suppose
that \(A\PFtoTF B\), \(P\in \semPFaux{\PLsometr{l}{A}}{S}\), and
\(\typing{\wf}{\Gamma}{P}\). By \(P\in \semPFaux{\PLsometr{l}{A}}{S}\),
there must exist \(Q\) and \(l'\) such that \(P\redwith{l'}Q\) with
\(\restrictL{l'}{S} = l\) and \(Q\in\semPFaux{A}{S}\).
By Theorem~\ref{thm:subject-reduction}, there exists \(\Delta\) such that
\(\Gamma \TEredwith{\labPtoT{l'}}\Delta\) and \({\Delta}\p {Q}\). 
By Lemma~\ref{lem:exclude-TEcom} in Appendix, we have
\(\exclude{\Gamma}{S}\TEredwith{\labPtoT{l}}\exclude{\Delta}{S}\).
By the assumption
\(A\PFtoTF B\), we have \(\Delta\in \semTFaux{B}{S}\), that is,
\(\exclude{\Delta}{S}\in \semTF{B}\). 
So, we have \(\exclude{\Gamma}{S}\in \semTF{\PLsometr{l}{B}}\),
that is, \(\Gamma\in \semTFaux{\PLsometr{l}{B}}{S}\) as required.
The soundness of \rname{F-Ev} follows similarly.

To show the soundness of \rname{F-Par}, suppose
\(A_1\PFtoTF B_1\), \(A_2\PFtoTF B_2\), \(P\in \semPFaux{A_1\PAR A_2}{S}\),
and \(\typing{\wf}{\Gamma}{P}\) 
with \(\wf(\Gamma)\). By the assumption \(P\in \semPFaux{A_1\PAR A_2}{S}\),
there exists \(P_1, P_2, \seq{x_1},\ldots,\seq{x_k}\) such that
\[
\begin{array}{l}
P \SPCONG \nuexpbseq{x}{1}{k}(P_1\PAR P_2)\\
P_1\in \semPFaux{A_1}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}}\\
P_2\in \semPFaux{A_2}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}}
\end{array}
\]
%%%By Lemma~\ref{lem:semPF-restriction}, we have
%%%\[
%%%\begin{array}{l}
%%%\nuexpbseq{x}{1}{k}P_1\in \semPFaux{A_1}{S\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\\
%%%\nuexpbseq{x}{1}{k}P_2\in \semPFaux{A_2}{S}
%%%\end{array}
%%%\]
By Lemma~\ref{lem:typing-closed-under-spcong}, we have
\(\Gamma\p {\nuexpbseq{x}{1}{k}(P_1\PAR P_2)}\).
By Theorem~\ref{thm:normal-derivation}, we have
\[
\begin{array}{l}
\typing{\wf}{\Delta_1}{P_1}\\
\typing{\wf}{\Delta_2}{P_2}\\
\Gamma\subTE \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}} \TEPAR
              \exclude{\Delta_2}{\set{\seq{x_1},\ldots,\seq{x_n}}}\\
\wf(\project{(\Delta_1\PAR\Delta_2)}{\set{\seq x_i}}) \mbox{ for }i=1,\ldots,k\\
%%%\FV(\exclude{(\Delta_1\PAR\Delta_2)}{\set{\seq{x_i},\ldots,\seq{x_k}}})\cap\set{\seq{x_i}}
%%%    =\emptyset \mbox{ for }i=1,\ldots,k\\\\
%%%\Gamma_k = \Delta_1\PAR\Delta_2\\
%%%\Gamma_{i-1}=\exclude{\Gamma_i}{\set{\seq{x_i}}}\mbox{ for }i=1,\ldots,k\\
%%%\reliable(\project{\Gamma_i}{\set{\seq{x_i}}}) \mbox{ for }i=1,\ldots,k\\
%%%\Gamma \subTE \Gamma_0
%%%\exclude{(\Delta_1\TEPAR\Delta_2)}{\set{\seq{x_1},\ldots,\seq{x_k}}}
%%%           (= \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_k}}}
%%%             \TEPAR \exclude{\Delta_2}{\set{\seq{x_1},\ldots,\seq{x_k}}})
\end{array}
\]
Note that \(\wf(\Delta_1)\) and \(\wf(\Delta_2)\) follows from the last two conditions and
\(\wf(\Gamma)\). 
So, by the assumptions 
\(A_1\PFtoTF B_1\) and \(A_2\PFtoTF B_2\), we have
\(\Delta_1 \in \semTFaux{B_1}{S\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\)
and 
\(\Delta_2 \in \semTFaux{B_2}{S\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\),
which implies 
\(\exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}} \in \semTFaux{B_1}{S}\)
and 
\(\exclude{\Delta_2}{\set{\seq{x_1},\ldots,\seq{x_n}}} \in \semTFaux{B_2}{S}\).
By 
\(\Gamma\subTE \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}} \TEPAR
              \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}}\), 
we have \(\Gamma\in \semTFaux{B_1\PAR B_2}{S}\) as required.
%%%From the last two conditions and the assumption \(\wf(\Gamma)\), 
%%%we get \(\wf(\Delta_1)\) and \(\wf(\Delta_2)\).
%%%Therefore, by the assumptions 
%%%\(A_1\PFtoTF B_1\) and \(A_2\PFtoTF B_2\), 
%%%we have \(\Delta_1 \in \semTFaux{B_1}{S\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\)
%%%and  \(\Delta_2 \in \semTFaux{B_2}{S\cup\set{\seq{x_1},\ldots,\seq{x_k}}}\).
%%%By Lemma~\ref{lem:semTF-restriction}, 
%%%we have \(\exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_k}}} \in \semTFaux{B_1}{S}\)
%%%and \(\exclude{\Delta_2}{\set{\seq{x_1},\ldots,\seq{x_k}}} \in \semTFaux{B_2}{S}\).
%%%Since \(\Gamma\subTE \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}} \TEPAR
%%%              \exclude{\Delta_1}{\set{\seq{x_1},\ldots,\seq{x_n}}}\), 
%%%we have \(\Gamma\in \semTFaux{B_1\PAR B_2}{S}\) as required.
%%%
%%%By the assumptions 
%%%By the condition \(\wf(\project{\Gamma_i}{\set{\seq{x_i}}})\), we have
%%%\(\wf(\project{\Delta_{ji}}{\set{\seq{x_i}}})\) 
%%%for 
%%%\(j\in\{1,2\}, i\in\{1,\ldots,k\})\). So, by repeatedly applying \rname{T-New}
%%%By the assumptions \(A_1\PFtoTF B_1\) and \(A_2\PFtoTF B_2\),
%%%we have:
%%%\[
%%%\begin{array}{l}
%%%\Delta_1\in \semPF{B_1}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}\\
%%%\Delta_2\in \semPF{B_2}{S\cup \set{\seq{x_1},\ldots,\seq{x_k}}
%%%\end{array}
%%%\]
%%%
%%%Let us define \(\Delta_{ij} (i\in\{1,2\}, j\in\{0,\ldots,k\})\) by:
%%%\[
%%%\begin{array}{l}
%%%\Delta_{ik} =\Delta_i\\
%%%\Delta_{ij-1} = \exclude{\Delta_{ij}}{\set{\seq{x_j}}}\mbox{ for }i=1,\ldots,k\\
%%%\end{array}
%%%\]
%%%Then, we have \(\Gamma_i = \Delta_{1i}\PAR \Delta_{2i}\).
%%%By the condition \(\wf(\project{\Gamma_i}{\set{\seq{x_i}}})\), we have
%%%\(\wf(\project{\Delta_{ji}}{\set{\seq{x_i}}})\) 
%%%for 
%%%\(j\in\{1,2\}, i\in\{1,\ldots,k\})\). So, by repeatedly appying \rname{T-New}
%%%to \(\Delta_i\p P_i\), we obtain 
%%%\(\tjudge{\wf}{\Delta_{i0}}{\nuexpbseq{x}{1}{k}P_i}\) for \(i=1, 2\).
%%%By applying induction hypothesis to \(A_i\PFtoTF B_i\), we obtain
%%%\(\Delta_{i0}\in \semTF{B_i}\). Finally, since
%%%\(\Gamma\subTE\Gamma_0 = \Delta_{00}\TEPAR\Delta_{10}\), we get
%%%\(\Gamma\in \semTF{B_1\PAR B_2}\).

To show the soundness of \rname{F-Neg1}, suppose 
that \(A\TFtoPF B\), \(P\in \semPFaux{\neg B}{S}\), and
\({\Gamma}\p {P}\). It suffices to show \(\Gamma\not\in \semTFaux{A}{S}\).
Suppose \(\Gamma\in \semTFaux{A}{S}\). Then, by \(A\TFtoPF B\), it must be the case
that \(P\in\semPFaux{B}{S}\). But this contradicts with the assumption
\(P\in \semPFaux{\neg B}{S}= \PSET\setdif \semPFaux{B}{S}\).
The proof of the soundness of \rname{F-Neg2} is similar.
\end{pf}
\fi

By using Lemma~\ref{lem:soundness-of-logic},
we can show that for any negative formula \(A\) defined below,
a process \(P\) satisfies \(A\) (i.e., \(P\in \semPF{A}\)) if 
its process type \(\Gamma\) satisfies the same formula \(A\). 
Therefore, our type system can be used at least for reasoning about
properties described using negative formulas.
\begin{defn}[positive/negative formulas]
The set \(\PosF\) (\(\NegF\), resp.) of positive (negative, resp.) 
formulas are the least set 
satisfying the following rules:
\[
\begin{array}{lcl}
\PLTRUE \in \PosF\cap \NegF\\
\PLout{x}{\ev}{n}, \PLin{x}{\ev}{n}\in \PosF\\
%%%A \mbox{ does not contain a formula of the form }
%%%  \PLout{x}{\ev}{n} \mbox{ or }\PLin{x}{\ev}{n}\imply\\
%%%\myquad  {A \in \PosF\cap \NegF}\\
A, B\in \PosF \imply \iffull\else\\
\myquad\fi A\PAR B, A\lor B, \PLsometr{\redlab}A, \eventual(A),
   \exists x.A, \exists \ev.A, \exists \ivar\COL{}C.A \in \PosF\\
A, B\in \NegF \imply %%%\PLsometr{\redlab}A, A\PAR B, 
   A\lor B, 
   \exists x.A, \exists \ev.A, \exists \ivar\COL{}C.A \in \NegF\\
A \in \PosF \imply \neg A\in \NegF\\
A \in \NegF \imply \neg A\in \PosF
\end{array}
\]
\end{defn}
Intuitively, a formula is positive (negative, resp.) if sub-formulas of the form
\(A\PAR B\), \(\PLsometr{\redlab}A\), \(\eventual(A)\),
\(\PLout{x}{\ev}{n}\), \(\PLin{x}{\ev}{n}\) appear only in positions
where the negation is applied an even (odd, resp.) number of times.

\begin{theorem}
\label{thm:property-logic}
Suppose \(\Gamma\p P\) and \(\conTE(\Gamma)\).  For any \(S \subseteq
\VAR\), if \(A\in \NegF\) with \(\FIV(A) = \emptyset\) and
\(\Gamma\in \semTFaux{A}{S}\), then \(P \in \semPFaux{A}{S}\)  holds.
Conversely,  for any \(S \subseteq \VAR\), if \(A\in\PosF\)  with
\(\FIV(A) = \emptyset\) and \(P\in \semPFaux{A}{S}\), then \(\Gamma\in
\semTFaux{A}{S}\) holds.

\end{theorem}
\iffull
\begin{pf}
%%%Since
%%%\(\tjudge{\reliable}{\Gamma}{P}\) implies 
%%%\(\tjudge{\wf}{\Gamma}{P}\) for any consistency condition \(\reliable\),
%%%it suffices to show the case for \(\reliable = \wf\).
The proof proceeds by induction on the size of \(A\).
The cases for 
\(\PLout{x}{\ev}{n}\), \(\PLin{x}{\ev}{n}\), \(A_1\PAR A_2\),
\(\PLsometr{\redlab}A'\), \(\eventual(A')\), and \(\neg A'\)
follow immediately from Lemma~\ref{lem:soundness-of-logic}.

Suppose \(A=A_1\lor A_2\in \NegF\) and \(\Gamma\in \semTF{A}\).
By the definition of \(\NegF\), it must be the case that
\(A_1, A_2\in \NegF\). By the assumption \(\Gamma\in \semTF{A}\),
\(\Gamma\in \semTF{A_i}\) for \(i=1\) or \(2\). By using induction hypothesis,
we obtain \(P\in \semPF{A_i} \subseteq \semPF{A}\) as required.
The other cases are similar.
\end{pf}
\begin{lemma}
\label{lem:redundant-new}
If \(\set{\seq x}\cap \FV(P)=\emptyset\), then
\(P\in \semPF{A}\) if and only if \(\nuexp{\seq x}P\in\semPF{A}\).
\end{lemma}
\begin{proof}
This follows by straightforward induction on the structure of \(A\).
\end{proof}
\else
\begin{pfsketch}
This follows by induction on the structure of \(A\). The cases for
\(\PLsometr{\redlab}A\) and \(\eventual(A)\) follow from 
Theorem~\ref{thm:subject-reduction} and the cases for 
\(\PLout{x}{\ev}{n}\), \(\PLin{x}{\ev}{n}\), and \(A\PAR B\) follow
from Theorem~\ref{thm:normal-derivation} and 
Corollary~\ref{cor:normal-derivation}. The other cases follow immediately
from the definitions of \(\semPF{A}\) and \(\semTF{A}\).
\end{pfsketch}
\fi
%%%\begin{lemma}
%%%\label{lem:semTF-restriction}
%%%Suppose that \(\Gamma\in \TSET\), \(A\in \FSET\), and \(S\cup \set{\seq x}\subseteq \VAR\).
%%%Suppose also that \(S\cap \set{\seq x}=\emptyset\).
%%%If \(A\) is a positive formula and \(\Gamma\in \semTFaux{A}{S\cup{\seq x}}\),
%%%then \(\exclude{\Gamma}{\set{\seq x}} \in \semTFaux{A}{S}\) holds.
%%%If \(A\) is a negative formula and
%%%\(\exclude{\Gamma}{\set{\seq x}}\in \semTFaux{A}{S}\), then 
%%%  \(\Gamma\in \semTFaux{A}{S\cup \set{\seq x}}\) holds.
%%%\end{lemma}
%%%\begin{remark}
%%%The converse does not hold.
%%%Let \(A = \PLout{x}{\ev}{n}\), \(\Gamma = \zeroTE\), 
%%%\(S=\emptyset\). If \(\emptyset\subTE \OutTEatom{x}{\ev}{\,}\),
%%%then \(\exclude{\Gamma}{\set{\seq x}} \in \semTFaux{A}{S}\) holds but
%%%\(\Gamma\not\in \semTFaux{A}{S\cup\set{\seq x}}\).
%%%Or let \(A = \PLsometr{\labcom{\epsilon}{\ev_1}{\ev_2}}\PLTRUE\),
%%%\(P = \outatom{x}{\,}{\ev_1}\PAR \inexp{y}{\,}{\ev_2}\zeroexp\),
%%%and \(\seq{x} = \{x, y\}\).
%%%\end{remark}
%%%
%%%\begin{lemma}
%%%\label{lem:semTF-closed-under-subTE}
%%%Suppose that \(\Gamma\subTE \Gamma'\). 
%%%If \(A\) is a positive formula and \(\Gamma'\in \semTFaux{A}{S}\), then
%%%\(\Gamma\in \semTFaux{A}{S}\). If \(A\) is a negative formula and
%%%\(\Gamma\in \semTFaux{A}{S}\), then \(\Gamma'\in \semTFaux{A}{S}\).
%%%\end{lemma}

\begin{corollary}[type soundness]
\label{cor:general-soundness}
Let \(A\in \NegF\) and \(P\) be a closed process.
Suppose that \(\reliable(\Gamma)\) implies \(\Gamma\in\semTF{A}\)
for any \(\Gamma\in\TSET\).
Suppose also that \(\Gamma\p P\) and \(\reliable(\Gamma)\).
Then, if \(P\red^* \SPCONG \nuexpseq{x}\nuexp{\seq{y}}Q\),
then \(\nuexpseq{x}Q\in\semPF{A}\).
\end{corollary}
\iffull
\begin{pf}
By applying Theorem~\ref{thm:subject-reduction} to 
\(\Gamma\p P\) and \(P\red^* \SPCONG \nuexpbseq{x}{1}{k}\nuexp{\seq{y}}Q\), we have
\(\Gamma'\p \nuexpbseq{x}{1}{k}\nuexp{\seq{y}}Q\) for some \(\Gamma'\) with
\(\reliable(\Gamma')\).
By Theorem~\ref{thm:normal-derivation}, we have \(\Delta\) such that
\(\Delta \p Q\) with \(\Gamma' \subTE \exclude{\Delta}{\set{\seq{x_1},\ldots,\seq{x_k},
\seq{y}}}\) and \(\reliable(\project{\Delta}{\set{\seq y}})\).
By the assumption, we have \(\project{\Delta}{\set{\seq y}} \in \semTF{A}\).
Let \(\set{\seq w} = \FV(\Delta)\setdif\set{\seq{x_1},\ldots,\seq{x_k},\seq{y}}\).
Since \(\project{\Delta}{\set{\seq y}} = 
\exclude{\Delta}{\set{\seq{x_1},\ldots,\seq{x_k},\seq{w}}}\),
we have \(\Delta \in \semTFaux{A}{\set{\seq{x_1},\ldots,\seq{x_k},\seq{w}}}\).
By using Theorem~\ref{thm:property-logic}, we obtain
\(Q \in \semPFaux{A}{\set{\seq{x_1},\ldots,\seq{x_k},\seq{w}}}\),
which implies \(\nuexp{\seq w}\nuexpbseq{x}{1}{k}Q\in \semPF{A}\) by Lemma~\ref{lem:semPF-restriction}.
By Lemma~\ref{lem:redundant-new}, we have \(\nuexpbseq{x}{1}{k}Q\in \semPF{A}\) as required.
\end{pf}
\fi

Intuitively, the last sentence of the above corollary means that 
all the channels created during reductions of \(P\) 
are used according to \(A\).
The corollary implies that, in order to guarantee that property,
it suffices to define the consistency condition \(\reliable\) 
by \(\reliable(\Gamma) \IFF
\conTE(\Gamma)\land \Gamma \models \invariant(A)\) 
(where \(\invariant(A)= \neg \eventual(\neg A)\)).

%%%As we show in Section~\ref{sec:application},
%%%the soundness of various instances follows immediately from 
%%%the above corollary.
Using the above corollary, we can obtain various type systems.
For example, we can obtain a variant of the linear channel type system~\cite{KobayashiTOPLAS:LinearPi}.
Let \(A\) be \(\neg \exists x.\exists \ev_1,\ev_2,\ev_3.\exists \ivar.\eventual(
   \PLsometr{\labcom{x}{\ev_1}{\ev_2}}\eventual(\PLout{x}{\ev_3}{\ivar}\lor \PLin{x}{\ev_3}{\ivar}))\);
Then it is guaranteed that every channel is used at most once.
More examples are given in Section~\ref{sec:application}.

Note that our generic type system can be used also for
reasoning about properties described by some non-negative formulas:
Indeed, 
the deadlock-freedom property is not described as a non-negative formula,
but as we show in Section~\ref{sec:application},
we can obtain 
a type system for deadlock-freedom as an instance of our generic type system
and show its soundness (by using not the above corollary but more basic theorems
presented in Section~\ref{subsec:common-properties}).
%%%It is left for future work to obtain a more general version of
%%%the above corollary that can deal with such properties as deadlock-freedom.


==> Implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented a prototype resource usage analyzer
based on the extended type system described in Section~\ref{sec:extension}.
We have tested all the examples given in the present paper.
The implementation can be tested at \url{http://www.yl.is.s.u-tokyo.ac.jp/~kohei/usage-pi/}.

The analyzer takes a pi-calculus program as an input, and uses \typical{}\cite{TyPiCal}
to annotate each input or output action
with an attribute on whether the action is guaranteed to succeed
automatically
(recall the syntax of extended processes in Section~\ref{sec:extension}).
The annotated program is then analyzed based on the
algorithm described in Section~\ref{sec:inference}.

The followings are some design decisions we made in the current implementation.
We restrict the resource usage specification (\(\spec\)) to the regular languages,
although in future we may extend it based on Remark~\ref{rem:petri-lang-as-spec}.
In Step 3-1 of the algorithm for checking \(\etraces{x}{A} \subseteq \spec\),
 we blindly approximate \(A\) by pushing all of its \(\nu\)-prefixes to the top-level.
In future we might utilize an existing model checker to handle the case where \(A\)
is already finite.
In Step 3-4 for solving
the reachability problems of Petri nets, we approximate  the number of tokens in each place by
 an element of the finite set \(\set{0, 1, 2, \mbox{``$3$ or more''}}\). That approximation
reduces Petri nets to finite state machines, so we can use 
 BDD to compute an approximation of the reachable states.

Figure~\ref{fig:samplerun} shows a part of a successful run of the analyzer.
The first process (on the second line) of the input program runs a server,
which returns a new, initialized resource.
We write \verb|!| and \verb|?| for output and input actions.
The resource access specification is here expressed by the number \(1\) of
\verb|newR 1, x|, which refers to the built-in specification \(\prefixclos{I(R+W)^*C\conv}\).
The second process runs infinitely many client processes, each of which
sends a request for a new resource, and after receiving it, reads and closes it.
The third process (on the 6th line) is a tail-recursive version of the replicated service
in Example~\ref{ex:repeatread}. Here, a
boolean is passed as the first argument of \(s\) instead of an integer, as the current
system is not adapted to handle integers; it does not affect the analysis, since the system
ignores the value and simply inspects both branches of the conditional.
%%%The input program shown on top of the figure recurses on channel \verb|repeat|,
%%%and repeatedly run the part \verb|if b then 0 else ...|, which
%%%is a combination of Examples~\ref{ex:cobegin}
%%%and \ref{ex:repeatread}  and
%%%a replicated service which receives a resource and returns the initialized one
%%%Recursive calls in the example has been replaced by a tail-recursive one.
Note that the program creates infinitely many resources and has infinitely many states.
%%%so that we cannot apply
%%%finite-state model checking and some of the previous type-based analyses that can only reason
%%%about the global state
%%%Some of the previous analyses can reason about only the global state~\cite{Rathke2005,Skalka04}.
%%%They would fail to infer that \emph{each} resource is eventually closed and
%%%if they were ever applied to this kind of program, since after a close
%%%which checks whether the following example is partially live:
%%%% the example in Figure~\ref{ex:repeatread} is partially live.
%%%\[
%%%\begin{array}{l}
%%%\nuexp{\rep}\nuexp{\repread}\\
%%%\repexp (\inexp{\repread}{b,x,r}{}\ \ifexp{b}{\outexp{r}{}{}}{\accexp{\Read}{x} \outexp{\repread}{b,x,r}{}}) \PAR\\
%%%\repexp (\inexp{\repread}{b}{} \IF\ b\ \THEN\ \zeroexp\ \ELSE\\
%%%\quad (\outexp{\repread}{b}{} \PAR\\
%%%\quad\quad \nurexp{y}{\prefixclos{\Init\ \Read^*\ \Close}} \nuexp{c_1} \nuexp{c_2}\\
%%%\quad\quad\quad(\accexp{\Init}{y} (\outexp{c_1}{}{} \PAR \outexp{c_1}{}{}) \PAR\\
%%%\quad\quad\quad\inexp{c_1}{}{} \outexp{\repread}{b,y,c_2}{} \PAR\\
%%%\quad\quad\quad\inexp{c_1}{}{} \outexp{\repread}{b,y,c_2}{} \PAR\\
%%%\quad\quad\quad\inexp{c_2}{}{} \inexp{c_2}{}{} \accexp{\Close}{y}))\\
%%%\end{array}
%%%\]
%%%The input program for the analyzer and
The first output is the annotated version of the input program produced by
\typical{}, where \verb|!!| and \verb|??| are
an output and an input with the attribute \(\capable\) (recall Section~\ref{sec:extension}).
% The input program for the analyzer is shown in Figure~\ref{fig:sampleinput}.
%%%\verb|newR 1, x in...| in the input corresponds to a process expression
%%%\(\nurexp{x}{\spec}\ldots\). The integer \verb|1| denotes a specification
%%%\(I R^* C\). We write \verb|acc(x,I)|, \verb|c!()| and \verb|c?()|
%%%for \(\accexp{I}{x}\), \(\outexp{c}{}{}\) and \(\inexp{c}{}{}\).

%%%The first part of the output shows the result of deadlock-freedom analysis.
%%%In the output, \verb|!!| and \verb|??| denote output and input actions
%%%annotated with \(\capable\). Actions annotated by \(\mayfail\) are expressed
%%%by \verb|!| and \verb|?|.

The remaining part shows the trace inclusion constraint and
the constructed Petri net.
%%%In reducing constraints, the analyzer does not expand
%%%subtyping constraints as we mentioned in Section~\ref{sec:reducing-constrints}
%%%to keep the size of constraints small.
The final line reports that the verification has succeeded,
which implies that both the safety property (in Section~\ref{sec:typing}) and
the partial liveness property (in Section~\ref{sec:extension}) are
satisfied.

%%%The analyzer shows the initial marking,
%%%the set of places and the set of transitions.
%%%Places are annotated with corresponding behavioral types.
%%%Transitions are expressed by labels of transitions,
%%%firing conditions and difference of the number of tokens
%%%after and before a transition fires.
%%%
%%%In the end, the analyzer reports result and
%%%a state decided to be errornous if any.
%%%%% In the example, the analyzer reports that
%%%%% the input is not partially live.
%%%%% This is due to the limitation of \typical{}
%%%%% (see the following remark).
%%%In the example, no errors are found.

%% \begin{figure}
%% \begin{verbatim}
%% new repeat in
%% new repeat_read in
%% *(repeat_read?(b, x, r).
%%    if b then r!()
%%    else acc(x,read).repeat_read!(b,x,r)) |
%% *(repeat?(b).
%%   if b then O else
%%    (repeat!(b) |
%%     (newR 1, y in new c1 in new c2 in
%%      (acc(y,init).(c1!() | c1!()) |
%%       c1?().repeat_read!(b,y,c2) |
%%       c1?().repeat_read!(b,y,c2) |
%%       c2?().c2?().acc(y,close)))))
%% \end{verbatim}
%% \caption{A Sample Input the Corresponds to Example~\ref{ex:repeatread}.}
%% \label{fig:sampleinput}
%% \end{figure}

%% \begin{figure}
%% \begin{verbatim}
%% (*** The result of lock-freedom analysis ***)
%% new repeat in
%% new repeat_read in
%% *(repeat_read?(b, x, r).
%%    if b then r!!(). O
%%    else acc(x, read). repeat_read!!(b, x, r). O) |
%% *(repeat?(b).
%%   if b then O else
%%    (repeat!!(b). O |
%%     (newR 1,y in new c1 in new c2 in
%%      (acc(y, init). (c1!!(). O | c1!!(). O) |
%%       c1??(). repeat_read!!(b, y, c2). O |
%%       c1??(). repeat_read!!(b, y, c2). O |
%%       c2??(). c2??(). acc(y, close). O))))

%% (*** Optimized Constrs ***)
%% \$28 <= (c2!!. O) & (acc(y, read). \$28)
%% \$26 <= (c2!!. O) & \$26
%% \$24 <= O & (\$24 | c1!!. O | c1!!. O | (c1??. (c2!!. O) & (c2!!. O & \$26)) |
%%              (c1??. (c2!!. O) & (c2!!. O & \$26)) | (c2??. c2??. O))
%% \$23<=(P(3)!!. O) & (acc(P(2), read). \$23)
%% trace(y,acc(y, init). (c1!!. O| c1!!. O)|
%%         c1??. (c2!!. O) & ((acc(y, read). (c2!!. O) & (acc(y, read). \$28))) |
%%         c1??. ((c2!!. O)) & ((acc(y, read). (c2!!. O) & (acc(y, read). \$28))) |
%%         c2??. c2??. acc(y, close). O) is included in 1

%% (*** initial marking ***)
%% 1 * 19 | 1 * 8 | 2 * 4 | 1 * 0

%% (*** Used Places ***)
%% (*** 22 Places ***)
%% 0: c2??. c2??. acc(y, close). O
%% 1: c2??. acc(y, close). O
%% 2: acc(y, close). O
%% 3: O
%% 4: c1??. ((c2!!. O)) & ((acc(y, read). ((c2!!. O)) & ((acc(y, read). \$28))))
%% 5: c2!!. O
%% 6: acc(y, read). ((c2!!. O)) & ((acc(y, read). \$28))
%% 7: acc(y, read). \$28
%% 8: acc(y, init). (c1!!. O| c1!!. O)
%% 9: c1!!. O
%% 10: P(3)!!. O
%% 11: acc(P(2), read). \$23
%% 12: ((P(3)!!. O)) & ((acc(P(2), read). \$23))
%% 13: c2??. c2??. O
%% 14: c2??. O
%% 15: c1??. ((c2!!. O)) & (((c2!!. O)) & (\$26))
%% 16:
%% O & (\$24 | (c1!!. O) | (c1!!. O) |
%% (c1??. (c2!!. O) & ((c2!!. O) & \$26)) |
%% (c1??. (c2!!. O) & ((c2!!. O) & \$26)) | (c2??. c2??. O))
%% 17: (c2!!. O) & \$26
%% 18: ((c2!!. O)) & ((acc(y, read). \$28))
%% 19: sp1 false
%% 20: sp2 false
%% 21: sp3 true

%% (*** Used transitions ***)
%% (*** 18 Transitions ***)
%% @@: 1 * 5 | 1 * 0 -> -1 * 5 | 1 * 3 | 1 * 1 | -1 * 0
%% @@: 1 * 5 | 1 * 1 -> -1 * 5 | 1 * 3 | 1 * 2 | -1 * 1
%% @@: 1 * 9 | 1 * 4 -> -1 * 9 | 1 * 5 | -1 * 4 | 1 * 3
%% @@: 1 * 9 | 1 * 4 -> -1 * 9 | 1 * 6 | -1 * 4 | 1 * 3
%% @@: 1 * 12 -> -1 * 12 | 1 * 10
%% @@: 1 * 12 -> -1 * 12 | 1 * 11
%% @@: 1 * 13 | 1 * 5 -> 1 * 14 | -1 * 13 | -1 * 5 | 1 * 3
%% @@: 1 * 14 | 1 * 5 -> -1 * 14 | -1 * 5 | 2 * 3
%% @@: 1 * 15 | 1 * 9 -> -1 * 15 | -1 * 9 | 1 * 5 | 1 * 3
%% @@: 1 * 15 | 1 * 9 -> -1 * 15 | -1 * 9 | 1 * 5 | 1 * 3
%% @@: 1 * 15 | 1 * 9 -> 1 * 17 | -1 * 15 | -1 * 9 | 1 * 3
%% @@: 1 * 16 -> -1 * 16 | 1 * 3
%% @@: 1 * 16 -> 2 * 15 | 1 * 13 | 2 * 9
%% @@: 1 * 17 -> -1 * 17 | 1 * 5
%% @@: 1 * 17 ->
%% @@: 1 * 18 -> -1 * 18 | 1 * 5
%% @@: 1 * 18 -> -1 * 18 | 1 * 7
%% (y, close): 1 * 20 | 1 * 2 -> -1 * 20 | 1 * 21 | 1 * 3 | -1 * 2
%% (y, init): 1 * 19 | 1 * 8 -> -1 * 19 | 1 * 20 | 2 * 9 | -1 * 8
%% (y, read): 1 * 20 | 1 * 6 -> -1 * 6 | 1 * 5
%% (y, read): 1 * 20 | 1 * 6 -> 1 * 7 | -1 * 6
%% (y, read): 1 * 20 | 1 * 7 -> 1 * 18 | -1 * 7

%% No error found
%% \end{verbatim}
%% \caption{A Sample Output of the Analyzer.}
%% \label{fig:samplerun}
%% \end{figure}

\begin{figure}
\small \textbf{Input:}
%% new rep, s in
%%   *(s?(b,x,r).if b then r!() else acc(x,R).s!(b,x,r))
%% | *(rep?(b).if b then O else
%%    (rep!(b)
%%     | (newR 1,y in new c1, c2 in
%%        (acc(y,I).(c1!() | c1!())
%%         | c1?().s!(b,y,c2) | c1?().s!(b,y,c2)
%%         | c2?().c2?().acc(y,C)))))
%% | rep!(true)
\begin{verbatim}
new create,s in
  *(create?(r).newR 1,x in acc(x,init).r!(x))
| *(new r in create!(r)
     | r?(y).new c in s!(false,y,c) | s!(false,y,c)
                    | c?().c?().acc(y,close))
| *(s?(b,x,r).if b then r!()
              else acc(x,read).s!(b,x,r))
\end{verbatim}
\textbf{Output:}
%% new rep, s in
%% *(s?(b, x, r).
%%    if b then r!!(). O
%%    else acc(x, R). s!!(b, x, r). O) |
%% *(rep?(b).
%%   if b then O else
%%    (rep!!(b). O |
%%     (newR 1,y in new c1 in new c2 in
%%      (acc(y, I). (c1!!(). O | c1!!(). O) |
%%       c1??(). s!!(b, y, c2). O |
%%       c1??(). s!!(b, y, c2). O |
%%       c2??(). c2??(). acc(y, C). O))))

%%       c1??. (c2!!. O) & acc(y, R). (c2!!. O) & acc(y, R). $28) |
%%       c1??. (c2!!. O) & acc(y, R). (c2!!. O) & acc(y, R). $28) |

%% 1: c2??. acc(y, C). O
%% 2: acc(y, C). O

%% @@: 1 * 5 | 1 * 0 -> -1 * 5 | 1 * 3 | 1 * 1 | -1 * 0
%% @@: 1 * 5 | 1 * 1 -> -1 * 5 | 1 * 3 | 1 * 2 | -1 * 1

%%%%%%% 7/15

%% new rep, s in
%%   *(s?(b,x,r).if b then r!() else acc(x,R).s!(b,x,r))
%% | *(rep?(b).if b then O else
%%      ....
%%         | c2??().c2??().acc(y,C)))))
%% | rep!!(true)

\begin{verbatim}
(*** The result of lock-freedom analysis ***)
new create, s in
  *create??(r). newR 1,x in acc(x, I). r!!(x)
| *(new r in create!!(r)
     | r??(y).new c in s!!(false,y,c) | s!!(false,y,c)
                    | c??().c??().acc(y,close))
...
(*** Constraints ***)
etrace(x,acc(x, init).(c!! & acc(x, read). $16 | $16 |
         c??. c??. acc(x, close). O)) is included in 1
...
(*** initial marking ***)
1 * 11 | 1 * 7
(*** 14 Places ***)
0: c!!. O
...
(*** 9 Transitions ***)
(x,close): 1*12 | 1*10 -> -1*12 | 1*13 | -1*10 | 1*1
...
No error found
\end{verbatim}
\caption{A Sample Run of the Analyzer.}
\label{fig:samplerun}
\end{figure}

%%%The followings are the current limitation of the prototype analyzer.
%%%\begin{itemize}
%%%%%%\item We have not yet implented a parser for regular expressions and a translator
%%%%%%into an minimized deterministic automaton. Only a fixed set of resource usage
%%%%%%specifications can be declared. (This is just a limitation of the front end,
%%%%%%and will be removed soon.)
%%%%%%\item In the final phase of deciding \(\etraces{x}{A}\subseteq \spec\)
%%%%%%(recall Section~\ref{sec:constraint-solving}),
%%%%%%no heursitic algorithm has been implemented to find a basis of \(\project{A}{\set{x}}\);
%%%%%%The approximation of pushing  all the \(\nu\)-prefixes to the top-level
%%%%%%is blindly applied to \(\project{A}{\set{x}}\).
%%%\item Petri nets are approximated to finite state machines when we solve
%%%the reachability problems of Petri nets. More specifically, the number of tokens
%%%in each place is
%%%abstracted to an element of the finite set \(\set{0, 1, 2, \mbox{``$3$ or more''}}\),
%%%and BDD is used to compute an approximation of the reachable states.
%%%\item The anlayzer suffers from the current limitation of \typical{}, which cannot infer
%%%that the input on channel \textit{rep} will eventually succeed in the program of
%%%Example~\ref{ex:repeatread}.
%%%As a result, the analyzer cannot infer that the resource is eventually closed.
%%%\item The current implementation is not tuned enough (especially the BDD library),
%%%so that it does not work for large programs. Various optimizations and
%%%possible utilization of an existing model checker as a back-end are left for
%%%future work.
%%%\end{itemize}


==> Inference.tex <==
\section{Type Inference Algorithm}
\label{sec:inference}
This section discusses an algorithm which takes a closed process \(P\) as an input
and checks whether \(\tjudge{\emptyset}{P}{\Tzero}\) holds.
%
As in similar type systems~\cite{IK05TOPLAS,Kobayashi05ActInf},
the algorithm consists of the following steps.
\begin{enumerate}
\item Extract constraints on type variables based on the (syntax-directed version of)
typing rules.
\item Reduce constraints to trace inclusion constraints of the form \\
\( \set{\traces{x_1}{A_1}\subseteq \spec_1, \ldots, \traces{x_n}{A_n}\subseteq \spec_n}\)
\item Decide whether the constraints are satisfied.
\end{enumerate}
%%%As in our previous work~\cite{Kobayashi05ActInf}, we use reduction of behavioral types
%%%into Petri nets in Step 3. Unlike in the previous work,
%%%however, we need to apply approximation, so that 
The algorithm for Step 3 is sound but not complete. 

We give an overview of each step below. The first two steps are almost the same as
those in the previous work.
%the algorithms for previous type systems~\cite{IK05TOPLAS,Kobayashi05ActInf}.

\subsection{Step 1: Extracting Constraints}

The typing rules presented in Section~\ref{sec:typing} can be transformed to
the syntax-directed typing rules shown in Figure~\ref{fig:sd-typing}.
In the figure, \(\Gamma_1\TEcup \Gamma_2\) is the type environment obtained by merging
both bindings, and defined only if
\(\Gamma_1(x)=\Gamma_2(x)\) for every \(x\in\dom(\Gamma_1)\cap \dom(\Gamma_2)\).
Type equality here is syntactic equality up to $\alpha$-renaming.
And \(\WF(\Gamma_1\cup \Gamma_2)\) means that \(\Gamma_1\cup \Gamma_2\) is well-defined.
The two sets of typing rules are equivalent in the following sense:
If \(\tjudge{\Gamma}{P}{A}\) is derivable,
then there exists \(A'\) such that \(A'\newsubtype A\) holds
and \(\sdtjudge{\Gamma}{P}{A'}\) is derivable. Conversely,
 if \(\sdtjudge{\Gamma}{P}{A}\) is derivable, so is \(\tjudge{\Gamma}{P}{A}\).
%Actually, this step 1 is fairly standard so that I even wonder if
%we should Theorem 4.1 as a theorem. If we run out of the space,
%some or most of the material here could be moved to Appendix.

\input{SyntaxDirectedTyping}

Based on the syntax-directed rules, we obtain the algorithm in
Figure~\ref{fig:algorithm-PT}, which takes a process \(P\) and outputs a triple
consisting of a type environment \(\Gamma\), a behavioral type \(A\), and
a set \(C\) of constraints.
In Figure~\ref{fig:algorithm-PT}, \(\Gamma_1\Tcup \cdots \Tcup \Gamma_n\) is defined to be
\((\Gamma, C)\) where \(\Gamma\) and \(C\) are given by:
\[
\begin{array}{l}
\dom(\Gamma) = \dom(\Gamma_1)\cup \cdots \cup \dom(\Gamma_n)\\
\Gamma(x) = \Gamma_i(x) \mbox{ where $x\in \dom(\Gamma_i)\setdif
   (\dom(\Gamma_1)\cup \cdots\cup \dom(\Gamma_{i-1}))$}\\
C = \set{\Gamma_i(x)=\Gamma_j(x) \mid x\in \dom(\Gamma_i)\cap \dom(\Gamma_j)}
\end{array}
\]

The triple \((\Gamma,A,C)\) output by \(\PT\) satisfies the following properties:
\begin{itemize}
\item \(\tjudge{\theta\Gamma}{P}{\theta A}\)
holds for any substitution \(\theta\) such that \(\models \theta C\).
\item If \(\tjudge{\Gamma'}{P}{A'}\), then there exists a substitution \(\theta\) such that
\(\theta\Gamma \subseteq \Gamma'\) and \(\theta A\newsubtype A'\).
\end{itemize}
Here, \(\Gamma\) and \(A\) may contain variables representing unknown behavioral types
and value types. \(C\) is a set of constraints on them, and
the substitution $\theta$ above replaces them with closed behavioral types
and value types. Intuitively, the triple \((\Gamma, A, C\) expresses a set of
type judgments for \(P\). The first property above says that the triple contains only valid
judgments, while the second property says that every valid judgment is subsumed by the triple.

We do not give a formal proof of the above properties; As usual, they can be proved
by induction on the structure of \(P\).

\iftwocol
\begin{figure}[tbp]
\else
\begin{figure}[tbp]
\fi
\begin{center}
\fbox{\small
\begin{minipage}{\figwidth}
\begin{tabbing}
\(\PTv(x) = \) \= \((x\COL\Tvvar, \Tvvar)\) (where $\Tvvar$ fresh)\\
\(\PTv(b) = \) \> \((\emptyset, \Tbool)\) \mbox{ if $b\in \set{\TRUE,\FALSE}$}\\
\rulesp{}\\
\( \PT(\zeroexp) = \)\= \((\emptyset, \Tzero, \emptyset) \)  \\
\( \PT(\outexp{x}{\seq{v}}{}P_0) = \) \\ \>
\(    \PLET\)\= \((\Gamma_i, \mvtype_i) = \PTv(v_i) \) \\ \> \>
                \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
\(    (\Gamma, C) = \Gamma_0 \Tcup (x\COL\Tchan{(\seq{y}\COL{}\seq{\mvtype})\Tbvar})\Tcup
    \Gamma_1\Tcup \cdots \Tcup \Gamma_n\) \\ \>
\(\PIN (\Gamma, \Tout{x}(\Tsubst{\Tbvar}{\seq{y}}{\seq{v}}\PAR A_0), C)\)
 (where $\Tbvar$ fresh)\\
\( \PT(\inexp{x}{\seq{y}}{}P_0) = \) \\ \>
\(    \PLET\)\= \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
  \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tchan{(\seq{y}\COL{}\seq{\Tvvar})\Tbvar})
            \Tcup (\seq{y}\COL\seq{\Tvvar})\)\\ \>
\(\PIN (\Gamma\setdif{\seq{y}}, \Tin{x}{\exclude{A_0}{\set{\seq{y}}}},
        C_0\cup C_1 \cup \set{\Tbvar\subtype \project{A_0}{\set{\seq{y}}}})\)\\ \> \>
  (where $\Tbvar$, $\seq{\Tvvar}$ fresh)\\
\( \PT(P_0\PAR P_1) = \) \\ \>
\(    \PLET\)\= \((\Gamma_0,A_0,C_0) = \PT(P_0)\)\\\>\>
   \((\Gamma_1,A_1,C_1) = \PT(P_1)\)\\\>\>
  \((\Gamma_2, C_2) = \Gamma_0\Tcup \Gamma_1\)\\ \>
\(\PIN (\Gamma_2, A_0\TPAR A_1, C_0\cup C_1\cup C_2)\)\\
\( PT(\ifexp{v}{P_0}{P_1}) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
   \((\Gamma_1,A_1,C_1) = \PT(P_1)\)\\\>\>
   \((\Gamma_2, \mvtype) = \PTv(v)\)\\ \>\>
   \((\Gamma, C_2) = \Gamma_0\Tcup \Gamma_1\Tcup \Gamma_2\)\\\>
\(    \PIN (\Gamma, A_0\TOR A_1, C_0\cup C_1 \cup C_2\cup \set{\mvtype=\Tbool}) \)\\
\( PT(\nuexp{x}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
\( C_1 = \PIF x\in \dom(\Gamma_0)\PTHEN
   \set{\isTchan(\Gamma_0(x))} \PELSE \emptyset\)\\ \>
\(    \PIN (\Gamma_0\restrictTE{\set{x}}, \Thiding{x}{A_0}, C_0\cup C_1) \)\\
\( PT(\repexp P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \>
\(    \PIN (\Gamma_0, \Trep{A_0}, C_0) \)\\
\( PT(\accexp{\acclab}{x}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
    \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tres)\)\\ \>
\(    \PIN (\Gamma_1, \Tacc{\acclab}{x}{A_0}, C_0\cup C_1) \)\\
\( PT(\nurexp{x}{\spec}P_0) = \) \\ \>
\(    \PLET (\Gamma_0, A_0, C_0) = PT(P_0) \) \\ \> \>
    \((\Gamma_1, C_1) = \Gamma_0\Tcup (x\COL\Tres)\)\\ \>
\(    \PIN (\Gamma_1\restrictTE{\set{x}}, \exclude{A_0}{\set{x}},
   C_0\cup C_1\cup \set{\traces{x}{A_0}\subseteq \spec}) \)
\end{tabbing}
\end{minipage}
}
\caption{A Type Inference Algorithm}
\label{fig:algorithm-PT}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi

%%%The following is a standard theorem about the correctness of the constraint extraction
%%%algorithm. Its correctness follows immediately from the equivalence of the
%%%typing rules in Section~\ref{sec:typing} and the syntax-directed rules. In it, the substitutions
%%%$\theta$ replace behavioral type variables $\alpha$ and value type variables $\rho$.
%%%\begin{thm}
%%%Suppose that \(\PT(P) = (\Gamma, A, C)\). Then, the following conditions hold.
%%%\begin{itemize}
%%%\item \(\tjudge{\theta\Gamma}{P}{\theta A}\)
%%%holds for any substitution \(\theta\) such that \(\models \theta C\).
%%%\item If \(\tjudge{\Gamma'}{P}{A'}\), then there exists a substitution \(\theta\) such that
%%%\(\theta\Gamma \subseteq \Gamma'\) and \(\theta A\newsubtype A'\).
%%%\end{itemize}
%%%\end{thm}

\subsection{Step 2: Reducing Constraints}
Given a closed process \(P\), \(\PT(P)\) produces a triple \((\emptyset, A, C)\).
The set \(C\) of constraints consists of unification constraints on value types
(where all the behavioral types occurring in them are variables),
constraints of the form \(\isTchan(\mvtype)\) (which means that \(\mvtype\) is
a channel type), subtype constraints on
behavioral types of the form \(\Tbvar \subtype A\), and constraints of the form
\(\traces{x}{A}\subseteq \spec\).
We can remove the first two kinds of constraints (unification constraints on value types
and \(\isTchan(\mvtype)\)) by applying the standard unification algorithm.
Thus, we obtain the following constraints:
\[
\begin{array}{l}
 \set{\Tbvar_1 \subtype A_1, \ldots, \Tbvar_n \subtype A_n, \\
 \traces{x_1}{B_1}\subseteq \spec_1, \ldots, \traces{x_m}{B_m}\subseteq \spec_m}
\end{array}
\]
Here, we can assume that \(\Tbvar_1,\ldots,\Tbvar_n\) are different from each other,
since \(\Tbvar\subtype A_1\) and \(\Tbvar\subtype A_2\) can be replaced with
\(\Tbvar \subtype A_1\TOR A_2\) by Lemma~\ref{le:subtyping-properties}.
We can also assume that \(\set{\Tbvar_1,\ldots,\Tbvar_n}\) contains all the type variables
in the constraint, since otherwise we can always add the tautology \(\Tbvar\subtype\Tbvar\).
Each subtype constraint \(\Tbvar\subtype A\) can also be replaced by
\(\Tbvar \subtype \Trec{\Tbvar}{A}\), by using Lemma~\ref{le:subtyping-properties}.
Therefore, the above constraints can be further reduced, by Lemma~\ref{le:subtyping-properties}, to:
\[
\begin{array}{l}
 \set{\traces{x_1}{\subst{\seq{\Tbvar}}{\seq{A}'}B_1}\subseteq \spec_1, \ldots,
  \traces{x_m}{\subst{\seq{\Tbvar}}{\seq{A}'}B_m}\subseteq \spec_m}
\end{array}
\]
Here, \(A_1',\ldots,A_n'\) are the least solutions for the subtype constraints.

Thus, we have reduced type checking to the validity of
trace inclusion constraints of the form \(\traces{x}{A}\subseteq \spec\).
%Kohei: Did we mentioned that we will replace $\traces{x}{A}$ with $\traces{x}{\project{A}{x}}$ somewhere?
%In the beginning of Step 3, it seems that we implicitly use this.
%Lucian: it is mentioned now! and is part of the definition.

\begin{exa}
\label{ex:inference-recursion}
Recall Example~\ref{ex:repeatread}.
By applying the algorithm \(\PT\) and the first part of Step~2,
we obtain the following constraints:
\[
\begin{array}{l}
\traces{x}{\Thiding{r} (\Tacc{I}{x} \Tout{\repread} \Tbvar_1 \TPAR \Tin{r} \Taccatom{C}{x})} \subseteq \prefixclos{IR^*C}\\
% \traces{x}{\Thiding{r} (\Tacc{I}{x} \Tbvar_1 \TPAR \Tin{r} \Taccatom{C}{x})} \subseteq \prefixclos{IR^*C}\\
\Tbvar_1 \subtype \project{\Tout{r} \Tbvar_2 \TOR \Thiding{r'} (\Tout{\repread} \Tren{\Tbvar_1}{r}{r'} \TPAR \Tin{r'} \Tacc{R}{x} \Tout{r} \Tbvar_2)}{\set{n,x,r}}\\
\Tbvar_2\subtype \Tbvar_2
% \Tbvar_1 \subtype \project{\Tout{r} \Tbvar_2 \TOR \Thiding{r'} (\Tren{\Tbvar_1}{r}{r'} \TPAR \Tin{r'} \Tacc{R}{x} \Tout{r'} \Tbvar_2)}{\set{b,x,r}}\\
% \Tbvar_3 \subtype \project{\Taccatom{C}{x}}{\emptyset} \TOR \project{\Tacc{R}{x} \Tout{r'} \Tbvar_2}{\emptyset}\\
\end{array}
\]
%%%where \(\Tbvar_2\) is a behavioral type variable on which there are no constraints.
% Kohei - Actually, constraints above are obtained by replacing \(\traces{x}{A}\) with \(\traces{x}{\project{A}{x}}\)
% Lucian - not needed, since Project{A}{x} is part of the definition of \traces.
By applying the second part of Step 2, we obtain
\(\traces{x}{A_1} \subseteq \prefixclos{IR^*C}\) where
\[
\begin{array}{rcl}
% \traces{x}{\Thiding{r} (\Tacc{I}{x} \Tout{\repread} A_1 \TPAR \Tin{r} \Taccatom{C}{x})} \subseteq \prefixclos{IR^*C}\\
A_1 &=& \Thiding{r} (\Tacc{I}{x} \Tout{\repread} A_2 \TPAR \Tin{r} \Taccatom{C}{x})\\
A_2 &=& \Trec{\Tbvar_1}{\project{\Tout{r}A_3 \TOR \Thiding{r'} (\Tout{\repread} \Tren{\Tbvar_1}{r}{r'} \TPAR \Tin{r'} \Tacc{R}{x} \Tout{r}A_3)}{\set{n,x,r}}}\\
A_3 &=& \Trec{\Tbvar_2}{\Tbvar_2}.
\end{array}
\]
%%%Since \(\traces{x}{A_1} = \traces{x}{\project{A_1}{\set{x_1}}}\),
%%%we omit the actions on \(s\) and \(A_3\) in Step 3 discussed below.
%%%\eoe{}
\end{exa}

\subsection{Step 3: Constraint Solving}
\label{sec:constraint-solving}
We present an approximation algorithm for checking a
trace inclusion constraint \(\traces{x}{A}\subseteq \spec\)
when the trace set \(\spec\) is a regular language.
(Actually, we can extend the algorithm to deal with the case
where \(\spec\) is a deterministic Petri net language: see
Remark~\ref{rem:petri-lang-as-spec}.)

We first describe the algorithm with an example. In
Example~\ref{ex:inference-recursion} above, we have reduced the typability of
the process to the equivalent constraint $\traces{x}{A_1} \subseteq \spec$ where
$\spec = \prefixclos{IR^*C}$ and
\begin{eqnarray*}
  \project{A_1}{\set{x}} & \eqtype & \Thiding{r}{(\Tacc{I}{x}A_2'' \mathrel{|} \Tin{r}\Taccatom{C}{x})} \\
  A_2'' & = & \Toutatom{r} \TOR \Thiding{r'}{(\Tren{A_2''}{r}{r'} \mathrel{|} \Tin{r'}\Tacc{R}{x}\Toutatom{r})}
\end{eqnarray*}
Here, we have removed \(A_3=\Trec{\Tbvar}{\Tbvar}\) since \(A_3\eqtype \Tzero\).

\textbf{Step 3-1.}
Approximate the behavior of \(\project{A_1}{\set{x}}\) 
by a Petri net~\cite{PetriBook} \(\petrinet{A_1}{x}\).
This part is similar to the translation of usage expressions into Petri nets in
Kobayashi's previous work~\cite{Kobayashi00CONCUR,Kobayashi05ActInf,TyPiCal}.
Since the behavioral types are more expressive (having recursion, hiding, and renaming), however,
we need to approximate the behavior of a behavioral type unlike in the previous work.
In this case $\project{A_1}{\set{x}}$ is infinite. 
To make it tractable we make a sound approximation $A_1'$ by pushing $(\nu)$ to top
level, and we eliminate $\csubst{r}{r'}$:
\begin{eqnarray*}
  A_1' & = & \Thiding{r,r'}{(\Tacc{I}{x}A_2' \mathrel{|} \Tin{r}\Taccatom{C}{x})} \\
  A_2' & = & \Toutatom{r} \TOR (A_3' \mathrel{|} \Tin{r'}\Tacc{R}{x}\Toutatom{r}) \\
  A_3' & = & \Toutatom{r'} \TOR (A_3' \mathrel{|} \Tin{r'}\Tacc{R}{x}\Toutatom{r'})
\end{eqnarray*}
Then $\petrinet{A_1'}{x}$ is as pictured. (Here we treat $A_1 \TOR A_2$ as $\tau.A_1 \TOR \tau.A_2$ for clarity.
We also use a version of Petri nets with labeled transitions.)
\[ \includegraphics[scale=1.25]{behavior} \]
The rectangles are the places of the net, and the dots labeled by \(\tau, x^R\), etc. are
the transitions of the net.
Write $i_x$ for the number of tokens at node $B_x$. The behavior $A_1'$ corresponds
to the initial marking $\{i_1{=}1,\, i_{10}{=}1\}$. We say that the nodes $\seq{B}$
together with the restricted names ($r,r'$) constitute a \emph{basis} for $A_1'$.
Note here that \(\traces{x}{A_1}\subseteq \traces{x}{A_1'} = 
\ptraces{\petrinet{A_1'}{x}}\) where \(\ptraces{\petrinet{A_1'}{x}}\) is the set of
traces of the Petri net. Thus, 
\(\ptraces{\petrinet{A_1'}{x}}\subseteq \spec\) is a sufficient condition
for  \(\traces{x}{A_1}\subseteq \spec\) .
The key point here is that
\(A_1'\) still has infinite states, but all its reachable states can be expressed in
the form \(\Thiding{r,r'}(i_1B_1 \TPAR \cdots \TPAR i_{11} B_{11})\)
(where \(i_kB_k\) is the parallel composition of \(i_k\) copies of \(B_k\)),  
a linear combination of finitely many processes \({\seq{B}}\).
That is why we could express \(A_1'\) by the Petri net as above.

\textbf{Step 3-2.} Construct a deterministic, minimized
 automaton \(M_\spec\) that accepts the language \(\spec\).
Here the initial marking is $\{i_{12}{=}1\}$.
\[ \includegraphics[scale=1.25]{spec} \]

\textbf{Step 3-3.} Construct another Petri net \(\Pcompose{\petrinet{A_1'}{x}}{\automaton{\spec}}\) from
\(\petrinet{A_1'}{x}\) and \(\automaton{\spec}\), which
 simulates the behavior of \(P_A\) and \(M_\spec\) simultaneously, so that
the problem of \(\traces{x}{A_1'}(=\ptraces{\petrinet{A_1'}{x}})\subseteq \spec\) 
is equivalent to a reachability problem
of \(\Pcompose{\petrinet{A_1'}{x}}{\automaton{\spec}}\). 
In the example, \(\Pcompose{\petrinet{A_1'}{x}}{\automaton{\spec}}\) has 
the initial marking $\{i_1{=}1,\, i_{10}{=}1,\, i_{12}{=}1\}$ and transitions such as 
 \(B_1 | B_{12} \Predwith{{I}} B_2 | B_{13}\).
\(\ptraces{\petrinet{A_1'}{x}}\subseteq \spec\) if and only if
the following unsafe state is unreachable.
\[
  (i_1{>}0 \wedge i_{12}{=}0) \vee (i_7{>}0 \wedge i_{13}{=}0) \vee (i_9{>}0 \wedge i_{13}{=}0) \vee (i_{11}{>}0 \wedge i_{13}{=}0)
\]
To explain, if $i_1>0\land i_{12}{=}0$ then the behavior is able to make an $R$ transition
but the specification automaton \(\automaton{\spec}\) is not able. 
%%Each disjunct has a similar form,
%%and together they characterize all unsafe states.

\textbf{Step 3-4.} Use an approximation algorithm to decide the reachability problem of
\(\Pcompose{\petrinet{A_1'}{x}}{\automaton{\spec}}\),
 in a manner similar to Kobayashi's type-based analyzer \texttt{TyPiCal}~\cite{TyPiCal}
for the \(\pi\)-calculus. 
%%%In the example we form (a possibly over-approximation of)
%%%the set of all reachable states
%%%from the initial marking, and check if any states satisfy the `unsafe' predicate:
%%%\[
%%%  (i_1{>}0 \wedge i_{12}{=}0) \vee (i_7{>}0 \wedge i_{13}{=}0) \vee (i_9{>}0 \wedge i_{13}{=}0) \vee (i_{11}{>}0 \wedge i_{13}{=}0)
%%%\]
%%%To explain, if $i_1>0$ then the behavior is able to make an $x^R$ transition
%%%but the specification is not able. Each disjunct has a similar form,
%%%and together they characterize all unsafe states.
%%%

The above steps 3-1, 3-2, and 3-3 are described in more detail below.
See Section~\ref{sec:implementation} for Step 3-4.
\subsubsection{Step 3-1: Construction of $\petrinet{A}{x}$}
\label{sec:petrinet-construction}
We first introduce the notion of a {\em basis}. The basis is analogous to
that of a vector space; Each state is expressed as a linear combination
of elements of the basis.
\begin{defi}
A pair \((\set{y_1,\ldots,y_m}, \set{B_1,\ldots,B_n})\) is a {\em basis} of
\(A\) if all of the following conditions are satisfied:
\begin{itemize}
\item
\(A \eqtype \Thiding{y_1}\cdots\Thiding{y_m}(i_1 B_1 \TPAR \cdots \TPAR i_n B_n)\)
for some \(i_1,\ldots,i_n\in\Nat\).
\item If \(B_j \Tredwith{\act} C\), then
there exist \(i_1,\ldots,i_n\in\Nat\) such that
\(C \eqtype i_1 B_1 \TPAR \cdots \TPAR i_n B_n\).
\item For each \(B_j\), there are only finitely many \(C\) (up to \(\eqtype\))
such that \(B_j \Tredwith{\act} C\).
\end{itemize}
\end{defi}
Note that if \((\set{\seq{y}}, \set{B_1,\ldots,B_n})\) is a basis of \(A\),
then whenever \(A\Treds A'\), there exist \(i_1,\ldots,i_n\) such that
\(A'\eqtype \Thiding{\seq{y}}(i_1 B_1 \TPAR \cdots \TPAR i_n B_n)\).
Let us write \(\baseindex(C)\) for \((i_1,\ldots,i_n)\) such that \(C\eqtype
i_1B_1\TPAR \cdots i_nB_n\). (If there are more than one such tuple,
\(\baseindex(C)\) picks one among them.)
Therefore, if \(\project{A}{\set{x}}\) has a basis, the behavior of \(\project{A}{\set{x}}\) is simulated by
the (labeled) Petri net \(\petrinetaux{A}{x}{(\set{\seq{y}},\set{\seq{B}})}\) given below.
Here, we use a process-like syntax to represent the elements of a Petri net rather
than the standard tuple notation \((P,T,F,W,M_0)\). A marking state
\(m\) which has \(i_k\) tokens for each place \(p_k\) (\(k\in\set{1,\ldots,n}\))
is written \(i_1p_1 \PPAR \cdots \PPAR i_np_n\). A transition that consumes
a marking \(m_1\) and produces \(m_2\) is expressed by \(m_1\Predwith{\gamma}m_2\),
where \(\gamma\) is the label of the transition.
\begin{itemize}
\item The set \(\Places\) of places is \(\set{\Place{B_1},\ldots,\Place{B_n}}\).
\item The initial marking \(\Marking_I\) is \(i_1\Place{B_1}\PAR \cdots \PAR i_n \Place{B_n}\)\\
where \(\project{A}{\set{x}} \eqtype \Thiding{\seq{y}}(i_1B_1\PAR \cdots \PAR i_nB_n)\).
\item The set of transitions consists of:
\begin{itemize}
\item %A net transition
\( %t:
   \Place{B_j} \Predwith{\tau} i_1 \Place{B_1} \PPAR \cdots \PPAR i_n \Place{B_n}\) \\
where \(\baseindex(C) = (i_1,\ldots,i_n)\),
for each %transition
\(B_j\redwith{\tau} C\).
\item %A net transition
\( %t:
   \Place{B_j} \Predwith{\acclab} i_1 \Place{B_1} \PPAR \cdots \PPAR i_n \Place{B_n}\) \\
where \(\baseindex(C) = (i_1,\ldots,i_n)\),
for each \(B_j\redwith{\actracc{\acclab}{x}}C\).
\item
\( %t:
   \Place{B_j}\PPAR \Place{B_{j'}} \Predwith{\tau} (i_1+i'_1) \Place{B_1} \PPAR \cdots
\PPAR (i_n + i'_n)\Place{B_n}\)
where \(\baseindex(C) = (i_1,\ldots,i_n)\) and \(\baseindex(C') = (i'_1,\ldots,i'_n)\),
for each pair of transitions
\(B_j \Tredwith{\actout{z}}C\) and
\(B_{j'}\Tredwith{\actin{z}}C'\) such that \(z\in \set{\seq{y}}\).
\end{itemize}
\end{itemize}

From now on we omit the basis and just write \(\petrinet{A}{x}\) for
\(\petrinetaux{A}{x}{(\set{\seq{y}},\set{\seq{B}})}\).
Let us write \(\ptraces{\petrinet{A}{x}}\) for the set:
\[ \set{\acclab_1 \cdots \acclab_k \mid \Marking_I \Predswith{\acclab_1} \cdots \Predswith{\acclab_k}\Marking'}\]
where \(\Predswith{\acclab}\) means \(\Predwith{\tau}^* \Predwith{\acclab}\Predwith{\tau}^*\).
By the construction of \(\petrinet{A}{x}\), \(\ptraces{\petrinet{A}{x}} = \traces{x}{A}\).

%%%We say that a behavioral type \(A\) is {\em atomic} if it satisfies all of the following conditions.
%%%\begin{itemize}
%%%\item \(A\)'s outermost constructor is not \(\TPAR\).
%%%\item \(A\) does not contain a constructor \(\exclude{\cdot}{S}\).
%%%\item The renaming operators \(\subst{\seq{y}}{\seq{x}}\) are only applied to
%%%   type variables and recursive behavioral types.
%%%\item If \(A\) is of the form \(\Thiding{x}{(A_1\TPAR \cdots\TPAR A_n)}\),
%%%  then every \(A_i\) contains a free occurrence of \(x\).
%%%\item \(A\) does not contain an unnecessary unfolding of
%%%recursion of the form \([\Trec{\Tbvar}A_1/\Tbvar]A_1\).
%%%\end{itemize}
%%%A behavioral type is in {\em normal form} if it is a parallel composition of atomic behavioral types.
%%%For any behavioral type \(A\), there is a normal form \(B\) such that \(A\eqtype B\).
%%%See Appendix~\ref{sec:normalization} for how to transform behavioral types into normal form.
%%%
%%%Let \(A\) be an atomic type.
%%%We define \(\Deriv(A)\) to be the least set satisfying the following rules.
%%%\[
%%%\begin{array}{l}
%%%\Deriv{A} \supseteq \set{A} \cup \bigcup\{\Deriv{A_1},\ldots,\Deriv{A_n}
%%%    \mid A \Tredwith{l} B\\
%%%\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad\myquad
%%% \mbox{and  $A_1\PAR \cdots \PAR A_n$ is a normal form of $B$}
%%%\}
%%%\end{array}
%%%\]
%%%Intuitively, \(\Deriv{A}\) is the set of atomic types that is sufficient for
%%%expressing all the possible transitions of \(A\) (up to equivalence of types).
%%%We extend \(\Deriv\) for non-atomic type, by defining
%%%\(\Deriv{A}= \Deriv{A_1}\cup \cdots \Deriv{A_n}\), where \(A_1\TPAR \cdots \TPAR A_n\)
%%%(here, we assume that we have some canonical way to choose one normal form).
%%%

The construction of \(\petrinet{A}{x}\) outlined above can be applied only when
a basis of \(\project{A}{x}\) can be found (by some heuristic algorithm).
If \(\project{A}{x}\) has no basis or cannot be found, we approximate \(\project{A}{x}\)
by moving all the \(\nu\)-prefixes to the top-level; for example,
\(\Tin{y}{\Thiding{x}A}\), \(\Trep{\Thiding{x}{A}}\) and
\(\Trec{\Tbvar}{\Thiding{x}{A}}\) are replaced by \(\Thiding{x}(\Tin{y}{A})\),
\({\Thiding{x}{\Trep{A}}}\), and
\(\Thiding{x}{\Trec{\Tbvar}{{A}}}\) respectively.
Let \(A'\) be the approximation of \(\project{A}{\set{x}}\).
It is easy to prove that \(A'\) is a sound approximation of \(\project{A}{\set{x}}\),
in the sense that \(\traces{x}{A}\subseteq \traces{x}{A'}\).

We can compute a basis of \(A'\) as follows
(see Appendix~\ref{sec:basis-of-behavioral-type} for more details).
Since \(\nu\)-prefixes do not appear inside recursion,
we can first eliminate the constructors \(\exclude{\cdot}{S}\), \(\project{\cdot}{S}\),
and \(\csubst{\seq{x}}{\seq{y}}\). Let \(\nuexp{\seq{y}}A''\) be the resulting
expression, where \(A''\) does not contain \(\exclude{\cdot}{S}\),
\(\csubst{\seq{x}}{\seq{y}}\), or \(\Thiding{x}\). Let \(\mathbf{B}\)
be the set of behavioral types that are
subexpressions of the behavioral types obtained from \(A''\) by
expanding recursive types and do not contain ``unnecessary'' unfolding
\(\subst{\Tbvar}{\Trec{\Tbvar}{A}}A\).
Then, \(\mathbf{B}\) is a finite set, and \((\set{\seq{y}}, \mathbf{B})\) is
a basis of \(A'\).
We can therefore construct a Petri net \(\petrinet{A'}{x}\).
By the construction, \(\ptraces{\petrinet{A'}{x}}=\traces{x}{A'} \supseteq \traces{x}{A}\),
so that \(\ptraces{\petrinet{A'}{x}}\subseteq \spec\) is a sufficient condition
for \(\traces{x}{A}\subseteq \spec\).


%%%Now we show how to construct \(\petrinetwithnu{A}{x}{\seq{y}}\).
%%%Let \(A\eqtype \nuexp{\seq{y}}(B_1\PAR cdots \PAR B_n)\) where
%%%\(B_1,\ldots,B_n\) are atomic.
%%%If the set \(\Deriv{B_1}\cup \cdots \cup \Deriv{B_n}\) is infinite (or at least cannot be decided to
%%%be finite in a reasonable amount of time),
%%%we first approximate each recursive type \(\Trec{\Tbvar}{A_1}\) occurring inside
%%%\(A\) with \(\subst{\Tbvar}{\Trec{\Tbvar}{A_1'}}A_1\) where \(A_1'\) is
%%%the type obtained from \(A_1\) by removing all the hiding constructors.
%%%Let the resulting type be \(A'\). Then \(\Deriv{B_1'}\cup \cdots \Deriv{B_n'}\)
%%%(where \(A' \eqtype \nuexp{\seq{y}'}(B_1\PAR \cdots \PAR B_n)\)) is a finite set,
%%%so we shall use \(A'\) instead of \(A\) below.
%%%Note that \(\traces{x}{A'}\subseteq \spec\) is a sufficient condition for
%%%\(\traces{x}{A}\subseteq \spec\), since \(\traces{x}{A'}\subtype \traces{x}{A}\).

%\begin{exa}
%\finish{Show how to obtain the approximation of the following type, and construct
%the Petri net for the approximation}
%\(\Trec{\Tbvar}{(\Toutatom{x}\TOR \Thiding{y}([y/x]\Tbvar\PAR \Tin{y}\Toutatom{x}))}\)
%is approximated.
%\end{exa}

%%%\finish{Treatment of bound variables are not sufficient below,
%%%so I will revise the remainder of this section.}
%%%
%%%Now assuming that the set \(\Deriv{A}\) is finite,
%%%we can define \(\petrinet{A}{x}{N}\) as follows.
%%%\begin{itemize}
%%%\item The set \(S\) of places is
%%%\[ \set{s_{B} \mid B\in \Deriv{B_1}\cup\cdots\cup \Deriv{B_n}}\]
%%%\item The initial marking \(m_I\) is \(n_1B_1\PAR n_kB_k\), where \(n_1B_1\PAR n_kB_k\) is a normal
%%%form of \(\project{A}{\set{x}}\).
%%%\item The set of transitions
%%%consists of (\(B,B',A_1,\ldots,A_k\) ranges over \(\Deriv{B_1}\cup\cdots\cup\Deriv{B_n}\) below):
%%%\begin{itemize}
%%%\item
%%%A net transition
%%%\[ t: s_B \Predwith{\tau} n_1 s_{A_1} \PPAR \cdots \PPAR n_k s_{A_k}\]
%%%for each transition \(B\redwith{\tau}\eqtype n_1A_1\TPAR\cdots\TPAR n_k A_k\).
%%%\item A net transition
%%%\[ t: s_B \Predwith{\acclab} n_1 s_{A_1} \PPAR \cdots \PPAR n_k s_{A_k}\]
%%%for each \(B\redwith{\actracc{\acclab}{x}}\eqtype n_1A_1\TPAR\cdots\TPAR n_k A_k\).
%%%\item A net transition
%%%\[ t: s_B \Predwith{\tau} n_1 s_{A_1} \PPAR \cdots \PPAR n_k s_{A_k}\]
%%%for each \(B\PAR B'\redwith{\tau}\eqtype n_1A_1\TPAR\cdots\TPAR n_k A_k\).
%%%\end{itemize}
%%%Here, \(nA\) represents parallel composition of \(n\) copies of \(A\).
%%%\end{itemize}
%%%Then,
%%%\[\traces{x}{A} =  \set{\acclab_1\cdots\acclab_m \mid m_I \Tredswith{\acclab_1}\cdots \Tredswith{\acclab_m}}\]

\subsubsection{Steps 3-2 and 3-3:
Construction of $\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}$ and
reduction of $\traces{x}{A}$ to a reachability problem}
% This section should also include discussions on an algorithm to decide
% \(\traces{x}{A}\subseteq \prefixclos{\spec}\);
% in particular, we will show that if \(A\) can be encoded as a petri net
% and if \(\spec\) can be encoded as a restricted form of petri net (``deterministic''
% petri net which we discussed in Redmond), then the problem is decidable (by
% a reduction to the reachability problem of Petri nets).
%%%Let \(\petrinet{A}{x}\) be a petri net that encodes behavior of \(\project{A}{x}\)
%%%and
Let \(\places{\petrinet{A}{x}}\)
and \(\transitions{\petrinet{A}{x}}\) be the sets of places and transitions of \(\petrinet{A}{x}\)
respectively.
%%%We assume that \(\petrinet{A}{x}\) is complete in the sense that
%%%\(\acclab_1\cdots\acclab_n \in \traces{x}{\project{A}{x}}\) if and only if
%%%\(m_1 \Predssilent\Predwith{\acclab_I}\Predssilent\cdots\Predssilent\Predwith{\acclab_n}\Predssilent m_n\)
%%%for some \(m_n\) where \(m_I\) is the initial state.
Let \(\automaton{\spec}\) be a minimized deterministic automaton\footnote{Note that since \(\spec\) is prefix-closed, all the states
of the minimized automaton are accepting states.}
that accepts \({\spec}\), and let \(\states{\spec}\) be its set of states and
\(\trans{\spec}\) be its transition function.

\begin{defi}
\label{def:composition-petrinet}
The \emph{composition} of
\(\petrinet{A}{x}\) and \(\automaton{\spec}\), written
\(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\), is defined as follows:
\begin{itemize}
\item The set of places is \(\places{\petrinet{A}{x}} \cup \states{\spec}\)
\item The set of transitions is:
\[
\begin{array}{l}
\set{ %t:
      (\Marking{|}q) \Predwith{\acclab} (\Marking'{|}q')
    \mid (%t:
          \Marking {\stackrel{\acclab}{\rightarrow}} \Marking') \in \transitions{\petrinet{A}{x}}\land
   \trans{\spec}(q, \acclab) = q'}\\
\cup
\set{ %t:
      \Marking \Predwith{\tau}\Marking'
    \mid (%t:
          \Marking {\stackrel{\tau}{\rightarrow}}\Marking')\in \transitions{\petrinet{A}{x}}}
%%%\{t: \s_1 \PPAR \cdots \PPAR s_n \PPAR q\Predwith{\acclab} k_1 s_1' \PPAR \cdots \PPAR k_m s'_m \PPAR q'\\
%%%  \mid (t: s_1 \PPAR \cdots \PPAR s_n \Predwith{\acclab} k_1 s_1' \PPAR \cdots \PPAR k_m s_m)\in
%%%      \transitions{\petrinet{A}{x}} \land \trans{\spec}(q, \acclab) = q'\}
\end{array}
\]
%%%\begin{itemize}
%%%\item A transition \(t' : s_1 \PPAR \cdots \PPAR s_n \PPAR q \Predwith{\acclab} k_1 s_1' \PPAR \cdots \PPAR k_m s_m \PPAR q'\) for each transition
%%% \((t: s_1 \PPAR \cdots \PPAR s_n \Predwith{\acclab} k_1 s_1' \PPAR \cdots \PPAR k_m s_m)\)
%%%of  \(\in \transitions{\petrinet{A}{x}}\) and \(\trans{\spec}(q, \acclab) = q'\).
%%%\item A transition
%%%\end{itemize}
\item Initial state is \(\Marking_I \PPAR q_I\) where \(m_I\) is the initial state of
\(\petrinet{A}{x}\) and \(q_I\) is the initial state of \(\automaton{\spec}\).
\end{itemize}
%%%We write \(\PDerivedTransition{t}{t'}\)
%%%if \(t'\) is obtained from \(t\)
%%%(i.e. \(t' : s_1 \PPAR \cdots \PPAR s_n \PPAR q_j \Predwith{l} k_1 s_1' \PPAR \cdots \PPAR k_m s_m \PPAR q_j'\) and \((t: s_1 \PPAR \cdots \PPAR s_n \Predwith{l} k_1 s_1' \PPAR \cdots \PPAR k_m s_m) \in \transitions{\petrinet{A}{x}}\) and
%%%\(\trans{\spec}(q_j, l) = q_j'\)
%%%%% if \((t: m_i \Predwith{l} m_i') \in \transitions{\petrinet{A}{x}}\) and
%%%%% \(\trans{\spec}(q_j, l) = q_j'\)
%%%for some \(m_i\) and \(m_i'\) and \(l\) and \(q_j\) and \(q_j'\)).
\end{defi}
%
Now, \(\ptraces{\petrinet{A}{x}}\subseteq \spec\) can be reduced to the reachability problems of
\(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\).
\begin{thm}
\label{le:petrinet-reachability}
\(\ptraces{\petrinet{A}{x}} \subseteq {\spec}\)
if and only if no marking \(\Marking\PPAR q\) that satisfies the following conditions is reachable:
\begin{itemize}
%%%\item \(\Marking\PPAR q\) is reachable by \(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\).
\item \(\Marking \Predwith{\acclab}\Marking'\) for some \(\Marking'\) and \(\acclab\) in \(\petrinet{A}{x}\).
\item \(\trans{\spec}(q, \acclab)\) is undefined.
\end{itemize}
\end{thm}
%
Thus, we can reduce
\(\ptraces{\petrinet{A}{x}}\subseteq \spec\) to a finite set of reachability problems of
\(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\). Hence
\(\ptraces{\petrinet{A}{x}}\subseteq \spec\) is decidable~\cite{MayrPetriNet}.

\begin{cor}
\(\ptraces{\petrinet{A}{x}} \subseteq {\spec}\)
if and only if
for every transition rule of the form \(%t:
                                        \Marking_1 \Predwith{\acclab} \Marking_2\)
 of \(\petrinet{A}{x}\) and \(q\) such that \(\trans{\spec}(q,\acclab)\) is undefined,
no marking \(\Marking\) such that \(\Marking \geq \Marking_1\PAR q\) is reachable by
\(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\).
%%%
%%%no marking \(\Marking\PPAR q\) that satisfies the following conditions is reachable:
%%%No \(m\) such that \(\Illmark{m}\) is reachable if and only if
%%%\(k_1 s_1 \PPAR \cdots \PPAR k_n s_n\) where \(k_i > 0\) is unreachable
%%%for every \(t: s_1 \PPAR \cdots \PPAR s_n \PPAR q_i \Predwith{l} m' \PPAR q_j\)
%%%in \(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\).
\end{cor}

\begin{rem}
\label{rem:petri-lang-as-spec}
We can actually extend the above algorithm for
checking \(\traces{x}{A}\subseteq \spec\) to deal with the case where
\(\spec\) belongs to the class of
deterministic Petri net languages (more precisely, the class of P-type languages
of \(\lambda\)-free, deterministic Petri nets~\cite{PetriBook,Pelz87}).
If \(\spec\) is the P-type language of a \(\lambda\)-free, deterministic Petri net,
then its complement \(\overline{\spec}\) is a Petri net language~\cite{Pelz87}.
Therefore, we can construct a Petri net that accepts the intersection of
the language of \(\petrinet{A}{x}\) and \(\overline{\spec}\)~\cite{PetriBook}),
so that \(\ptraces{\petrinet{A}{x}}\subseteq \spec\) can be reduced to the
emptiness problem of the Petri net, which is decidable due to the decidability
of the reachability problem.

Some of the useful resource usage specifications are not regular languages but
are deterministic Petri net language. For example, consider a stack-like resource on which,
at any point of program execution,
the number of times the operation \textit{pop} has been performed is less
than the number of times \textit{push} has been performed. Such specification is
expressible as a deterministic Petri net language.
\end{rem}



%%%\begin{defi}
%%%\(\dup{\petrinet{A}{x}}\) is a petri net derived from \(\petrinet{A}{x}\) as follows:
%%%\begin{itemize}
%%%\item \(\places{\dup{\petrinet{A}{x}}} = \places{\petrinet{A}{x}} \cup \set{\coplace{s} | s \in \places{\petrinet{A}{x}}}\)
%%%\item \(\transitions{\dup{\petrinet{A}{x}}}\) consists of the following transitions:
%%%\begin{itemize}
%%%\item \(s_i \Predwith{} \coplace{s_i}\) for every \(s_i \in \petrinet{A}{x}\).
%%%\item \(2 \coplace{s_i} \Predwith{} \coplace{s_i}\) for every \(s_i \in \petrinet{A}{x}\)
%%%\item \(\coplace{s_1} \PPAR \cdots \PPAR \coplace{s_n} \Predwith{l} k_1 s_1' \PPAR \cdots \PPAR k_m s_m'\)
%%%for every \((s_1 \PPAR \cdots \PPAR s_n \Predwith{l} k_1 s_1' \PPAR \cdots \PPAR k_m s_m') \in \transitions{\petrinet{A}{x}}\)
%%%\end{itemize}
%%%\end{itemize}
%%%\end{defi}
%%%
%%%\begin{lemma}
%%%\(k_1 s_1 \PPAR \cdots \PPAR k_n s_n\) where \(k_i > 0\) is unreachable
%%%for every \(t: s_1 \PPAR \cdots \PPAR s_n \PPAR q_i \Predwith{l} m' \PPAR q_j\)
%%%in \(\Pcompose{\petrinet{A}{x}}{\automaton{\spec}}\)
%%%if and only if
%%%\(\coplace{s_1} \PPAR \cdots \PPAR \coplace{s_n}\) is unreachable
%%%for every \(t: \coplace{s_1} \PPAR \cdots \PPAR \coplace{s_n} \PPAR q_i \Predwith{l} m' \PPAR q_j\)
%%%in \(\Pcompose{\dup{\petrinet{A}{x}}}{\automaton{\spec}}\).
%%%\end{lemma}


==> Intro.tex <==
\section{Introduction}
\label{sec:intro}

Computer programs access many external resources, such as files,
library functions, device drivers, etc. Such resources are often associated with
certain access protocols; for example, an opened file should be eventually closed
and after the file has been closed, no read/write access is allowed.
The aim of resource usage analysis~\cite{IK05TOPLAS} is to statically check that programs conform to such
access protocols.
Although a number of approaches, including type systems and model checking,
have been proposed so far for the resource usage analysis or similar
analyses~\cite{DeLine01PLDI,DeLine02PLDI,Aiken02PLDI,IK05TOPLAS,SLAM},
most of them focused on analysis of sequential programs, and did not treat concurrent programs,
especially those involving dynamic creation/passing of channels and resources.
%%%in a satisfactory manner.

In the present paper, we propose a type-based method of resource usage analysis for
{\em concurrent languages}.
Dealing with concurrency is especially important because concurrent programs are hard to debug,
and also because actual programs accessing resources are often concurrent.
We use the \(\pi\)-calculus (extended with resource primitives)
as a target language so that our analysis can be applied to
a wide range of concurrency primitives (including 
those for dynamically creating and passing channels) in a uniform manner.

%% We explain the main idea of our type-based analysis below.
%% In Igarashi and Kobayashi's type-based resource usage analysis
%% for the \(\lambda\)-calculus~\cite{IK05TOPLAS}, resource types
%% were extended with information about how the resources can be accessed.
%% For example, a read-only file was given the type \((\textbf{File}, R^*C)\), where
%% \(R\) denotes a read operation, and \(C\) denotes a close operation.
%% We follow the same approach, and extend resource types and channel types
%% with information about how they are accessed and used for communications.
%% We infer the extended types through type inference and then check that
%% the inferred access sequences conform to the specification of each resource.

A main new difficulty in dealing with concurrent programs is that 
control structures are more complex in concurrent programs
than in sequential programs.
For example, consider the following process \(P_1\):
\[
  \nuexp{c}(\Read(x).\outatom{c}{\,}{}\PAR \inexp{c}{\,}{}\Close(x))
\]
Here, \(\Read(x).\outatom{c}{\,}{}\) reads \(x\) and then sends a signal on channel
\(c\), and in parallel to that, \(\inexp{c}{\,}{}\Close(x)\) waits for a signal on
channel \(c\) and then closes \(x\). Because of the synchronization through channel
\(c\), \(x\) is closed only after being read. To capture this kind of causal dependency
between communications and resource access, we use CCS processes
as extra type information (which are called behavioral types).
For example, the above process is given the behavioral type
\(\nuexp{c}(\Tacc{R}{x}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{x})\).

Using the behavioral types introduced above, we can construct a type system for resource usage analysis
in a manner similar to previous behavioral
type systems for the \(\pi\)-calculus~\cite{Kobayashi03TCS,Rehof02POPL}.
A type judgment is of the form \( \tjudge{\Gamma}{P}{A}\),
where \(\Gamma\) is the usual type environment and \(A\) is a behavioral type approximating the behavior of
\(P\) on the free channels and resources.
For example, the above process \(P_1\) is typed
\(\tjudge{x\COL\Tres}{P_1}{\nuexp{c}(\Tacc{R}{x}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{x})}\).
Behavioral types are also used to augment channel types.
The judgment for \(\inexp{s}{x}{}P_1\) is given by:
\[
\tjudge{\Gamma\ \ }
   {\ \ \inexp{s}{x}{}P_1\ \ }
   {\ \ \Tinatom{s}}
 \]
where \(\Gamma = s{:}\Tchan{(x{:}\Tres)\nuexp{c}(\Tacc{R}{x}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{x})}\).
Here, the behavioral type of \(\inexp{s}{x}{}P_1\) is simply a single input command \(s\):
the characteristic feature of this kind of type system is that the behavior of the input continuation is
accounted for at output, not at input.
The channel \(s\) has \emph{argument type} \((x{:}\Tres)\nuexp{c}(\Tacc{R}{x}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{x})\), which
specifies that the resource sent along channel \(s\) will be read first and then closed.
Using the same type environment, the output process \(\outatom{s}{r}{}\) is typed as:
\[
\tjudge{\Gamma, r{:}\Tres\ \ }
{\ \ \outatom{s}{r}{}\ \ }
{\ \ \Tout{s}\nuexp{c}(\Tacc{R}{r}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{r})} \]
Here the behavioral type is an output followed by a continuation.
The continuation\\
\(\nuexp{c}(\Tacc{R}{r}\Toutatom{c}\TPAR \Tin{c}\Taccatom{C}{r})\)
has been obtained by substituting \(r\) for \(x\) in the argument type of \(s\).
In this way, the types propagate information about how resources and channels passed thorough channels
are accessed.

An important property of our type system is that
types express abstract behavior
of processes, so that certain properties of processes can be verified
by verifying the corresponding properties of their types, using, for example,
model checking techniques.
The latter properties (of behavioral types) are more amenable 
to automatic verification techniques like model checking than the former ones,
because the types do not have channel mobility and also because the types typically
represent only the behavior of a part of the entire process.

The technical contributions of the present work are summarized as follows.
\begin{itemize}
\item Formalization of type systems for resource usage analysis for the \(\pi\)-calculus,
% We have formalized type systems for resource usage analysis for the \(\pi\)-calculus,
and proof of their soundness.
We have augmented previous behavioral types for the \(\pi\)-calculus
with hiding and renaming constructors, and adapted them to the problem of resource usage analysis.
CCS-like processes have been used as types also in previous work on type systems
for the \(\pi\)-calculus~\cite{Kobayashi03TCS,Rehof02POPL}.
Igarashi and Kobayashi~\cite{Kobayashi03TCS}, however, used a fragment without
hiding and renaming, and Chaki et al.~\cite{Rehof02POPL} used a fragment without
renaming, while the present paper uses both hiding and renaming. The inclusion of hiding and
renaming is important both for accuracy and for automatic inference
(see Remark~\ref{rem:combination-of-hiding-and-renaming}).
%% \item We have developed a type inference algorithm, which includes a procedure to
%% check the conformance of inferred usage with respect to a resource usage specification
%% (expressed using a regular language); the algorithm for checking conformance was left
%% open in Igarashi and Kobayashi's resource usage analysis for the \(\lambda\)-calculus.
\item Realization of fully automatic verification (while making the analysis 
% We realized fully automatic verification (while making the analysis 
 more precise than \cite{Kobayashi03TCS}).
Igarashi and Kobayashi~\cite{Kobayashi03TCS} gave only an abstract type system,
without giving a concrete type inference algorithm. 
Chaki et al.~\cite{Rehof02POPL} requires type annotations.
The full automation was enabled
by a combination of a number of small ideas, like inclusion of hiding and renaming
as type constructors, and 
%% (Igarashi and Kobayashi~\cite{Kobayashi03TCS} used a fragment without
%% hiding and renaming, and Chaki et al.~\cite{Rehof02POPL} used a fragment without
%% renaming), 
approximation of a CCS-like type by a Petri net (to reduce the problem of
checking conformance of inferred types to resource usage specification).
\item Verification of not only the usual safety property that an invalid resource
access does not occur, but also an extended safety (which we call {\em partial liveness})
that necessary resource accesses (e.g. closing of a file) are eventually performed
unless the whole process diverges. The partial liveness is not guaranteed by
Chaki et al.'s type system~\cite{Rehof02POPL}.
A noteworthy point about our type system for guaranteeing the partial liveness is that it is parameterized by
a mechanism that guarantees deadlock-freedom (in the sense of Kobayashi's
definition~\cite{Kobayashi02IC}). So, our type system can be combined with {\em any} mechanism
(model checking, abstract interpretation, another type system, or whatever) to verify deadlock-freedom
for deadlock- or lock-freedom (e.g., Yoshida's graph type system~\cite{Yoshida96FST}).
\item Implementation of a prototype resource usage analyzer based on the proposed method.
The implementation can be tested at \url{http://www.yl.is.s.u-tokyo.ac.jp/~kohei/usage-pi/}.
\end{itemize}
%% Technically, the closest to our type system is the type system of Chaki et al.~\cite{Rehof02POPL}.
%% The main differences (besides the obvious difference that Chaki et al.~\cite{Rehof02POPL}
%%  does not treat resources as primitives; see Remark~\ref{rem:resources}) are (1) our analysis does not require any
%% type annotations except for annotations to specify (not to assist) how resources should
%% be used, while Chaki et al.'s type system requires heavy annotations on channel types,
%% and (2) the extension of our analysis in Section~\ref{sec:extension} can
%% infer partial liveness, like the requirement that a file be eventually closed,
%% while Chaki et al.'s type system cannot.

The rest of this paper is structured as follows.
Section~\ref{sec:syntax} introduces an extension of the \(\pi\)-calculus with
primitives for creating and accessing resources. Section~\ref{sec:typing} introduces a type system
for resource usage analysis, which guarantees that well-typed processes
never perform an invalid resource access. Section~\ref{sec:inference}
gives a type inference algorithm for the type system.
Section~\ref{sec:extension} extends the type system to guarantee that necessary resource
accesses (such as closing of opened files) are eventually performed (unless the program diverges).
%% A noteworthy point about the extended type system is that it is parameterized by
%% a type system that guarantees deadlock- or lock-freedom (in the sense of Kobayashi's
%% definition~\cite{Kobayashi02IC}). So, our type system can be combined with {\em any} type system
%% for deadlock- or lock-freedom (e.g., Yoshida's graph type system~\cite{Yoshida96FST}).
Section~\ref{sec:implementation} describes a prototype resource usage analyzer we have implemented based
on the present work.
Section~\ref{sec:related} discusses related work.
Section~\ref{sec:conclusion} concludes.


==> Normalization.tex <==

\section{Normalization of Behavioral Types}
\label{sec:normalization}
\def\excludeaux#1#2#3#4{{#3}\uparrow_{#4}^{#1,#2}}

\(\exclude{A}{S}\) can be removed as follows:
\[
\begin{array}{l}
\exclude{A}{S} = \excludeaux{\emptyset}{\emptyset}{A}{S}\\
\excludeaux{D}{F}{\Tzero}{S} = \Tzero\\
\excludeaux{D}{F}{\Tact{\act}{A}}{S} = \Tact{(\act\backslash{S})}{\excludeaux{D}{F}{A}{S}}\\
\excludeaux{D}{F}{\Tbvar}{S} = 
  \left\{
   \begin{array}{ll}
       A & \mbox{if $F(\Tbvar,S) = A$}\\
       \Trec{\beta}{\excludeaux{D}{F\set{(\Tbvar,S)\mapsto \beta}}{D(\Tbvar)}{S}}
        & \mbox{if $(\Tbvar,S)\not\in \dom(F)$}
   \end{array}\right.\\
\excludeaux{D}{F}{\Trec{\Tbvar}{A}}{S} =
  \excludeaux{D\set{\Tbvar\mapsto A}}{F\set{(\Tbvar,S)\mapsto A}}{\Trec{\Tbvar}{A}}{S}\\
\excludeaux{D}{F}{[\seq{y}/\seq{x}]A}{S} =
  \excludeaux{D}{F}{A}{\set{z \mid [\seq{y}/\seq{x}]z\in S}}\\
\excludeaux{D}{F}{\Thiding{x}{A}}{S} =
   \Thiding{x}{\excludeaux{D}{F}{A}{S}} \mbox{ (we assume that $x$ does not ocur in $D,F,S$)}\\
\cdots
\end{array}
\]
Here, \(D\) keeps recursive definitions and \(F\) is a cache.

[*** How can we show that \(\exclude{A}{S}\) given above is well-defined?
 --- probably because \(S\) can contain only free variables, so that
 \(F\) ranges over a finite set ***]

We also assume that renamings are applied only to variables
\(\Tbvar\) and recursive types \(\Trec{\Tbvar}{A}\).
\def\rename#1#2{[{#2}/{#1}]}
\[
\begin{array}{l}
\rename{\seq x}{\seq y}\Tzero = \Tzero\\
\rename{\seq x}{\seq y}\Tact{\act}A =
   \Tact{\rename{\seq x}{\seq y}\act}\rename{\seq x}{\seq y}A\\
\rename{\seq x}{\seq y}(A_1\PAR A_2) =
  (\rename{\seq x}{\seq y}A_1) \PAR (\rename{\seq x}{\seq y}A_2) \\
\rename{\seq x}{\seq y}\rename{\seq x'}{\seq y'}A =
  (\rename{\seq x}{\seq y}\circ \rename{\seq x'}{\seq y'})A\\
\cdots
\end{array}
\]
\begin{remark}
It is not trivial to remove \([y/x]\Trec{\Tbvar}{A}\) as well.
Consider
\[ [y/x]\Trec{\Tbvar}x.y.[z/x]\Tbvar\]
We need a definition similar to that of \(\excludeaux{D}{F}{A}{S}\),
and again we are left with the question of whether the definition is well-formed.
\end{remark}

We can also push operators \(\Thiding{x}{}\) and \(\Trep\) inside as much as possible:
\[
\begin{array}{l}
\Trep{(A_1|A_2)} = \Trep{A_1}\PAR \Trep{A_2}\\
\Thiding{x}{(A_1|A_2)} = \Thiding{x}{A_1} \PAR A_2 \mbox{ if $x$ is not free in $A_2$}\\
\Thiding{x}{A} = A \mbox{ if $x$ is not free in $A$}\\
\end{array}
\]



==> Object.tex <==
\section{Further Applications: Analysis of Race and Deadlock of Concurrent
Objects}
\label{sec:object}

The type systems for race- and deadlock-freedom, presented in the last
section, are indeed powerful enough to guarantee some useful properties
about concurrent objects.  In essence, a concurrent object is regarded as
a  set of processes that provides a collection of services 
(e.g., methods)~\cite{Jones93CONCUR,Pierce95TPPP,Kobayashi95TAPOS}, just as a
sequential object is a set of functions.  Clients refer to an object
through a record of channels that represent locations of those services.
Hence, by giving an appropriate type to the record, we can enforce a certain
protocol that clients should respect.  Since our type system can capture,
in particular,  temporal dependency on the invoked services, it is
possible to guarantee race-freedom of accesses to methods, studied by
Abadi, Flanagan and Freund~\cite{Flanagan99CONCUR,Flanagan00PLDI}, 
and deadlock-freedom for objects with non-uniform
service availability, studied by Puntigam~\cite{Puntigam99SAC}.  
Note that, so far, these properties
have been discussed only for languages with primitive notion of objects. 
This section demonstrates how our type system can guarantee these properties.
%%at the level of the \(\pi\)-calculus.

We first describe how to enforce race-free accesses to methods.  For
example, the following
process %% expression \(P\) 
waits for a request on {\it newob}, and upon receiving a request,
creates an object with a lock \(l\) and 
a method \(m\) to print out the string ``Hello, '' appended to a given
string, and exports
its interface \([l, m]\) through the reply channel \(r\). 
\[
%%P \stackrel{\mbox{\tiny def}}{=}
\begin{array}{l}
\repexp \inexp{newob}{r}{\,}
\nuexp{l, m}( \\
\quad \;\;\outnilatom{l}{\ev'} \PAR \repexp \inexp{m}{s,r'}{\ev'}
             \outexp{print}{\mbox{``Hello, ''}}{\ev'}
             \outexp{print}{s}{\ev'}
             \outnilatom{r'}{\ev'} \\
\quad \PAR \outatom{r}{l,m}{}
)
\end{array}
\]
% (The expression \(\{l=lc,m=mc\}\) is a record of channels \(lc\) and \(mc\)
% with labels \(l\) and \(m\), respectively.)
Since the method \(m\) should not be invoked concurrently,%
\footnote{We do not want an output like ``Hello, Hello, ''.} clients
should acquire and release the lock \(l\) before and after the
invocation of \(m\), respectively.  Indeed by using \(\reliable_2\),
it is guaranteed that there are no simultaneous outputs to \(m\):

The exported interface \([l,m]\) (through which clients access to the
object) can be given a type:
\[
       \typ{l,m}{\TREPA \InTEnil{l}{\ev'}
           \OutTEatom{m}{\typ{s \COL \mathit{String},r}{( 
              \OutTEatom{r}{\typ{}{\OutTEnilatom{l}{\ev'}}{}}{\ev'})}}{\ev} 
               },
\]
where \(\TREPA\Gamma\) abbreviates \(\recty{\tev}{(\zeroTE\TIOR
  (\Gamma\TEPAR\tev))}\), meaning that the tuple can be used according
to \(\Gamma\) by arbitrarily many processes. (Here, we assume that the
subtyping relation \(\subTE\) satisfies \(\evTE{\ev}\PrTy\TEcong
\PrTy\) and that \textit{String} is some unary tuple type; the
notation \(\typ{s \COL \mathit{String}, r}{\Gamma}\) stands for
\(\typ{s, r}{(\appty{\mathit{String}}{s} \TEPAR \Gamma)}\).)  The
process type 
\(
\InTEnil{l}{\ev'} \OutTEatom{m}{\typ{s \COL
    \mathit{String},r}{(
    \OutTEatom{r}{\typ{}{\OutTEnilatom{l}{\ev'}}{}}{\ev'})}}{\ev}
\)
means that (1) the lock must be acquired (by an input from \(l\))
before the method is invoked (by an output to \(m\)); (2) the method
argument must be a pair of string \(s\) and a reply channel \(r\); and
(3) the lock must be released (by an output to \(l\))
but only after the reply from the object is sent to \(r\).  Note that
the tuple type \(\typ{s \COL \mathit{String} ,r}
{(\OutTEatom{r}{\typ{}{\OutTEnilatom{l}{\ev'}}{}}{\ev'})}\) refers to
the lock \(l\) as a free variable, making it possible to express
temporal dependency between \(l\), which is \emph{not} passed to the
method body, and the reply channel \(r\).

Then, a client
\[
%%\outexp{newob}{r}{\ev'}\inexp{r}{l,m}{\ev'}(
\begin{array}{l}
\;\; \nuexp{r_1}(\innil{l}{\ev'}\outexp{m}{\mbox{``Atsushi''},r_1}{\ev}
    \innil{r_1}{\ev'}\outnilatom{l}{\ev'}) \\
\PAR
\nuexp{r_2}(\innil{l}{\ev'}\outexp{m}{\mbox{``Naoki''},r_2}{\ev}
    \innil{r_2}{\ev'}\outnilatom{l}{\ev'})
\end{array}
\]
is well typed, but neither 
\[
\nuexp{r_3}(\outexp{m}{\mbox{``Atsushi''}, r_3}{\ev}\innil{r_3}{\ev'}P) 
\]
nor 
\[
\nuexp{r_4}(\innil{l}{\ev'}\outexp{m}{\mbox{``Naoki''},r_4}{\ev}(
    \innilatom{r_4}{\ev'} \PAR \outnilatom{l}{\ev'}))
\]
 is.
The above type of the interface roughly corresponds to  the object
type \([m:\varsigma(l)String\rightarrow Unit\cdot\{l\}\cdot+]\) of
Abadi and Flanagan's type system~\cite{Flanagan99CONCUR}, which means
that the method \(m\) can be invoked only after the lock on the object
is acquired.  
%
\finishlater{
In Flanagan and Abadi's type system~\cite{Flanagan99CONCUR}, the
above tuple type roughly corresponds to their object type
\([m:\varsigma(l)String\rightarrow Proc\cdot\{l\}\cdot+]\), which means an
object with the method \(m\), invoked only after acquisition of the lock on
the object.  
}
%
Unfortunately, our type system is less expressive than theirs
in some respects.  As the example shows, channels representing a
lock \(l\) and a method \(m\) guarded by the lock must be created
at once; % and, moreover, those channels always have to be carried together;
Otherwise, our type system will lose dependency among those
channels.  See Section~\ref{sec:extension} for a possible remedy against
the problem.


Similarly, we can express non-uniform service availability in our type
system.
For example, this is a process that creates a one-place buffer:
\[
\begin{array}{l}
\repexp\inexp{\mbox{\it newbuf\/}}{r}{\,}\nuexp{put, get, b}( \\
\quad \;\; \outnilatom{b}{} 
\PAR \repexp\innil{b}{}\inexp{put}{x}{}\inexp{get}{r'}{}
(\outatom{r'}{x}{}\PAR \outnilatom{b}{}) \\
\quad \PAR \outatom{r}{put,get}{})
\end{array}
\]
Now, two methods \(put\) and \(get\) are provided but they are
available only alternately.  
%%%Thus, clients are required to use the method
%%%\(get\) only {\em after\/} the method \(put\) is invoked.
%%%Again, this protocol can be enforced by using \(\reliable_3\).
%%Assume the event ordering \(\EOrd\) such that \(\ev' \EOrd \ev\).
By using \(\reliable_4\), we can guarantee that
 invocations of the methods \(put\) and \(get\) never
get deadlocked. The interface \([put,get]\) can be given a type:
%%%\[
%%%\TEREP \outTEatom{\mbox{\it newbuf\/}}{
%%%  \outtyatom{1}{
%%%    \TREP (\outtyatom{1}{\tau}{\ev'}{1} \TEPAR
%%%           \recty{\tv}(\evty{\ev'}\tv \TEIOR 
%%%                       \outtyatom{2}{\outtyatom{1}{\tau}{\ev}{1}}{\ev}{1}))\,
%%%  }{}{2}
%%%}{}{1} \TEPAR \cdots
%%%\]
\[
   \typ{put,get}{
      \evTE{\evmax}\recTE{\tev}{(\zeroty\TEIOR
           (\OutTEatom{put}{\tau}{\ev} \TEPAR
           \evTE{\evmax}
                       \OutTE{get}{(r)\OutTEatom{r}{\tau}{\ev}}{\ev}
                       \evTE{\evmax}\tev))}},
\]
which says that an output to \(put\) must come in parallel to or before an
output to \(get\). (Here, \(\evTE{\evmax}\Gamma\) abbreviates
\(\recTE{\tev}{(\Gamma\TEIOR
\evTE{\ev_1}\tev\TEIOR\cdots\TEIOR\evTE{\ev_n}\tev)}\) 
where \(\{\ev_1,\ldots,\ev_n\}\) is the set of events occurring in the program.
It means that it is allowed to wait for arbitrary events before using the value
according to \(\Gamma\).)
Then, both 
\[
%%\outexp{\mbox{\it newbuf\/}}{r}{}\inexp{r}{put,get}{}(
\outatom{put}{v}{\ev}
\PAR 
\nuexp{r}\outexp{get}{r}{\ev}\inexp{r}{x}{}\cdots
\]
and 
\[
%%\outexp{\mbox{\it newbuf\/}}{r}{}\inexp{r}{put,get}{}
\outexp{put}{v}{\ev}\nuexp{r}\outexp{get}{r}{\ev}\inexp{r}{x}{}\cdots
\]
are well-typed (and hence never get deadlocked on \(put!\) and \(get!\)) while
\(
%%\outexp{\mbox{\it newbuf\/}}{r}{}\inexp{r}{put,get}{}
\nuexp{r'}\outexp{get}{r'}{\ev}\inexp{r'}{x}{}\outexp{put}{v}{\ev}\cdots
\)
is not.

\endinput


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% By putting \(P \PAR \outatom{l}{}{\ev'}\) and clients of the
% object under the type environment
% \[
% \begin{array}{cl}
% & \outTEatom{l}{\zeroty}{\ev'}{0} \\
% \TEPAR &
% \TEREP (\inTE{m}{1:String \TPAR \outtyatom{2}{\zeroty}{\ev'}{0}}{\ev}{2}
%        \evty{\ev'}\evty{\ev'}\evtyatom{\ev'}) \\
% \TEPAR & \TEREP (\outTEatom{print}{1:String}{\ev'}{1}) \\
% \TEPAR & \TEREP (\inTE{l}{\zeroty}{\ev'}{0}
%        \outTE{m}{1:String \TPAR \outtyatom{2}{\zeroty}{\ev'}{0}}{\ev}{2}
%        \evty{\ev'}\outTEatom{l}{\zeroty}{\ev'}{0})
% \end{array}
% \]
% we can indeed guarantee that the method \(m\) will never be invoked
% simultaneously.  The last part
% \[
% (\inTE{l}{\zeroty}{\ev'}{0}
%        \outTE{m}{1:String \TPAR \outtyatom{2}{\zeroty}{\ev'}{0}}{\ev}{2}
%        \evty{\ev'}\outTEatom{l}{\zeroty}{\ev'}{0})
% \]
%  enforces that each invocation of \(m\) must be preceded by the acquisition
% of a lock and be followed by the release of the lock.  


% The above type environment allows exactly one access to \(m\) between the
% acquisition and release of the lock \(l\).  More generally, we can allow
% multiple sequential accesses to multiple methods \(m_1, \ldots, m_k\)
% by the following type environment: 
% \[
% \TEREP \inTE{l}{\zeroty}{\ev'}{0}\recty{\rho}
% (\outTE{l}{\zeroty}{\ev'}{0}\TIOR \outTE{m_1}{\tau_1}{\ev}{n_1}\rho
% \TIOR \cdots \TIOR \outTE{m_k}{\tau_k}{\ev}{n_k}\rho)
% \]
% After acquiring a lock, a process well-typed under the above type
% environment can immediately release the lock or invoke one of the methods
% \(m_1\) through \(m_k\).  The recursive type expresses that the process,
% after invoking a method, gets back to the point where the choice was made.









% from the corresponding channel, manipulates the object's state, which is
% also represented by a channel, and returns a result to the callee.
% The process expression below shows a typical pattern:
% \[
% \repexp (\inexp{m_1}{x,r}{\ev_1} \cdots . \outatom{r}{result}{\ev_2})
% \PAR \cdots \PAR
% \repexp (\inexp{m_k}{x,r}{\ev_3} \cdots . \outatom{r}{result}{\ev_4})
% \]
% Since object states do not play an important role in our examples,
% we don't deal with the states of objects explicitly and an object is
% represented by just a set of replicated input processes.

\subsection{Race-free Method Invocations}

As Abadi and Flanagan's type system~\cite{}, our type system can prevent a
group of methods from being invoked simultaneously.  We consider a variant
of the second type system in the last section, where a race condition on
the {\em output\/} with the event \(\ev\) is prevented.  
% by associating a channel to represent a lock on the object.

\subsection{Deadlock Freedom for Objects with Non-Uniform Services}

An object's available methods may depend on the state of the object and
vary from time to time.  For example, consider the
following process expression 
\[
P \stackrel{\mbox{\tiny def}}{=}
\nuexp{b}(\outexp{b}{}{\ev'}
\PAR
\repexp \inexp{b}{}{\ev'}\inexp{put}{x}{\ev'}\inexp{get}{r}{\ev}
        \outexp{r}{x}{\ev'}\outexp{b}{}{\ev'}
)
\]
representing a one-place buffer object: It can accept invocations of the
methods put and get, but only alternately.  
By using the third type system
in the last section, we can guarantee that the invocation of get never gets
stuck: Clients are enforced to respect a protocol such that each invocation
of get comes with exactly one invocation of put performed before get.

First, the process expression \(P\) is well typed under the following type
environment: 
\[
\Gamma_1 \stackrel{\mbox{\tiny def}}{=}
\evTEatom{\ev'} \TEPAR 
\evTE{\ev'}\inTE{put}{\tau}{\ev'}{1}\inTE{get}{\intyatom{1}{\tau}{\ev'}{1}}{\ev}
 \evTE{\ev'}\evTEatom{\ev'}
\]
and the following type environment represents abstract behavior of clients:
\[
\Gamma_2 \stackrel{\mbox{\tiny def}}{=}
\TEREP (\outTEatom{put}{\tau}{\ev'}{1} \TEPAR
        \recTE{\tev}(\evTE{\ev'}\tev \TEIOR 
                     \outTEatom{get}{\outtyatom{1}{\tau}{\ev}{1}}{\ev}{1})
\]
For example, both 
\(
\outatom{put}{v}{\ev'}
\PAR 
\nuexp{r}(\outexp{get}{r}{\ev}\inexp{r}{x}{\ev''}\cdots)
\)
and 
\(
\outexp{put}{v}{\ev'}\nuexp{r}(\outexp{get}{r}{\ev'}\inexp{r}{x}{\ev''}\cdots)
\)
are well typed under \(\Gamma_2 \TEPAR \cdots\).
Since \(\reliable(\Gamma_1 \TEPAR \Gamma_2)\) holds with the event ordering
\(\EOrd\) such that \(\ev' \EOrd \ev\), outputs to \(get\) are indeed
guaranteed to succeed. 

Previous type systems for deadlock freedom~\cite{} cannot capture such
non-uniform availability of methods because they do not take into account
dependency between two channels unless one channel is passed through the
other.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Process.tex <==
\section{Processes}
\label{sec:syntax}

\iffull
This section introduces the syntax and the operational semantics of
our target language.
\fi

\subsect{Syntax}


\begin{defi}[processes]
The set of processes is defined by the following syntax.
\def\prdefone{\zeroexp\mid G_1+\cdots+G_n \mid (P\PAR Q)}
\def\prdeftwo{\mid \nuexp{x_1,\ldots,x_n}{P}\mid \repexp{P}}
\def\prdefthree{\outexp{x}{y_1,\ldots,y_n}{\ev}P\mid \inexp{x}{y_1,\ldots,y_n}{\ev}P}
\[
\begin{array}{lcl}
P \mbox{ (processes)}&::= &
\zeroexp
\mid \outexp{x}{v_1,\ldots,v_n}{}P
\mid \inexp{x}{y_1,\ldots,y_n}{}P\\
& & \mid (P\PAR Q)
\mid \ifexp{v}{P}{Q}\\
& & \mid \nuexp{x}P
\mid \repexp{P}
\mid \accexp{\acclab}{x}{P}
\mid \nurexp{x}{\spec}P\\
v \mbox{ (values)} &::=& x \mid \TRUE \mid \FALSE
\end{array}
\]
Here, \(x\), \(y\), and \(z\) range over a countably infinite set \(\VAR\) of
variables. \(\acclab\) ranges over a set of labels called {\em access labels}.
\(\spec\), called a {\em trace set},
 denotes a set of sequences of access labels that is prefix-closed.
The prefixes (like $(\nu x)$ and
 $(\NUR^\spec x)$) bind tighter than the parallel composition \(\PAR\).
\end{defi}

An access label specifies the kind of an access operation. Typical access labels
that we are going to use in this paper are:
\(I\) for initialization, \(R\) for read, \(W\) for write,
and \(C\) for close.

Process \(\accexp{\acclab}{x}P\) accesses the resource \(x\), and
then behaves like \(P\). We will often write \(\Init(x).P\),
\(\Read(x).P\), \(\Write(x).P\), and \(\Close(x).P\) for
\(\accexp{I}{x}P\), \(\accexp{R}{x}P\), \(\accexp{W}{x}P\),
\(\accexp{C}{x}P\). Process \(\nurexp{x}{\spec}P\) creates a new
resource with the bound name \(x\) that should be accessed according to \(\spec\), and then
behaves like \(P\). \(\spec\) specifies a set of acceptable sequences
of operations that are allowed for the new resource \(x\). For
example, \(\nurexp{x}{\prefixclos{I(R+W)^*C}}P\) creates a resource
that should be first initialized, read or written an arbitrary
number of times, and then closed. Here, \(\prefixclos{S}\) is the
prefix closure of \(S\), i.e., \(\set{s \mid s s'\in S}\).
We write \(\emptyseq\) for the empty sequence.

We often abbreviate a sequence \(v_1,\ldots,v_n\) to \(\seq{v}\),
and write \(\outexp{x}{\seq{v}}{}P\)
and \(\inexp{x}{\seq{y}}{}P\) for \(\outexp{x}{v_1,\ldots,v_n}{}P\) and
\(\inexp{x}{y_1,\ldots,y_n}{}P\).
We often omit trailing \(\zeroexp\) and write \(\outatom{x}{\seq{v}}{}\) and
\(\accatom{\acclab}{x}\) for
\(\outexp{x}{\seq{v}}{}{\zeroexp}\) and
\(\accexp{\acclab}{x}\zeroexp\) respectively.

The bound and free variables of \(P\) are defined in a customary manner;
also \(\nurexp{x}{\spec}P\) binds \(x\).
We identify processes up to \(\alpha\)-conversion,
and assume that \(\alpha\)-conversion is implicity applied so that
bound variables are always different from each other and from free variables.

%% \begin{figure}[h]
%% \fbox{
%% \begin{minipage}{\hfigwidth}
%% \end{minipage}
%% }
%% \caption{An example of a process.}
%% \label{fig:repeatread}
%% \end{figure}


\subsect{Operational Semantics}
\label{sec:op-sem}

We now formally define the operational semantics of our process calculus
The operational semantics is almost the same as the standard reduction semantics for
the \(\pi\)-calculus, except that trace sets \(\spec\) (which represent how resources
should be accessed in future) may change during reduction.

\begin{defi}
The {\em structural preorder} \(\SPCONG\) is the least
reflexive and transitive relation closed under the rules
in Figure~\ref{fig:spcong}
(\(P\SCONG Q\) stands for \((P\SPCONG Q)\land(Q\SPCONG P)\)).
\end{defi}
\begin{rem}
As in our previous behavioural type systems for the 
\(\pi\)-calculus~\cite{Kobayashi03TCS,Kobayashi02IC,Kobayashi05ActInf}, the structural relation
is asymmetric. If the standard, symmetric structural relation were used, the type preservation property
would not hold: \(\tjudge{\Gamma}{\repexp{P}\PAR P}{A}\) does not
necessarily imply \(\tjudge{\Gamma}{\repexp{P}}{A}\)) for the type system introduced in the next
section.
\end{rem}
\iftwocol
\begin{figure*}
\else
\begin{figure}
\fi
\begin{center}
\fbox{\small
\begin{minipage}{14.7 cm}
\iftwocol
\begin{minipage}[t]{7.25cm}
\typicallabel{SP-Commut}
\fi\small
\Infax[SP-Zero]{P\PAR \zeroexp\SCONG P}
\vspace*{2ex}
\Infax[SP-Commut]{P\PAR Q\SCONG Q\PAR P}
\vspace*{2ex}
\Infax[SP-Assoc]{P\PAR (Q\PAR R)\SCONG (P\PAR Q)\PAR R}
\vspace*{2ex}
\Infax[SP-Rep]{\repexp{P}\SPCONG \repexp{P}\PAR P}
\rulesp
\Infax[SP-New]
  {\nuexp{{x}}P \PAR Q  \SPCONG \nuexp{{x}}(P\PAR Q)
   \mbox{(if ${x}$ not free in $Q$)}}
\rulesp
\Infax[SP-NewR]
  {\nurexp{x}{\spec}P \PAR Q  \SPCONG \nurexp{{x}}{\spec}(P\PAR Q)
   \mbox{(if ${x}$ not free in $Q$)}}
\iftwocol
\end{minipage}
\hspace*{0.5cm}
\begin{minipage}[t]{7.25cm}
\typicallabel{SP-CNew}
\fi
%%%\infax[SP-New2]
%%%  {\nuexp{\seq{x}}\nuexp{\seq{y}}P \SPCONG \nuexp{\seq{x},\seq{y}}P}
\rulesp
\Infrule[SP-Par]{P\SPCONG P'\andalso Q\SPCONG Q'}{P\PAR Q\SPCONG P'\PAR Q'}
%%%\infrule[SP-Out]
%%%   {P\SPCONG Q}{\outexp{x}{\seq v}{\ev}P\SPCONG \outexp{x}{\seq v}{\ev}Q}
%%%\infrule[SP-In]
%%%   {P\SPCONG Q}{\inexp{x}{\seq y}{\ev}P\SPCONG \inexp{x}{\seq y}{\ev}Q}
\rulesp
\Infrule[SP-CNew]
   {P\SPCONG Q}{\nuexp{{x}}{P}\SPCONG \nuexp{{x}}Q}
\rulesp
\Infrule[SP-CNewR]
   {P\SPCONG Q}{\nurexp{{x}}{\spec}{P}\SPCONG \nurexp{{x}}{\spec}Q}
%%%\infrule[SP-CRep]
%%%   {P\SPCONG Q}{\repexp{P}\SPCONG \repexp{Q}}
%%%\infrule[SP-If]
%%%   {P\SPCONG P'\andalso Q\SPCONG Q'}
%%%   {\ifexp{v}{P}{Q}\SPCONG \ifexp{v}{P'}{Q'}}
\iftwocol
\end{minipage}
\fi
\end{minipage}
}
\caption{Structural Preorder}
\label{fig:spcong}
\end{center}
\iftwocol
\end{figure*}
\else
\end{figure}
\fi
\def\labcom{dummy}
\begin{defi} \label{def:target1}
The set of {\em reduction labels}, ranged over by
\(\pact\), is \(\set{\redlabacc{\acclab}{x} \mid x\in\VAR}\cup
\{\tau\}\).
We define \(\acctarget{\pact}\) by:
\[
\acctarget{\redlabacc{\acclab}{x}} = \set{x} \qquad
\acctarget{\tau} = \emptyset
\]
\end{defi}
\begin{defi}
Let \(\spec\) be a set of sequences of access labels.
\(\diffspec{\spec}{\acclab}\) is defined by:\quad
\(\diffspec{\spec}{\acclab} = \set{ s \mid \acclab s \in \spec}.\)
\end{defi}

\begin{defi}
The reduction relation \(\redwith{\redlab}\) is the least relation closed
under the rules in Figure~\ref{fig:os}.
\end{defi}
%
We write \(P\red Q\) when \(P\redwith{\redlab}Q\) for some \(\redlab\).
We write \(\red^*\) for the reflexive and transitive closure of \(\red\).

\iftwocol
\begin{figure*}
\else
\begin{figure}
\fi
\begin{center}
\fbox{
%\begin{minipage}{16.5cm}
%\begin{minipage}{9 cm}{\small\hoffset=-2 cm
  \hskip-40 pt\begin{parbox}{8 cm}{\small
\Infax[R-Com]{\outexp{x}{\seq z}{}{P}
   \PAR \inexp{x}{\seq y}{}Q
     \redwith{\redinside} P\PAR \subst{\seq y}{\seq z}Q}
\rulesp{}
\Infax[R-Acc]{\accexp{\acclab}{x}P \redwith{\redlabacc{\acclab}{x}} P}
\rulesp{}
\Infrule[R-Par]{P\redwith{\redlab}Q}
       {P\PAR R\redwith{\redlab}Q\PAR R}
\rulesp{}
\Infax[R-IfT]{\ifexp{\TRUE}{P}{Q} \redwith{\redinside} P}
\Infax[R-IfF]{\ifexp{\FALSE}{P}{Q} \redwith{\redinside} Q}

}
%\end{minipage}
\end{parbox}
  \hskip-40 pt\begin{parbox}{9 cm}{\small

\Infrule[R-New]{P \redwith{L} Q\andalso x\not\in\acctarget{\redlab}}
        {\nuexp{x}P \redwith{L} \nuexp{x}Q}

\rulesp{}
\Infrule[R-NewR1]{P\redwith{\redlabacc{\acclab}{x}}Q}
%%%\andalso \diffspec{\spec}{x}\neq \emptyset}
        {\nurexp{x}{\spec}P \redwith{\redinside} \nurexp{x}{\diffspec{\spec}{\acclab}}Q}
\rulesp{}
\Infrule[R-NewR2]{P\redwith{\redlab}Q\!\!\andalso\!\! x\not\in\acctarget{\redlab}}
        {\nurexp{x}{\spec}P \redwith{\redlab}\nurexp{x}{\spec}Q}

%%%\Infrule[R-New2]{P \redwith{\redlab} Q\andalso
%%%(\redlab=\labcom{\epsilon}{\ev}{\ev'})\lor (\redlab=\labcom{y}{\ev}{\ev'}\land
%%% y\not\in\{\seq{x}\})}
%%%        {\nuexp{\seq{x}}P \redwith{\redlab} \nuexp{\seq{x}}Q}
\rulesp{}
\Infrule[R-SP]{P\SPCONG P'\!\!\! \andalso\!\!\! P'\redwith{\redlab}Q'\!\!\!\andalso\!\!\! Q'\SPCONG Q}
     {P\redwith{\redlab}Q} }
\iftwocol
\end{parbox}
%\end{minipage}
\else
\end{parbox}
%\end{minipage}
\fi
}
\caption{Reduction Relation}
\label{fig:os}
\end{center}
\iftwocol
\end{figure*}
\else
\end{figure}
\fi

Notice that when an invalid access to a resource occurs (i.e. when the program accesses
$\xi$ but the specification $\spec$ has no $\xi$-prefixes), then
resource specification \(\spec\) is set to \(\emptyset\) by
\rname{R-NewR1}. On the other hand \(\spec\supseteq\{\emptyseq\}\) indicates a resource
that has been correctly used so far, and \(\spec=\{\emptyseq\}\) indicates
one that has been correctly and completely used.
\begin{defi}
A process \(P\) is {\em resource-safe} if it does not contain
a sub-expression of the form \(\nurexp{x}{\emptyset}Q\).
\end{defi}
We give  a type system guaranteeing that any resource-safe, well-typed process
cannot be reduced to a non-safe process (in other words, any resource-safe,
well-typed process never performs an invalid access) in Section~\ref{sec:typing}.


%%%\subsection{Deadlock-Freedom and Livelock-Freedom}
%%%\begin{defn}
%%%A predicate \(\waiting\) on processes is the least unary
%%%relation satisfying the following conditions:
%%%(i) \(\waiting(\outexp{x}{\tilde v}{\caponly}P)\),
%%%(ii) \(\waiting(\inexp{x}{\tilde y}{\caponly}P)\),
%%%(iii) \(\forall i\in\{1,\ldots,n\}.\waiting(G_i)\)  implies
%%%\(\waiting(G_1+\cdots+G_n)\),
%%%and (iv) \(\waiting(P)\) implies \(\waiting(P\PAR Q)\),
%%%\(\waiting(Q\PAR P)\), \(\waiting(\repexp{P})\), and
%%%\(\waiting(\nuexp{x}P)\).
%%%\end{defn}
%%%\begin{defn}[deadlock, deadlock-freedom]
%%%\label{def:deadlock}
%%%A process \(P\) is in {\em deadlock} if\\ (i) \(\waiting(P)\)
%%%and (ii) there is no \(P'\) such that \(P\red P'\).
%%%A process \(P\) is {\em deadlock-free} if there exists no \(Q\) such that
%%%\(P\red^* Q\) and \(Q\) is in deadlock.
%%%\end{defn}

\begin{exa}
\label{ex:cobegin}
The following process first creates a resource \(x\) that should be first initialized, read
an arbitrary number of times, and then closed. It then spawns four processes; they
synchronize through channels \(c_1\) and \(c_2\), so that
\(x\) is accessed in a valid order.
\[
\begin{array}{l@{}l}
\nurexp{x}{\prefixclos{IR^*C}}
\nuexp{c_1}\nuexp{c_2}\big(\\
\myquad \Init(x).(\outatom{c_1}{\,}{}\PAR \outatom{c_1}{\,}{})
  & \mbox{\emph{/* initialize x, and send signals */}}\\
\myquad \PAR
  \inexp{c_1}{\,}{}\Read(x).\outatom{c_2}{\,}{}
 &\mbox{\emph{/* wait for a signal on \(c_1\),}}\\
 &\mbox{\emph{then read $x$, and signal on $c_2$*/}}\\
\myquad \PAR
   \inexp{c_1}{\,}{}\Read(x).\outatom{c_2}{\,}{}
 & \mbox{\emph{/* wait for a signal on \(c_1\),}}\\
 & \mbox{\emph{then read $x$, and signal on $c_2$*/}}\\
\myquad \PAR
  \inexp{c_2}{\,}{}\inexp{c_2}{\,}{}\Close(x)\,\big)
  & \mbox{\emph{/* wait on $c_2$, then close $x$ */}}
\end{array}
\]
\eoe{}
\end{exa}

% [Kohei] added
\begin{exa}
\label{ex:repeatread}
The following program is prototypical of recursive functions.
There is a replicated service which listens on channel $\repread$;
it either terminates the recursion by sending a message
back on the reply channel $r$, or it recursively invokes
a sub-instance of itself which will reply on a private channel $r'$.
In this example each recursive step does a $\Read(x)$.
The following program use an integer to decide whether or not to recurse.
Though our language does not have integers and operations on them as primitives,
it is trivial to extend our language and type system with those primitives.

%
%spawns two processes.
%The first one receives three values thorough a channel
%\(\repread\): a boolean value \(b\), a resource \(x\) and
%a channel \(r\) which is used for transmitting acknowledgement.
%If \(b\) is \(\TRUE\),
%then the process sends an acknowledgement through \(r\).
%If \(b\) is \(\FALSE\), the process creates
%a fresh channel \(r'\) and spawns two processes;
%one sends \(b'\) and \(x'\) and \(\rep''\) through \(\repread\),
%and the other waits for an acknowledgement through \(\rep''\),
%reads the resource \(x'\) and sends acknowledgement through \(\rep'\).
%
%The second one creates a resource \(y\) which should be initialized,
%read an arbitrary times and closed, and creates a channel \(\rep\),
%and spawns two processes.
%The first one initializes the resource \(y\) and sends a boolean
%value \(b\) and the resource \(y\) and the channel \(\rep\) through \(\repread\).
%The second one waits for an acknowledgement through \(\rep\)
%and closes \(y\).
%
%
\begin{tabular}{l}
$\nuexp{\repread}\big(\ \repexp{(\inexp{\repread}{n,x,r}{}}\IF\ n=0\ \THEN\ \outatom{r}{}{}\)\\
\qquad\qquad $\ELSE\ \nuexp{r'}(\outatom{\repread}{n-1,x,r'}{} \PAR \inexp{r'}{}{}\Read(x).\outatom{r}{}{}) $\\
\qquad\  $\PAR\ \nurexp{x}{\prefixclos{IR^*C}} \nuexp{r}(\Init(x).\outatom{\repread}{100,x,r}{} \PAR \inexp{r}{}{}\Close(x) ) \,\big)$
%\quad\quad \((\accexp{I}{y} \outexp{\repread}{b,y,\rep}{} \PAR \inexp{\rep}{}{} \accexp{C}{y})\)
\end{tabular}\\
\eoe{}
The above program corresponds to the following higher-level program:
\begin{verbatim}
init(x); parbegin read(x); read(x) parend; close(x)
\end{verbatim}
\end{exa}
%%%Appendix~\ref{sec:another-example} gives another example.

\begin{exa}
\newcommand{\producer}{\mathit{producer}}
\newcommand{\consumer}{\mathit{consumer}}
\newcommand{\accput}{\mathbf{P}}
\newcommand{\accget}{\mathbf{G}}
\newcommand{\buf}{\mathit{buf}}
%%%Other kinds of synchronization patterns can be easily expressed in the
%%%\(\pi\)-calculus, and analyzed by our system.
Consider the following producer/consumer program:%
\footnote{This is an example taken from an ealier version of \cite{Rathke2005}
and modified.}
\[
\begin{array}{l}
\nuexp{\producer} \nuexp{\consumer}\\
\repexp (\inexp{\producer}{b,p,c}{} \inexp{p}{}{} \accexp{\accput}{b} (\outatom{c}{}{}
\PAR \outatom{\producer}{b,p,c}{})) \PAR\\
\repexp (\inexp{\consumer}{b,p,c}{} \inexp{c}{}{} \accexp{\accget}{b} (\outatom{p}{}{} \PAR \outatom{\producer}{b,p,c}{})) \PAR\\
\nurexp{\buf}{\prefixclos{(\accput\ \accget)^*}} \nuexp{x} \nuexp{y}\\
\quad \repexp(\outatom{\producer}{\buf,x,y}{}) \PAR \repexp(\outatom{\consumer}{\buf,x,y}{}) \PAR \outatom{x}{}{}
\end{array}
\]
The first two processes \(\repexp(\inexp{\producer}{b,p,c}{}\cdots)\)
and \\ \(\repexp(\inexp{\consumer}{b,p,c}{}\cdots)\)
define the behavior of producers and consumers.
A producer repeatedly waits to receive a signal on \(p\), performs a put on the buffer \(b\)
(by \(\accatom{\accput}{b}\)), and then sends a signal on \(c\).
A consumer repeatedly waits to receive a signal on \(c\), performs a get on the buffer \(b\)
(by \(\accatom{\accput}{b}\)), and then sends a signal on \(p\).
The third process creates a new buffer on which put and get should be applied only alternately,
 creates two channels \(x\) and \(y\) used for synchronization,
and runs infinitely many producers and consumers.
\end{exa}
%%%Our prototype analyer can correctly judge that the program is safe, i.e.,
%%%puts and gets can occur only alternately.
%%%More examples will be given
%%%at \url{http://www.yl.is.s.u-tokyo.ac.jp/~kohei/usage-pi/}.

\begin{rem} \label{rem:resources}
We treat resources as primitives in this paper, but
we could alternatively express a resource as a tuple of channels,
each of which corresponds to each access operation.
For example, the resource in Example~\ref{ex:cobegin} can be expressed
as a tuple consisting of three channels \(\Init, \Read\), and \(\Close\).
If we did so, we could directly reuse the previous type
systems~\cite{Kobayashi03TCS,Rehof02POPL} to infer some of the properties
discussed in this paper (with different precision).
Treating resources as primitives, however, simplifies the type systems
introduced in later sections and clarifies the essence:
if we expressed a resource as a tuple of channels,
we would need primitives for simultaneous creation of multiple channels
as in \cite{Kobayashi03TCS}, and need to care about whether communications on
the resource access channels succeed or not.
On the other hand, our resource access primitives are non-blocking,
which simplifies in particular the extended type system discussed
in Section~\ref{sec:extension}.
\end{rem}


==> Proof-of-Sec3.tex <==
\subsect{Proof of Subject Reduction Theorem (Theorem~\ref{thm:subject-reduction})}
\label{sec:proofSR}

%%%\begin{lemma}
%%%\label{lem:TEcomb-recovers-splittedTEs}
%%%\((\project{\Gamma}{S})\TEcomb (\exclude{\Gamma}{S}) = \Gamma\).
%%%\end{lemma}
%%%\begin{proof}
%%%By straightforward induction on the structure of \(\Gamma\).
%%%\end{proof}

\begin{lemma}
\label{lem:exclude-is-commutative}
\(\exclude{(\exclude{\Gamma}{S_1})}{S_2} = 
 \exclude{(\exclude{\Gamma}{S_2})}{S_1} = 
 \exclude{\Gamma}{S_1\cup S_2}\).
\end{lemma}
\begin{proof}
By induction on the structure of \(\Gamma\).
\end{proof}

%%%\begin{lemma}
%%%If \(\Gamma\subTE \Delta\) and \(\Delta\TEredwith{}\Delta'\),
%%%then there exists \(\Gamma'\) such that
%%%\(\Gamma\TEredwith{}\Gamma'\) and \(\Gamma'\subTE \Delta'\).
%%%\end{lemma}
%%%\begin{remark}
%%%$B$3$l$O:G>.$N(B\(\subTE\)$B$K$D$$$F$O@.$jN)$D$H;W$o$l$k$,!$Dj5A(B\ref{def:subTE}
%%%$B$N>r7o$rK~$?$9G$0U$N(B\(\subTE\)$B$K$D$$$F$O@.$jN)$D$H$O$$$($J$$$N$G!$(B
%%%$BK\Mh(B\(\subTE\)$B$N>r7o$K2C$($k$Y$-!%!J$H$$$&$3$H$O!$(B\(\subTE\)$B$H(B\(\TEred\)$B$O(B
%%%$BF1;~$KDj5A$9$kI,MW$"$j!)!K(B
%%%\end{remark}
\begin{lemma}[inversion]
\label{lem:inversion}
Suppose \(\Gp P\).
\begin{enumerate}
\item If \(P = P_1 \PAR P_2\), then there exist \(\Gamma_1\) and
\(\Gamma_2\) such that \(\Gamma_i \p P_i\) for \(i=1,2\) and
\(\Gamma \subTE \Gamma_1 \TEPAR \Gamma_2\).

\item If \(P = P_1 + \cdots + P_n\), then there exist \(\Gamma_1, \ldots,
\Gamma_n\) such that \(\Gamma_i \p P_i\)  
for \(i=1,\ldots, n\) and \(\Gamma \subTE \Gamma_1+\cdots+\Gamma_n\).

\item If \(P = \outexp{x}{\tilde z}{\ev}P_0\), then there exist
\(\Gamma_1\) and \(\Gamma_2\) such that \(\Gamma_1 \p P_0\) and
\(\Gamma \subTE \OutTE{x}{(\tilde y)\Gamma_2}{\ev}(\Gamma_1 \TEPAR
\subst{\tilde y}{\tilde z}\Gamma_2)\).

\item If \(P = \inexp{x}{\tilde y}{\ev}P_0\), then there exist
\(\Gamma_1\) and \(\Gamma_2\) such that \(\Gamma_1 \TEPAR \Gamma_2 \p P_0\)
 and
\(\Gamma \subTE \InTE{x}
  {(\tilde y)\Gamma_2}{\ev}\Gamma_1\) with
\(\FV(\Gamma_1) \cap \set{\tilde y} = \emptyset\).

\item If \(P = \nuexp{\tilde x}P_0\), then there exists
\(\Gamma_0\) such that \(\Gamma_0 \p P_0\) and \(\Gamma \subTE
\exclude{\Gamma_0}{\set{\tilde x}}\) with
\(\reliable(\project{\Gamma}{\set{\tilde x}})\) and
\(\FV(\exclude{\Gamma_0}{\set{\tilde x}}) \cap \set{\tilde x} = \emptyset\).

\item If \(P = \repexp P_0\), then there exists \(\Gamma_0\) such
that \(\Gamma_0 \p P_0\) and \(\Gamma \subTE \TEREP\Gamma_0\).
\end{enumerate}
\end{lemma}
\begin{proof}
Immediate from the fact that a type derivation of \(\Gp P\) must end with
an application of the rule corresponding to the form of \(P\), followed by
zero or more applications of the rule \rn{T-Sub}. 
\end{proof}

\begin{lemma}
\label{lem:exclude-TEcom}
If \(\Gamma \TEredwith{\tyredlab} \Gamma'\), then 
\(\exclude{\Gamma}{\set{\tilde x}} 
   \TEredwith{\tyredlab'} \exclude{\Gamma'}{\set{\tilde x}}\) where
\(\tyredlab'\) is defined by:
\[
\tyredlab' = 
\left\{
\begin{array}{ll}
\labTEcom{\epsilon}{\ev_1}{\ev_2}
  & \mbox{if \(\tyredlab = \labTEcom{y}{\ev_1}{\ev_2}\) and \(y \in \set{\tilde x}\)} \\
\tyredlab & \mbox{otherwise}
\end{array}
\right.
\]
\end{lemma}
\begin{proof}
By induction on the derivation of
\(\Gamma \TEredwith{\tyredlab} \Gamma'\) with 
a case analysis on the last rule used.  We show only the main base case
below; The other cases are easy.
\begin{rneqncase}{TER-Com}{
  \Gamma =  \cdots+\OutTE{y}{\tau_1}{\ev_1}\Gamma_1+\cdots
  \TEPAR \cdots+\InTE{y}{\tau_2}{\ev_2}\Gamma_2+\cdots \\
\Gamma' = \Gamma_1 \TEPAR \Gamma_2 
\qquad
\tyredlab = \labTEcom{y}{\ev_1}{\ev_2} \qquad
\tau_1 \subtype \tau_2
}
We have two subcases according to whether \(y \in \{\tilde x\}\) or
not.  
We will show the subcase where \(y=x_i\).
% \begin{eqnsubcase}{y = x_i}
Since \(\exclude{\Gamma}{\set{\tilde x}} = 
\cdots+\evTE{\ev_1} \exclude{\Gamma_1}{\set{\tilde x}}+\cdots 
   \TEPAR
   \cdots+\evTE{\ev_2}\exclude{\Gamma_2}{\set{\tilde x}}+\cdots 
\), by rule \rn{TER-Com2},
\[
\exclude{\Gamma}{\set{\tilde x}}
\TEredwith{\labTEcom{\epsilon}{\ev_1}{\ev_2}}
\exclude{\Gamma_1}{\set{\tilde x}} \TEPAR
\exclude{\Gamma_2}{\set{\tilde x}}
\]
finishing the subcase. The other subcase is easy. 
% \end{eqnsubcase} 
% \begin{eqnsubcase}{y \neq \set{\tilde x}}
% Easy.  Notice that the rule \rn{TER-Com} can still be applied to
% \(\exclude{\Gamma}{\set{\tilde x}}\).
% \endofpf
% \end{eqnsubcase}
\end{rneqncase}
\end{proof}

\begin{lemma}
\label{lem:TEcomb-preserves-wf}
If \(\wf(\project{\Gamma}{S})\) and
\(\wf(\exclude{\Gamma}{S})\), 
then \(\wf(\Gamma)\).
\end{lemma}
\begin{proof}
Suppose \(\wf(\Gamma)\) does not hold.
Then, there exist \(x\), \(\tau_1\), \(\tau_2\), \(\ev_1\), \(\ev_2\),
 \(\Gamma_1\), \(\Gamma_2\), and \(\Gamma_3\)
such that
\[
\Gamma\TEred^* 
\cdots+\OutTE{x}{\tau_1}{\ev_1}\Gamma_1+\cdots 
 \TEPAR \cdots+\InTE{x}{\tau_2}{\ev_2}\Gamma_2+\cdots\TEPAR \Gamma_3
\]
and \(\tau_1 \nsubtype \tau_2\).
By using Lemma~\ref{lem:exclude-TEcom} repeatedly, either
\[
\exclude{\Gamma}{S} \TEred^*
\cdots+\OutTE{x}{\tau_1}{\ev_1}(\exclude{\Gamma_1}{S})+\cdots 
 \TEPAR \cdots+\InTE{x}{\tau_2}{\ev_2}(\exclude{\Gamma_2}{S})+\cdots
\TEPAR \exclude{\Gamma_3}{S}
\]
or
\[
\project{\Gamma}{S} \TEred^*
\cdots+\OutTE{x}{\tau_1}{\ev_1}(\project{\Gamma_1}{S})+\cdots
 \TEPAR \cdots+\InTE{x}{\tau_2}{\ev_2}(\project{\Gamma_2}{S})+\cdots
\TEPAR \project{\Gamma_3}{S},
\]
contradicting the assumptions \(\conTE(\project{\Gamma}{S})\) and
\(\conTE(\exclude{\Gamma}{S})\).
\end{proof}

% \begin{lemma}
% \label{lem:subTE-is-closed-under-substitution}
% If \(\Gamma_1\subTE\Gamma_2\), then 
% \(\subst{x}{y}\Gamma_1\subTE\subst{x}{y}\Gamma_2\).
% \end{lemma}
% \begin{proof}
% Suppose \(\Gamma_1\subTE\Gamma_2\).
% By the definition of \(\subTE\), there exist 
% a substitution \(\theta = [\subs{1}{z_1},\ldots,\subs{n}{z_n}]\) 
% and types \(\tau_1\) and \(\tau_2\) such  that \(\Gamma_1=\theta\tau_1\),
% \(\Gamma_2=\theta\tau_2\), and \(\tau_1\subtype\tau_2\).
% Because \(\subst{x}{y}\Gamma_i = 
%  (\subst{x}{y}\circ \theta)\tau_i\), 
% \(\subst{x}{y}\Gamma_1\subTE\subst{x}{y}\Gamma_2\) follows by the definition
% of \(\subTE\).
% \end{proof}

\begin{lemma}[substitution]
\label{lem:substitution}
If \(\Gamma\p P\), then 
\(\subst{\seq{x}}{\seq{y}}\Gamma\p \subst{\seq{x}}{\seq{y}}P\).
\end{lemma}
\begin{proof}
By straightforward induction on the derivation of \(\Gamma\p P\).
%The proof proceeds by induction on the derivation of \(\Gamma\p P\).
%We use the rule \rn{Sub-Subst}
%%%and the fact that \(\Gamma_1 \subTE \Gamma_2\) implies
%%%\(\subst{x}{y}\Gamma_1 \subTE \subst{x}{y}\Gamma_2\) and
%and the fact that \(x \not \in \set{\tilde x}\) implies
%\(\project{\subst{x}{y}\Gamma}{\set{\tilde x}}
% = \project{\Gamma}{\set{\tilde x}}\).
%%%Both of them are immediate
%%%from the definitions of \(\Gamma_1 \subTE \Gamma_2\) and
%%%\(\project{\Gamma}{S}\), respectively.
\end{proof}

\begin{lemma}
\label{lem:typing-closed-under-spcong}
If \(\Gamma\p P\) and \(P\SPCONG Q\), then \(\Gamma\p Q\).
\end{lemma}
\begin{proof}
By structural induction on the derivation of \(P\SPCONG Q\) with
a case analysis of the last rule used.
We show a few interesting cases below;  The other cases are easy.

\begin{eqncase}{
  P = \nuexp{\seq{x}}P_1 \PAR P_2 &
  Q = \nuexp{\seq{x}}(P_1 \PAR P_2) &
  \mbox{if \(\seq{x}\) are not free in \(P_2\)}
}
By Lemma~\ref{lem:inversion}, there exist \(\Gamma_1\), \(\Gamma_1'\), and 
\(\Gamma_2\) such that \(\Gamma_i \p P_i\) for \(i \in \set{1,2}\) and
\(\Gamma \subTE \Gamma_1' \TEPAR \Gamma_2\) and 
\(\Gamma_1' \subTE \exclude{\Gamma_1}{\set{\seq{x}}}\) with
\(\reliable(\project{\Gamma_1}{\set{\seq{x}}})\).
%
By the rule \rn{T-Par}, \(\Gamma_1 \TEPAR \Gamma_2 \p P_1 \PAR P_2\).
%
Without loss of generality, we can assume \(\seq{x}\) are not free in
 \(\Gamma_2\) so that \(\exclude{\Gamma_2}{\set{\seq{x}}}=\Gamma_2\) and 
\(\nullTE(\project{\Gamma_2}{\set{\seq{x}}})\).
Then, \(\exclude{(\Gamma_1 \TEPAR \Gamma_2)}{\set{\seq{x}}} =
\exclude{\Gamma_1}{\set{\seq{x}}} \TEPAR \Gamma_2\) and,
by the third condition in Definition~\ref{def:consistency},
\(\reliable(\project{(\Gamma_1 \TEPAR \Gamma_2)}{\set{\seq{x}}})\). 
%
Thus, 
\[
  \exclude{\Gamma_1}{\set{\seq{x}}} \TEPAR \Gamma_2 \p
  \nuexp{\seq{x}}{(P_1 \PAR P_2)}
\]
by the rule \rn{T-New}.
Finally, it is easy to show \(\Gamma \subTE
\exclude{\Gamma_1}{\set{\seq{x}}} \TEPAR \Gamma_2 \), and so, by the rule
\rn{T-Sub}, \(\Gp Q\).
\end{eqncase}

\begin{eqncase}{
  P = \repexp P_0 &
  Q = \repexp P_0 \PAR P_0
}
By Lemma~\ref{lem:inversion}, we have 
\(\Gamma_0 \p P_0\) and \(\Gamma \subTE \TEREP \Gamma_0\).
   Then, by the rule \rn{T-Par},
\(\Gamma_0 \TEPAR \TEREP \Gamma_0 \p P_0 \PAR \repexp P_0\).
Since \(\TEREP \Gamma_0 \subTE \Gamma_0 \TEPAR \TEREP \Gamma_0\),
by using the rule \rn{T-Sub}, \(\Gp Q\).
\endofpf
\end{eqncase}
\end{proof}

\begin{proofof}{Theorem~\ref{thm:subject-reduction}}
By induction on the derivation of \(P \redwith{\redlab} Q\) with a case
analysis on the last rule used.  \iffull\else We show only main cases
below. \fi

\begin{rneqncase}{R-Com}{
%\multicolumn{4}{@{}l}{
P = \cdots +  \outexp{x}{\tilde z}{\ev}{P_0} + \cdots
 \PAR \cdots + \inexp{x}{\tilde y}{\ev'}Q_0 + \cdots  \\
Q = P_0\PAR [\subs{\tilde y}{\tilde z}]Q_0 \qquad
l = \labcom{x}{\ev}{\ev'} 
}
By Lemma~\ref{lem:inversion} and the subtyping rules, there exist
\(\Gamma_1\), \(\Gamma_2\), \(\Gamma_3\), and \(\Gamma_4\) such that
\[
\begin{array}{l}
\Gamma \subTE \cdots + 
\OutTE{x}{\typ{\tilde w}{\Gamma_2}}{\ev}
          (\Gamma_1 \TEPAR [\subs{\tilde w}{\tilde z}] \Gamma_2)+ \cdots 
 \TEPAR \cdots + \InTE{x}{\typ{\tilde y}{\Gamma_4}}{\ev'}\Gamma_3 + \cdots\\
\Gamma_1 \p P_0 \qquad \Gamma_3 \TEPAR \Gamma_4 \p Q_0 \qquad
\FV(\Gamma_3) \cap \set{\tilde y} = \emptyset.
\end{array}
\]
Then, since \(\wf(\Gamma)\), it must be the case that 
\(\typ{\tilde w}{\Gamma_2} \subtype \typ{\tilde
y}{\Gamma_4}\), that is, 
\(\Gamma_2 \subtype [\subs{\tilde y}{\tilde w}]\Gamma_4\).  We can show  
\[
\Gamma \TEredwith{\labTEcom{x}{\ev}{\ev'}} 
\Gamma_1 \TEPAR [\subs{\tilde w}{\tilde y}](\Gamma_3 \TEPAR \Gamma_4)
\]
by the following calculation:
\[
\begin{array}{rcl}
\Gamma &\TEredwith{\labTEcom{x}{\ev}{\ev'}} &
   \Gamma_1 \TEPAR
   [\subs{\tilde w}{\tilde z}]\Gamma_2 \TEPAR
   \Gamma_3 \\
& \subTE & 
   \Gamma_1 \TEPAR
   [\subs{\tilde w}{\tilde z}][\subs{\tilde y}{\tilde w}] \Gamma_4 \TEPAR \Gamma_4 \\
& = & 
   \Gamma_1 \TEPAR
   [\subs{\tilde y}{\tilde z}] \Gamma_4 \TEPAR \Gamma_3 \\
& = & 
   \Gamma_1 \TEPAR
   [\subs{\tilde y}{\tilde z}] (\Gamma_4 \TEPAR \Gamma_3 ) \quad
   (\FV(\Gamma_3) \cap \set{\tilde y} = \emptyset) \\
\end{array}
\]
By Lemma~\ref{lem:substitution},
\(
[\subs{\tilde y}{\tilde z}](\Gamma_3 \TEPAR \Gamma_4)
 \p [\subs{\tilde y}{\tilde z}]Q_0
\).
Finally, by the rule \rn{T-Par}, 
\(
\Gamma_1 \TEPAR [\subs{\tilde y}{\tilde z}](\Gamma_3 \TEPAR \Gamma_4)
\p P_0\PAR [\subs{\tilde y}{\tilde z}]Q_0
\),
finishing the case.
\end{rneqncase}

\begin{rneqncase}{R-Par}{
P = P_0 \PAR R &
P_0 \redwith{\redlab} Q_0 &
Q = Q_0 \PAR R
}
By Lemma~\ref{lem:inversion}, there exist \(\Gamma_1\) and \(\Gamma_2\)
such that
\[
\begin{array}{lll}
\Gamma \subTE \Gamma_1 \TEPAR \Gamma_2 &
\Gamma_1 \p P_0 & 
\Gamma_2 \p R 
\end{array}
\]

To use the induction hypothesis, we show \(\wf(\Gamma_1)\) by
contradiction.  Suppose \(\wf(\Gamma_1)\) does not hold.
Then, \(\wf(\Gamma_1 \TEPAR \Gamma_2)\) does not hold, either;  It means
\(\wf(\Gamma)\) does not hold.  Thus, \(\wf(\Gamma_1)\).

By the induction hypothesis, there exists \(\Gamma'_1\) such that
\(\Gamma_1 \TEredwith{\labPtoT{\redlab}} \Gamma'_1\) and
\(\Gamma'_1 \p Q_0\).
By the rules \rn{TER-Skip}, \rn{TER-Par}, and \rn{TER-Sub},
\(\Gamma \TEredwith{\labPtoT{\redlab}} \Gamma'_1 \TEPAR
\Gamma_2\). 
By the rule \rn{T-Par}, \(\Gamma'_1 \TEPAR \Gamma_2 \p Q_0 \PAR R\),
finishing the case.
\end{rneqncase}

\begin{rneqncase}{R-New}{
P = \nuexp{\seq{x}}P_0 &
P_0 \redwith{\redlab'} Q_0 &
Q = \nuexp{\seq{x}}Q_0 &
\redlab = \restrictL{\redlab'}{\set{\seq{x}}}
}
We show the subcase where \(\redlab' = \labcom{x_i}{\ev}{\ev'}\)
for some \(i\), thus \(\redlab = \labcom{\epsilon}{\ev}{\ev'}\);
The other cases (\(\redlab' = \labcom{\epsilon}{\ev}{\ev'}\) or
\(\redlab' = \labcom{y}{\ev}{\ev'}\) with \(y \not \in \set{\seq{x}}\))
are similar.
By Lemma~\ref{lem:inversion}, there exists \(\Gamma_0\) such that
\[
\begin{bcpcasearray}
\Gamma_0 \p P_0 &
\Gamma \subTE \exclude{\Gamma_0}{\set{\seq{x}}} &
\reliable(\project{\Gamma_0}{\set{\seq{x}}}) &
\FV(\exclude{\Gamma_0}{\set{\seq{x}}}) \cap \set{\seq{x}} = \emptyset.
\end{bcpcasearray}
\]
Since \(\wf(\project{\Gamma_0}{\set{\seq{x}}})\)
and \(\wf(\exclude{\Gamma_0}{\set{\seq{x}}})\)
from the assumptions, we have
\(\wf(\Gamma_0)\) by Lemma~\ref{lem:TEcomb-preserves-wf}. 
By the induction hypothesis, there exists \(\Gamma'_0\) such that
\(\Gamma_0 \TEredwith{\labTEcom{x_i}{\ev}{\ev'}} \Gamma'_0\) and
\(\Gamma_0' \p Q_0\).
By Lemma~\ref{lem:exclude-TEcom}, \(\exclude{\Gamma_0}{\set{\seq{x}}}
\TEredwith{\labTEcom{\epsilon}{\ev}{\ev'}}
\exclude{\Gamma'_0}{\set{\seq{x}}}\) and
\(\project{\Gamma_0}{\set{\seq{x}}}
\TEredwith{\labTEcom{x_i}{\ev}{\ev'}}
 \project{\Gamma'_0}{\set{\seq{x}}}\).
Then, \(\reliable(\project{\Gamma'_0}{\set{\seq{x}}})\).
It is easy to show \(\Gamma \TEredwith{\tyredlab}\Gamma'\) implies
\(\FV(\Gamma) \supseteq \FV(\Gamma')\), thus
\(\FV(\exclude{\Gamma'_0}{\set{\seq{x}}}) \cap \set{\seq{x}} = \emptyset\).
Finally, by the rule \rn{T-New}, \(\exclude{\Gamma'_0}{\set{\seq{x}}} \p
\nuexp{\seq{x}}Q_0\), finishing the case.
\iffull\else \endofpf \fi
\end{rneqncase}

\iffull
\begin{rneqncase}{R-SP}{
P \SPCONG P' & 
P' \redwith{l} Q' &
 Q' \SPCONG Q'
}
Immediate from Lemma~\ref{lem:typing-closed-under-spcong} and the induction
hypothesis.
\endofpf
\end{rneqncase}
\fi

\end{proofof}

%%%\begin{proofof}{Theorem~\ref{thm:type-soundness}}
%%%By mathematical induction on the length of the reduction sequence
%%%\(P \red \cdots \red Q\), using Theorem~\ref{thm:subject-reduction} and
%%%the fact that \(\reliable\) is preserved by reduction (of type
%%%environments).
%%%\end{proofof}


==> Proof-of-Sec4.tex <==
\subsection{Proof of Theorem~\protect\ref{thm:correctness-of-deadlock}}
\label{sec:proof-of-sec4}

We first show properties of \(\leq_1\) and \(\leq_2\).
\begin{lemma}
\label{lem:least-subtyping}
Let \(\subtype\) be \(\leq_i\) (\(i\in \set{1,2}\)).  Then, the following
conditions hold:
\begin{itemize}
\item \(\Gamma \models \PLout{x}{\ev}{\ivar}\), then \(\Gamma\TEcong
 \cdots+\OutTE{x}{\tau}{\ev}\Delta_1+\cdots \TEPAR \Delta_2\)
 for some \(\tau\), \(\Delta_1\), and \(\Delta_2\).
\item \(\Gamma \models \PLin{x}{\ev}{\ivar}\), then \(\Gamma\TEcong
 \cdots+\InTE{x}{\tau}{\ev}\Delta_1+\cdots \TEPAR \Delta_2\)
 for some \(\tau\), \(\Delta_1\), and \(\Delta_2\).
\item \(\Gamma\models \PLsometr{\ev}\PLTRUE\), then 
  \(\Gamma \TEcong \cdots+\evTE{\ev}\Delta_1+\cdots \TEPAR \Delta_2\)
 for some \(\Delta_1\) and \(\Delta_2\).
\item \(\Gamma \models \PLout{x}{\ev}{\ivar}\PAR \PLin{x}{\ev}{\ivar}\), 
  then \(\Gamma\TEcong \cdots+\OutTE{x}{\tau_1}{\ev}\Delta_1+\cdots \TEPAR 
\cdots+\InTE{x}{\tau_2}{\ev}\Delta_2+\cdots \TEPAR\Delta_3\).
 for some \(\tau_1\), \(\tau_2\), \(\Delta_1\), \(\Delta_2\) and \(\Delta_3\).
\end{itemize}
\end{lemma}
\begin{proof}
  By the definition of \(\models\), \(\Gamma\models
  \PLout{x}{\ev}{\ivar}\) if and only if \(\Gamma \subTE
  \cdots+\InTE{x}{\tau}{\ev}\Delta_1+\cdots \TEPAR \Delta_2\) for some
  \(\Delta_1\) and \(\Delta_2\). Therefore, the first property
  follows, for both \(\leq_1\) and \(\leq_2\),  by
  straightforward induction on derivation of the subtyping relation.
  Proofs of the other properties are similar.
\end{proof}

We check the necessary condition for Theorem~\ref{thm:type-soundness} below.
\begin{lemma}
\label{lem:deadlock}
Let \(\subtype\) be \(\leq_i\) (\(i \in \set{1,2}\)), and
let \(\reliable\) be \(\reliable_4\). If \(\Gamma\p P\) and 
\(\reliable(\Gamma)\), then \(p_4(P)\) holds.
\end{lemma}
\begin{proof}
The proof proceeds by well-founded induction on \(\ev\). 
Suppose \(\Gamma\p P\), \(\reliable(\Gamma)\), and
\(P\SPCONG \nuexpbseq{w}{1}{k}Q\) with 
\(Q \models \PLout{x}{\ev}{\ivar}\lor \PLin{x}{\ev}{\ivar}\) 
for some \(x, \ivar\). It suffices to show that
\(Q \models \exists x.\exists \ev_1,\ev_2.(
                   \PLsometr{\labcom{x}{\ev_1}{\ev_2}}{\PLTRUE}\lor 
                   \PLsometr{\labcom{\epsilon}{\ev_1}{\ev_2}}{\PLTRUE})\),
that is, \(Q\red R\) for some \(R\).
We show only the case for \(Q\models \PLout{x}{\ev}{\ivar}\):
The case for \(Q\models \PLin{x}{\ev}{\ivar}\) is similar.
By Lemma~\ref{lem:typing-closed-under-spcong} and Theorem~\ref{thm:normal-derivation},
we have 
\[
\begin{array}{l}
\Delta \pN Q\\
\Delta \models \PLout{x}{\ev}{\ivar}\\
\Gamma \subTE \exclude{\Delta}{\set{\seq{w_1},\ldots,\seq{w_k}}}
\end{array}
\]
Moreover, since \(\reliable(\Gamma)\), there exists a set \(S\) such that
\(x\in S\) and \(\reliable(\project{\Delta}{S})\).
(Let \(S\) be \(\set{\seq{w_i}}\) if \(y\in \set{\seq{w_i}}\), and
 \(\FV(\Delta)\setdif\set{\seq{w_1},\ldots,\seq{w_k}}\) otherwise.)
So, by the definition of \(\reliable_4\), there exist 
\(y, \ev_2,\ev_3\) such that \(\project{\Delta}{S} \models 
\PLsometr{\labcom{y}{\ev_2}{\ev_3}}{\PLTRUE}\) or
\(\project{\Delta}{S} \models 
\PLsometr{\ev_2}{\PLTRUE}\land \ev_2\EOrd \ev\).
In the former case, 
\(\Delta \models \PLout{y}{\ev_2}{\ivar}\PAR \PLin{y}{\ev_3}{\ivar}\).
By Theorem~\ref{lem:property-of-normal-derivation} and Lemma~\ref{lem:least-subtyping}, 
we have \(Q\redwith{\labcom{y}{\ev_2}{\ev_3}} R\) for some \(R\)
 as required.
In the latter case, 
by Theorem~\ref{lem:property-of-normal-derivation} and Lemma~\ref{lem:least-subtyping}, 
we have \(Q'\models \PLout{y}{\ev_2}{\ivar}\lor \PLin{y}{\ev_2}{\ivar}\)
and \(Q \SPCONG \nuexpbseq{u}{1}{l}Q'\)
for some \(y, \seq{u_1},\ldots,\seq{u_l}\).
By the induction hypothesis, we have \(Q\red R\) for some \(R\), as required.
\end{proof}

%%%\fi
\begin{pfof}{Theorem~\ref{thm:correctness-of-deadlock}}
%%%\iffull
This follows immediately from Lemma~\ref{lem:deadlock}
and Theorem~\ref{thm:type-soundness}.
%%%\else
%%%This follows immediately from Lemmas~\ref{lem:arity-mismatch} and 
%%%\ref{lem:deadlock}, 
%%%and Theorem~\ref{thm:type-soundness}.
%%%\fi
\end{pfof}

==> ProofPartialLiveness.tex <==
\section{Proofs of the Lemma for Theorem~\ref{th:partial-liveness}}
\label{sec:proof-of-partial-liveness}

This section gives a proof of the lemma ``\textbf{Disabled}''
used in the proof of Theorem~\ref{th:partial-liveness}.

\begin{lem}[Disabled]
\label{le:esafety:disabled}
If \(\wellannot{P}\) and \(\etjudge{\Gamma}{P}{A}\) with
\(\Tbool\not\in\codom(\Gamma)\), then
\(P\notred\) implies \(\disabled{A}{S}\) for any \(S\).
\end{lem}
\proof %\begin{proof}
We first note that \(\wellannot{P}\) and  \(P\notred\) imply
\(\neg\Penabled(P)\) by the definition of \(\wellannot{P}\).
So, it is sufficient to show (i)\(\etjudge{\Gamma}{P}{A}\), (ii)\(P\notred\), 
(iii)\(\neg\Penabled(P)\), and (iv) \(\Tbool\not\in\codom(\Gamma)\)
imply \(\disabled{A}{S}\) for any \(S\).
We prove this by induction on the derivation of 
\(\etjudge{\Gamma}{P}{A}\), with case analysis on the last rule.
\begin{itemize}
\item Case \rname{T-Zero}: In this case, \(A=\Tzero\), so we have \(\disabled{A}{S}\) for 
any \(S\).
\item Case \rname{T-Out}: In this case, \(P = \Exoutexp{x}{\dltag}{\seq{v}}{}P_1\)
and\\ \(A = \ExTout{x}{\dltag}(\csubst{\seq{y}}{\seq{v}}A_1\PAR A_2)\). 
Since \(\neg\Penabled(P)\), \(\dltag=\mayfail\). So, we have \(\disabled{A}{S}\) for any \(S\).
\item Case \rname{T-In}: In this case, \(P = \Exinexp{x}{\dltag}{\seq y}{}P_1\) and
\(A = \ExTin{x}{\dltag}(\exclude{A_2}{\set{\seq{y}}})\). 
Since \(\neg\Penabled(P)\), \(\dltag=\mayfail\). So, we have \(\disabled{A}{S}\) for any \(S\).
\item Case \rname{T-Par}: In this case, \(P={P_1}\PAR P_2\) and \(A={A_1}\PAR A_2\)
with \(\etjudge{\Gamma}{P_1}{A_1}\) and \(\etjudge{\Gamma}{P_2}{A_2}\). 
Note that \(P\notred\) implies \(P_1\notred\) and \(P_2\notred\).
\(\neg\Penabled{(P)}\) implies \(\neg\Penabled{(P_1)}\) and \(\neg\Penabled{(P_2)}\).
So, by the induction hypothesis, we get \(\disabled{A_1}{S}\) and \(\disabled{A_2}{S}\)
for any \(S\),
which implies \(\disabled{A}{S}\).
\item Case \rname{T-Rep}: In this case, \(P=\repexp{P_1}\) and \(A=\Trep{A_1}\),
with \(\etjudge{\Gamma}{P_1}{A_1}\). 
\(\neg\Penabled(P)\) and \(P\notred\) imply \(\neg\Penabled(P_1)\) and
 \(P_1\notred\). So, by the induction hypothesis, we get \(\disabled{A_1}{S}\) for
any \(S\), which also implies \(\disabled{A}{S}\) as required.
\item Case \rname{T-If}: This case cannot happen; by the condition (iv), 
\(P\) must be of the form \(\ifexp{\TRUE}{P_1}{P_2}\)\\ or \(\ifexp{\FALSE}{P_1}{P_2}\),
which contradicts with \(P\notred\).
\item Case \rname{T-New}: In this case, \(P=\nuexp{x}{P_1}\), \(A=\Thiding{x}{A_2}\),
and \(\tjudge{\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}{P_1}{A_2}\).
\(\neg\Penabled(P)\) and \(P\notred\) imply \(\neg\Penabled(P_1)\) and
 \(P_1\notred\). So, by the induction hypothesis, 
we get \(\disabled{A_2}{S}\) for any \(S\). By the definition of \(\disabled{\cdot}{S}\),
we get \(\disabled{A}{S}\).
\item Case \rname{T-Acc}: This case cannot happen, since \(P\) must be of the form
\(\accexp{\acclab}{x}P_1\), which contradicts with \(P\notred\).
\item Case \rname{T-NewR}: Similar to the case for \rname{T-New}.
\item Case \rname{T-Sub}: \(\etjudge{\Gamma}{P}{A}\) must be derived from
\(\etjudge{\Gamma}{P}{A'}\) for some \(A'\newsubtype A\). By the induction hypothesis,
for any \(S\), we get \(\disabled{A'}{S}\). By the condition \(A'\newsubtype A\),
we have \(\disabled{A}{S}\) for any \(S\).\qed
\end{itemize}
%\end{proof}


%%%Extended safety talks about the absence of reductions, so we first need some lemmas
%%%about the absence of reductions.
%%%
%%%\begin{lem} \ \label{le:absence}
%%%\begin{enumerate}
%%%\item $P_1 | P_2 \not\rightarrow$ implies $P_1\not\rightarrow$ and $P_2\not\rightarrow$
%%%      \label{le:absence:par}
%%%\item $a.P \not\rightarrow$ and $x^\xi.P\not\rightarrow$
%%%      \label{le:absence:act}
%%%\item $*P \not\rightarrow$ implies $P\not\rightarrow$
%%%      \label{le:absence:replication}
%%%\item $(\nu x)P\not\rightarrow$ implies $P\not\rightarrow$
%%%      \label{le:absence:nu}
%%%\item $(\IF\ x\ \THEN\ P\ \ELSE\ Q) \not\rightarrow$
%%%      \label{le:absence:if}
%%%\end{enumerate}
%%%\end{lem}
%%%\proof %\begin{proof} Obvious by inspection. We remark for Part~\ref{le:absence:if}
%%%that $(\IF\ \TRUE\ \ldots)$ has a reduction step, as does $(\IF\ \FALSE\ \ldots)$,
%%%but when the operand is just a variable then no reduction step is possible.
%%%\end{proof}
%%%
%%%
%%%\begin{lem} \label{le:extended}
%%%The following lemmas from Appendix~A (which applied to simulation
%%%$\geq$ and judgments $\p$) also hold for extended simulation $\geq$
%%%and extended judgments $\p_{df}$:
%%%\begin{enumerate}
%%%\item \label{le:extended:precongruent} Lemma~\ref{le:subtype-precongruent} (Precongruence)
%%%\item \label{le:extended:structure} Lemma~\ref{le:subtype-structure} (Structure)
%%%\item \label{le:extended:substitution} Lemma~\ref{le:subtype-substitution} (Substitution)
%%%\item \label{le:extended:exclusion} Lemma~\ref{le:subtype-exclusion} (Exclusion)
%%%\item \label{le:extended:simulation} Lemma~\ref{le:subtype-simulation} (Simulation)
%%%\item \label{le:extended:judgement} Lemma~\ref{le:judgement-substitution} (Judgment substitution)
%%%\item \label{le:extended:subject-reduction} Lemma~\ref{le:subject-reduction} (Subject-reduction)
%%%\end{enumerate}
%%%\end{lem}
%%%\proof %\begin{proof}
%%%\todo{extended proofs}
%%%\end{proof}
%%%
%%%\begin{lem}[Extended safety] \
%%%\label{le:esafety}
%%%\begin{enumerate}
%%%\item \label{le:esafety:inactive} If $\wellannot{P}$ and $P\not\rightarrow$ then $\neg\active{P}$.
%%%\item \label{le:esafety:disabled} If $\etjudge{\Gamma}{P}{A}$ and $\neg\active{P}$ then $\disabled{A}{S}$
%%%for all $S$.\todo{probably needs $\Tbool\notin codom(\Gamma)$}
%%%\item \label{le:esafety:SPCONG} If $\wellannot{P}$ and $P \preceq P'$ then
%%%$\wellannot{P'}$.
%%%\item \label{le:esafety:reduction} If $\wellannot{P}$ and $P \rightarrow^* P'$ then $\wellannot{P'}$.
%%%\item \label{le:esafety:nus} If $\wellannot{\,(\seq{\nu}\seq{N})P\,}$ then
%%%$\wellannot{P}$.
%%%\item \label{le:esafety:esafety} Safety: if $\wellannot{P}$ and $\etjudge{\Gamma}{P}{A}$ then either (1) $P
%%%\rightarrow P'$ and $\wellannot{P'}$, or (2) $P \not\rightarrow$ and
%%%if $P \preceq(\seq{\nu}\seq{\NUR})\big(\, \nurexp{y}{\spec}Q
%%%\mathrel{|} R\,\big)$ then ${\downarrow}\in\Phi$.
%%%\end{enumerate}
%%%\end{lem}
%%%\proof %\begin{proof}
%%%\textbf{Part~\ref{le:esafety:inactive}} is obvious from Definition~\ref{def:wellannot}
%%%of $\wellannot{}$.
%%%
%%%\textbf{Part~\ref{le:esafety:disabled}.} A straightforward induction
%%%on the derivation of $\etjudge{\Gamma}{P}{A}$. We elaborate three interesting cases.
%%%\begin{enumerate}
%%%\item The process $\outexp{x}{\vv}{t}P$, which is associated with
%%%the judgment
%%%$\etjudge{\Gamma}{P}{\Toutatom{x}_t.(\csubst{\yy}{\vv}A_1|A_2)}$.
%%%By Lemma~\ref{le:absence}.\ref{le:absence:act} the process
%%%makes no reductions. Note the assumption that
%%%it is well-formed. That means that if $t{=}c$ then it would have a
%%%reduction. Therefore $t{=}\emptyset$, giving
%%%$\disabled{\Toutatom{x}_t.(\csubst{\yy}{\vv}A_1|A_2}{S}$ as
%%%required.
%%%\item The process $P_1|P_2$, which is associated with the judgment
%%%$\etjudge{\Gamma}{P_1|P_2}{A_1|A_2}$ from $\etjudge{\Gamma}{P_1}{A_1}$
%%%and $\etjudge{\Gamma}{P_2}{A_2}$. By Lemma~\ref{le:absence}.~\ref{le:absence:par}
%%%we have $P_1\not\rightarrow$ and $P_2\not\rightarrow$. By the induction
%%%hypothesis, $\disabled{A_1}{S}$ and $\disabled{A_2}{S}$ and hence
%%%$\disabled{A_1|A_2}{S}$ as required.
%%%\item The process $\accexp{\xi}{x}P$. This does undergo a reduction,
%%%so the lemma is immediately true.
%%%\end{enumerate}
%%%
%%%\textbf{Parts~\ref{le:esafety:SPCONG} and~\ref{le:esafety:reduction}and~\ref{le:esafety:nus}} are
%%%straightforward.
%%%
%%%\textbf{Part~\ref{le:esafety:esafety}.} Option (1) is
%%%satisfied by Part~\ref{le:esafety:reduction}. For
%%%option (2), there are three tasks. First, $P \SPCONG
%%%(\seq{\nu}\seq{\NUR})\big(\, \nurexp{y}{\spec}Q|R\,\big)$ by
%%%assumption, $\SPCONG (\seq{\nu}\seq{\NUR})\nurexp{y}{\spec}(Q|R)$ by
%%%assuming $y$ distinct through alpha-renaming. By
%%%Parts~\ref{le:esafety:SPCONG} and~\ref{le:esafety:nus},
%%% \[ \wellannot{Q|R}. \]
%%%Second, the assumption $P \not\rightarrow$ and
%%%Lemma~\ref{le:absence} give
%%% \[ Q|R \not\rightarrow. \]
%%%Third, the assumption $\etjudge{\Gamma}{P}{A}$ and
%%%Lemma~\ref{le:extended}.\ref{le:extended:subject-reduction} yield
%%%$\etjudge{\Gamma}{(\seq{\nu}\seq{\NUR})\nurexp{y}{\spec}(Q|R)}{A}$,
%%%which must have been deduced from some
%%% \[ \etjudge{\Gamma'}{Q|R}{A'} \qquad \etraces{y}{Q|R} \subseteq \spec. \]
%%%These two parts together with Part~\ref{le:esafety:disabled} give
%%%$\disabled{A'}{\{\yy\}}$. And so by definition of $\textbf{etraces}$ we
%%%get ${\downarrow} \in \spec$ as required.
%%%\end{proof}


==> ProofSubjectReduction.tex <==
\section{Proof of the Subject Reduction Property}
\label{sec:app:subject-reduction}

In this section, we prove the subject reduction property used in
the proofs of Theorems~\ref{th:safety} and~\ref{th:partial-liveness}. 
As in Appendix~\ref{sec:app:subtyping},
we prove it for the basic and extended cases simultaneously.

\begin{lem}[Weakening]
\label{le:weakening} 
\begin{enumerate}
\item If \(\Gamma\p v:\mvtype\) and \(x\not\in\dom(\Gamma)\), then
\(\Gamma,x\COL \mvtype'\p v:\tau\).
\item If
 $\tjudge{\Gamma}{P}{A}$ and $x\notin\FV(P)$
% and $x$ not in $\Gamma$ or $A$ then $\tjudge{\Gamma,\,x\COL
and $x$ not in $\dom(\Gamma)$ or $\FV(A)$ then $\tjudge{\Gamma,\,x\COL
\mvtype}{P}{A}$.
\end{enumerate}
\end{lem}
\proof
\text{Part~1} is straightforward. \text{Part~2} is proved by
straightforward induction on the derivation of $\tjudge{\Gamma}{P}{A}$.\qed
%\end{proof}

\begin{lem}[Judgement substitution] \
\label{le:judgement-substitution}
\begin{enumerate}
\item \label{le:judgement-substitution:substval}
\textit{(For values)} If $\Gamma,\xx\COL\seq{\mvtype} \p y \COL \mvtype$
and $\Gamma \p \vv\COL\seq{\mvtype}$ then $\Gamma \p \subst{\xx}{\vv}y
\COL \sigma$.
\item \label{le:judgement-substitution:substproc} \textit{(For processes)} If
$\tjudge{\Gamma, \xx\COL\seq{\mvtype}}{P}{A}$ and $\Gamma \p
\vv\COL\seq{\mvtype}$ then
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
\end{enumerate}
\end{lem}
\proof
\textbf{Part~\ref{le:judgement-substitution:substval}.} Either
$y=x_i$ for some $i$, in which case \(\subst{\xx}{\vv}y=v_i\)
and \(\sigma = \mvtype_i\), so that the result follows from
\(\Gamma \p \vv\COL\seq{\mvtype}\).
Or $y\notin\xx$, in which case $\subst{\xx}{\vv}y = y$ and
$y\COL \mvtype$ is in $\Gamma$. We remark that types $\mvtype$ never
have free names.

\textbf{Part~\ref{le:judgement-substitution:substproc}.} By
induction on the derivation of $\tjudge{\Gamma}{P}{A}$. Most cases
follow straightforwardly on Lemma~\ref{le:subtype-substitution}. We
consider four particular cases.
\begin{enumerate}
\item Case \rname{T-Sub}, where $\tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A}$ is inferred
from
\[\begin{array}{c}
  \tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A'} \qquad A' \newsubtype A
\end{array}\]
From the induction hypothesis,
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A'}$. By
Lemma~\ref{le:subtype-precongruent}.\ref{le:subtype-precongruent:subst}
and assumption $A' \newsubtype A$ we get $\csubst{\xx}{\vv}A' \newsubtype
\csubst{\xx}{\vv}A$, and hence as required
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
%
\item Case \rname{T-NewR}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\nurexp{z}{\spec}P}{\exclude{A}{\{z\}}}$
is inferred from
\[\begin{array}{c}
  \tjudge{\Gamma,\xx\COL\seq{\tau},z\COL\Tres}{P}{A} \qquad
  \traces{z}{A} \subseteq \spec
\end{array}\]
Assume by alpha-renaming that $z$ does not clash with $\xx$ or $\vv$. From
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude1}
%% we get $\project{A}{\{z\}} \eqtype \project{(\csubst{\xx}{\yy}A)}{\{z\}}$,
%% giving $\traces{z}{A} = \traces{z}{\csubst{\xx}{\yy}A}$ and hence
%% $\traces{z}{\csubst{\xx}{\yy}A} \subseteq \spec$. 
we get $\project{A}{\{z\}} \eqtype \project{(\csubst{\xx}{\vv}A)}{\{z\}}$,
giving $\traces{z}{A} = \traces{z}{\csubst{\xx}{\vv}A}$ and hence
$\traces{z}{\csubst{\xx}{\vv}A} \subseteq \spec$. 
From $\Gamma \p \vv\COL\seq{\tau}$ and Lemma~\ref{le:weakening}, 
we get \(\Gamma, z\COL\Tres \p \vv\COL\seq{\tau}\). So, by the induction
hypothesis,
$\tjudge{\Gamma,z\COL\Tres}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
These two together give
 \[ \tjudge{\Gamma}{\nurexp{z}{\spec}\subst{\xx}{\vv}P}{\exclude{(\csubst{\xx}{\vv}A)}{\{z\}}}. \]
For the process $\nurexp{z}{\spec}\subst{\xx}{\vv}P$, we can push
the substitution out by definition of the substitution operator and
because $z\not\in\set{\seq{x},\seq{v}}$. For the behavior
$\exclude{(\csubst{\xx}{\vv}A)}{\{z\}}$ we use
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude1}
to push it out. Hence as required,
 \[ \tjudge{\Gamma}{\subst{\xx}{\vv}\nurexp{z}{\spec}P}{\csubst{\xx}{\vv}(\exclude{A}{\{z\}})}. \]
\beginextended{} Just replace \(\TRACES\) with \(\ETRACES\) in the above reasoning.
%
\item Case \rname{T-Out}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\outexp{z}{w}{}P}{\Tout{z}(\csubst{\yy}{\seq{w}}A_1
| A_2)}$ is inferred from
\[\begin{array}{c}
 \tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A_2} \qquad
 \Gamma,\xx\COL\seq{\tau} \p \seq{w}\COL\seq{\sigma} \\
 \Gamma,\xx\COL\seq{\tau} \p z\COL\Tchan{(\yy:\seq{\sigma})A_1}
\end{array}\]
Part~\ref{le:judgement-substitution:substval} implies $\Gamma \p
\subst{\xx}{\vv}\seq{w} \COL \seq{\sigma}$ and $\Gamma \p
\subst{\xx}{\vv}z \COL \Tchan{(\yy:\seq{\sigma})A_1}$. From the
induction hypothesis, we get
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A_2}$. These
three give
 \[
 \tjudge{\Gamma}{\outexp{\subst{\xx}{\vv}z}{\subst{\xx}{\vv}\seq{w}}{}\subst{\xx}{\vv}P}{\Tout{\subst{\xx}{\vv}z}(\csubst{\yy}{\subst{\xx}{\vv}\seq{w}}A_1 | \csubst{\xx}{\vv}A_2)}
 \]
For the process we push the substitution out by definition of the
substitution operator. For the behavior we push it out using several
parts of Lemma~\ref{le:subtype-substitution}.
%
\item Case \rname{T-In}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\inexp{z}{\yy}{}P}{\Tin{z}(\exclude{A_2}{\{\yy\}})}$
is inferred from
\[\begin{array}{c}
 \tjudge{\Gamma,\yy\COL\seq{\sigma},\xx\COL\seq{\tau}}{P}{A_2}
 \qquad
 \Gamma,\xx\COL\seq{\tau} \p z\COL\Tchan{(\yy:\seq{\sigma})A_1} \\
 \project{A_2}{\{\yy\}}\newsubtype  A_1 
\end{array}\]
We use three deductions. First from
Part~\ref{le:judgement-substitution:substval} we get $\Gamma \p
\subst{\xx}{\vv}z \COL\Tchan{(\yy:\seq{\sigma})A_1}$. Second, from
assumption $ \project{A_2}{\{\yy\}}\newsubtype A_1$ and
Lemma~\ref{le:subtype-precongruent}.\ref{le:subtype-precongruent:subst}
we get $\csubst{\xx}{\vv}(\project{A_2}{\{\yy\}}) \newsubtype \csubst{\xx}{\vv}A_1$. 
% The substitution on the left
The substitution on the right
disappears because $\FV(A_1)\subseteq\{\yy\}$ and we can assume by
alpha-renaming that $\yy$ does not clash with $\{\xx,\vv\}$. The substitution on the
% right can be pushed inside by
left can be pushed inside by
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude1}.
%%%\todo{This is not true if we directly apply Lemma~\ref{le:subtype-substitution:exclude1}..}
These together give $
\project{(\csubst{\xx}{\vv}A_2)}{\{\yy\}}\newsubtype A_1$. And third, from the induction
hypothesis we get
$\tjudge{\Gamma,\yy\COL\seq{\sigma}}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A_2}$.
These three give
 \[
 \tjudge{\Gamma}{\inexp{\subst{\xx}{\vv}z}{\yy}{}\subst{\xx}{\vv}P}{\Tin{\subst{\xx}{\vv}z}(\exclude{(\csubst{\xx}{\vv}A_2)}{\{\yy\}})}
 \]
As in the previous case we push the substitution out in the process
and the behavior to get, as required,
 \[\hbox to123 pt{\hfil}
 \tjudge{\Gamma}{\subst{\xx}{\vv}(\inexp{z}{\yy}{}P)}{\csubst{\xx}{\vv}(\Tin{z}(\exclude{A_2}{\{\yy\}}))}.
 \hbox to122 pt{\hfil}\qEd
\]
\end{enumerate}
%\end{proof}


\begin{lem}[Subject-reduction] \
\label{le:subject-reduction}
\begin{enumerate}
\item If $\tjudge{\Gamma}{P}{A}$ and $P \SPCONG Q$ then $\tjudge{\Gamma}{Q}{A}$. \label{le:subject-reduction:SPCONG}
\item \label{le:subject-reduction:subject-reduction} \textit{(Subject-reduction)} If $P \stackrel{L}{\rightarrow} P'$
and $\tjudge{\Gamma}{P}{A}$ then $A \Tredswith{L} A'$ and $\tjudge{\Gamma}{P'}{A'}$
for some \(A'\).
\end{enumerate}
\end{lem}
\proof
%%%\textbf{Part~\ref{le:subject-reduction:weakening}} is a
%%%straightforward on the derivation of $\tjudge{\Gamma}{P}{A}$.
%%%
\textbf{Part~\ref{le:subject-reduction:SPCONG}.} By induction on the
derivation of $P \SPCONG Q$. Most cases use
Lemma~\ref{le:subtype-structure}. %%%\todo{THREE CASES. NIL and NEW and NUR, which is already here}
The case for $\nuexp{x}P | Q
\preceq \nuexp{x}(P|Q)$ uses
Lemma~\ref{le:weakening}.
The only interesting case is that for $\nurexp{x}{\spec}P|Q \preceq
\nurexp{x}{\spec}(P|Q)$ with $x\notin\FV(Q)$. The judgement
$\tjudge{\Gamma}{\nurexp{x}{\spec}P|Q}{A}$ must have been inferred
from
\[\begin{array}{c}
 \tjudge{\Gamma,x\COL\Tres}{P}{A_3} \qquad
 \traces{x}{A_3}\subseteq \Phi \qquad
 \exclude{A_3}{\{x\}} \newsubtype A_1 \\
 \tjudge{\Gamma}{Q}{A_2} \qquad
 A_1|A_2 \newsubtype A
\end{array}\]
From these and Lemma~\ref{le:weakening}, we infer
\[ \tjudge{\Gamma, x\COL\Tres}{P|Q}{A_3|A_2}. \]
By alpha-renaming assume $x\notin\FV(A_2)$. By
Lemmas~\ref{le:subtype-exclusion}.\ref{le:subtype-exclusion:par}
and~\ref{le:subtype-exclusion}.\ref{le:subtype-exclusion:nil} we get
$\project{(A_3|A_2)}{\{x\}} \eqtype \project{A_3}{\{x\}} | \project{A_2}{\{x\}}
\newsubtype \project{A_3}{\{x\}}$, and then by
Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:traces} we get
$\traces{x}{A_3|A_2}\subseteq\traces{x}{A_3}$, and so $\traces{x}{A_3|A_2}
\subseteq \spec$. This gives
\[ \tjudge{\Gamma}{\nurexp{x}{\spec}(P|Q)}{\exclude{(A_3|A_2)}{\{x\}}}. \]
Finally $\exclude{(A_3|A_2)}{\{x\}}
\newsubtype \exclude{A_3}{\{x\}} | A_2 \newsubtype A_1 \TPAR A_2 \newsubtype A$. This gives as required
\[ \tjudge{\Gamma}{\nurexp{x}{\spec}(P|Q)}{A}. \]
\beginextended{} Just replace \(\TRACES\) with \(\ETRACES\) in the above reasoning.

\textbf{Part~\ref{le:subject-reduction:subject-reduction}.} By
induction on the derivation of $P \redwith{L} P'$. We show main cases.
The other cases are straightforward.
\begin{itemize}
\item Case \rname{R-Com}:
We are given
\[ \tjudge{\Gamma}{\outexp{x}{\seq{v}}{}P_1 \PAR \inexp{x}{\seq{y}}{}P_2}{A}. \]
%% This must have been deduced from
%% \[\begin{array}{c}
%%   \tjudge{\Gamma}{P_1}{A_2} \qquad
%% \qquad \Gamma\p x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}
%%   \Gamma \p v_i\COL \mvtype_i \\
%%   \Tout{x}(\csubst{\yy}{\vv}A_1 \PAR A_2) \newsubtype A_3 \qquad
%%   \tjudge{\Gamma,\yy\COL\seq{\mvtype}}{P_2}{A_4} \\
%%   \project{A_4}{\{\yy\}}\newsubtype A_1 \qquad \Tin{x}(\exclude{A_4}{\{\yy\}}) \newsubtype A_5 \qquad
%%   A_3|A_5 \newsubtype A
%% \end{array}\]
This must have been deduced from
\begin{gather}
  \tjudge{\Gamma}{\outexp{x}{\seq{v}}{}P_1}{A_1} \notag\\
  \tjudge{\Gamma}{\inexp{x}{\seq{y}}{}P_2}{A_2} \notag\\
  A_1|A_2 \newsubtype A.
\end{gather}
\(\tjudge{\Gamma}{\outexp{x}{\seq{v}}{}P_1}{A_1}\) and
\(\tjudge{\Gamma}{\inexp{x}{\seq{y}}{}P_2}{A_2}\) must have been deduced from
\begin{gather}
  \tjudge{\Gamma}{P_1}{A_3}\\
  \Gamma\p x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_4}\\
  \Gamma \p v_i\COL \mvtype_i\\
  \Tout{x}(\csubst{\yy}{\vv}A_4 \PAR A_3) \newsubtype A_1
\end{gather}
and
\begin{gather}
  \tjudge{\Gamma,\yy\COL\seq{\mvtype}}{P_2}{A_5}\\
  \Gamma\p x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_4} \notag\\
  \project{A_5}{\{\yy\}}\newsubtype A_4\\
  \Tin{x}(\exclude{A_5}{\{\yy\}}) \newsubtype A_2
\end{gather}
respectively.
We must show \(A \Rightarrow A'\) and
\(\tjudge{\Gamma}{P_1 | \subst{\yy}{\vv}P_2}{A'}\) for some \(A'\).
%% We must show some $A'$ for which $A \Rightarrow A'$ and
%% $\tjudge{\Gamma}{P_1 | \subst{\yy}{\vv}P_2}{A'}$. 
We pick some
$A'$ such that $A \Rightarrow A'$ and $A' \subtype \csubst{\yy}{\vv}A_4 | A_3 | \exclude{A_5}{\{\yy\}}$.
The existence of such $A'$ is guaranteed by 
\(A \subtype 
\Tout{x}(\csubst{\yy}{\vv}A_4 | A_3) | \Tin{x}(\exclude{A_5}{\{\yy\}})
\red \csubst{\yy}{\vv}A_4 | A_3 |
\exclude{A_5}{\{\yy\}}\),
which follows from (B.1) and (B.5) and (B.8),
%% and
%% \(\Tout{x}(\csubst{\yy}{\vv}A_4 | A_3) |
%% \Tin{x}(\exclude{A_5}{\{\yy\}}) \red \csubst{\yy}{\vv}A_4 | A_3 |
%% \exclude{A_5}{\{\yy\}}\),
and the definition
of the subtyping relation (Definition~\ref{def:subtype}).
%% Because we have 
%% \(A \subtype 
%% \Tout{x}(\csubst{\yy}{\vv}A_4 | A_3) | \Tin{x}(\exclude{A_5}{\{\yy\}})\)
%% from (B.1) and (B.5) and (B.8),
%% and because 
%% \(\Tout{x}(\csubst{\yy}{\vv}A_4 | A_3) |
%% \Tin{x}(\exclude{A_5}{\{\yy\}}) \red \csubst{\yy}{\vv}A_4 | A_3 |
%% \exclude{A_5}{\{\yy\}}\),
%% the existence of such $A'$ is guaranteed by the definition
%% of the subtyping relation (Definition~\ref{def:subtype}).
%% $A
%% \subtype \Tout{x}(\csubst{\yy}{\vv}A_1 | A_2) |
%% \Tin{x}(\exclude{A_4}{\{\yy\}}) \red \csubst{\yy}{\vv}A_1 | A_2 |
%% \exclude{A_4}{\{\yy\}}$. 
It remains to prove $\tjudge{\Gamma}{P_1 |
\subst{\yy}{\vv}P_2}{A'}$. We start with the judgment (B.6),
\[ \tjudge{\Gamma,\yy\COL\seq{\mvtype}}{P_2}{A_5}. \]
By
Lemma~\ref{le:judgement-substitution}.\ref{le:judgement-substitution:substproc},
\[ \tjudge{\Gamma}{\subst{\yy}{\vv}P_2}{\csubst{\yy}{\vv}A_5}. \]
Hence
\[ \tjudge{\Gamma}{P_1 | \subst{\yy}{\vv}P_2}{A_3 | \csubst{\yy}{\vv}A_5}. \]
Therefore, the required result \(\tjudge{\Gamma}{P_1 \PAR \subst{\yy}{\vv}P_2}{A'}\) 
follows by \rname{T-Sub}, if we show
\(A_3 \TPAR \csubst{\yy}{\vv}{A_5} \newsubtype A'\).
It follows by:
\[
\begin{array}{rclr}
A_3 \TPAR \csubst{\yy}{\vv}A_5 &\newsubtype& A_3 \TPAR \csubst{\yy}{\vv}(\project{A_5}{\{\yy\}} \TPAR \exclude{A_5}{\{\yy\}}) & \mbox{(Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:separate})}\\
                               &\newsubtype& A_3 \TPAR \csubst{\yy}{\vv}(\project{A_5}{\{\yy\}}) \TPAR \csubst{\yy}{\vv}(\exclude{A_5}{\{\yy\}}) & \mbox{(Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:par})}\\
                               &\newsubtype& A_3 \TPAR \csubst{\yy}{\vv}(\project{A_5}{\{\yy\}}) \TPAR \exclude{A_5}{\{\yy\}} & \mbox{(Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude2})}\\
                               &\newsubtype& A_3 \TPAR \csubst{\yy}{\vv}A_4 | \exclude{A_5}{\{\yy\}} & \mbox{(assumption B.7 above)}\\
                               &\newsubtype& A' & \mbox{(the definition of \(A'\)).}
\end{array}
\]
%% Now $A_2\TPAR \csubst{\yy}{\vv}A_4 
%% \newsubtype A_2\TPAR \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}|\exclude{A_4}{\{\yy\}})$
%%  (by
%% Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:separate}), \\
%% $\newsubtype A_2\TPAR \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}) |
%%   \csubst{\yy}{\vv}(\exclude{A_4}{\{\yy\}}) $ (by
%% Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:par}), \\
%% $\newsubtype A_2\TPAR \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}) |
%% \exclude{A_4}{\{\yy\}} $ (by
%% Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude2}), \\
%% $\newsubtype A_2 \TPAR \csubst{\yy}{\vv}A_1 | \exclude{A_4}{\{\yy\}} $ (by
%% assumption $\exclude{A_4}{\{\yy\}} \newsubtype A_1$), \\
%% $\newsubtype A'$ (by definition of $A'$).
%% This gives as required
%% \[ \tjudge{\Gamma}{P_1 | \subst{\yy}{\vv}P_2}{A'}. \]
\item Case \rname{R-Acc}:
We are given \(\tjudge{\Gamma}{\accexp{\acclab}{x} P_1}{A}\).
This must have been derived from
\begin{itemize}
\item \(\tjudge{\Gamma}{P_1}{A_1}\)
\item \(\tjudge{\Gamma}{x}{\Tres}\)
\item \(\Tacc{\acclab}{x} A_1\newsubtype A\).
\end{itemize}
We have to show that
\begin{itemize}
\item \(\tjudge{\Gamma}{P_1}{A'}\)
\item \(A \Tredswith{\Tredlabacc{x}{\acclab}} A'\).
\end{itemize}
Let \(A'\) be a behavioral type that satisfies
\(A \Tredsacc{x}{\acclab} A'\) and \(A' \subtype A_1\).
Such \(A'\) is guaranteed to exist by \(A \subtype \Tacc{\acclab}{x} A_1\Tredwith{\Tredlabacc{x}{\acclab}}A_1\).
Then, \(\tjudge{\Gamma}{P_1}{A'}\) follows from
\(\tjudge{\Gamma}{P_1}{A_1}\) and \(A' \subtype A_1\).

\item Case \rname{R-NewR1}:
We are given \(\tjudge{\Gamma}{\nurexp{x}{\spec} P_1}{A}\)
This must have been derived from
\begin{itemize}
\item \(\tjudge{\Gamma, x:\Tres}{P_1}{A_1}\)
\item \(\traces{x}{A_1} \subseteq \spec\)
\item \(A \subtype \exclude{A_1}{\set{x}}\).
\end{itemize}
We have to show that there exists \(A'\) such that
\begin{itemize}
\item \(\tjudge{\Gamma}{\nurexp{x}{\diffspec{\spec}{\acclab}}P_1'}{A'}\)
\item \(A \Treds A'\)
\end{itemize}
where \(P_1 \redacc{\acclab}{x} P_1'\).

By the induction hypothesis, there exists \(A_1'\) that satisfies
\(\tjudge{\Gamma,x:\Tres}{P_1'}{A_1'}\) and
\(A_1 \Tredswith{\Tredlabacc{x}{\acclab}} A_1'\).
Using \rname{Tr-Project}, we get 
\(\project{A_1}{\set{x}} \Tredswith{\Tredlabacc{x}{\acclab}} \project{A_1'}{\set{x}}\).
So, from the definition of \(\TRACES\)
and \(\traces{x}{A_1}\subseteq \spec\), 
 we get \(\traces{x}{A_1'}\subseteq \diffspec{\spec}{\acclab}\).
By using \rname{T-NewR}, we get \(\tjudge{\Gamma}{\nurexp{x}{\diffspec{\spec}{\acclab}}P_1'}
{\exclude{A_1'}{\set{x}}}\).

It remains to show there exists \(A'\) such that \(\exclude{A_1'}{\set{x}}\newsubtype A'\)
and \(A \Treds A'\). That follows from \(A \subtype \exclude{A_1}{\set{x}} 
\Treds \exclude{A_1'}{\set{x}}\). Here, the latter relation follows from
\(A_1\Tredswith{\Tredlabacc{x}{\acclab}}A_1'\) and rule \rname{Tr-Exclude}.\\
\beginextended{} Just replace \(\TRACES\) with \(\ETRACES\) in the above reasoning.
%%%
%%%Let \(A'\) be a behavioral type that satisfies
%%%\(A \Tredsilent A'\) and \(A' \subtype \exclude{A_1'}{\set{x}}\).
%%%Such \(A'\) is guaranteed to exist by \(A \subtype \exclude{A_1}{\set{x}}\) and
%%%\(A_1 \Tredacc{x}{\acclab} A_1'\).
%%%From \(\tjudge{\Gamma,x:\Tres}{P_1'}{A_1'}\) and \(A' \subtype \exclude{A_1'}{\set{x}}\),
%%%we are left to show that \(\traces{x}{A_1'} \subseteq \diffspec{\spec}{\acclab}\),
%%%which follows from Lemma~\ref{le:safety:phiminus}.
\item Case \rname{R-SP}: This follows immediately from Part~\ref{le:subject-reduction:SPCONG}
and the induction hypothesis.\qed
\end{itemize}
%\end{proof}



==> ProofSubtyping.tex <==
\section{Properties of the Subtyping Relation}
\label{sec:app:subtyping}

This section states and proves the properties of the subtyping relation,
which are used in the proof of type soundness (Theorems~\ref{th:safety}
and \ref{th:partial-liveness}, in particular the proofs of the lemmas
in Appendices~\ref{sec:app:subject-reduction} and \ref{sec:proof-of-partial-liveness}),
and in the type inference algorithm described in Section~\ref{sec:inference}
(in particular, for transforming constraints on behavioral types).

Actually, there are two subtyping relations; the basic one
in Definition~\ref{def:subtype} and the extended one in 
Definition~\ref{def:ex-subtype}. Since the proofs are almost the same,
we state and prove the properties of the basic and extended ones simultaneously.
In a few places, we have an additional condition to check for the extended case.
Such places will be marked by ``\extendedonly{}.''
When we are discussing the basic case, attributes attached to actions 
should be ignored. We also omit them even for the extended case when they
are not important.



\begin{lem}[Simulation relation] \
\label{le:relation}
\begin{enumerate}
\item \label{le:relation:transitive} 
 The subtyping relation is reflexive and transitive. %%%$A \subtype B \subtype C$ implies $A \subtype C$
%%%\item $A \subtype A$
\item \label{le:relation:upto} {(Simulation-up-to)} Let $\R$ be a relation on behavioral types such that whenever $A_1
\R A_2$ then 
\begin{itemize}
\item[(i)] $A_1 \stackrel{l}{\rightarrow} A_1'$ implies $A_2
\Tredswith{l} A_2'$ and $A_1'\R {\newsubtype}
A_2'$ for some $A_2'$ and 
\item[(ii)] \(\disabled{A_1}{S}\) implies \(\disabled{A_2}{S}\).
\end{itemize}
Then $\R \subseteq {\newsubtype}$.
Condition (ii) is required only for the extended case.
\end{enumerate}
\end{lem}
\proof 
\textbf{Part~\ref{le:relation:transitive}} is trivial by the definition.
To show \textbf{Part~\ref{le:relation:upto}}, suppose \(\R\) is a simulation up to.
We show that $\R' = (\R{\newsubtype})\cup \R$ is a simulation, i.e.,
whenever \(A_1\R' A_2\), (i) $A_1 \Tredwith{l} A_1'$ implies $A_2
\Tredswith{l} A_2'$ and $A_1'\R'
A_2'$ for some $A_2'$ and (\extendedonly{}) (ii) 
\(\disabled{A_1}{S}\) implies \(\disabled{A_2}{S}\).
Suppose \(A_1\R' A_2\). The case where \(A_1\R A_2\) is trivial by the definition of 
the simulation-up-to.
To check the other case, suppose \(A_1 {\R} A_3 \newsubtype A_2 \).
To show (i), suppose also that $A_1 \Tredwith{l} A_1'$. Since \(\R\) is a simulation up to,
there exists \(A_3'\) such that \(A_3\Tredswith{l}A_3'\) and \(A_1'\mathrel{\R}\newsubtype A_3'\).
By \(A_3\Tredswith{l}A_3'\) and \(A_3\newsubtype A_2\), we have \(A_2'\) such that 
\(A_2\Tredswith{l} A_2'\) and \(A_3'\newsubtype A_2'\). Since \(\newsubtype\) is transitive,
we have \(A_1'\mathrel{\R}\newsubtype A_2'\), which implies \(A_1'\R' A_2'\).\\
\beginextended{} To show (ii), suppose 
\(\disabled{A_1}{S}\). Since
\(\R\) is a simulation up to, we have \(\disabled{A_3}{S}\), which implies \(\disabled{A_2}{S}\).\qed
%%%
%%%By a chain of assumptions, $A_1
%%%\stackrel{l}{\Rightarrow} A_1'$ with
%%% \[ A_1' \subtype A_1''' \mathrel{{\subtype}{\R}{\subtype}} A_2'''
%%% \subtype A_2'. \]
%%%By Part~\ref{le:relation:transitive} we get $A_1'
%%%\mathrel{{\subtype}{\R}{\subtype}} A_2'$ as required. Hence
%%%${\subtype}{\R}{\subtype} \subseteq {\subtype}$. It is clear that
%%%$\ID \subseteq {\subtype}$ where $\ID = \set{(A, A)}$. Hence ${\R}
%%%\subseteq {\subtype}$.
%\end{proof}

%%%\begin{lem}[Replication] \label{le:replication}
%%%If $*A \stackrel{l}{\rightarrow} A'$, then one of the following holds:
%%%(we write $nA$ for $n$ copies of $A$ in parallel)
%%%\begin{enumerate}
%%%\item $A {\stackrel{x}{\rightarrow}} A_1$ and $A 
%%%{\stackrel{\overline{y}}{\rightarrow}} A_2$ and $l=\{x,\overline{y}\}$ and 
%%%$A' =  nA\,|\,A_1\,|\,mA\,|\,A_2\,|\,*A$
%%%\item $A {\stackrel{x}{\rightarrow}} A_1$ and $A 
%%%{\stackrel{\overline{y}}{\rightarrow}} A_2$ and $l=\{x,\overline{y}\}$ and 
%%%$A' =  nA\,|\,A_2\,|\,mA\,|\,A_1\,|\,*A$
%%%\item $A {\stackrel{x}{\rightarrow}} A_1$ and $A 
%%%{\stackrel{\overline{x}}{\rightarrow}} A_2$ and $l=\tau$ and $A' = 
%%%nA\,|\,A_1\,|\,mA\,|\,A_2\,|\,*A$
%%%\item $A {\stackrel{x}{\rightarrow}} A_1$ and $A 
%%%{\stackrel{\overline{x}}{\rightarrow}} A_2$ and $l=\tau$ and $A' = 
%%%nA\,|\,A_2\,|\,mA\,|\,A_1\,|\,*A$
%%%\item $A {\stackrel{l}{\rightarrow}} A_1$ and $A' = nA\,|\,A_1\,|\,*A$
%%%\end{enumerate}
%%%\end{lem}
%%%\proof By induction on the derivation of $*A 
%%%\stackrel{l}{\rightarrow} A'$. There
%%%are six cases.
%%%\begin{enumerate}
%%%\item $A \Tredwith{l} A_1$ \\
%%%      $A|*A \Tredwith{l} A_1 | *A$ (by \rname{Tr-Par1a}) \\
%%%      $*A \Tredwith{l} A_1 | *A$ (by \rname{Tr-Rep}) \\
%%%      Then Part~5 holds.
%%%\item $*A \Tredwith{l} A'$ \\
%%%      $A | *A \Tredwith{l} A | A'$ (by \rname{Tr-Par1b}) \\
%%%      $*A \Tredwith{l} A | A'$ (by \rname{Tr-Rep}) \\
%%%      The induction hypothesis applies to the first line. And placing an $A$ 
%%%in front of $A'$ preserves the induction hypothesis.
%%%\item $A {\Tredwith{x}} A_1$ and $*A {\Tredwith{\Tout{y}}} A'$ \\
%%%      $A|*A \Tredwith{\{x,\overline{y}\}} A_1|A'$ (by \rname{Tr-Par2a}) \\
%%%      $*A \Tredwith{\{x,\overline{y}\}} A_1|A'$ (by \rname{Tr-Rep}) \\
%%%      By the induction hypothesis Part~5 holds for the first line. Therefore 
%%%Part~2 holds for the last line.
%%%\item $A {\Tredwith{\overline{y}}} A_1$ and $*A {\Tredwith{x}} A'$. This 
%%%case is largely the same as the previous.
%%%\item $A | *A \Tredwith{\{x,\overline{x}\}} A'$ (deduced as in Case~3 or~4) 
%%%\\
%%%      $*A \Tredwith{\{x,\overline{x}\}} A'$ (by \rname{Tr-Rep}) \\
%%%      $*A \Tredwith{\tau} A'$ (by \rname{Tr-Com}) \\
%%%      The same analysis applies as in Case~3 or~4.
%%%\item $A | *A \Tredwith{\{x,\overline{x}\}} A'$ (deduced as in Case~3 or~4) 
%%%\\
%%%      $A | *A \Tredwith{\tau} A'$ (by \rname{Tr-Com}) \\
%%%      $*A \Tredwith{\tau} A'$ (by \rname{Tr-Rep}) \\
%%%      The same analysis applies as in Case~3 or~4.
%%%\end{enumerate}
%%%\end{proof}


\newcommand{\simR}{\mathrel{\mathcal{R}}}

\begin{lem}[Structural congruence]
\label{le:subtype-structure} \
\begin{enumerate}
\item $A{|}\textbf{0} \eqtype A$
\item $A{|}B \eqtype B{|}A$
\item $A{|}(B{|}C) \eqtype (A{|}B){|}C$
\item $A{\TOR}B \eqtype B{\TOR}A$
\item $A{\TOR}(B{\TOR}C) \eqtype (A{\TOR}B){\TOR}C$
\item ${*}A \eqtype A | {*}A$
\item $(\nu x)(A|B) \eqtype (\nu x)A\,|\,B$ if $x\notin\FV(B)$
\item $(\nu x)(A{\TOR}B) \eqtype (\nu x)A\,{\TOR}\,B$ if $x\notin\FV(B)$
\item $\subst{\alpha}{\mu\alpha.A}{A} \eqtype \mu\alpha.A$
\end{enumerate}
\end{lem}
\proof These proofs are all standard.\qed
%\end{proof}

We next show that \(\newsubtype\) is a precongruence.
We first show it for some basic type constructors.
\begin{lem}[Precongruence, simple cases] \label{le:subtype-precongruent}
If $A \newsubtype A'$ then
\begin{enumerate}
%%%\item $a_t.A \newsubtype a_t.A'$
%%%\item $x^\xi.A \newsubtype x^\xi.A'$
%%%\item $\tau.A \newsubtype \tau.A'$
%%%\item ${*}A \newsubtype {*}A'$
\item \label{le:subtype-precongruent:par} $A{|}B \newsubtype A'{|}B'$ if $B 
\newsubtype B'$
\item \label{le:subtype-precongruent:subst} $\csubst{y}{x}A \newsubtype 
\csubst{y}{x}A'$
\item $(\nu x)A \newsubtype (\nu x)A'$
\item $\exclude{A}{S} \newsubtype \exclude{A'}{S}$
\item $\project{A}{S} \newsubtype \project{A'}{S}$
%%%\item $A{\TOR}B \newsubtype A'{\TOR}B'$ if $B \newsubtype B'$
\end{enumerate}
\end{lem}
\proof 
These follow from the fact that the following relations are all simulations-up-to.
\[
\begin{array}{l}
\simR_1 = \set{(A\TPAR B, A'\TPAR B') \mid A\newsubtype A', B\newsubtype B'}\\
\simR_2 = \set{(\csubst{\seq{x}}{\seq{y}}A, \csubst{\seq{x}}{\seq{y}}A')\mid A\newsubtype A'}\\
\simR_3 = \set{(\Thiding{x}{A}, \Thiding{x}{A'}) \mid A\newsubtype A'}\\
\simR_4 = \set{(\exclude{A}{S}, \exclude{A'}{S}) \mid A\newsubtype A'}\\
\simR_5 = \set{(\project{A}{S}, \project{A'}{S}) \mid A\newsubtype
A'}\rlap{\hskip 165pt\qEd}
\end{array}
\]
%%%
%%%Construct a relation $\simR$ which contains $\Tzero \simR
%%%\Tzero$
%%%and which is a precongruence (i.e. which is closed with respect to all
%%%constructions in the statement of
%%%the Lemma). We will prove that it is a simulation by induction on the
%%%construction of $\simR$. These
%%%are the cases:
%%%\begin{enumerate} \setcounter{enumi}{-1}
%%%\item Case $\Tzero \simR \Tzero$. No transitions.
%%%\item Case $a_t.A \simR a_t.A'$ with $A \simR A'$. The right-hand transition
%%%$a_t.A' \Tredwith{a_t} A'$ is matched
%%%by the left-hand $a_t.A \Tredwith{a_t} A \simR A'$.
%%%\item Case $x^\xi.A \simR x^\xi.A'$. Similar to the previous case.
%%%\item Case $\tau.A \simR \tau.A'$. Similar to the previous case.
%%%\item Case $*A \simR *A'$ with $A \simR A'$. By Lemma~\ref{le:replication}
%%%there are five possibilities. We
%%%elaborate only the case of Lemma~\ref{le:replication}.1: the right hand side
%%%makes a transition
%%%$*A' \Tredwith{\{x,\overline{y}\}} nA' | A_1' | mA' | A_2' | *A'$ with $A'
%%%\Tredwith{x} A_1'$ and
%%%$A' \Tredwith{\overline{y}} A_2'$. By assumption $A \simR A'$ we have $A
%%%\Tredswith{x} A_1 \simR A_1'$
%%%and $A \Tredswith{\overline{y}} A_2 \simR A_2'$. With repeated applications
%%%of \rname{Tr-Par} and \rname{Tr-Rep}
%%%we get $\*A \Tredswith{\{x,\overline{y}\}} nA | A_1 | mA | A_2 | *A$. And
%%%finally
%%%$nA | A_1 | mA | A_2 | *A \simR nA' | A_1' | mA' | A_2' | *A'$ by
%%%construction.
%%%\item Case $\csubst{y}{x}A \simR \csubst{y}{x}A'$ with $A \simR A'$. There
%%%are two possibilities: \\
%%%(1) Either the right hand side makes a transition $\csubst{y}{x}A'
%%%\Tredwith{\subst{y}{x}l} \csubst{y}{x}A_1'$ with
%%%$A' \Tredwith{l} A_1'$. By assumption $A \Tredswith{l} A_1 \simR A_1'$ and
%%%hence
%%%$\csubst{y}{x}A \Tredswith{\subst{y}{x}l} \csubst{y}{x}A'$, which is $\simR
%%%\csubst{y}{x}A_1'$ by
%%%construction. \\
%%%(2) Or the right hand side makes a transition $\csubst{y}{x}A'
%%%\Tredwith{\tau} \csubst{y}{x}A_1'$ with
%%%$A' \Tredwith{\{z_1,\overline{z}_2\}} A_1'$ and $\subst{y}{x}z_1 =
%%%\subst{y}{x}z_2$.
%%%Then we proceed much as before.
%%%\item Case $(\nu x)A \simR (\nu x)A'$. There are two possibilities: \\
%%%(1) Either the right hand side makes a transition $(\nu x)A' \Tredwith{l}
%%%(\nu x)A_1'$ with $A' \Tredwith{l} A_1'$ and
%%%$\acctarget{l}{\cap}\{x\}{=}\emptyset$. By assumption, $A \Tredswith{l} A_1
%%%\simR A_1'$,
%%%and so $(\nu x)A \Tredswith{l} (\nu x)A_1 \simR (\nu x)A_1'$ as required.
%%%(2) Or the right hand side makes a transition $(\nu x)A' \Tredwith{\tau}
%%%(\nu x)A_1'$ with $(\nu x)A' \Tredwith{\{y,\overline{y}\}} (\nu x)A_1'$,
%%%as before.
%%%\item Case $\exclude{A}{S} \simR \exclude{A'}{S}$ with $A \simR A'$. Similar
%%%to the previous case.
%%%\item Case $\project{A}{S} \simR \project{A'}{S}$. Similar to the previous
%%%case.
%%%\item Case $A{|}B \simR A'{|}B'$ with $A \simR A'$ and $B \simR B'$. This
%%%is largely similar to the case for replication.
%%%\item Case $A{\TOR}B \simR A'{\TOR}B'$ with $A \simR A'$ and $B \simR B'$.
%%%There are four possibilities. \\
%%%(1) Either the right hand side makes a transition
%%%    $A'{\TOR}B' \Tredwith{l} A_1'$ with $A' \Tredwith{l} A_1'$.
%%%    By assumption, $A \Tredswith{l} A' \simR A_1'$, and so $A{\TOR}B
%%%\Tredswith{l} A' \simR A_1'$
%%%    as required. \\
%%%(2) Or the right hand side makes a transition
%%%    $A'{\TOR}B' \Tredwith{\tau} A_1'$ with $A' \Tredwith{\{x,\overline{x}\}}
%%%A_1'$. Then
%%%    we proceed much as before. \\
%%%(3,4) Or the right hand side makes transitions originating in $B'$, which
%%%are similar to the
%%%first two cases.
%%%\end{enumerate}
%%%\todo{Go through all of these for the extended case.}
%\end{proof}

We now show that \(\newsubtype\) is closed under arbitrary type constructors.
\(\FTV(B)\) below is the set of free (i.e., not bound by \(\mu\)) behavioral type
variables.
\begin{lem}[Precongruence, general cases] \label{le:rec1}
If $A \newsubtype A'$ and $\FTV(B)\subseteq \{\alpha\}$,
then $\subst{\alpha}{A}B \newsubtype \subst{\alpha}{A'}B$.
\end{lem}
\proof
%We will prove Part~\ref{le:subtype-precongruent:rec}. All the other cases can be derived
%from it. For instance, to derive the case $a_t.A \newsubtype a_t.A'$, 
%%we use $\subst{\alpha}{A}a_t.\alpha \newsubtype \subst{\alpha}{A'}a_t.\alpha$.
%And to derive the case $A{|}B \newsubtype A'|B'$ we use 
%%$\subst{\alpha}{A}\alpha|B \newsubtype \subst{\alpha}{A'}\alpha|B$
%and then $\subst{\alpha}{B}A'|\alpha \newsubtype 
%%%\subst{\alpha}{B'}A'|\alpha$ and Lemma~\ref{le:relation}.\ref{le:relation:transitive}.
%
%For Part~\ref{le:subtype-precongruent:rec},
Let $\simR = \{ (\subst{\alpha}{A}B,\, \subst{\alpha}{A'}B)\}$. We will 
prove (i) if $\subst{\alpha}{A}B \Tredwith{l} B_1$ then
$\subst{\alpha}{A'}B \Tredswith{l} B_1'$ with $B_1 
\mathrel{{\simR}{\newsubtype}} B_1'$, by induction on
the derivation of $\subst{\alpha}{A'}B \Tredwith{l}B_1'$. We will also prove 
(ii) $\disabled{\subst{\alpha}{A}B}{S}$ implies
$\disabled{\subst{\alpha}{A'}B}{S}$, by induction on the structure of $B$
in the extended case.
In other words, $\simR$ is a simulation-up-to.
Hence (Lemma~\ref{le:relation}.\ref{le:relation:upto}) it is in 
$\newsubtype$. 

We start with (i), with case analysis on the last rule used.
If \(B=\alpha\), then the required condition follows immediately from
\(A\newsubtype A'\). So we consider the case \(B\neq \alpha\) below.
%%for how the transition $\subst{\alpha}{A}B \Tredwith{l}$ is derived:
\begin{enumerate}
\item Case \rname{TR-Act}.
%%%  There are two possibilities. First is that $B=\alpha$ and 
%%%$\subst{\alpha}{A}B = A \Tredwith{l} A_1$.
%%%  By assumption $A {\newsubtype} A'$ we get $\subst{\alpha}{A'}B = A' 
%%%\Tredswith{l} A_1'$ with
%%%  $A_1 \newsubtype A_1'$. Because $\text{id} \in {\simR}$ we get $A_1 \simR 
%%%A_1 \newsubtype A_1'$ as
%%%  required. Actually, the case $B=\alpha$ reoccurs for every case, and is 
%%%exactly the same,
%%%  so we henceforth ignore it. \\
  In this case, $B=\act.B_x$, so
  \[ \subst{\alpha}{A}B = l.\subst{\alpha}{A}B_x \Tredwith{l} 
\subst{\alpha}{A}B_x = B_1.\]
  We also have
  \[ \subst{\alpha}{A'}B = l.\subst{\alpha}{A}B_x \Tredwith{l} 
\subst{\alpha}{A'}B_x = B_1'.\]
  By construction of $\simR$, we have $B_1 \simR B_1' \newsubtype B_1'$ as 
required.
%
\item Case \rname{Tr-Par1}. We show only the left case.
   $B = B_x|B_y$ and we assumed $\subst{\alpha}{A}B_x \Tredwith{l} 
B_{x1}$ to make
  \[ \subst{\alpha}{A}B = \subst{\alpha}{A}B_x | \subst{\alpha}{A}B_y 
\Tredwith{l} B_{x1} | \subst{\alpha}{A}B_y = B_1. \]
  By the induction hypothesis, $\subst{\alpha}{A'}B_x \Tredswith{l} B_{x1}'$ 
with $B_{x1} \mathrel{{\simR}{\newsubtype}} B_{x1}'$.
  (Note that $\alpha$ is not free in $B_{x1}$ or $B_{x1}'$.
%%\todo{I think this requires \(A\) and \(A'\) do not contain free \(\Tbvar\).}
%%\todo{$A$ and $A'$ being closed is implicitly assumed by $A\newsubtype A'$ -Naoki}
)
  That gives
  \[ \subst{\alpha}{A'}B = \subst{\alpha}{A'}B_x | \subst{\alpha}{A'}B_y 
\Tredswith{l} B_{x1}' | \subst{\alpha}{A'}B_y = B_1'.\]
  It remains to prove $B_1 \mathrel{{\simR}{\newsubtype}} B_1'$.
By the condition $B_{x1} \mathrel{{\simR}{\newsubtype}} B_{x1}'$,
there exists \(C\) such that
\[
B_{x1} = \subst{\Tbvar}{A}C \qquad 
\subst{\Tbvar}{A'}C \newsubtype B_{x1}'
\]
So, we get:
\[ 
\begin{array}{lcl}
B_1 = \subst{\Tbvar}{A}(C\TPAR B_y) \simR \subst{\Tbvar}{A'}(C\TPAR B_y)\\
\myquad = \subst{\Tbvar}{A'}C \TPAR \subst{\Tbvar}{A'}B_y \newsubtype B_{x1}'\TPAR \subst{\Tbvar}{A'}B_y = B_1'.
\end{array}
\]
Here, we have used Lemma~\ref{le:subtype-precongruent}, Part~\ref{le:subtype-precongruent:par}.
%%%  \todo{Now what? I don't think we can do this. I think we need to enlarge 
%%%the construction of $\simR$, so that if
%%%  $B_{x1} \simR B_{x1}''$ and $\subst{\alpha}{A}B_y \simR 
%%%\subst{\alpha}{A'}B_y$ then their parallel composition
%%%  is also in $\simR$.}
%
\item Case \rname{Tr-Par2}. We show only the left case.
 $B = B_x|B_y$ and we assumed $\subst{\alpha}{A}B_x \Tredwith{x} B_{x1}$ and
$\subst{\alpha}{A}B_y \Tredwith{\actout{y}} B_{y1}$ to make 
  \[ \subst{\alpha}{A}B = \subst{\alpha}{A}B_x | \subst{\alpha}{A}B_y 
\Tredwith{\actcom{x}{\actout{y}}} B_{x1} | B_{y1} = B_1.\]
By the induction hypothesis, 
\(\subst{\alpha}{A'}B_x \Tredswith{x} B_{x1}'\) and
\(\subst{\alpha}{A'}B_y \Tredswith{x} B_{y1}'\)
with \(B_{x1}\mathrel{{\simR}{\newsubtype}} B_{x1}'\)
and \(B_{y1}\mathrel{{\simR}{\newsubtype}} B_{y1}'\).
 That gives
\[ \subst{\alpha}{A'}{B} =\subst{\alpha}{A'}B_x \TPAR
\subst{\alpha}{A'}B_y \Tredswith{\actcom{x}{\actout{y}}}
B_{x1}'\TPAR B_{y1}'= B_1'.\]
It remains to prove $B_1 \mathrel{{\simR}{\newsubtype}} B_1'$.
From \(B_{x1}\mathrel{{\simR}{\newsubtype}} B_{x1}'\)
and \(B_{y1}\mathrel{{\simR}{\newsubtype}} B_{y1}'\), 
there exist \(C_x\) and \(C_y\) such that
\[
\begin{array}{l}
B_{x1} = \subst{\Tbvar}{A}C_x \qquad
\subst{\Tbvar}{A'}C_x \newsubtype B_{x1}'\\
B_{y1} = \subst{\Tbvar}{A}C_y \qquad
\subst{\Tbvar}{A'}C_y \newsubtype B_{y1}'
\end{array}
\]
Hence, \(B_1 =\subst{\Tbvar}{A}(C_x\TPAR C_y) \simR
             \subst{\Tbvar}{A'}(C_x\TPAR C_y) \newsubtype B_1'\).
%
\item Cases \rname{Tr-Com} and \rname{Tr-Or}. These cases 
follow immediately from the induction hypothesis.
\item Case \rname{Tr-Rep}.
  Then $B = *B_x$ and $\subst{\alpha}{A}B = *\subst{\alpha}{A}B_x 
\Tredwith{l}$. \(\subst{\alpha}{A}B \redwith{l} B_1\) must have been
derived from \[\subst{\alpha}{A}(B_x\TPAR \Trep B_x) = 
\subst{\alpha}{A}B_x\TPAR \Trep\subst{\alpha}{A}B_x
\Tredwith{l} B_1.\]
By the induction hypothesis, 
there exists \(B_1'\) such that 
$$B_1\mathrel{{\simR}{\newsubtype}} B_1'\quad\hbox{and}\quad
\subst{\alpha}{A'}(B_x\TPAR \Trep B_x) \Tredswith{l} B_1'\ .$$
Using \rname{Tr-Rep}, we get \(\subst{\alpha}{A'}B\Tredswith{l}B_1'\) 
as required.
%%%
%%%
%%%  Lemma~\ref{le:replication} gives five possibilities for how this might 
%%%have
%%%  been derived. We elaborate only the first possibility. In this case
%%%  $\subst{\alpha}{A}B_x \Tredwith{x} B_{x1}$ and $\subst{\alpha}{A}B_x 
%%%\Tredwith{\overline{y}} B_{x2}$ giving
%%%  \[ *\subst{\alpha}{A}B_x \Tredwith{\{x,\overline{y}\}} 
%%%n\subst{\alpha}{A}B_x | B_{x1} | m\subst{\alpha}{A}B_x | B_{x2} | 
%%%*\subst{\alpha}{A}B_x = B_1. \]
%%%  By the induction hypothesis, $\subst{\alpha}{A'}B_x \Tredswith{x} B_{x1}'$ 
%%%and $B_{x1} \mathrel{{\simR}{\newsubtype}} B_{x1}'$. \\
%%%  Also by induction hypothesis, $\subst{\alpha}{A'}B_x \Tredswith{x} 
%%%B_{x2}'$ and $B_{x2} \mathrel{{\simR}{\newsubtype}} B_{x2}'$. \\
%%%  These allow us to deduce
%%%  \[ \subst{\alpha}{A'}B = *\subst{\alpha}{A'}B_x 
%%%\Tredswith{\{x,\overline{y}\}} n\subst{\alpha}{A'}B_x | B_{x1}' | 
%%%m\subst{\alpha}{A'}B_x | B_{x2}' | *\subst{\alpha}{A'}B_x = B_1'. \]
%%%  It remains to prove $B_1 \mathrel{{\simR}{\newsubtype}} B_1'$. This is 
%%%substantially the same
%%%  as the case for \rname{Tr-Par1a}.
%%%%
\item Case \rname{Tr-Rec}. 
%%%The first possibility is that $B = 
%%%\mu\alpha.B_x$, so $\subst{\alpha}{A}B = \subst{\alpha}{A'}B = B$.
%%%  This is trivial. The second possibility is that $B = \mu\beta.B_x$ to make
Then, we have $B = \Trec{\beta}{B_x}$ to make
  \[ \subst{\alpha}{A}B = \Trec{\beta}{\subst{\alpha}{A}B_x} \Tredwith{l} 
B_{1}\]
  where we assumed 
$\subst{\beta}{\Trec{\beta}{\subst{\alpha}{A}B_x}}\subst{\alpha}{A}B_x 
\Tredwith{l} B_1$.
  But $\beta$ does not clash with $A$ or $\alpha$ so these two substitutions 
swap around, giving
  \[ \subst{\alpha}{A} \subst{\beta}{\mu\beta.B_x}B_x \Tredwith{l} B_1. \]
  By the induction hypothesis,
  \[ \subst{\alpha}{A'} \subst{\beta}{\mu\beta.B_x} B_x \Tredswith{l} B_1' 
\]
  with $B_1 \mathrel{{\simR}{\newsubtype}} B_1'$. Hence
  \[ \subst{\alpha}{A'}B = \mu\beta.\subst{\alpha}{A'}B_x \Tredswith{l} B_1' 
\]
  as required.
\item Case \rname{Tr-Rename}.
Then, \(B = \csubst{\seq{x}}{\seq{y}}B_x\).
\(\subst{\alpha}{A}B\Tredwith{\subst{\seq x}{\seq y}l} \csubst{\seq{x}}{\seq{y}}B_{x1} = B_1\)
must have been derived from \(\subst{\alpha}{A}B_x \Tredwith{l} B_{x1}\).
From the induction hypothesis, we get 
\[ \subst{\alpha}{A'}B_x \Tredwith{l} B_{x1}'
  \qquad B_{x1} \mathrel{{\simR}{\newsubtype}} B_{x1}'.\]
Let \(B_1' = \csubst{\seq{x}}{\seq{y}}B_{x1}'\). It remains to 
% It remains to 
% prove \(B_1 \mathrel{{\simR}{\newsubtype}} B_{x1}\).
prove \(B_1 \mathrel{{\simR}{\newsubtype}} B_1'\).
% prove \(B_1 \mathrel{{\simR}{\newsubtype}} \csubst{\seq{x}}{\seq{y}}B_{x1}'\).
By 
\(B_{x1} \mathrel{{\simR}{\newsubtype}} B_{x1}'\),
there exists \(C\) such that 
\[ B_{x1} = \subst{\alpha}{A}C \qquad \subst{\alpha}{A'}C \newsubtype B_{x1}'.\]
So, we have:
\[\begin{array}{l}
 B_1 = \subst{\alpha}{A}\csubst{\seq{x}}{\seq{y}}C
   \simR \subst{\alpha}{A'}\csubst{\seq{x}}{\seq{y}}C\\
\qquad   = \csubst{\seq{x}}{\seq{y}}\subst{\alpha}{A'}C
   \newsubtype \csubst{\seq{x}}{\seq{y}}B_{x1}' = B_1'.
\end{array}\]
Here, we used the fact that \(\newsubtype\) is preserved by \(\csubst{\seq{x}}{\seq{y}}\)
(Lemma~\ref{le:subtype-precongruent}, Part~\ref{le:subtype-precongruent:subst}).
\item Cases \rname{Tr-Hiding}, \rname{Tr-Exclude}, and \rname{Tr-Project}:
Similar to \rname{Tr-Rename}.
We use the fact that \(\newsubtype\) is preserved by 
\(\nu\), \(\project{\cdot}{S}\), and \(\exclude{\cdot}{S}\)
(Lemma~\ref{le:subtype-precongruent}).
\end{enumerate}
\beginextended{}
In addition we need to show that $\disabled{\subst{\alpha}{A}B}{S}$ implies
$\disabled{\subst{\alpha}{A'}B}{S}$. This follows by 
straightforward induction on the structure of $B$.\qed
%\end{proof}

%%%\begin{lem}[Precongruence] \label{le:subtype-precongruent}
%%%If $A \subtype A'$ then
%%%\begin{enumerate}
%%%\item $a_t.A \subtype a_t.A'$
%%%\item $x^\xi.A \subtype x^\xi.A'$
%%%\item ${*}A \subtype {*}A'$
%%%\item \label{le:subtype-precongruent:subst} $\csubst{y}{x}A \subtype \csubst{y}{x}A'$
%%%\item $(\nu x)A \subtype (\nu x)A'$
%%%\item $\exclude{A}{S} \subtype \exclude{A'}{S}$
%%%\item $\project{A}{S} \subtype \project{A'}{S}$
%%%\end{enumerate}
%%%If also $B \subtype B'$ then
%%%\begin{enumerate} \setcounter{enumi}{7}
%%%\item $A{|}B \subtype A'{|}B'$
%%%\item $A{\TOR}B \subtype A'{\TOR}B'$
%%%\end{enumerate}
%%%If $B_i \subtype B_i'$ for each $i\in\{1\ldots n\}$ implies
%%%$\subst{\seq{\alpha}}{\seq{B}}A \subtype \subst{\seq{\alpha}}{\seq{B'}}A'$, then
%%%\begin{enumerate} \setcounter{enumi}{9}
%%%\item $\mu\alpha_1\ldots\mu\alpha_n.A \subtype \mu\alpha_1\ldots\mu\alpha_n.A'$
%%%\end{enumerate}
%%%\end{lem}
%%%\proof These proofs are all standard. \end{proof}



\begin{lem}[Substitution]
%%%\todo{The following statements were about \(\csubst{y}{x}A\).
%%%But this lemma is used in the form \(\csubst{\xx}{\yy}A\), 
%%%so I rewrote these statement and a part of the proof.
%%%In case I am wrong, all the old contents are in comments. --Kohei}
\label{le:subtype-substitution} \
\begin{enumerate}
%% \item $\csubst{y}{x}\textbf{0} \eqtype \textbf{0}$
%% \item $\csubst{y}{x}(a.A) \eqtype (\subst{y}{x}a).\csubst{y}{x}A$
%% \item $\csubst{y}{x}(z^\acclab.A) \eqtype (\subst{y}{x}z)^\acclab.\csubst{y}{x}A$
%% \item \label{le:subtype-substitution:par} $\csubst{y}{x}(A|B) \eqtype \csubst{y}{x}A\ |\ \csubst{y}{x}B$
%% \item $\csubst{y}{x}(A{\TOR}B) \eqtype \csubst{y}{x}A\ \TOR\ \csubst{y}{x}B$
%% \item $\csubst{y}{x}({*}A) \eqtype *(\csubst{y}{x}A)$
%% \item $\csubst{y}{x}\csubst{a}{b}A \eqtype
%% \csubst{a}{\subst{y}{x}b}\csubst{y}{x}A$ if $\acctarget{a}{\cap}\{x,y\}{=}\emptyset$
%% \item $\csubst{y}{x}(\nu z)A \eqtype (\nu z)(\csubst{y}{x}A)$ if $\{z\}{\cap}\{x,y\}{=}\emptyset$
%% \item \label{le:subtype-substitution:exclude1}
%%    $\csubst{y}{x}(\exclude{A}{S}) \eqtype \exclude{(\csubst{y}{x}A)}{S}$, and \\
%%    $\csubst{y}{x}(\project{A}{S}) \eqtype \project{A}{S}$, \\
%%    if $S{\cap}\{x,y\}{=}\emptyset$
%% \item \label{le:subtype-substitution:exclude2}
%%   $\csubst{y}{x}(\exclude{A}{S}) \eqtype \exclude{A}{S}$, and \\
%%   $\csubst{y}{x}(\project{A}{S}) \eqtype \project{(\csubst{y}{x}A)}{S}$, \\
%%   if $\{y\}\subseteq S$
\item $\csubst{\xx}{\yy}\textbf{0} \eqtype \textbf{0}$
\item $\csubst{\xx}{\yy}(a.A) \eqtype (\subst{\xx}{\yy}a).\csubst{\xx}{\yy}A$
\item $\csubst{\xx}{\yy}(z^\acclab.A) \eqtype (\subst{\xx}{\yy}z)^\acclab.\csubst{\xx}{\yy}A$
\item \label{le:subtype-substitution:par} $\csubst{\xx}{\yy}(A|B) \eqtype \csubst{\xx}{\yy}A\ |\ \csubst{\xx}{\yy}B$
\item $\csubst{\xx}{\yy}(A{\TOR}B) \eqtype \csubst{\xx}{\yy}A\ \TOR\ \csubst{\xx}{\yy}B$
\item $\csubst{\xx}{\yy}({*}A) \eqtype *(\csubst{\xx}{\yy}A)$
\item $\csubst{\xx}{\yy}\csubst{a}{b}A \eqtype
\csubst{a}{\subst{\xx}{\yy}b}\csubst{\xx}{\yy}A$ if $\acctarget{a}{\cap}\{\xx,\yy\}{=}\emptyset$
\item $\csubst{\xx}{\yy}(\nu z)A \eqtype (\nu z)(\csubst{\xx}{\yy}A)$ if $\{z\}{\cap}\{x,y\}{=}\emptyset$
%%%\todo{We need to think more about the following two branches.
%%%At least, in the case \rname{T-In} in the proof of B.2, 
%%%\(\csubst{\xx}{\yy}(\project{A}{S}) \eqtype \project{\csubst{\xx}{\yy}A}{S}\) is required under \(S{\cap}\{x,y\}{=}\emptyset\).}
\item \label{le:subtype-substitution:exclude1}
   $\csubst{\xx}{\yy}(\exclude{A}{S}) \eqtype \exclude{(\csubst{\xx}{\yy}A)}{S}$, and \\
   $\csubst{\xx}{\yy}(\project{A}{S}) \eqtype \project{\csubst{\xx}{\yy}A}{S}
    \eqtype \project{A}{S}$, \\
   if $S{\cap}\{x,y\}{=}\emptyset$
\item \label{le:subtype-substitution:exclude2}
  $\csubst{\xx}{\yy}(\exclude{A}{S}) \eqtype \exclude{A}{S}$, 
%%%  $\csubst{\xx}{\yy}(\project{A}{S}) \eqtype \project{(\csubst{\xx}{\yy}A)}{S}$, \\
  if $\{\xx\}\subseteq S$
\end{enumerate}
\end{lem}
\proof 
Most parts are straightforward, although \textbf{Part~\ref{le:subtype-substitution:par}} is non-obvious in
the case of labels $\{x,\overline{y}\}$. For
Part~\ref{le:subtype-substitution:par}, we construct a relation
% $\mathcal{S} = \{ ( \csubst{y}{x}(A|B), \csubst{y}{x}A | \csubst{y}{x}B) \}$ 
$\mathcal{S} = \{ ( \csubst{\xx}{\yy}(A|B), \csubst{\xx}{\yy}A | \csubst{\xx}{\yy}B) \}$ 
and prove $\mathcal{S}$ and $\mathcal{S}^{-1}$ are simulations.
The interesting case is when we infer
%% \[ \csubst{y}{x}A | \csubst{y}{x}B \stackrel{\tau}{\rightarrow}
%% \csubst{y}{x}A' | \csubst{y}{x}B' \] from
%% \[ A \stackrel{z_1}{\rightarrow} A' \qquad
%%    B \stackrel{\overline{z_2}}{\rightarrow} B' \qquad
%%    \subst{y}{x}z_1 = \subst{y}{x}z_2.
%% \]
\[ \csubst{\xx}{\yy}A | \csubst{\xx}{\yy}B \stackrel{\tau}{\rightarrow}
\csubst{\xx}{\yy}A' | \csubst{\xx}{\yy}B' \] from
\[ A \stackrel{z_1}{\rightarrow} A' \qquad
   B \stackrel{\overline{z_2}}{\rightarrow} B' \qquad
   \subst{\xx}{\yy}z_1 = \subst{\xx}{\yy}z_2.
\]
This gives
 \[ A|B \stackrel{\{z_1,\overline{z_2}\}}{\rightarrow} A'|B'. \]
Hence
%%  \[ \csubst{y}{x}(A|B) \stackrel{\{\subst{y}{x}z_1,\subst{y}{x}\overline{z_2}\}}{\longrightarrow} \csubst{y}{x}(A'|B'). \]
%% And hence as required
%%  \[ \csubst{y}{x}(A|B) \stackrel{\tau}{\rightarrow} \csubst{y}{x}(A'|B'). \]
 \[ \csubst{\xx}{\yy}(A|B) \stackrel{\{\subst{\xx}{\yy}z_1,\subst{\xx}{\yy}\overline{z_2}\}}{\longrightarrow} \csubst{\xx}{\yy}(A'|B'). \]
And hence as required
 \[ \csubst{\xx}{\yy}(A|B) \stackrel{\tau}{\rightarrow} \csubst{\xx}{\yy}(A'|B'). \]

\textbf{Part~\ref{le:subtype-substitution:exclude1}.} Here we
construct $\mathcal{S} = \{ (\,\csubst{\xx}{\yy}(\exclude{A}{S}),\
\exclude{(\csubst{\xx}{\yy}A)}{S}\,) \}$ where $S$ does not clash
with $\{\xx,\yy\}$, and we prove that $\mathcal{S}$ and $\mathcal{S}^{-1}$
are simulations. We focus on two cases.
\begin{enumerate}
\item Suppose $\exclude{(\csubst{\xx}{\yy}A)}{S}
\stackrel{\subst{\xx}{\yy}l}{\longrightarrow}
\exclude{(\csubst{\xx}{\yy}A')}{S}$ is inferred from $$A
\stackrel{l}{\rightarrow} A'\quad\hbox{and}\quad\acctarget{\subst{\xx}{\yy}l}
{\cap}S=\emptyset.$$ We must infer that $\csubst{\xx}{\yy}(\exclude{A}{S})
\stackrel{\subst{\xx}{\yy}l}{\longrightarrow}
\csubst{\xx}{\yy}(\exclude{A'}{S})$. This requires $\acctarget{l}
{\cap}S=\emptyset$, which we prove as follows. It is assumed that
$S$ does not clash, so $\{\xx,\yy\}{\cap}S = \emptyset$. We also
have $\acctarget{\subst{\xx}{\yy}l} {\cap}S=\emptyset$, and so
$\subst{\xx}{\yy}(\acctarget{l}){\cap}S=\emptyset$. Let $T =
\acctarget{l}$. Suppose $z\in T$. Then either $z\in\xx$ so $z\notin
S$, or $z\in\yy$ so $z\notin S$, or $z\notin\{\xx,\yy\}$ so
$z\in\subst{\xx}{\yy}T$ so $z\notin S$. In all cases $z\notin S$, so
$T{\cap}S = \emptyset$ as required.
%
\item Suppose $\exclude{(\csubst{\xx}{\yy}A)}{S}
\stackrel{\tau}{\rightarrow} \exclude{(\csubst{\xx}{\yy}A')}{S}$ is
inferred from $A \stackrel{l}{\rightarrow} A'$ and
$\acctarget{\subst{\xx}{\yy}l} \subseteq S$. We must infer
$\csubst{\xx}{\yy}(\exclude{A}{S}) \stackrel{\tau}{\rightarrow}
\csubst{\xx}{\yy}(\exclude{A'}{S})$. This requires $\acctarget{l}
\subseteq S$, which we prove as follows. Once again let $T =
\acctarget{l}$. We have $\{\xx,\yy\}{\cap}S = \emptyset$ and
$\subst{\xx}{\yy}T \subseteq S$. Suppose $z\in T$. Then
$\subst{\xx}{\yy}z \in \subst{\xx}{\yy}T$, and $\subst{\xx}{\yy}z
\in S$. Either $z\in\xx$ so $y\in S$, which is a contradiction. Or
% $z\in\yy$ so $y\in S$, which is a contradiction. Or
\(z\not\in\xx\), so \(\subst{\xx}{\yy}z = z\in S\).
%%%\todo{There was a sentence ``$z\in\yy$ so $y\in S$'' here.
%%%But we do not assume \(\xx \cap \yy = \emptyset\),
%%%so the argument in this sentence holds only in the case \(z \in \set{\yy}\setdif\set{\xx}\)--Kohei}
%%%$z\in\set{\yy}\setdif\set{\xx}$ so $y\in S$, which is a contradiction. Or
%%%$z\notin\{\xx,\yy\}$ so $z\in S$. 
Hence $T \subseteq S$ as required.\qed
\end{enumerate}
%\end{proof}

\begin{lem}[Exclusion and Projection] \
\label{le:subtype-exclusion}
\setbox0=\hbox{$\exclude{(A{\TOR}B)}{S} {\eqtype} \exclude{A}{S} {\TOR} \exclude{B}{S}$}\newlength{\excolwidth}\setlength{\excolwidth}{\wd0}
\begin{enumerate}
\item \makebox[\excolwidth][l]{$\exclude{\textbf{0}}{S} {\eqtype} \textbf{0}$}
      \makebox[\excolwidth][l]{$\project{\textbf{0}}{S} {\eqtype} \textbf{0}$}
\item \makebox[\excolwidth][l]{$\exclude{(a_t.A)}{S} {\eqtype} a_t.(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{(a_t.A)}{S} {\eqtype} \tau_t.(\project{A}{S})$}
      \makebox[0pt][l]{if $\acctarget{a}{\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{(a_t.A)}{S} {\eqtype} \tau_t.\exclude{A}{S}$}
      \makebox[\excolwidth][l]{$\project{(a_t.A)}{S} {\eqtype} a_t.\project{A}{S}$}
      \makebox[0pt][l]{if $\acctarget{a}{\subseteq}S$}
\item \makebox[\excolwidth][l]{$\exclude{(z^\xi.A)}{S} {\eqtype} z^\xi.(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{(z^\xi.A)}{S} {\eqtype} \tau_c.\project{A}{S}$}
      \makebox[0pt][l]{if $\acctarget{z^\xi}{\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{(z^\xi.A)}{S} {\eqtype} \tau_c.\exclude{A}{S}$}
      \makebox[\excolwidth][l]{$\project{(z^\xi.A)}{S} {\eqtype} z^\xi.(\project{A}{S})$}
      \makebox[0pt][l]{if $\acctarget{z^\xi}{\subseteq}S$}
\item \makebox[\excolwidth][l]{$\exclude{(A|B)}{S} {\eqtype} \exclude{A}{S}\ |\ \exclude{B}{S}$}
      \makebox[\excolwidth][l]{$\project{(A|B)}{S} {\eqtype} \project{A}{S}\ |\ \project{B}{S}$}
      \label{le:subtype-exclusion:par}
\item \makebox[\excolwidth][l]{$\exclude{(A{\TOR}B)}{S} {\eqtype} \exclude{A}{S} {\TOR} \exclude{B}{S}$}
      \makebox[\excolwidth][l]{$\project{(A{\TOR}B)}{S} {\eqtype} \project{A}{S} {\TOR} \project{B}{S}$}
\item \makebox[\excolwidth][l]{$\exclude{({*}A)}{S} {\eqtype} {*}(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{({*}A)}{S} {\eqtype} {*}(\project{A}{S})$}
\item \makebox[\excolwidth][l]{$\exclude{(\exclude{A}{S})}{T} {\eqtype} \exclude{A}{S\cup T}$}
      \makebox[\excolwidth][l]{$\project{(\project{A}{S})}{T} {\eqtype} \project{A}{S\cap T}$}
\item \makebox[\excolwidth][l]{$\exclude{A}{S} {\eqtype} A$}
      \makebox[\excolwidth][l]{$\project{A}{S} {\newsubtype} \Tzero$}
      \makebox[0pt][l]{if $\FV(A){\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{A}{S} {\newsubtype} \Tzero$}
      \makebox[\excolwidth][l]{$\project{A}{S} {\eqtype} A$}
      \makebox[0pt][l]{if $\FV(A){\subseteq}S$}
      \label{le:subtype-exclusion:nil}
\end{enumerate}
\end{lem}
\proof Straightforward.\qed
%\end{proof}

\begin{lem}[Simulation] \
\label{le:subtype-simulation}
\begin{enumerate}
\item \label{le:subtype-simulation:traces} If $A_1 \newsubtype A_2$ then $\traces{x}{A_1} \subseteq
\traces{x}{A_2}$ for any $x$.
\item \label{le:subtype-simulation:sequence} If $A \stackrel{\{x,\overline{y}\}}{\longrightarrow} A'$ then
$A \stackrel{x}{\rightarrow}\stackrel{\overline{y}}{\rightarrow}
A'$.
\item $A \newsubtype A{\TOR}B $
%%%\item $A \subtype \textbf{0}$
\item $A{\TOR}A \newsubtype A $
\item \label{le:subtype-simulation:separate} $A\newsubtype \exclude{A}{S} \mathrel{|}
\project{A}{S} $
\item \label{le:subtype-simulation:rec} 
If $\subst{\alpha}{B}A\newsubtype B$ then $\mu\alpha.A\newsubtype B$
\item $B_1{\TOR}B_2\newsubtype A $ if and only if $B_1\newsubtype A$ 
and $B_2\newsubtype A$
\end{enumerate}
\end{lem}
\proof These proofs are largely standard.

\textbf{Part~\ref{le:subtype-simulation:traces}} follows immediately from the
definitions of subtyping and traces.
%Let \(\accseq\) ba a sequence of access labels. Suppose that
%\(\accseq\in \traces{x}{A_2}\). We show \(\accseq \in
%\traces{x}{A_1}\) by induction on the length of \(\accseq\).
%\begin{itemize}
%\item Case \(\accseq = \emptyuselab\):
%It must be the case that there exists \(A_2'\) such that \(A_2
%\Tredswith{\Tredlabsilent} A_2'\). From \(A_1 \subtype A_2\), there
%exists \(A_1'\) such that \(A_1 \Tredswith{\Tredlabsilent}\TSPCONG
%A_1'\). Thus, \(\emptyuselab \in A_1\).
%\item Case \(\accseq = \acclab \cdot \accseq_1\):
%It must be the case that there exists \(A_2'\) such that \(A_2
%\Tredswith{\acclab} A_2'\) and \(\accseq_1 \in \traces{x}{A_2'}\).
%From \(A_1 \subtype A_2\), there exists \(A_1'\) such that \(A_1
%\Tredswith{\acclab} A_1'\) and \(A_1' \subtype A_2'\). From the
%induction hypothesis, we have \(\accseq_1 \in \traces{x}{A_1'}\).
%Thus, \(\accseq \in \traces{x}{A_1}\).
%\end{itemize}

\textbf{Part~\ref{le:subtype-simulation:rec}.}
%%%\todo{Done for representative cases, but I'm not sure the following proof is correct --Kohei.}
Suppose \(\Tsubst{A}{\Tbvar}{B} \newsubtype B\). 
Let \(\R\) be
\[\set{(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A},\Tsubst{A'}{\Tbvar}{B})\mid 
   \FTV(A')=\set{\Tbvar}}.\]
By Lemma~\ref{le:subtype-precongruent}.\ref{le:relation:upto}, 
It suffices to prove that \(\R\)
is a simulation up to.

Suppose that \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \mathrel{\R} 
\Tsubst{A'}{\Tbvar}{B}\) and
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\).
We show that there exists \(B'\) such that \(\Tsubst{A'}{\Tbvar}{B}
\Tredswith{l} B'\) and \(A'' \mathrel{{\R}{\newsubtype}} B'\)
by induction on the derivation of
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\), with case analysis
on the last rule used. We show main cases; the other cases are similar or straightforward.
%% We show that \(\R\) is a simulation up to \(\subtype\), so that \(\R \subseteq \subtype\),
%% by induction on the derivation of \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\).
%% In the following cases, we show that there exists \(B'\) such that
%% \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{l} B'\) and \(B' \subtype \R \subtype A''\).
\begin{itemize}
\item Case \rname{TR-Act}:
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\) is derived from\\
\(\Tin{l}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}} \Tredwith{l} \Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}\)
where \(A' = \Tin{l}A_1\) and \(A'' = \Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}\).
Thus, \(\Tsubst{A'}{\Tbvar}{B} = \Tin{l}{\Tsubst{A_1}{\Tbvar}{B}} \Tredwith{l} \Tsubst{A_1}{\Tbvar}{B}\).
\item Case \rname{TR-Par1}:
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\) is derived from\\
\(\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{l} A_1'\)
where \(A' = A_1 \TPAR A_2\) and \(A'' = A_1' \TPAR \Tsubst{A_2}{\Tbvar}{\Trec{\Tbvar}{A}}\).
By the induction hypothesis, there exists \(B_1'\) such that
\(\Tsubst{A_1}{\Tbvar}{B} \Tredswith{l} B_1'\) and \(A_1' \mathrel{{\R}{\newsubtype}} B_1'\). Thus, we have \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{l} B_1' \TPAR \Tsubst{A_2}{\Tbvar}{B}\). 
It remains to show 
\(A''=
A_1' \TPAR \subst{\Tbvar}{\Trec{\Tbvar}{A}}{A_2}
\mathrel{{\R}{\newsubtype}} B_1' \TPAR \Tsubst{A_2}{\Tbvar}{B}\).
From \(A_1' \mathrel{{\R}{\newsubtype}} B_1'\), we get
\[ A_1' = \subst{\Tbvar}{\Trec{\Tbvar}{A}}C \qquad 
 \subst{\Tbvar}{B}C \newsubtype B_1'\]
for some \(C\). So, 
\[
\begin{array}{l}
 A''=A_1' \TPAR \subst{\Tbvar}{\Trec{\Tbvar}{A}}{A_2}
 = \subst{\Tbvar}{\Trec{\Tbvar}{A}}{(C\TPAR A_2)}\\
 \simR
\subst{\Tbvar}{B}{(C\TPAR A_2)}
 = \subst{\Tbvar}{B}C\TPAR \subst{\Tbvar}{B}A_2
 \newsubtype B_1' \TPAR \Tsubst{A_2}{\Tbvar}{B}
\end{array}
\]
%% It must be the case that
%% \begin{itemize}
%% \item \(A' = A_1 \TPAR A_2\)
%% \item \(A'' = \Tsubst{(A_1' \TPAR A_2)}{\Tbvar}{\Trec{\Tbvar}A}\)
%% \item \(A_1 \Tredwith{l} A_1'\)
%% \end{itemize}
%% for some \(A_1\) and \(A_1'\) and \(A_2\). Thus,
%% \(\Tsubst{A'}{\Tbvar}{B} \Tredwith{x} \Tsubst{(A_1' \TPAR
%% A_2)}{\Tbvar}{B}\). From the definition of \(\R\), we have
%% \(\Tsubst{(A_1' \TPAR A_2)}{\Tbvar}{B} \R A''\).

\item Case \rname{TR-Par2}:
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{\actcom{x}{\actout{y}}} A''\) is derived from
\(\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{x} A_1'\) and
\(\Tsubst{A_2}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{\actout{y}} A_2'\)
where \(A' = A_1 \TPAR A_2\) and \(A'' = A_1' \TPAR A_2'\).
From the induction hypothesis, there exist \(B_1'\) and \(B_2'\) such that
\(\Tsubst{A_1}{\Tbvar}{B} \Tredswith{x} B_1'\) and \(A_1' \mathrel{{\R}{\newsubtype}} B_1'\) and
\(\Tsubst{A_2}{\Tbvar}{B} \Tredswith{\actout{y}} B_2'\) and \(A_2' \mathrel{{\R}{\newsubtype}} B_2'\).
Thus, we have \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{\actcom{x}{\actout{y}}} B_1' \TPAR B_2'\). 
From \(A_1' \mathrel{{\R}{\newsubtype}} B_1'\) and
\(A_2' \mathrel{{\R}{\newsubtype}} B_2'\), we get 
\(A_1' \TPAR A_2' \mathrel{{\R}{\newsubtype}} B_1' \TPAR B_2'\) as required.
%%%We need to show that
%%%\(A_1' \TPAR A_2' \mathrel{{\R}{\newsubtype}} B_1' \TPAR B_2'\).
%%%Let \(A_1' \mathrel{\R} B_1'' \newsubtype B_1'\) and \(A_2' \mathrel{\R} B_2'' \newsubtype B_2'\).
%%%Then, \(B_1'' \TPAR B_2'' \mathrel{\newsubtype} B_1' \TPAR B_2'\) and
%%%\(A_1' \TPAR A_2' \mathrel{\R} B_1'' \TPAR B_2''\) follows,
%%%so that \(A_1' \TPAR A_2' \mathrel{{\R}{\newsubtype}} B_1' \TPAR B_2'\)
%%%follows as required.
%% It must be the case that
%% \begin{itemize}
%% \item \(l = \actcom{x}{\actout{y}}\)
%% \item \(A' = A_1 \TPAR A_2\)
%% \item \(A_1 \Tredwith{x} A_1'\)
%% \item \(A_2 \Tredwith{\actout{y}} A_2'\)
%% \item \(A'' = \Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{\Trec{\Tbvar}A}\)
%% \end{itemize}
%% for some \(A_1\) and \(A_2\) an d\(A_1'\) and \(A_2'\) and \(x\) and \(y\).
%% Thus, \(\Tsubst{A'}{\Tbvar}{B} \Tredwith{\actcom{x}{\actout{y}}} \Tsubst{(A_1' \TPAR
%% A_2)}{\Tbvar}{B}\). From the definition of \(\R\), we have
%% \(\Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{B} \R A''\).

%%%\item Case \rname{TR-Com}:
%%%\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredsilent A''\) is derived from
%%%\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{\actcom{x}{\actout{x}}} A''\).
%%%From the induction hypothesis, there exists \(B'\) such that
%%%\(\Tsubst{A'}{\Tbvar}{B} \Tredswith{\actcom{x}{\actout{x}}} B'\) and \(A'' \mathrel{{\R}{\newsubtype}} B'\).
%%%Thus, we have \(\Tsubst{A'}{\Tbvar}{B} \Tredsilent^* B'\), as required.
%% It must be the case that
%% \begin{itemize}
%% \item \(\act = \Tredlabsilent\)
%% \item \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{\actcom{x}{\actout{x}}} A''\)
%% \end{itemize}
%% for some \(x\).
%% From the induction hypothesis,
%% we have \(\Tsubst{A'}{\Tbvar}{B} \subtype \Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}{A}}\),
%% so that \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{\actcom{x}{\actout{x}}} B'\)
%% and \(B' \subtype A''\) for some \(B'\).

\item Case \rname{TR-Rec}:
\begin{itemize}
\item Case \(A' = \Trec{\beta}A_1\):
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\) is derived from
\[
\begin{array}{l}
\Tsubst{\Tsubst{A_1}{\beta}{\Trec{\beta}{A_1}}}{\Tbvar}{\Trec{\Tbvar}{A}}\\
=\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}
  \Tredwith{l} A''.
\end{array}
\]
Here, we assumed without loss of generality
% that \(\Tbvar\) is not free in \(A\) and \(B\).
%%%\todo{There was \(\Tbvar\) in place of \(\beta\).
%%%I think \(\beta\) is correct. --Kohei}
that \(\beta\) is not free in \(A\) and \(B\).
%%%\(\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}}\) and
%%%we can assume that \(\beta\) does not freely occur in \(A\).
Thus, by the induction hypothesis, there exists \(B'\) such that
\[
\begin{array}{l}
\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}} 
=
\Tsubst{\Tsubst{A_1}{\beta}{\Trec{\beta}{A_1}}}{\Tbvar}{B} 
\Tredswith{l} B'
\end{array}
\]
and
\(A'' \mathrel{{\R}{\newsubtype}} B'\).
%%%We can assume that \(\beta\) does not freely occur in \(B\).
%%%Thus, \(\Tsubst{\Tsubst{A_1}{\beta}{\Trec{\beta}{A_1}}}{\Tbvar}{B}\)
%%%is syntactically equal to
%%%\(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}}\), so that
Using \rname{Tr-Rec}, we obtain
\(\Tsubst{A'}{\Tbvar}{B}=\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}} \Tredswith{l} B'\) as required.
%% Thus, we have \(\Tsubst{A'}{\Tbvar}{B} \Tredsilent^* B'\), as required.
%% We can assume that \(\beta\) does not freely occur in \(B\).
%% Thus, \(\Tsubst{\Tsubst{A_1}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}}}}{\Tbvar}{B}\) is equal to
%% \(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}\)

%% We can assume that \(\beta\) does not freely occur in \(A\) and \(B\).
%% It must be the case that
%% \begin{itemize}
%% \item \(A' = \Trec{\beta}A_1\)
%% \item \(\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}} \Tredwith{l} A''\)
%% \end{itemize}
%% for some \(A_1\).
%% From the induction hypothesis, we have \(\Tsubst{A_1}{\Tbvar}{B} \subtype \Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}\),
%% so that \(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}}\) \(\subtype\)\\
%% \(\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}\).
%% Thus, there exists \(B'\) such that
%% \(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}} \Tredswith{l} B'\), so that \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{l} B'\),
%% and \(B' \subtype A''\).

\item Case \(A' = \Tbvar\):
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}\) is equal to \(\Trec{\Tbvar}A\).
From \(\Trec{\Tbvar}A \mathrel{\newsubtype} B\),
there exists \(B'\) such that \(B \Tredswith{l} B'\) and
\(A'' \mathrel{\newsubtype} B'\) as required.
%% It must be the case that
%% \begin{itemize}
%% \item \(A' = \Tbvar\)
%% \item \(\Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{l} A''\)
%% \end{itemize}
%% From the induction hypothesis, we have
%% \(\Tsubst{A}{\Tbvar}{B} \subtype \Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}}\),
%% so that there exists \(B'\) such that
%% \(\Tsubst{A}{\Tbvar}{B} \Tredswith{l} B'\) and
%% \(B' \subtype A''\).
\end{itemize}
\end{itemize}
\beginextended{}
We also need to prove that 
$$\disabled{\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}}{S}
% implies \(\Tsubst{A'}{\Tbvar}{B}\) for any \(A'\).
\quad\hbox{implies}\quad
\disabled{\Tsubst{A'}{\Tbvar}{B}}{S}\quad\hbox{for any}\quad A'\ .$$
This is proved by induction on the derivation of 
\(\disabled{\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}}{S}\).
We show the only non-trivial case, where 
\(\disabled{\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}}{S}\) has been derived 
by using the last rule in Figure~\ref{fig:disabledness}.
The other cases follow immediately from the induction hypothesis.

There are two cases to consider.
\begin{itemize}
\item Case where \(A'=\Tbvar\):
Then, \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}= \Trec{\Tbvar}A\) and
\(\disabled{\Trec{\Tbvar}A}{S}\) must have been deduced from\\
\(\disabled{\subst{\Tbvar}{\Trec{\Tbvar}{A}}A}{S}\). 
By the induction hypothesis, we have 
\(\disabled{\subst{\Tbvar}{B}A}{S}\). By the assumption 
\(\Tsubst{A}{\Tbvar}{B} \newsubtype B\), we have \(\disabled{B}{S}\) as required
(note that \(\subst{\Tbvar}{B}A'=B\) in this case).
\item Case where \(A' = \Trec{\beta}{C}\).
Let \(C'\) be \(\subst{\Tbvar}{\Trec{\Tbvar}{A}}C\).
Then, \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}= \Trec{\beta}{C'}\),
and \(\disabled{\Trec{\beta}{C'}}{S}\) must have been derived from
\( \disabled{\subst{\beta}{\Trec{\beta}{C'}}C'}{S}\).
Here, we note 
\[ \subst{\beta}{\Trec{\beta}{C'}}C' = \subst{\Tbvar}{\Trec{\Tbvar}{A}}
 \subst{\beta}{\Trec{\beta}C}C.\]
So, from the induction hypothesis, we get \\
\(\disabled{\subst{\Tbvar}{B}\subst{\beta}{\Trec{\beta}C}C}{S}\), i.e.,
\[ \disabled{\subst{\beta}{\Trec{\beta}\subst{\Tbvar}{B}C}\subst{\Tbvar}{B}C}{S}.\]
By using the last rule of Figure~\ref{fig:disabledness}, we get
\(\disabled{\subst{\Tbvar}{B}A'}{S}\) as required.\qed
\end{itemize}
%\end{proof}


==> ProofTypeSoundness.tex <==

\section{Proof of Theorem~\ref{th:safety}}
\label{sec:app:safety}

We have written the following lemmas generically so they can apply
to both the main type system and also the extended type system. When
reading the lemmas for the main type system
(Section~\ref{sec:typing}) the subscript in actions $a_t.A$ should
be taken as $0$ always. The proofs in this appendix apply to the
main type system. In the following appendix the lemmas will address
the extended type system of Section~\ref{sec:extension}, $a_t.A$
is as defined in that section, and Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:traces}
applies to $\etraces{x}{}$ instead of $\traces{x}{}$, and
proofs will be for that extended type system.


\begin{lemma}[Precongruence] \label{le:subtype-precongruent}
If $A \subtype A'$ then
\begin{enumerate}
\item $a_t.A \subtype a_t.A'$
\item $x^\xi.A \subtype x^\xi.A'$
\item ${*}A \subtype {*}A'$
\item \label{le:subtype-precongruent:subst} $\csubst{y}{x}A \subtype \csubst{y}{x}A'$
\item $(\nu x)A \subtype (\nu x)A'$
\item $\exclude{A}{S} \subtype \exclude{A'}{S}$
\item $\project{A}{S} \subtype \project{A'}{S}$
\end{enumerate}
If also $B \subtype B'$ then
\begin{enumerate} \setcounter{enumi}{7}
\item $A{|}B \subtype A'{|}B'$
\item $A{\TOR}B \subtype A'{\TOR}B'$
\end{enumerate}
If $B_i \subtype B_i'$ for each $i\in\{1\ldots n\}$ implies
$\subst{\seq{\alpha}}{\seq{B}}A \subtype \subst{\seq{\alpha}}{\seq{B'}}A'$, then
\begin{enumerate} \setcounter{enumi}{9}
\item $\mu\alpha_1\ldots\mu\alpha_n.A \subtype \mu\alpha_1\ldots\mu\alpha_n.A'$
\end{enumerate}
%\item If also $B_i \subtype B_i'$ for each $i$, and
%$\seq{B},\seq{B}'$ contain no free recursion variables,
%then $\subst{\seq{\alpha}}{\seq{B}}A \subtype
%\subst{\seq{\alpha}}{\seq{B}'}A'$ where
%$\seq{\alpha}$ are the free recursion
%variables in $A,A'$.
\end{lemma}
\proof %\begin{proof} 
These proofs are all standard.\qed
%\end{proof}

\begin{lemma}[Simulation relation] \
\label{le:relation}
\begin{enumerate}
\item \label{le:relation:transitive} $A \subtype B \subtype C$ implies $A \subtype C$
\item $A \subtype A$
\item \label{le:relation:upto} (Simulation-up-to) Let $\R$ be a relation on behavioral types such that whenever $A_1
\R A_2$ then $A_2 \stackrel{l}{\rightarrow} A_2'$ implies $A_1
\stackrel{l}{\Rightarrow} A_1'$ and $A_1'{\subtype} \R {\subtype}
A_2'$ for some $A_1'$. Then $\R \subseteq {\subtype}$.
\end{enumerate}
\end{lemma}
\proof %\begin{proof} We elaborate only
\textbf{Part~\ref{le:relation:upto}.} First we show that
${\subtype}\R{\subtype}$ is a simulation. Suppose
 \[ A_1 \subtype A_1'' \mathrel{\R} A_2'' \subtype A_2 \]
and $A_2 \stackrel{l}{\rightarrow}$. By a chain of assumptions, $A_1
\stackrel{l}{\Rightarrow} A_1'$ with
 \[ A_1' \subtype A_1''' \mathrel{{\subtype}{\R}{\subtype}} A_2'''
 \subtype A_2'. \]
By Part~\ref{le:relation:transitive} we get $A_1'
\mathrel{{\subtype}{\R}{\subtype}} A_2'$ as required. Hence
${\subtype}{\R}{\subtype} \subseteq {\subtype}$. It is clear that
$\ID \subseteq {\subtype}$ where $\ID = \set{(A, A)}$. Hence ${\R}
\subseteq {\subtype}$.\qed
%\end{proof}


\begin{lemma}[Structural congruence]
\label{le:subtype-structure} \
\begin{enumerate}
\item $A{|}\textbf{0} \eqtype A$
\item $A{|}B \eqtype B{|}A$
\item $A{|}(B{|}C) \eqtype (A{|}B){|}C$
\item $A{\TOR}B \eqtype B{\TOR}A$
\item $A{\TOR}(B{\TOR}C) \eqtype (A{\TOR}B){\TOR}C$
\item ${*}A \eqtype A | {*}A$
\item $(\nu x)(A|B) \eqtype (\nu x)A\,|\,B$ if $x\notin\FV(B)$
\item $(\nu x)(A{\TOR}B) \eqtype (\nu x)A\,{\TOR}\,B$ if $x\notin\FV(B)$
\item $\subst{\alpha}{\mu\alpha.A} \eqtype \mu\alpha.A$
\end{enumerate}
\end{lemma}
\proof %\begin{proof} 
These proofs are all standard.\qed
%\end{proof}

\begin{lemma}[Substitution]
\label{le:subtype-substitution} \
\begin{enumerate}
\item $\csubst{y}{x}\textbf{0} \eqtype \textbf{0}$
\item $\csubst{y}{x}(a.A) \eqtype (\subst{y}{x}a).\csubst{y}{x}A$
\item $\csubst{y}{x}(z^\acclab.A) \eqtype (\subst{y}{x}z)^\acclab.\csubst{y}{x}A$
\item \label{le:subtype-substitution:par} $\csubst{y}{x}(A|B) \eqtype \csubst{y}{x}A\ |\ \csubst{y}{x}B$
\item $\csubst{y}{x}(A{\TOR}B) \eqtype \csubst{y}{x}A\ \TOR\ \csubst{y}{x}B$
\item $\csubst{y}{x}({*}A) \eqtype *(\csubst{y}{x}A)$
\item $\csubst{y}{x}\csubst{a}{b}A \eqtype
\csubst{a}{\subst{y}{x}b}\csubst{y}{x}A$ if $\acctarget{a}{\cap}\{x,y\}{=}\emptyset$
\item $\csubst{y}{x}(\nu z)A \eqtype (\nu z)(\csubst{y}{x}A)$ if $\{z\}{\cap}\{x,y\}{=}\emptyset$
\item \label{le:subtype-substitution:exclude1}
   $\csubst{y}{x}(\exclude{A}{S}) \eqtype \exclude{(\csubst{y}{x}A)}{S}$, and \\
   $\csubst{y}{x}(\project{A}{S}) \eqtype \project{A}{S}$, \\
   if $S{\cap}\{x,y\}{=}\emptyset$
\item \label{le:subtype-substitution:exclude2}
  $\csubst{y}{x}(\exclude{A}{S}) \eqtype \exclude{A}{S}$, and \\
  $\csubst{y}{x}(\project{A}{S}) \eqtype \project{(\csubst{y}{x}A)}{S}$, \\
  if $\{y\}\subseteq S$
\end{enumerate}
\end{lemma}
\proof %\begin{proof} Most parts are straightforward, although \textbf{Part~\ref{le:subtype-substitution:par}} is non-obvious in
the case of labels $\{x,\overline{y}\}$. For
Part~\ref{le:subtype-substitution:par}, we construct a relation
$\mathcal{S} = \{ ( \csubst{y}{x}(A|B), \csubst{y}{x}A |
\csubst{y}{x}B) \}$ and prove $\mathcal{S}$ and $\mathcal{S}^{-1}$ are simulations.
The interesting case is when we infer
\[ \csubst{y}{x}A | \csubst{y}{x}B \stackrel{\tau}{\rightarrow}
\csubst{y}{x}A' | \csubst{y}{x}B' \] from
\[ A \stackrel{z_1}{\rightarrow} A' \qquad
   B \stackrel{\overline{z_2}}{\rightarrow} B' \qquad
   \subst{y}{x}z_1 = \subst{y}{x}z_2.
\]
This gives
 \[ A|B \stackrel{\{z_1,\overline{z_2}\}}{\rightarrow} A'|B'. \]
Hence
 \[ \csubst{y}{x}(A|B) \stackrel{\{\subst{y}{x}z_1,\subst{y}{x}\overline{z_2}\}}{\longrightarrow} \csubst{y}{x}(A'|B'). \]
And hence as required
 \[ \csubst{y}{x}(A|B) \stackrel{\tau}{\rightarrow} \csubst{y}{x}(A'|B'). \]

\textbf{Part~\ref{le:subtype-substitution:exclude1}.} Here we
construct $\mathcal{S} = \{ (\,\csubst{\xx}{\yy}(\exclude{A}{S}),\
\exclude{(\csubst{\xx}{\yy}A)}{S}\,) \}$ where $S$ does not clash
with $\{\xx,\yy\}$, and we prove that $\mathcal{S}$ and $\mathcal{S}^{-1}$
are simulations. We focus on two cases.
\begin{enumerate}
\item Suppose $\exclude{(\csubst{\xx}{\yy}A)}{S}
\stackrel{\subst{\xx}{\yy}l}{\longrightarrow}
\exclude{(\csubst{\xx}{\yy}A')}{S}$ is inferred from $A
\stackrel{l}{\rightarrow} A'$ and $\acctarget{\subst{\xx}{\yy}l}
{\cap}S=\emptyset$. We must infer that $\csubst{\xx}{\yy}(\exclude{A}{S})
\stackrel{\subst{\xx}{\yy}l}{\longrightarrow}
\csubst{\xx}{\yy}(\exclude{A'}{S})$. This requires $\acctarget{l}
{\cap}S=\emptyset$, which we prove as follows. It is assumed that
$S$ does not clash, so $\{\xx,\yy\}{\cap}S = \emptyset$. We also
have $\acctarget{\subst{\xx}{\yy}l} {\cap}S=\emptyset$, and so
$\subst{\xx}{\yy}(\acctarget{l}){\cap}S=\emptyset$. Let $T =
\acctarget{l}$. Suppose $z\in T$. Then either $z\in\xx$ so $z\notin
S$, or $z\in\yy$ so $z\notin S$, or $z\notin\{\xx,\yy\}$ so
$z\in\subst{\xx}{\yy}T$ so $z\notin S$. In all cases $z\notin S$, so
$T{\cap}S = \emptyset$ as required.
%
\item Suppose $\exclude{(\csubst{\xx}{\yy}A)}{S}
\stackrel{\tau}{\rightarrow} \exclude{(\csubst{\xx}{\yy}A')}{S}$ is
inferred from $A \stackrel{l}{\rightarrow} A'$ and
$\acctarget{\subst{\xx}{\yy}l} \subseteq S$. We must infer
$\csubst{\xx}{\yy}(\exclude{A}{S}) \stackrel{\tau}{\rightarrow}
\csubst{\xx}{\yy}(\exclude{A'}{S})$. This requires $\acctarget{l}
\subseteq S$, which we prove as follows. Once again let $T =
\acctarget{l}$. We have $\{\xx,\yy\}{\cap}S = \emptyset$ and
$\subst{\xx}{\yy}T \subseteq S$. Suppose $z\in T$. Then
$\subst{\xx}{\yy}z \in \subst{\xx}{\yy}T$, and $\subst{\xx}{\yy}z
\in S$. Either $z\in\xx$ so $y\in S$, which is a contradiction. Or
$z\in\yy$ so $y\in S$, which is a contradiction. Or
$z\notin\{\xx,\yy\}$ so $z\in S$. Hence $T \subseteq S$ as required.\qed
\end{enumerate}
%\end{proof}

\begin{lemma}[Exclusion and Projection] \
\label{le:subtype-exclusion}
\setbox0=\hbox{$\exclude{(A{\TOR}B)}{S} {\eqtype} \exclude{A}{S} {\TOR} \exclude{B}{S}$}\newlength{\excolwidth}\setlength{\excolwidth}{\wd0}
\begin{enumerate}
\item \makebox[\excolwidth][l]{$\exclude{\textbf{0}}{S} {\eqtype} \textbf{0}$}
      \makebox[\excolwidth][l]{$\project{\textbf{0}}{S} {\eqtype} \textbf{0}$}
\item \makebox[\excolwidth][l]{$\exclude{(a_t.A)}{S} {\eqtype} a_t.(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{(a_t.A)}{S} {\eqtype} \tau_t.(\project{A}{S})$}
      \makebox[0pt][l]{if $\acctarget{a}{\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{(a_t.A)}{S} {\eqtype} \tau_t.\exclude{A}{S}$}
      \makebox[\excolwidth][l]{$\project{(a_t.A)}{S} {\eqtype} a_t.\project{A}{S}$}
      \makebox[0pt][l]{if $\acctarget{a}{\subseteq}S$}
\item \makebox[\excolwidth][l]{$\exclude{(z^\xi.A)}{S} {\eqtype} z^\xi.(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{(z^\xi.A)}{S} {\eqtype} \tau_c.\project{A}{S}$}
      \makebox[0pt][l]{if $\acctarget{z^\xi}{\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{(z^\xi.A)}{S} {\eqtype} \tau_c.\exclude{A}{S}$}
      \makebox[\excolwidth][l]{$\project{(z^\xi.A)}{S} {\eqtype} z^\xi.(\project{A}{S})$}
      \makebox[0pt][l]{if $\acctarget{z^\xi}{\subseteq}S$}
\item \makebox[\excolwidth][l]{$\exclude{(A|B)}{S} {\eqtype} \exclude{A}{S}\ |\ \exclude{B}{S}$}
      \makebox[\excolwidth][l]{$\project{(A|B)}{S} {\eqtype} \project{A}{S}\ |\ \project{B}{S}$}
      \label{le:subtype-exclusion:par}
\item \makebox[\excolwidth][l]{$\exclude{(A{\TOR}B)}{S} {\eqtype} \exclude{A}{S} {\TOR} \exclude{B}{S}$}
      \makebox[\excolwidth][l]{$\project{(A{\TOR}B)}{S} {\eqtype} \project{A}{S} {\TOR} \project{B}{S}$}
\item \makebox[\excolwidth][l]{$\exclude{({*}A)}{S} {\eqtype} {*}(\exclude{A}{S})$}
      \makebox[\excolwidth][l]{$\project{({*}A)}{S} {\eqtype} {*}(\project{A}{S})$}
\item \makebox[\excolwidth][l]{$\exclude{(\exclude{A}{S})}{T} {\eqtype} \exclude{A}{S\cup T}$}
%      \makebox[\excolwidth][l]{$\project{(\project{A}{S})}{T} {\eqtype} \project{A}{S\cup T}$}
  \todo{Fixed. --Kohei}
      \makebox[\excolwidth][l]{$\project{(\project{A}{S})}{T} {\eqtype} \project{A}{S\cap T}$}
\item \makebox[\excolwidth][l]{$\exclude{A}{S} {\eqtype} A$}
      \makebox[\excolwidth][l]{$\project{A}{S} {\eqtype} \textbf{0}$}
      \makebox[0pt][l]{if $\FV(A){\cap}S{=}\emptyset$}
\item \makebox[\excolwidth][l]{$\exclude{A}{S} {\eqtype} \textbf{0}$}
      \makebox[\excolwidth][l]{$\project{A}{S} {\eqtype} A$}
      \makebox[0pt][l]{if $\FV(A){\subseteq}S$}
      \label{le:subtype-exclusion:nil}
\end{enumerate}
\end{lemma}
\proof %\begin{proof}
 Straightforward.\qed
%\end{proof}

\begin{lemma}[Simulation] \
\label{le:subtype-simulation}
\begin{enumerate}
\item \label{le:subtype-simulation:traces} If $A_1 \subtype A_2$ then $\traces{x}{A_1} \supseteq
\traces{x}{A_2}$ for any $x$.
\item \label{le:subtype-simulation:sequence} If $A \stackrel{\{x,\overline{y}\}}{\longrightarrow} A'$ then
$A \stackrel{x}{\rightarrow}\stackrel{\overline{y}}{\rightarrow}
A'$.
\item $A{\TOR}B \subtype A$
\item $A \subtype \textbf{0}$
\item $A \subtype A{\TOR}A$
\item \label{le:subtype-simulation:separate} $\exclude{A}{S} \mathrel{|}
\project{A}{S} \subtype A$
\item \label{le:subtype-simulation:rec} If $B \subtype \subst{\alpha}{B}A$ then $B \subtype \mu\alpha.A$
\item $A \subtype B_1{\TOR}B_2$ if and only if $A\subtype B_1$ and $A \subtype B_2$
\end{enumerate}
\end{lemma}
\proof %\begin{proof} These proofs are largely standard.

\textbf{Part~\ref{le:subtype-simulation:traces}} follows immediately from the
definitions of subtyping and traces.
%Let \(\accseq\) ba a sequence of access labels. Suppose that
%\(\accseq\in \traces{x}{A_2}\). We show \(\accseq \in
%\traces{x}{A_1}\) by induction on the length of \(\accseq\).
%\begin{itemize}
%\item Case \(\accseq = \emptyuselab\):
%It must be the case that there exists \(A_2'\) such that \(A_2
%\Tredswith{\Tredlabsilent} A_2'\). From \(A_1 \subtype A_2\), there
%exists \(A_1'\) such that \(A_1 \Tredswith{\Tredlabsilent}\TSPCONG
%A_1'\). Thus, \(\emptyuselab \in A_1\).
%\item Case \(\accseq = \acclab \cdot \accseq_1\):
%It must be the case that there exists \(A_2'\) such that \(A_2
%\Tredswith{\acclab} A_2'\) and \(\accseq_1 \in \traces{x}{A_2'}\).
%From \(A_1 \subtype A_2\), there exists \(A_1'\) such that \(A_1
%\Tredswith{\acclab} A_1'\) and \(A_1' \subtype A_2'\). From the
%induction hypothesis, we have \(\accseq_1 \in \traces{x}{A_1'}\).
%Thus, \(\accseq \in \traces{x}{A_1}\).
%\end{itemize}

\textbf{Part~\ref{le:subtype-simulation:separate}.} We construct
$\mathcal{S} = \{ (\project{A}{S}|\exclude{A}{S},B) \ |\ A \subtype
B \}$ and prove it is a simulation. In other words, assuming $B
\stackrel{l}{\rightarrow} B'$, we must show $\exclude{A}{S} |
\project{A}{S} \stackrel{l}{\Rightarrow} A'$ with $(A',B') \in
\mathcal{S}$. This is easy when $l{\cap}S = \emptyset$, and also
when $l{\subseteq}S$; the interesting case is when $B
\stackrel{\{x,\overline{y}\}}{\rightarrow} B'$ for $x{\in}S,\,
y{\notin}S$. By Part~\ref{le:subtype-simulation:sequence} and
assumption $A{\subtype}B$ we get $A \stackrel{x}{\Rightarrow} A_1
\stackrel{\overline{y}}{\Rightarrow} A' \subtype B'$. Hence
\[\begin{array}{c}
 \exclude{A}{S} \stackrel{\tau}{\Rightarrow} \exclude{A_1}{S}
 \stackrel{\overline{y}}{\Rightarrow} \exclude{A'}{S} \\
 \project{A}{S} \stackrel{x}{\Rightarrow} \project{A_1}{S}
 \stackrel{\tau}{\Rightarrow} \project{A'}{S}
\end{array}\]
Putting them in parallel, we get as required
\[ \exclude{A}{S} | \project{A}{S}
\stackrel{\{x,\overline{y}\}}{\Rightarrow} \exclude{A'}{S} |
\project{A'}{S}. \]

\textbf{Part~\ref{le:subtype-simulation:rec}.} 
\todo{Done for representative cases, but I'm not sure the following proof is correct --Kohei.}
Let \(\R\) be
\({\subtype} \cup \set{(\Tsubst{A'}{\Tbvar}{B},
\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A})}\). We will prove that \(\R\)
is a simulation up to \(\subtype\) if \(B \subtype
\Tsubst{A}{\Tbvar}{B}\). Then, we have \(\R \subseteq {\subtype}\),
so that \(B \subtype \Trec{\Tbvar}A\) from
Lemma~\ref{le:subtype-precongruent}.\ref{le:relation:upto}.

Suppose that \(\Tsubst{A'}{\Tbvar}{B} \mathrel{\R}
\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A}\) and
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\). 
We will show that there exists \(B'\) such that \(\Tsubst{A'}{\Tbvar}{B}
\Tredswith{l} B'\) and \(B' \mathrel{{\subtype}{\R}{\subtype}} A''\)
by induction on the derivation of
\(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\).
%% We show that \(\R\) is a simulation up to \(\subtype\), so that \(\R \subseteq \subtype\),
%% by induction on the derivation of \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}A} \Tredwith{l} A''\).
%% In the following cases, we show that there exists \(B'\) such that
%% \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{l} B'\) and \(B' \subtype \R \subtype A''\).
\begin{itemize}
\item Case \rname{TR-In}:
It must be the case that
\begin{itemize}
\item \(A' = \Tin{x}A_1\)
\item \(A'' = \Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}\)
\item \(l = x\)
\end{itemize}
for some \(A_1\) and \(x\). Thus, \(\Tsubst{A'}{\Tbvar}{B}
\Tredwith{x} \Tsubst{A_1}{\Tbvar}{B}\). From the definition of
\(\R\), we have \(\Tsubst{A_1}{\Tbvar}{B} \R A''\).

\item Case \rname{TR-Par}:
It must be the case that
\begin{itemize}
\item \(A' = A_1 \TPAR A_2\)
\item \(A'' = \Tsubst{(A_1' \TPAR A_2)}{\Tbvar}{\Trec{\Tbvar}A}\)
\item \(A_1 \Tredwith{l} A_1'\)
\end{itemize}
for some \(A_1\) and \(A_1'\) and \(A_2\). Thus,
\(\Tsubst{A'}{\Tbvar}{B} \Tredwith{x} \Tsubst{(A_1' \TPAR
A_2)}{\Tbvar}{B}\). From the definition of \(\R\), we have
\(\Tsubst{(A_1' \TPAR A_2)}{\Tbvar}{B} \R A''\).

\item Case \rname{TR-Par2}:
It must be the case that
\begin{itemize}
\item \(l = \actcom{x}{\actout{y}}\)
\item \(A' = A_1 \TPAR A_2\)
\item \(A_1 \Tredwith{x} A_1'\)
\item \(A_2 \Tredwith{\actout{y}} A_2'\)
\item \(A'' = \Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{\Trec{\Tbvar}A}\)
\end{itemize}
for some \(A_1\) and \(A_2\) an d\(A_1'\) and \(A_2'\) and \(x\) and \(y\). 
Thus, \(\Tsubst{A'}{\Tbvar}{B} \Tredwith{\actcom{x}{\actout{y}}} \Tsubst{(A_1' \TPAR
A_2)}{\Tbvar}{B}\). From the definition of \(\R\), we have
\(\Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{B} \R A''\).

\item Case \rname{TR-Com}:
%% It must be the case that
%% \begin{itemize}
%% \item \(A' = A_1 \TPAR A_2\)
%% \item \(A'' = \Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{\Trec{\Tbvar}A}\)
%% \item \(A_1 \Tredwith{a} A_1'\)
%% \item \(A_2 \Tredwith{\Toutatom{a}} A_2'\)
%% \end{itemize}
%% for some \(A_1\) and \(A_1'\) and \(A_2\) and \(A_2'\) and \(a\).
%% Thus, \(\Tsubst{A'}{\Tbvar}{B} \Tredsilent \Tsubst{(A_1' \TPAR
%% A_2')}{\Tbvar}{B}\). From the definition of \(\R\), we have
%% \(\Tsubst{(A_1' \TPAR A_2')}{\Tbvar}{B} \R A''\).
It must be the case that
\begin{itemize}
\item \(\act = \Tredlabsilent\)
\item \(\Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{\actcom{x}{\actout{x}}} A''\)
\end{itemize}
for some \(x\).
From the induction hypothesis,
we have \(\Tsubst{A'}{\Tbvar}{B} \subtype \Tsubst{A'}{\Tbvar}{\Trec{\Tbvar}{A}}\),
so that \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{\actcom{x}{\actout{x}}} B'\)
and \(B' \subtype A''\) for some \(B'\).

\item Case \rname{TR-Rec}:
\begin{itemize}
\item Case \(A' = \Trec{\beta}A_1\): 
We can assume that \(\beta\) does not freely occur in \(A\) and \(B\).
It must be the case that
\begin{itemize}
\item \(A' = \Trec{\beta}A_1\)
\item \(\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}} \Tredwith{l} A''\)
\end{itemize}
for some \(A_1\).
\(\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}\) is
syntactically equal to \(\Tsubst{\Tsubst{A_1}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}}{\Tbvar}{\Trec{\Tbvar}{A}}\)
From the induction hypothesis, we have \(\Tsubst{A_1}{\Tbvar}{B} \subtype \Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}{A}}\),
so that \(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}}\) \(\subtype\)
\(\Tsubst{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{\Trec{\Tbvar}A}}}\).
Thus, there exists \(B'\) such that 
\(\Tsubst{\Tsubst{A_1}{\Tbvar}{B}}{\beta}{\Trec{\beta}{\Tsubst{A_1}{\Tbvar}{B}}} \Tredswith{l} B'\), so that \(\Tsubst{A'}{\Tbvar}{B} \Tredswith{l} B'\),
and \(B' \subtype A''\).

\item Case \(A' = \Tbvar\):
It must be the case that
\begin{itemize}
\item \(A' = \Tbvar\)
\item \(\Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{l} A''\)
\end{itemize}
From the induction hypothesis, we have
\(\Tsubst{A}{\Tbvar}{B} \subtype \Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}}\),
so that there exists \(B'\) such that
\(\Tsubst{A}{\Tbvar}{B} \Tredswith{l} B'\) and
\(B' \subtype A''\).\qed
\end{itemize}


\end{itemize}
%\end{proof}

\begin{lemma}[Judgement substitution] \
\label{le:judgement-substitution}
\begin{enumerate}
\item \label{le:judgement-substitution:substval}
\textit{(For values)} If $\Gamma,\xx\COL\seq{\tau} \p y \COL \sigma$
and $\Gamma \p \vv\COL\seq{\tau}$ then $\Gamma \p \subst{\xx}{\vv}y
\COL \sigma$.
\item \label{le:judgement-substitution:substproc} \textit{(For processes)} If
$\tjudge{\Gamma, \xx\COL\seq{\tau}}{P}{A}$ and $\Gamma \p
\vv\COL\seq{\tau}$ then
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
\end{enumerate}
\end{lemma}
\proof %\begin{proof}
\textbf{Part~\ref{le:judgement-substitution:substval}.} Either
$y=x_i$ for some $i$, in which case $y\COL \tau_i$ is already in
$\Gamma$. Or $y\notin\xx$, in which case $\subst{\xx}{\vv}y = y$ and
$y\COL \sigma$ is in $\Gamma$. We remark that types $\sigma$ never
have free names.

\textbf{Part~\ref{le:judgement-substitution:substproc}.} By
induction on the derivation of $\tjudge{\Gamma}{P}{A}$. Most cases
follow straightforwardly on Lemma~\ref{le:subtype-substitution}. We
consider four particular cases.
\begin{enumerate}
\item Case \rname{T-Sub}, where $\tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A}$ is inferred
from
\[\begin{array}{c}
  \tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A'} \qquad A \subtype A'
\end{array}\]
From the induction hypothesis,
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A'}$. By
Lemma~\ref{le:subtype-precongruent}.\ref{le:subtype-precongruent:subst}
and assumption $A \subtype A'$ we get $\csubst{\xx}{\vv}A \subtype
\csubst{\xx}{\vv}A'$, and hence as required
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
%
\item Case \rname{T-NewR}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\nurexp{z}{\spec}P}{\exclude{A}{\{z\}}}$
is inferred from
\[\begin{array}{c}
  \tjudge{\Gamma,\xx\COL\seq{\tau},z\COL\Tres}{P}{A} \qquad
  \traces{z}{A} \subseteq \spec
\end{array}\]
Assume by alpha-renaming that $z$ does not clash with $\xx$ or $\vv$. From
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude2}
we get $\project{A}{\{z\}} \eqtype \project{(\csubst{\xx}{\yy}A)}{\{z\}}$,
giving $\traces{z}{A} = \traces{z}{\csubst{\xx}{\yy}A}$ and hence
$\traces{z}{\csubst{\xx}{\yy}A} \subseteq \spec$. By the induction
hypothesis,
$\tjudge{\Gamma,z\COL\Tres}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A}$.
These two together give
 \[ \tjudge{\Gamma}{\nurexp{z}{\spec}\subst{\xx}{\vv}P}{\exclude{(\csubst{\xx}{\vv}A)}{\{z\}}}. \]
For the process $\nurexp{z}{\spec}\subst{\xx}{\vv}P$, we can push
the substitution out by definition of the substitution operator and
because $z$ is fresh. For the behavior
$\exclude{(\csubst{\xx}{\vv}A)}{\{z\}}$ we use
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude1}
to push it out. Hence as required,
 \[ \tjudge{\Gamma}{\subst{\xx}{\vv}\nurexp{z}{\spec}P}{\csubst{\xx}{\vv}(\exclude{A}{\{z\}})}. \]
%
\item Case \rname{T-Out}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\outexp{z}{w}{}P}{\Tout{z}(\csubst{\yy}{\seq{w}}A_1
| A_2)}$ is inferred from
\[\begin{array}{c}
 \tjudge{\Gamma,\xx\COL\seq{\tau}}{P}{A_2} \qquad
 \Gamma,\xx\COL\seq{\tau} \p \seq{w}\COL\seq{\sigma} \\
 \Gamma,\xx\COL\seq{\tau} \p z\COL\Tchan{(\yy:\seq{\sigma})A_1}
\end{array}\]
Part~\ref{le:judgement-substitution:substval} implies $\Gamma \p
\subst{\xx}{\vv}w \COL \seq{\sigma}$ and $\Gamma \p
\subst{\xx}{\vv}z \COL \Tchan{(\yy:\seq{\sigma})A_1}$. From the
induction hypothesis, we get
$\tjudge{\Gamma}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A_2}$. These
three give
 \[
 \tjudge{\Gamma}{\outexp{\subst{\xx}{\vv}z}{\subst{\xx}{\vv}\seq{w}}{}\subst{\xx}{\vv}P}{\Tout{\subst{\xx}{\vv}z}(\csubst{\yy}{\subst{\xx}{\vv}\seq{w}}A_1 | \csubst{\xx}{\vv}A_2)}
 \]
For the process we push the substitution out by definition of the
substitution operator. For the behavior we push it out using several
parts of Lemma~\ref{le:subtype-substitution}.
%
\item Case \rname{T-In}, where
$\tjudge{\Gamma,\xx\COL\seq{\tau}}{\inexp{z}{\yy}{}P}{\Tin{z}(\exclude{A_2}{\{\yy\}})}$
is inferred from
\[\begin{array}{c}
 \tjudge{\Gamma,\yy\COL\seq{\sigma},\xx\COL\seq{\tau}}{P}{A_2}
 \qquad
 \Gamma,\xx\COL\seq{\tau} \p z\COL\Tchan{(\yy:\seq{\sigma})A_1} \\
 A_1 \subtype \project{A_2}{\{\yy\}}
\end{array}\]
We use three deductions. First from
Part~\ref{le:judgement-substitution:substval} we get $\Gamma\p\subst{\xx}{\vv}z \COL\Tchan{(\yy:\seq{\sigma})A_1}$. Second, from
assumption $A_1 \subtype \project{A_2}{\{\yy\}}$ and
Lemma~\ref{le:subtype-precongruent}.\ref{le:subtype-precongruent:subst}
we get $\csubst{\xx}{\vv}A_1 \subtype
\csubst{\xx}{\vv}(\project{A_2}{\{\yy\}}$. The substitution on the left
disappears because $\FV(A_1)\subseteq\{\yy\}$ and we can assume by
alpha-renaming that $\yy$ does not clash with $\{\xx,\vv\}$. The substitution on the
right can be pushed inside by
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude1}.
These together give $A_1 \subtype
\project{(\csubst{\xx}{\vv}A_2)}{\{\yy\}}$. And third, from the induction
hypothesis we get
$\tjudge{\Gamma,\yy\COL\seq{\sigma}}{\subst{\xx}{\vv}P}{\csubst{\xx}{\vv}A_2}$.
These three give
 \[
 \tjudge{\Gamma}{\inexp{\subst{\xx}{\vv}z}{\yy}{}\subst{\xx}{\vv}P}{\Tin{\subst{\xx}{\vv}z}(\exclude{(\csubst{\xx}{\vv}A_2)}{\{\yy\}})}
 \]
A in the previous case we push the substitution out in the process
and the behavior to get, as required,
 \[\hbox to30 pt{\hfil}
 \tjudge{\Gamma}{\subst{\xx}{\vv}(\inexp{z}{\yy}{}P)}{\csubst{\xx}{\vv}(\Tin{z}(\exclude{A_2}{\{\yy\}}))}.
 \hbox to30 pt{\hfil}\qEd\]
\end{enumerate}
%\end{proof}


\begin{lemma}[Subject-reduction] \
\label{le:subject-reduction}
\begin{enumerate}
\item \label{le:subject-reduction:weakening} If
\textit{(Weakening)} If $\tjudge{\Gamma}{P}{A}$ and $x\notin\FV(P)$
and $x$ not in $\Gamma$ or $A$ then $\tjudge{\Gamma,\,x\COL
T}{P}{A}$.
\item If $\tjudge{\Gamma}{P}{A}$ and $P \SPCONG Q$ then $\tjudge{\Gamma}{Q}{A}$. \label{le:subject-reduction:SPCONG}
\item \label{le:subject-reduction:subject-reduction} \textit{(Subject-reduction)} If $P \stackrel{L}{\rightarrow} P'$
and $\tjudge{\Gamma}{P}{A}$ then $A \stackrel{L}{\rightarrow} A'$ and $\tjudge{\Gamma}{P'}{A'}$.
\end{enumerate}
\end{lemma}
\proof %\begin{proof}
\textbf{Part~\ref{le:subject-reduction:weakening}} is a
straightforward on the derivation of $\tjudge{\Gamma}{P}{A}$.

\textbf{Part~\ref{le:subject-reduction:SPCONG}.} By induction on the
derivation of $P \SPCONG Q$. Most cases use
Lemma~\ref{le:subtype-structure}. \todo{THREE CASES. NIL and NEW and NUR, which is already here}
The case for $\nuexp{x}P | Q
\preceq \nuexp{x}(P|Q)$ uses
Lemma~\ref{le:subject-reduction}.\ref{le:subject-reduction:weakening}.
The only interesting case is that for $\nurexp{x}{\spec}P|Q \preceq
\nurexp{x}{\spec}(P|Q)$ with $x\notin\FV(Q)$. The judgement
$\tjudge{\Gamma}{\nurexp{x}{\spec}P|Q}{A}$ must have been inferred
from
\[\begin{array}{c}
 \tjudge{\Gamma,x\COL\Tres}{P}{A_3} \qquad
 \traces{x}{A_3}\subseteq \Phi \qquad
 \exclude{A_3}{\{x\}} \newsubtype A_1 \\
 \tjudge{\Gamma}{Q}{A_2} \qquad
 A_1|A_2 \newsubtype A
\end{array}\]
From these we infer
\[ \tjudge{\Gamma, x\COL\Tres}{P|Q}{A_3|A_2}. \]
By alpha-renaming assume $x\notin\FV(A_2)$. By
Lemmas~\ref{le:subtype-exclusion}.\ref{le:subtype-exclusion:par}
and~\ref{le:subtype-exclusion}.\ref{le:subtype-exclusion:nil} we get
$\project{(A_3|A_2)}{\{x\}} \eqtype \project{A_3}{\{x\}} | \project{A_2}{\{x\}}
\eqtype \project{A_3}{\{x\}}$, and then by
Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:traces} we get
$\traces{x}{A_3|A_2}=\traces{x}{A_3}$, and so $\traces{x}{A_3|A_2}
\subseteq \spec$. This gives
\[ \tjudge{\Gamma}{\nurexp{x}{\spec}(P|Q)}{\exclude{(A_3|A_2)}{\{x\}}}. \]
Finally $\exclude{(A_3|A_2)}{\{x\}}
\newsubtype \exclude{A_3}{\{x\}} | A_2 \newsubtype A$. This gives as required
\[ \tjudge{\Gamma}{\nurexp{x}{\spec}(P|Q)}{A}. \]


\textbf{Part~\ref{le:subject-reduction:subject-reduction}.} By
induction on the derivation of $P \red P'$. There are two
interesting cases. That for \rname{R-SP} follows from
Part~\ref{le:subject-reduction:SPCONG}. That for \rname{R-Com} is as
follows. We are given
\[ \tjudge{\Gamma}{\outexp{x}{\seq{v}}{}P \PAR \inexp{x}{\seq{y}}{}Q}{A}. \]
This must have been deduced from
\[\begin{array}{c}
  \tjudge{\Gamma,x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}{P}{A_2} \qquad
  \Gamma \p v_i\COL \mvtype_i \\
  \Tout{x}(\csubst{\yy}{\vv}A_1 \PAR A_2) \newsubtype A_3 \\
  \tjudge{\Gamma,x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_1},\yy\COL\seq{\mvtype}}{Q}{A_4} \\\
  \project{A_4}{\{\yy\}}\newsubtype A_1 \qquad \Tin{x}(\exclude{A_4}{\{\yy\}}) \newsubtype A_5 \qquad
  A_3|A_5 \newsubtype A
\end{array}\]
We must show some $A'$ for which $A \Rightarrow A'$ and
$\tjudge{\Gamma}{P | \subst{\yy}{\vv}Q}{A'}$. We pick some
$A'$ such that $A \Rightarrow A'$ and $A' \subtype \csubst{\yy}{\vv}A_1 | A_2 | \exclude{A_4}{\{\yy\}}$.
The existence of such $A'$ is guaranteed by
$A \Rightarrow A'$ and $A
\subtype \Tout{x}(\csubst{\yy}{\vv}A_1 | A_2) |
\Tin{x}(\exclude{A_4}{\{\yy\}}) \red \csubst{\yy}{\vv}A_1 | A_2 |
\exclude{A_4}{\{\yy\}}$. It remains to prove $\tjudge{\Gamma}{P |
\subst{\yy}{\vv}Q}{A'}$. We start with
\[ \tjudge{\Gamma,\yy\COL\seq{\mvtype}}{Q}{A_4}. \]
By
Lemma~\ref{le:judgement-substitution}.\ref{le:judgement-substitution:substproc},
\[ \tjudge{\Gamma}{\subst{\yy}{\vv}Q}{\csubst{\yy}{\vv}A_4}. \]
Hence
\[ \tjudge{\Gamma}{P | \subst{\yy}{\vv}Q}{A_2 | \csubst{\yy}{\vv}A_4}. \]
Now $\csubst{\yy}{\vv}A_4 | A_2
\newsubtype \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}|\exclude{A_4}{\{\yy\}})
| A_2$ (by
Lemma~\ref{le:subtype-simulation}.\ref{le:subtype-simulation:separate}), \\
$\newsubtype \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}) |
\csubst{\yy}{\vv}(\exclude{A_4}{\{\yy\}}) | A_2$ (by
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:par}), \\
$\newsubtype \csubst{\yy}{\vv}(\project{A_4}{\{\yy\}}) |
\exclude{A_4}{\{\yy\}} | A_2$ (by
Lemma~\ref{le:subtype-substitution}.\ref{le:subtype-substitution:exclude2}), \\
$\newsubtype \csubst{\yy}{\vv}A_1 | \exclude{A_4}{\{\yy\}} | A_2$ (by
assumption $\exclude{A_4}{\{\yy\}} \newsubtype A_1$), \\
$\newsubtype A'$ (by definition of $A'$). 
This gives as required
\[ \tjudge{\Gamma}{P | \subst{\yy}{\vv}Q}{A'}. \]
\todo{MUST LIST ALL THESE CASES. Especially R-Acc, R-NewR1 are important.}

The case for \rname{R-Acc} is as follows.
We are given \(\tjudge{\Gamma}{\accexp{\acclab}{x} P_1}{A}\).
This must have been derived from
\begin{itemize}
\item \(\tjudge{\Gamma}{P_1}{A_1}\)
\item \(\tjudge{\Gamma}{x}{\Tres}\)
\item \(A \subtype \Tacc{\acclab}{x} A_1\).
\end{itemize}
We have to show that
\begin{itemize}
\item \(\tjudge{\Gamma}{P_1}{A'}\)
\item \(A \Tredacc{x}{\acclab} A'\).
\end{itemize}
Let \(A'\) be a behavioral type that satisfies
\(A \Tredsacc{x}{\acclab} A'\) and \(A' \subtype A_1\).
Such \(A'\) is guaranteed to exist by \(A \subtype \Tacc{\acclab}{x} A_1\).
Then, \(\tjudge{\Gamma}{P_1}{A'}\) follows from
\(\tjudge{\Gamma}{P_1}{A_1}\) and \(A' \subtype A_1\) and \rname{T-Sub}.

The case for \rname{R-NewR1} is as follows.
We are given \(\tjudge{\Gamma}{\nurexp{x}{\spec} P_1}{A}\)
This must have been derived from
\begin{itemize}
\item \(\tjudge{\Gamma, x:\Tres}{P_1}{A_1}\)
\item \(\traces{x}{A_1} \subseteq \spec\)
\item \(A \subtype \exclude{A_1}{\set{x}}\).
\end{itemize}
We have to show that there exists \(A'\) such that
\begin{itemize}
\item \(\tjudge{\Gamma}{\nurexp{x}{\diffspec{\spec}{\acclab}}P_1'}{A'}\)
\item \(A \Tredsilent A'\)
\end{itemize}
where \(P_1 \redacc{\acclab}{x} P_1'\).

From the induction hypothesis, there exists \(A_1'\) that satisfies
\(\tjudge{\Gamma,x:\Tres}{P_1'}{A_1'}\) and
\(A_1 \Tredacc{x}{\acclab} A'\).
Let \(A'\) be a behavioral type that satisfies
\(A \Tredsilent A'\) and \(A' \subtype \exclude{A_1'}{\set{x}}\).
Such \(A'\) is guaranteed to exist by \(A \subtype \exclude{A_1}{\set{x}}\) and
\(A_1 \Tredacc{x}{\acclab} A_1'\).
From \(\tjudge{\Gamma,x:\Tres}{P_1'}{A_1'}\) and \(A' \subtype \exclude{A_1'}{\set{x}}\),
we are left to show that \(\traces{x}{A_1'} \subseteq \diffspec{\spec}{\acclab}\),
which follows from Lemma~\ref{le:safety:phiminus}.
\todo{We need Lemma~\ref{le:safety:phiminus} here, so separate this from Lemma~\ref{le:safet}.}\qed
%\end{proof}

\begin{lemma}[Safety] \
\label{le:safety}
\begin{enumerate}
\item \label{le:safety:phiminus} If $A \stackrel{x^\xi}{\rightarrow} A'$ and $\traces{x}{A}
\subseteq \Phi$ then $\Phi^{{-}\xi} \not= \emptyset$ and
$\traces{x}{A'} \subseteq \Phi^{{-}\xi}$.
\item \label{le:safety:structure} If $P$ is safe and $P \preceq P'$ then $P'$ is safe.
\item \label{le:safety:reduction} If $P$ is safe and $\tjudge{\Gamma}{P}{A}$ and $P \rightarrow^* P'$
then $P'$ is safe.
\end{enumerate}
\end{lemma}
\proof %\begin{proof}
\textbf{Part~\ref{le:safety:phiminus}} follows immediately from the
definitions of traces and $\Phi^{{-}\xi}$.

\textbf{Part~\ref{le:safety:structure}.} Straightforward induction
on the derivation of $P \preceq Q$, since in every rule the
occurrences of $\nurexp{x}{\spec}$ are identical in $P$ and $Q$.

\textbf{Part~\ref{le:safety:reduction}.} We focus on just a single
step $P \red P'$.
Lemma~\ref{le:subject-reduction}.\ref{le:subject-reduction:subject-reduction}
means that judgements are preserved by reduction. We must show that
safety is preserved by reduction. This is by induction on the
derivation of reduction $P \red P'$. The only interesting case is
\rname{R-NewR1}, since the other rules do not alter trace-sets
$\spec$. In this case, we are given
\[\begin{array}{c}
 \tjudge{\Gamma}{P}{A} \qquad
 P \stackrel{x^\xi}{\rightarrow} P' \qquad
 P\ {\rm safe} \Rightarrow P'\ {\rm safe} \\
 \nurexp{x}{\spec}P \stackrel{\tau}{\rightarrow}
 \nurexp{x}{\spec^{-\xi}}P' \qquad
 \nurexp{x}{\spec}P \ {\rm safe}
\end{array}\]
and must deduce that $\nurexp{x}{\spec^{-\xi}}P'$ is safe. By
Lemma~\ref{le:subject-reduction}.\ref{le:subject-reduction:subject-reduction},
$A \stackrel{x^\xi}{\rightarrow} A'$ for some
$\tjudge{\Gamma}{P'}{A'}$. By Part~\ref{le:safety:phiminus},
$\nurexp{x}{\spec^{-\xi}}P'$ is safe.
\todo{Or, $\spec^{-\xi}\not=\emptyset$ follows from $\spec^{-\xi} \supseteq \traces{x}{A} \ni \{\emptyseq\}$.}\qed
%\end{proof}



%\begin{lemma}[Canonical Form]
%\label{le:canonical}
%If \(\Gamma \p v : \Tchan{(\seq{y}:\seq{\tau})A}\),
%then there exists \(x \in \dom(\Gamma)\) such that \(v = x\).%
%\end{lemma}
%
%\begin{lemma}
%\label{le:trace-substitution}
%\(\traces{x}{A} = \traces{\subst{\seq{y}}{\seq{z}}x}{\subst{\seq{y}}{\seq{z}}A}\).
%\end{lemma}


==> Proofs.tex <==
\section{Proofs of Theorems}
\label{sec:proofs}
\input{Proof-of-Sec3}

\input{Proof-of-Sec4}


==> Reconstruction.tex <==
\sect{Type Checking/Reconstruction}
\label{sec:reconstruct}

By using Theorem~\ref{thm:normal-derivation}, we can also formalize a
common part of type-check/reconstruction algorithms: By reading the
typing rules in a bottom-up manner, we can develop an algorithm that
inputs a process expression and outputs a process type with a set of
subtype constraints and consistency conditions on the type.  The pair
of a process type and a set of constraints is principal in the sense
that a process is typeable if and only if the set of constraints
output by the algorithm is satisfiable.  Indeed, the algorithm
presented here is essentially the same as the first half of an
existing type reconstruction algorithm~\cite{Kobayashi00CONCUR}.

To complete a type-check/reconstruction algorithm, it will be only
required to develop an algorithm to solve constraints on process
types.  Since the definitions of a subtype relation and a consistency
condition vary, such algorithms have to be developed for each
instance.  Some of them, which have prototype implementations, can be
found in the literature~\cite{Igarashi99IC,Kobayashi00CONCUR}.

In this section, we mainly discuss the common part: the definition of
principal typings and an algorithm to compute them.

\iffull
\subsect{Principal Typings}

We first define the notion of principal typings in our type system.  A
principal typing is defined as a pair of a process type including
\emph{process type variables} and a set of constraints on the process
type variables; all the possible process types, under which the
process expression is well typed, are obtained from the process type
in the pair, by replacing process type variables in the constraint so
that the constraint is satisfied.

To define principal typings, we introduce a countably infinite set of
process type variables, ranged over by \(\rho\), and extend the
definition of process types with the process type variables and the
expressions \(\project{\Gamma}{\set{x_1,\ldots,x_n}}\) and
\(\exclude{\Gamma}{\set{x_1,\ldots,x_n}}\).

\begin{defn}[extended process type]
  The set of process types is extended as follows.
\[
\Gamma ::= \cdots \mid \TEvar \mid
  \project{\Gamma}{\set{x_1,\ldots,x_n}} \mid
  \exclude{\Gamma}{\set{x_1,\ldots,x_n}} 
\]
\end{defn}

The metavariable \(C\) denotes a set of constraints of the form 
\(\Gamma_1 \subTE \Gamma_2\),
\(\FV(\Gamma) \cap \set{\seq x} = \emptyset\) or \(\reliable(\Gamma)\).

\begin{notation}
  We write \(\theta\) for a substitution of (non-extended) process
  types and tuple types for process type variables and tuple type
  variables, respectively.  We write \(\FTV(\Gamma)\) and \(\FTV(C)\)
  for the sets of (process and tuple) type variables appearing free in
  \(\Gamma\) and \(C\), respectively.
\end{notation}

Then, principal typings are defined as follows.

\begin{defn}[principal typing]
A pair \((\Gamma, C)\) of an extended process type and a set of 
constraints is a {\em principal typing\/} of a process \(P\) if it
satisfies the following conditions:
\begin{enumerate}
\item If \(\theta\) is chosen so that
 \(\dom(\theta) \supseteq \FTV(\Gamma) \cup \FTV(C)\) and 
\(\theta C\) is satisfied, then \(\theta\Gamma \p P\).
\item If \(\Gamma' \p P\), then there exists a substitution \(\theta\) such
that \(\theta C\) and \(\Gamma' \subTE \theta\Gamma\) hold.
\end{enumerate}
\end{defn}

\subsect{Algorithm to Compute Principal Typings}

% \begin{figure}[htbp]
% \fbox{%
% \begin{minipage}{0.97\textwidth}
% \leavevmode
% \infax[ST-Zero]{
%   \zeroTE \p \zeroexp
% }
% \infrule[ST-Par]{
%   \Gamma_1   \p P_1 \andalso 
%   \Gamma_2   \p P_2
% }{
%   \Gamma_1\TEPAR{}\Gamma_2 \p P_1\PAR P_2
% }
% \infrule[ST-Rep]{
%   \Gamma   \p P
% }{
%   \TEREP{\Gamma}   \p \repexp{P}
% }
% \infrule[ST-Choice]{
%   \Gamma_i   \p P_i \mbox{ for each $i\in \{1,\ldots,n\}$}
% }{
%   \Gamma_1+\cdots+\Gamma_n   \p P_1+\cdots+P_n
% }
% \infrule[ST-Out]{
%   \Gamma_1   \p P  \andalso
%   \Gamma'_1 \subTE \Gamma_1
% }{
%   \OutTE{x}{\typ{\seq y}{\Gamma_2}}{\ev}
%        {(\Gamma'_1\TEPAR \subst{\seq y}{\seq z}\Gamma_2)}
%            \p \outexp{x}{\seq z}{\ev}P
% }
% \infrule[ST-In]{
%   \Gamma \p P \andalso \Gamma_1 \TEPAR \Gamma_2 \subTE \Gamma
%     \andalso \FV(\Gamma_2)\cap \set{\seq y} = \emptyset
% }{
%   \InTE{x}{\typ{\seq y}\Gamma_1}{\ev}\Gamma_2
%          \p \inexp{x}{\seq y}{\ev}P
% }
% \infrule[ST-New]{
%   \Gamma  \p P \andalso
%   \reliable(\project{\Gamma}{\set{\seq x}}) \andalso
%   \FV(\exclude{\Gamma}{\set{\seq x}})\cap\set{\seq x} =\emptyset 
% }{
%   \exclude{\Gamma}{\set{\seq x}}  \p \nuexp{\seq x}P
% }
%   \end{minipage}
% }
%   \caption{Syntax-directed Typing Rules}
%   \label{fig:SDtypingrules}
% \end{figure}

Thanks to Theorem~\ref{thm:normal-derivation}, it is easy to derive
syntax-directed typing rules,
%, shown in Figure~\ref{fig:SDtypingrules},
by combining \rn{T-Sub} with \rn{T-Out} and \rn{T-In} from the
original ones.  Then, by reading the syntax-directed typing rules in a
bottom-up manner, we can obtain a principal typing algorithm, which
takes a process expression as an input and outputs its principal
typing.  The algorithm \(PT\) is shown in Figure~\ref{fig:PT}.

\begin{figure}
  \centering
\fbox{
  \begin{minipage}{0.97\textwidth}
\begin{tabbing}
\( PT(P) = (\Gamma, C): \) \\
\\ \hspace*{3em} \= 
\( PT(\zeroexp) = (\emptyset, \emptyset) \) \\ \\ \>
\( PT(P_1 \PAR P_2) = \) \\ \> \quad \= 
\( \PLET \) \= \((\Gamma_1, C_1) = PT(P_1)\) \\ \> \> \>
\(             (\Gamma_2, C_2) = PT(P_2) \) \\ \> \>
\(    \PIN (\Gamma_1 \TEPAR \Gamma_2, C_1 \cup C_2) \) \\ \\ \>
\( PT(\repexp P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = PT(P_0) \) \\ \> \>
\(    \PIN (\TEREP \Gamma_0, C_0) \) \\ \\ \>
\( PT(P_1+\cdots+P_n) = \) \\ \> \>
\(    \PLET\) \= \((\Gamma_1, C_1) = PT(P_1) \) \\ \> \> \>
\(                      \qquad \vdots \) \\ \> \> \>
\(          (\Gamma_n, C_n) = PT(P_n) \) \\ \> \>
\(    \PIN (\Gamma_1+\cdots+\Gamma_n, C_1 \cup \cdots \cup C_n) \) \\ \\ \>
\( PT(\outexp{x}{\tilde z}{\ev}P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = PT(P_0) \) \\ \> \>
\(    \PIN (\outty{x}{\tv}{\ev}{n}
            (\rho \TEPAR \appty{\tupty{\tv}{n}}{\seq z}),
          C_0 \cup \set{\rho \subTE \Gamma_0}) \) \\ \> \>
    (where \(\alpha\) and \(\rho\) are fresh)  \\ \\ \>
\( PT(\inexp{x}{\seq y}{\ev}P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = PT(P_0) \) \\ \> \>
\(    \PIN  (\inty{x}{\tv}{\ev}{n} \rho,
           C_0 \cup \set{(\rho\TEPAR \appty{\tupty{\tv}{n}}
                           {\seq y})  \subTE \Gamma_0, 
                         \FV(\rho) \cap \set{\seq y} = \emptyset}) \) \\ \> \>
     (where \(\tv\) and \(\rho\) are fresh)  \\ \\ \>
\( PT(\nuexp{\seq x}P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = PT(P_0) \) \\ \> \>
\(    \PIN (\exclude{\Gamma_0}{\set{\seq x}}, 
       C_0 \cup \set{\reliable(\project{\Gamma_0}{\set{\seq x}}),
                   \FV(\exclude{\Gamma_0}{\set{\seq x}})\cap \set{\seq x} = \emptyset}) \)
\end{tabbing}
  \end{minipage}
}
  \caption{Algorithm \(PT\)}
  \label{fig:PT}
\end{figure}

\begin{theorem}
  If \(PT(P) = (\Gamma, C)\), then \((\Gamma, C)\) is a principal typing of \(P\).
\end{theorem}
\begin{proof}
  Structural induction on \(P\).
\end{proof}

% \subsect{Constraint Solving}

% Since a given process \(P\) is typeable if and only if the set of
% constraints output by \(PT(P)\), the remaining work to develop a
% type-check/reconstruction algorithm for each specific type system is
% to develop an algorithm to solve constraints.  Such algorithms, though
% presented in their specific formalization, have already been developed
% for specific type systems~\cite{Igarashi99IC,Kobayashi00CONCUR}.

\else

The type reconstruction algorithm \PT{} given below takes a process
expression as input and outputs a pair of a type environment 
(extended with expressions like \(\exclude{\tev}{S}\) and
\(\project{\tev}{S}\)) and a set of
constraints on variables in the type environment.  Each constraint is of
the form either \(\reliable(\Gamma)\) or \(\tev \subTE \Gamma\).  The
obtained pair gives a principal typing of the input in the sense that all
the possible type environments, under which the process expression is well
typed, are obtained from the type environment in the pair, by replacing
free variables in the constraint so that the constraint is satisfied.

\begin{tabbing}
\hspace*{2em} \= \( \PT(P) = (\Gamma, C): \) \\
\\ \>
\( \PT(\zeroexp) = (\zeroTE, \emptyset) \) \\ \>
\( \PT(\outexp{x}{\tilde z}{\ev}P_0) = \) \\ \> \quad \=
\(    \PLET (\Gamma_0, C_0) = \PT(P_0) \) \\ \> \>
\(    \PIN (\OutTE{x}{\typ{\tilde z}{\tev_x}}{\ev}
            (\tev \TEPAR \tev_x),
          C_0 \cup \set{\tev \subTE \Gamma_0}) \) \\ \> \>
    (where \(\tev\) and \(\tev_x\) are fresh)  \\ \>
\( \PT(\inexp{x}{\tilde y}{\ev}P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = \PT(P_0) \) \\ \> \>
\(    \PIN  \)\=\((\InTE{x}{\typ{\tilde y}{
                             \project{\tev}{\set{\tilde y}}}}{\ev}
           (\exclude{\tev}{\set{\tilde y}}), 
               C_0 \cup \set{\tev \subTE \Gamma_0}) \) \\ \> \> 
     (where \(\tev\) is fresh)  \\ \>
\( \PT(P_1 \PAR P_2) = \) \\ \> \>
\(   \PLET \) \= \((\Gamma_1, C_1) = \PT(P_1)\) \\ \> \> \>
\(             (\Gamma_2, C_2) = \PT(P_2) \) \\ \> \>
\(    \PIN (\Gamma_1 \TEPAR \Gamma_2, C_1 \cup C_2) \) \\ \>
\( \PT(P_1+\cdots+P_n) = \) \\ \> \>
\(    \PLET\) \= \((\Gamma_1, C_1) = \PT(P_1) \) \\ \> \> \>
\(                      \qquad \vdots \) \\ \> \> \>
\(          (\Gamma_n, C_n) = \PT(P_n) \) \\ \> \>
\(    \PIN (\Gamma_1+\cdots+\Gamma_n, C_1 \cup \cdots \cup C_n) \) \\ \>
\( \PT(\repexp P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = \PT(P_0) \) \\ \> \>
\(    \PIN (\TEREP \Gamma_0, C_0) \) \\ \>
\( \PT(\nuexp{\tilde x}P_0) = \) \\ \> \>
\(    \PLET (\Gamma_0, C_0) = \PT(P_0) \) \\ \> \>
\(    \PIN (\exclude{\Gamma_0}{\set{\tilde x}}, 
       C_0 \cup \set{\reliable(\project{\Gamma_0}{\set{\tilde x}})}) \)
\end{tabbing}

\fi



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> Related.tex <==
\section{Related Work}
\label{sec:related}

Resource usage analysis and similar analyses have recently been studied extensively,
and a variety of methods from type systems to model checking have been
proposed~\cite{DeLine01PLDI,DeLine02PLDI,Aiken02PLDI,IK05TOPLAS,SLAM,Marriott03,Skalka04}.
However, only a few of them deal with concurrent languages.
To our knowledge,
none of them deal with the partial liveness property (or the total liveness property) that we discussed
in Section~\ref{sec:extension}.
Nguyen and Rathke~\cite{Rathke2005} propose an effect-type system for a kind of resource usage analysis
for functional languages extended with threads and monitors. In their language,
neither resources nor monitors can be created dynamically.
On the other hand, our target language
is \(\pi\)-calculus, so that our type system can be applied to programs that may create infinitely many resources (due to the existence of primitives for dynamic creation of resources: recall
the example in Figure~\ref{fig:samplerun}), and also
to programs that use a wide range of communication and synchronization primitives.
Capability-based type systems can deal with concurrency to a certain degree
(\cite{DeLine01PLDI}, Section~4.2),
by associating each resource with a unique capability to access the resource.
The type system can control the resource access order,
by ensuring the uniqueness of the capability and keeping track
of what access is currently allowed by each capability. In this approach, however,
resource accesses are completely serialized and programmers have to care about
appropriately passing capabilities between threads.
% This part may be cryptic for people who are not familiar with the literature,
%but I am not sure whether we should go into more detail.
%In principle, if you want to ensure that a file is accessed as init;(read+write)*;close,
%a unique capability to access the file is created, and that is passed around.
%Only a process having the capability can access the file, and the type system
%keeps track of what access is currently associated with each capability. So,
%it is easy to ensure that the resources are used in the proper order, but
%accesses are completely serialized and programmers have to care about passing capabilities
%appropriately. For example, fork-join style synchronization of Example 1 cannot be expressed.}
Capability-based type systems~\cite{DeLine01PLDI,DeLine02PLDI} also require rather complex
type annotations.
%%%however, associating a resource with a unique
%%%capability and letting explicitly pass the capability between processes seems to restrict concurrent programs too much.
Igarashi and Kobayashi's type system for resource usage analysis
for \(\lambda\)-calculus~\cite{IK05TOPLAS} can be extended to deal with threads, by introducing
the following typing rule:
\infrule{\Gamma_1\p M_1:\tau_1 \andalso \Gamma_2 \p M_2:\tau_2}
     {\Gamma_1\otimes \Gamma_2 \p \textit{spawn}(M_1);M_2}
Here, \(\Gamma_1\otimes \Gamma_2\) describes resources that are used according to
\(\Gamma_1\) and \(\Gamma_2\) that are used in an interleaving manner. However, it is not obvious
how to accurately capture information about possible synchronizations between \(M_1\) and \(M_2\).

Model checking technologies~\cite{Ball02POPL} can of course be applicable to concurrent languages, but
they suffer from the 
state explosion problem, especially for expressive concurrent languages like \(\pi\)-calculus,
where resources and communication channels can be dynamically created and passed around.
Appropriate abstraction must be devised for effectively performing the resource usage analysis
for the \(\pi\)-calculus with model checking.
Actually, our type-based analysis can be considered a kind of abstract model checking.
The behavioral types extracted by (the first two steps of) the type inference algorithm are
abstract concurrent programs, each of which
 captures the access behavior on each resource. Then, conformance of the abstract program
with respect to the resource usage specification is checked as a model checking problem.
It would be interesting to study a relationship between the abstraction through our behavioral type and
the abstraction techniques for concurrent programs used in the model checking community.
From that perspective, an advantage of our approach is that our type, which
describes a resource-wise behavior, has much smaller state space than the whole program.
In particular, if infinitely many resources are dynamically created, the whole program has 
infinite states, but it is often the case that our behavioral types are still finite
(indeed so for the example in Figure~\ref{fig:samplerun}).
The limitation of our current analysis is that programs can be abstracted in
only one way; on the other hand, the usual abstract model checking techniques refine abstraction
step by step until the verification succeeds.

Technically, closest to our type system are that of Igarashi and Kobayashi~\cite{Kobayashi03TCS}
and that of Chaki, Rajamani, and Rehof~\cite{Rehof02POPL}. Those type systems
are developed for checking the communication behavior of a process, but by viewing a set of
channels as a resource, it is possible to use
those type systems directly for the resource usage analysis.
We summarize below similarities and differences between those type
systems~\cite{Kobayashi03TCS,Rehof02POPL} and the type system in the present paper.

%\begin{itemize}
%\item
\emph{(1) Whether types are supplied by the programmer or inferred automatically:}
Types are inferred automatically in
 Igarashi and Kobayashi's generic type~\cite{Kobayashi03TCS} and the type system of
the present paper, but the type of each channel must be annotated with
in Chaki et al.'s type system. The annotated type contains information
about how the values (channels, in particular)
sent along the channel are used by senders and receivers,
and that information is used to make the type checking process compositional.
For the purpose of the resource usage analysis discussed here,
we think that it is a burden for programmers to declare how channels are going to be used,
since their primary concern is how resources are accessed, not channels.
Ideal would be to allow the user to specify some types and infer the others, like in ML.
For that purpose, we need to develop an algorithm to check the conformance
\(A\newsubtype B\) of an inferred type \(A\) to a declared type \(B\).
That seems generally harder to decide than the trace inclusion constraint
\(\traces{x}{A}\subseteq \spec\), but we expect to be able to
develop a sound algorithm by properly restricting the language of declared types.

%\item
\emph{(2) The languages used as behavioral types:}
All the three type systems
use a fragment of CCS as the language of types to check cross-channel dependency
of communications. The types in
Igarashi and Kobayashi's generic type system for the \(\pi\)-calculus~\cite{Kobayashi03TCS},
however, lacks hiding, so that their type system cannot be applied to obtain precise information
about resource usage. In fact, their analysis would fail even for the program in
Example~\ref{ex:cobegin}.
Chaki et al.'s type system does use hiding, but lacks renaming as a
constructor. Without the renaming constructor, the most general type does not necessarily
exist, which hinders automatic type inference (recall Remark~\ref{rem:combination-of-hiding-and-renaming}).

%\item
\emph{(3) Algorithms for checking the conformance of inferred types with respect to
specifications:}
In Igarashi and Kobayashi's generic type system, how to check conformance of
inferred types with respect to the user-supplied specifications was left open,
and only suggested that it could be solved as a model checking problem.
In Chaki et al.'s type system~\cite{Rehof02POPL}, the conformance is expressed
as \(A \models F\) (for checking the global behavior, where \(F\) is an LTL-formula)
 and \(A\newsubtype A'\) (for checking the conformance of declared types with respect to
inferred types). In their type checker PIPER~\cite{Rehof02POPL}, those
conditions are verified using SPIN, so that \(A\) is restricted to a finite-state process.
Corresponding to the conformance check of the above work is the check of
trace inclusion constraints \(\traces{x}{A}\subseteq \spec\). Our algorithm based on
the reduction to Petri nets works even when \(A\) has infinite states.

%\item
\emph{(4) The guaranteed properties:}
Both Igarashi and Kobayashi's generic type~\cite{Kobayashi03TCS} and the extended type system of
the present paper can guarantee a certain lock-freedom property, that necessary communications
or resource accesses are eventually performed (unless the whole process diverges),
while Chaki et al.'s type system and
the type system in Section~\ref{sec:typing} of the present paper do not.
The guaranteed properties depend on the choice of the language of behavioral types and
the subtyping relation. In the latter type systems, the ordinary simulation relation is used, so that
a process's type describes only an upper-bound of the possible behavior of the process,
 not a lower-bound of the behavior like a certain resource access is eventually performed.
Rajamani et al.~\cite{Rehof04CAV,Rehof04ISOLA} recently introduced
a more elaborate notion of simulation relation called ``stuck-free conformance.''
Even with the stuck-free conformance relation, however, their type system~\cite{Rehof02POPL}
still cannot guarantee the lack of deadlock-freedom of a process.
On the other hand, by relying on an external analysis to check deadlock-freedom,
the extension in Section~\ref{sec:extension} keeps
the typing rules and the subtyping relation simple, while achieving the guarantee that
necessary resource accesses are eventually performed unless the whole process diverges.
%\end{itemize}

Kobayashi's type systems for deadlock-freedom and
livelock-freedom~\cite{Kobayashi00CONCUR,Kobayashi02IC,Kobayashi05ActInf} and
its implementation~\cite{TyPiCal}
form the basis of the extended type systems
for partial and total liveness properties discussed in Section~\ref{sec:extension},
and are used for producing well-annotated programs.
Conversely, the behavioral types introduced in this paper can be used to refine
the type systems for deadlock-freedom and livelock-freedom.
Yoshida and Honda have also studied type systems that
can guarantee certain lock-freedom properties~\cite{Yoshida96FST,Honda02POPL,Yoshida02liveness}.
So, their type systems can also be used for checking whether programs are well-annotated
in the sense of Section~\ref{sec:extension}.

In Section~\ref{sec:extension}, we have utilized the existing analysis for deadlock-freedom
to enhance the result of the resource usage analysis.
Other type systems for concurrent languages may also be useful. For example,
the type system for atomicity~\cite{Flanagan03PLDI} can be used to infer
the atomicity of a sequence of actions in a source program. By using the atomicity
information, we may be able to reduce the state space of behavioral types and check
the trace inclusion relation \(\etraces{x}{A}\subseteq \spec\) more efficiently.


==> Soundness.tex <==
%\section{Type Soundness}
%\label{sec:soundness}



The following theorem states that no well-typed process performs
an invalid access to a resource.
\begin{thm}[type soundness (safety)]
\label{th:safety}
Suppose that \(P\) is safe.
If \(\tjudge{\Gamma}{P}{A}\) and \(P\red^* Q\), then \(Q\) is safe.
\end{thm}
\proof
We make use of the following lemma:
\begin{itemize}
\item \textbf{Subject-reduction.} If $P \redwith{L} P'$
and $\tjudge{\Gamma}{P}{A}$ then $A \Tredswith{L} A'$ and $\tjudge{\Gamma}{P'}{A'}$.
Proof: see Appendix~\ref{sec:app:subject-reduction}.
\end{itemize}
For the proof of the theorem, we focus on just a single reduction step.
By the Lemma we know that judgements are preserved by reduction; we must show
that safety is also preserved, by induction on the derivation of reduction.
The only interesting case is \rname{R-NewR1}, 
\(\nurexp{x}{\spec}P \stackrel{\tau}{\rightarrow} \nurexp{x}{\spec^{-\xi}}P'\),
since the other rules do not alter trace-sets
$\spec$. In this case, we are given $\tjudge{\Gamma}{P}{A}$,
$\traces{x}{A}\subseteq \spec$, and $P \stackrel{x^\xi}{\rightarrow} P'$.
By the Lemma, $A \Tredswith{x^\xi} A'$ for some
$\tjudge{\Gamma}{P'}{A'}$. Assume $\nurexp{x}{\spec}P$ is safe; hence so is $P$; by
the induction hypothesis so is $P'$. From the conditions \(\traces{x}{A}\subseteq \spec\)
and $A \Tredswith{x^\xi} A'$, we get \(\xi\in \traces{x}{A}\subseteq \spec\), so that 
\(\emptyseq\in \spec^{-\xi}\neq \emptyset\). So, 
\(\nurexp{x}{\spec^{-\xi}}P'\) is safe.
\qed



%%%\begin{remark}
%%%The type system does not guarantee a {\em liveness} property;
%%%for example, \(\tjudge{\emptyset}{\nurexp{x}{\prefixclos{IR^*C}}P}{\Tzero} \) does not
%%%imply that \(x\) will be eventually closed.
%%%See Section~\ref{sec:extension} for how to extend the type system
%%%to guarantee the liveness property.
%%%%%%The extension for guaranteeing such a property is discussed in Section
%%%%%%To guarantee such a liveness property, we need to refine behavioral
%%%%%%types with the notion of capabilities/obligations to avoid deadlock and/or
%%%%%%livelock
%%%\end{remark}

%\finish{Give a proof sketch if there is enough space.
%The proof of subject reduction is routine, but we may still include
%the statement of subject reduction and the proof of Lemma A.8.
%Anyway, I do not strongly insist on including the proof sketch here.}


==> SyntaxDirectedTyping.tex <==
\iftwocol
\begin{figure}
\else
\begin{figure}
\fi
\begin{center}
\fbox{\small
\iftwocol
\begin{minipage}{\hfigwidth} %[t]{8cm}
\else
\begin{minipage}{14.5 cm} %{17cm}
\fi
\typicallabel{T-SD-Zero}

%%%\textbf{judgment for processes}
\infax[T-SD-Zero]
{\sdtjudge{\emptyset}{\zeroexp}{\Tzero}}

%\rulesp{}

%% \infrule[T-Out]
%%   {\Gamma, x:\Tchan{(x_1:\tau_1,\ldots,x_n:\tau_n)A_1}; A_2   \psd P\\
%%      \Gamma \psd v_i:\tau_i \mbox{ for each $i\in\{1,\ldots,n\}$}}
%%   {\Gamma, x:\Tchan{(x_1:\tau_1,\ldots,x_n:\tau_n)A_1}; 
%%     \Tout{x}(A_1[v_1/x_1,\ldots,v_n/x_n]\PAR A_2) \psd 
%%      \outexp{x}{v_1,\ldots,v_n}{}P}
\infrule[T-SD-Out]
  {\sdtjudge{\Gamma_0}{P}{A_2} \andalso
%%%   x:\Tchan{(\seq{y}\COL\seq{\mvtype})A_1} \in \Gamma \\
   \Gamma_i \p v_i\COL \mvtype_i \mbox{ (for each $i\in\set{1,\ldots,n}$)}}
  {\sdtjudge{\Gamma_0\TEcup \seq{\Gamma}\TEcup(x\COL\Tchan{(\seq{y}\COL\seq{\mvtype})A_1})}
   {\outexp{x}{\seq{v}}{}P}{\Tout{x}(\Tren{A_1}{\seq y}{\seq v} \PAR A_2)}}
%\rulesp{}

\infrule[T-SD-In]
   {   \sdtjudge{ \Gamma}{P}{A_2}\andalso
    \project{A_2}{\set{\seq{y}}}\newsubtype A_1\andalso
    \WF(\Gamma\TEcup \seq{y}\COL\seq{\mvtype})}
   {\sdtjudge{(\Gamma\restrictTE{\set{\seq{y}}})\TEcup x:\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}
    {\inexp{x}{\seq{y}}{}P}{\Tin{x}{\exclude{A_2}{\set{\seq{y}}}}}}
%% \infrule[T-In]
%%    {\Gamma, x:\Tchan{(y_1:\tau_1,\ldots,y_n:\tau_n)A_1}, 
%%     y_1:\tau_1,\ldots,y_n:\tau_n; A_2 \psd P\\
%%     A_1 \subtype \project{A_2}{\set{y_1,\ldots,y_n}}
%% %%%    \andalso  \set{x_1,\ldots,x_n}\cap \FV(\Gamma) = \emptyset
%%    }
%%    {\Gamma, x:\Tchan{(x_1:\tau_1,\ldots,x_n:\tau_n)A_1};
%%        \Tin{x}(\exclude{A_2}{\set{x_1,\ldots,x_n}})
%%          \psd \inexp{x}{\seq y}{}P}

%\rulesp{}

\infrule[T-SD-Par]
   {\sdtjudge{\Gamma_1}{P_1}{A_1} \andalso \sdtjudge{\Gamma_2}{P_2}{A_2}}
   {\sdtjudge{\Gamma_1\cup \Gamma_2}{P_1\PAR P_2}{A_1\TPAR A_2}}

%\rulesp{}
\infrule[T-SD-Rep]
   {\sdtjudge{\Gamma}{P}{A}}
   {\sdtjudge{\Gamma}{\repexp{P}}{\Trep{A}}}

%\rulesp{}

\infrule[T-SD-If]
  {\Gamma_0\p v:\Tbool\andalso 
   \sdtjudge{\Gamma_1}{P}{A_1} \andalso \sdtjudge{\Gamma_2}{Q}{A_2}\\
     A_1\newsubtype A \andalso A_2\newsubtype A}
  {\sdtjudge{\Gamma_0\TEcup\Gamma_1\TEcup \Gamma_2}{\ifexp{v}{P}{Q}}{A}}
%\rulesp{}


\infrule[T-SD-New]
   {\sdtjudge{\Gamma}{P}{A_2}\andalso
    \WF(\Gamma\TEcup (x:\Tchan{(\seq{x}\COL\seq{\tau})A_1}))}
%%%    \andalso x\not\in \FV(\Gamma)
   {\sdtjudge{\Gamma\restrictTE{\set{x}}}{\nuexp{x}P}{\Thiding{x}{A_2}}}
%\rulesp{}

\infrule[T-SD-Acc]
  {\sdtjudge{\Gamma}{P}{A}}
  {\sdtjudge{\Gamma\TEcup (x\COL\Tres)}{\accexp{\acclab}{x}P}{\Tacc{\acclab}{x}A}}

%\rulesp{}

\infrule[T-SD-NewR]
  {\sdtjudge{\Gamma}{P}{A}\andalso 
   \traces{x}{{A}} \subseteq {\spec} \andalso
   \WF(\Gamma\TEcup (x\COL\Tres))}
   % \Gamma; \exclude{A}{\set{x}} \psd \nurexp{x}{\spec}P
  {\sdtjudge{\Gamma\restrictTE{\set{x}}}{\nurexp{x}{\spec}P}{\exclude{A'}{\set{x}}}}
%% \infrule[T-NewR]
%%   {\Gamma, x\COL\Tres; A \psd P\andalso \traces{x}{\project{A}{x}} \subseteq \prefixclos{\spec}}
%%   {\Gamma; \exclude{A}{\set{x}} \psd \nurexp{x}{\spec}P}

%% \infrule[T-Sub]
%%   {\Gamma; A' \psd P\andalso A \subtype A'}
%%   {\Gamma; A  \psd P}

%% \textbf{judgment for values}
%% \infax[T-Var]{\Gamma, x\COL\tau \psd x:\tau}
%% \infrule[T-Bool]{b\in \set{\TRUE,\FALSE}}{\Gamma \psd b: \Tbool}
\end{minipage}
}
\caption{Syntax Directed Typing Rules}
\label{fig:sd-typing}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi


==> Typing.tex <==
\sect{Type System}
\label{sec:typing}
This section introduces a type system that prevents invalid access to resources.
The type system in this section
does not guarantee a liveness property that
all the necessary accesses are eventually made; extensions to guarantee that property
are discussed in Section~\ref{sec:extension}.
%The formal property guaranteed by the type system is discussed in the next section.
\subsect{Types}

We first introduce the syntax of types. We use two categories of types:
value types and behavioral types. The latter describes how a process accesses
resources and communicates through channels.
As mentioned in Section~\ref{sec:intro}, we use CCS processes for behavioral types.
\begin{defi}[types]
The sets of {\em value types} \(\mvtype\) and {\em behavioral types} \(A\) are defined by:
\[
\begin{array}{lcl}
\mvtype  &\!\!::=\!\!& \Tbool \mid \Tres
    \mid \Tchan{(x_1\COL{}\mvtype_1,\ldots,x_n\COL{}\mvtype_n)A}\\
%% A \mbox{ (behavioral types)} &::=&
%%     \Tzero \mid \Tin{x}A\mid \Tout{x}A \mid \Tacc{\acclab}{x}A\mid (A_1\PAR A_2)
%%     \mid A_1\TOR A_2
%%     \mid \Trep{A} \mid \Tbvar \mid \Tren{A}{\seq{x}}{\seq{y}}
%%     \mid \Thiding{x}{A}
%%     \mid \Trec{\Tbvar}{A}
A  &\!\!::=\!\!&
    \Tzero \mid \Tbvar \mid \Tact{\cact}A \mid
   \Tacc{\acclab}{x}A\mid \Tact{\tau}A\mid
  (A_1\PAR A_2)    \mid A_1\TOR A_2\mid \Trep{A} \\
    && \mid \csubstseq{y_1/x_1,\ldots,y_n/x_n}A
    \mid \Thiding{x}{A}
    \mid \Trec{\Tbvar}{A}
    \mid \exclude{A}{S} \mid \project{A}{S}\\
\multicolumn{3}{l}
{\cact \mbox{ (communication labels) } ::=
   \Tinatom{x} \mid \Toutatom{x}}
%%%a \mbox{ (communication labels) } &::=&
%%%   \Tinatom{x} \mid \Toutatom{x}
\end{array}
\]
%%%The metavariable \(\lab\) ranges over the set \(\IndexSet\) of positive
%%%integers, and \(m\) ranges over the set of non-negative integers.
\end{defi}
%
A behavioral type \(A\), which is a CCS process,
 describes what kind of communication and resource
access a process may perform.
\(\Tzero\) describes a process that performs no communication or resource
access.
The types \(\Tin{x}A\), \(\Tout{x}A\), \(\Tacc{\acclab}{x}A\) and \(\Tact{\tau}A\)
describe processes that first perform an action and then behave according to $A$; the actions
are, respectively, an input on $x$, an output on $x$, an access operation $\xi$ on $x$,
and the invisible action.
%%%The type \(\Tin{x}A\) describes a process that first performs an input on \(x\)
%%%and then behaves according to \(A\).
%%%The type \(\Tout{x}A\) describes a process that performs
%%% an output on \(x\) and then behaves according to \(A\).
%%%The behavioral type \(\Tacc{\acclab}{x}A\) describes a process that performs
%%%an operation described by \(\acclab\) to the resource \(x\), and then behaves
%%%according to \(A\).
\(A_1\PAR A_2\) describes a process that performs communications and
resource access according to \(A_1\) and \(A_2\), possibly in parallel.
\(A_1{\TOR}A_2\) describes a process that behaves according to
either \(A_1\) or \(A_2\).
\(\Trep{A}\) describes a process that behaves like
\(A\) an arbitrary number of times, possibly in parallel.
\(\csubstseq{y_1/x_1,\ldots,y_n/x_n}A\), abbreviated to
\(\Tren{A}{\seq{x}}{\seq{y}}\), denotes simultaneous renaming of
\(\seq{x}\) with \(\seq{y}\) in \(A\).
%%%(Note that the renaming is defined to be a constructor rather than an operator.)
\(\Thiding{x}{A}\) describes a process that behaves like \(A\) for
some hidden channel \(x\). For example,
\(\Thiding{x}{(\Tin{x}\Toutatom{y}\PAR \Toutatom{x})}\) describes a
process that performs an output on \(y\) after the invisible action on \(x\).
The type \(\Trec{\Tbvar}{A}\) describes a process that behaves like
a recursive process defined by \(\Tbvar \DEF A\).\footnote{The replication
\(\Trep{A}\) and \(\Trec{\Tbvar}{(A\TPAR \Tbvar)}\) have the same semantics in
this section, but they are differentiated in Section~\ref{sec:extension}
by the predicate \textit{disabled}.}
%% The type \(\project{\PrTy}{S}\) describes a processtrue
%% extracts from \(\PrTy\) information
%% on the usage of only the channels in \(S\),
%% while \(\exclude{\PrTy}{S}\) extracts information on the usage of
%% the channels not in \(S\).
The type \(\exclude{A}{S}\) describes a process
that behaves like \(A\), except that actions whose targets
are in \(S\) are replaced by the invisible action \(\tau\),
%%% [Kohei] added
while \(\project{A}{S}\) describes a process
that behaves like \(A\), except that actions whose targets
are not in \(S\) are replaced by \(\tau\).
The formal semantics of behavioral types is defined later using
labeled transition semantics.

As for value types, \(\Tbool\) is the type of booleans. \(\Tres\) is the type of resources.
%%%(For simplicity, we consider a single kind of resource in the
%%%formalization.)
The type
\(\Tchan{(x_1\COL{}\mvtype_1,\ldots,x_n\COL{}\mvtype_n)A}\),
abbreviated to \(\Tchan{(\seq{x}\COL\seq{\mvtype})A}\), describes channels carrying
tuples consisting of values of types \(\mvtype_1,\ldots,\mvtype_n\).
Here the type \(A\) approximates how a receiver on the channel may use the elements \(x_1,\ldots,x_n\) of each tuple
for communications and resource access.
For example, \(\Tchan{(x\COL\Tres,y\COL\Tres)\Tacc{R}{x}\Taccatom{C}{y}}\) describes
channels carrying a pair of resources, where a party who receives the actual pair
\((x',y')\) will first read $x'$ and then close $y'$.
We sometimes omit \(\seq{\mvtype}\) and write
\(\Tchan{(\seq{x})A}\) for \(\Tchan{(\seq{x}\COL\seq{\mvtype})A}\).
When \(\seq{x}\) is empty, we also write \(\Tchan{}\).
%%%\(A\) can be considered as a contract about the possible resource access and communication
%%%behaviors of receivers.
%%%A sender expects that any receiver will use values sent on the channel according to
%%%\(A\), and a receiver has to o



%\finish{Where should we say that the behavioral type \(A\) describes
%only an upper-bound of the behavior of processes?
%For example, a process having a type \(\Tacc{C}{x}\Tzero\) does not necessarily
%mean the process will close \(x\).}
%% Lucian -- the above comment has already been dealt with
%% in section 3.3, "A is an approximation... P may do less..."

Note that \(\csubst{\seq{x}}{\seq{y}}\) is treated as a constructor rather than
an operator for performing the actual substitution. We write \(\subst{\seq{x}}{\seq{y}}\)
for the latter throughout this paper.
\(\csubst{\seq{x}}{\seq{y}}A\) is slightly different from the \emph{relabeling}
of the standard CCS~\cite{Milner89CCS}: \(\csubst{x}{y}(\Tinatom{x}\PAR \Toutatom{y})\)
allows the communication on \(y\), but the relabeling of CCS does not.
This difference calls for the introduction of
a special transition label \(\actcom{x}{\actout{y}}\) in
Section~\ref{sec:semantics-of-types}.


%%%The following is the definition of free variables. Probably the definition is unnecessary.
\begin{defi}
The set of {\em free variables} of \(A\), written \(\FV(A)\), is defined by:
\[\begin{array}{rcl}
\FV(\Tzero) &=& \emptyset\\
\FV(\Tbvar) &=& \emptyset\\
\FV(\Tin{x}A) &=& \set{x}\cup \FV(A)\\
\FV(\Tout{x}A) &=& \set{x}\cup \FV(A)\\
\FV(\Tacc{\acclab}{x}A) &=& \set{x}\cup \FV(A)\\
\FV(\Tact{\tau}A) &=& \FV(A)\\
\FV(A_1\PAR A_2) &=& \FV(A_1)\cup \FV(A_2)\\
\FV(A_1\TOR A_2) &=& \FV(A_1)\cup \FV(A_2)\\
\FV(\Trep{A}) &=& \FV(A)\\
\FV(\Tren{A}{\seq{x}}{\seq{y}}) &=& (\FV(A) \setdif \set{\xx}) \cup \set{\yy}\\
\FV(\Thiding{x}{A}) &=& \FV(A)\setdif\set{x}\\
\FV(\Trec{\Tbvar}A) &=& \FV(A)\\
\FV(\exclude{A}{S}) &=& \FV(A)\setdif S\\
\FV(\project{A}{S}) &=& \FV(A) \cap S
%
%% \FV(A) &=& \FV^\emptymap(A)\\
%% \FV^F(\Tzero) &=& \emptyset\\
%% \FV^F(\Tbvar) &=& F(\Tbvar)\\
%% \FV^F(\Tin{x}A) &=& \set{x}\cup \FV^F(A)\\
%% \FV^F(\Tout{x}A) &=& \set{x}\cup \FV^F(A)\\
%% \FV^F(\Tacc{\acclab}{x}A) &=& \set{x}\cup \FV^F(A)\\
%% \FV^F(\Tact{\tau}A) &=& \FV^F(A)\\
%% \FV^F(A_1\PAR A_2) &=& \FV^F(A_1)\cup \FV^F(A_2)\\
%% \FV^F(A_1\TOR A_2) &=& \FV^F(A_1)\cup \FV^F(A_2)\\
%% \FV^F(\Tren{A}{\seq{x}}{\seq{y}}) &=& \set{ \subst{\seq{x}}{\seq{y}}{z}\mid z\in \FV^F(A)}\\
%% \FV^F(\Thiding{x}{A}) &=& \FV^F(A)\setdif\set{x}\\
%% \FV^F(\exclude{A}{S}) &=& \FV^F(A)\setdif S\\
%% %%% \FV^F(\project{A}{S}) &=& \FV^F(A) \cap S\\
%% \FV^F(\Trec{\Tbvar}A) &=&
%%     \bigcap \set{S \mid S \supseteq \FV^{\extmap{F}{\Tbvar}{S}}(A)}
\end{array}\]
\end{defi}
%
As defined above, \(\Thiding{x}{A}\), \(\Tren{A}{\seq{x}}{\seq{y}}\), and \(\exclude{A}{S}\) bind
\(x\), \(\seq{x}\), and the variables in \(S\) respectively.
We identify behavioral types up to renaming of bound variables.
In the rest of this paper, we require that
every channel type
\(\Tchan{(x_1\COL{}\mvtype_1,\ldots,x_n\COL{}\mvtype_n)A}\)
must satisfy \(\FV(A)\subseteq \set{x_1,\ldots,x_n}\).
For example, \(\Tchan{(x{:}\Tres)\Taccatom{R}{x}}\) is a valid type
but \(\Tchan{(x{:}\Tres)\Taccatom{R}{y}}\) is not.%
\footnote{This constraint can be removed if we assume that
the free variables in \(\codom(\Gamma)\) never clash
with the bound variables of \(P\)
in the judgment form \(\tjudge{\Gamma}{P}{A}\) given later. In particular,
we need an implicit assumption \(\{\yy\}{\cap}\FV(\Gamma){=}\emptyset\) in
Figure~\ref{fig:typing}, \rname{T-In}.}

% [Kohei] changed
% We write \(\project{A}{S}\) for \(\exclude{A}{\FV(A) \setdif S}\).
%%%We extend \(\csubst{\seq{x}}{\seq{y}}A\) to 
%%%By abuse of notation, we write \(\csubstseq{v_1/x_1,\ldots,v_n/x_n}A\) for
%%%\(\csubstseq{v_{i_1}/x_{i_1},\ldots,v_{i_k}/x_{i_k}}A\) where\\
%%%\(\set{v_{i_1},\ldots,v_{i_k}} = \set{v_1,\ldots,v_n}\setdif\set{\TRUE,\FALSE}\).
%%%For example,\\ \(\csubstseq{\TRUE/x, y/z}A\) stands for
%%%\(\csubstseq{y/z}A\).


%%%% We introduce exclude/project as primitives.
%% We define operations on types.
%% The operation \(\project{\PrTy}{S}\) defined below
%% extracts from \(\PrTy\) information
%% on the usage of only the channels in \(S\),
%% while \(\exclude{\PrTy}{S}\) extracts information on the usage of
%% the channels not in \(S\).
%% \begin{defi}
%% Let \(S\) be a finite subset of \(\VAR\).
%% Then, unary operations \(\project{\cdot}{S}\) and
%% \(\exclude{\cdot}{S}\)  are defined by:
%% %%%\[
%% \begin{eqnarray*}
%% \exclude{A}{\set{x_1,\ldots,x_n}} &=& \Thiding{x_1,\ldots,x_n}(A \PAR
%%                       \Trep{\Tinatom{x_1}} \PAR \Trep{\Toutatom{x_1}} \PAR \cdots \PAR
%%                             \Trep{\Tinatom{x_n}} \PAR \Trep{\Toutatom{x_n}})\\
%% \project{A}{S} &=& \exclude{A}{\FV(A)\setdif S}
%% \end{eqnarray*}
%% %%\]
%% \end{defi}


\subsect{Semantics of behavioral types}
\label{sec:semantics-of-types}
We give a labeled transition relation \(\Tredwith{\Tredlab}\) for behavioral types.
The transition labels $l$ (distinct from the reduction labels $L$ of Definition~\ref{def:target1}) are
\[ \act\ ::=\
   \Tinatom{x} \mid \Toutatom{x} \mid
   \Tredlabacc{x}{\acclab} \mid \Tredlabsilent\mid \actcom{x}{\actout{y}}
\]
The label $\actcom{x}{\actout{y}}$ indicates the potential
to react in the presence of a substitution that identifies $x$ and $y$.
We also extend \(\Acctarget{}\) to the function on transition labels by:
\[
\acctarget{x} = \acctarget{\Toutatom{x}} = \set{x} \qquad
\acctarget{\actcom{x}{\actout{y}}} = \set{x,y}
\]
%%%The structural relation \(\TSPCONG\) and the reduction relation
The transition relation
\(\Tredwith{\Tredlab}\) on behavioral types is
the least relation closed under the rules
in Figure~\ref{fig:red-behavioral-types}.
We write \(\Treds\) for the reflexive and transitive closure of
\(\Tredwith{\tau}\).
We also write \(\Tredswith{\act}\) for
\(\Treds\Tredwith{\Tredlab}\Treds\).
\iftwocol
\begin{figure}
\else
\begin{figure}
\fi
\begin{center}
\fbox{\small
\iftwocol
\begin{minipage}{\hfigwidth}
\else
\begin{minipage}{14.5 cm}
\fi
%% \paragraph{Evaluation contexts}
%% \[
%% \begin{array}{l}
%% %% \Tevalcontxt ::= \hole \mid \nuexp{x}\Tevalcontxt \mid \nurexp{x}{\spec}\Tevalcontxt
%% %%            \mid (\Tevalcontxt\TPAR A)
%% \Tevalcontxt ::= \hole \mid (\Tevalcontxt\TPAR A)
%% \end{array}
%% \]

% \textbf{Structural relation}
% ($A_1\TSCONG A_2\iff (A_1\TSPCONG A_2)\land (A_2\TSPCONG A_1)$)}
%% \infax{A_1\TPAR A_2\TSCONG A_2\TPAR A_1}
%% \infax{A_1\TPAR (A_2\TPAR A_3)\TSCONG (A_1\TPAR A_2)\TPAR A_3}
%% \infax{A_1\TOR A_2 \TSPCONG A_i  \ (i\in \set{1,2})}
%% \infax{\Trec{\Tbvar}{A} \TSPCONG \Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}}}
%% \infax{\Tren{(\Tin{x}{A})}{\seq{y}}{\seq{z}}\TSCONG
%%           \Tin{\rename{x}{\seq{y}}{\seq{z}}}{\Tren{A}{\seq{y}}{\seq{z}}}}
%% \infax{\Tren{(\Tout{x}{A})}{\seq{y}}{\seq{z}}\TSCONG
%%           \Tout{\rename{x}{\seq{y}}{\seq{z}}}{\Tren{A}{\seq{y}}{\seq{z}}}}
%% \infax{\Tren{(\Tacc{\acclab}{x}{A})}{\seq{y}}{\seq{z}}\TSCONG
%%           \Tacc{\acclab}{\rename{x}{\seq{y}}{\seq{z}}}{\Tren{A}{\seq{y}}{\seq{z}}}}
%% \Infax{\Tren{(A_1\TPAR A_2)}{\seq{x}}{\seq{y}} \TSCONG
%%   \Tren{A_1}{\seq{x}}{\seq{y}} \TPAR  \Tren{A_2}{\seq{x}}{\seq{y}}}
%% \infax{\Tren{(A_1\TOR A_2)}{\seq{x}}{\seq{y}} \TSCONG
%%   \Tren{A_1}{\seq{x}}{\seq{y}} \TOR  \Tren{A_2}{\seq{x}}{\seq{y}}}
%% \infax{\Tren{(\nuexp{x}A)}{\seq{y}}{\seq{z}} \TSCONG
%%           \nuexp{x}\Tren{A}{\seq{y}}{\seq{z}} \mbox{ (if $x\not\in \set{\seq{y}\cup\seq{z}}$})}
%% \infax{\Tren{\Trec{\Tbvar}{A}}{\seq{x}}{\seq{y}} \TSCONG
%%             \Trec{\Tbvar}{\Tren{A}{\seq{x}}{\seq{y}}}}
% \infax{\nuexp{x}A_1 \TPAR A_2 \TSPCONG \nuexp{x}(A_1\TPAR A_2)
%         \mbox{ (if $x\not\in \FV(A_2)$)}}
%% \infax{\nurexp{x}{\spec}A_1 \TPAR A_2 \TSPCONG \nurexp{x}{\spec}(A_1\TPAR A_2)
%%          \mbox{ (if $x\not\in \FV(A_2)$)}}
%% \infax{\project{A}{S}  \TSPCONG  \exclude{A}{\FV(A) \setdif S}}
%% \infrule{A_1\TSPCONG A_2}
%%         {\Tevalcontxt[A_1]\TSPCONG \Tevalcontxt[A_2]}

% \textbf{Reduction relation}
%%\textbf{Transition semantics}
%% \infax[TR-Com]{\Tin{x}{A_1}\TPAR \Tout{x}{A_2}\Tredsilent A_1\TPAR A_2}
%% \infax[TR-Acc]{\Tacc{\acclab}{x}A_1 \Tredacc{\acclab}{x} A_1}
%% \infrule[TR-Context]{A_1\Tredwith{\Tredlab}A_2}{\Tevalcontxt[A_1]\Tredwith{\Tredlab} \Tevalcontxt[A_2]}
%% \infrule[TR-Cong]{A_1\TSPCONG A_1' \andalso A_1'\Tredwith{\Tredlab}A_2'\andalso
%%     A_2'\TSPCONG A_2}
%%   {A_1\Tredwith{\Tredlab} A_2}
%% \end{minipage}
%% }
%%%\infax[TR-In]{\Tin{x}A \Tredwith{\Tinatom{x}} A}
%%%\infax[TR-Out]{\Tout{x}A \Tredwith{\Toutatom{x}} A}
%\infax[Tr-CAct]
%   {\Tact{\cact}A \Tredwith{\cact} A}
%\infax[Tr-Acc]
%   {\Tact{\actracc{\acclab}{x}}A \Tredwith{\actracc{\acclab}{x}} A}
%\infax[Tr-Tau]
%   {\Tact{\tau}A \Tredwith{\tau} A}
\infax[Tr-Act]
    {\Tact{\cact}A {\stackrel{\cact}{\rightarrow}} A \andalso
     \Tact{\actracc{\acclab}{x}}A \stackrel{x^{\xi}}{\rightarrow} A \andalso
     \Tact{\tau}A {\stackrel{\tau}{\rightarrow}} A}

%\infrule[Tr-Par1]
%{A_1 \Tredwith{l} A_1'}
%{A_1 \TPAR A_2 \Tredwith{l} A_1' \TPAR A_2}
%\infrule[Tr-Par2]
%{A_2 \Tredwith{l} A_2'}
%{A_1 \TPAR A_2 \Tredwith{l} A_1 \TPAR A_2'}
%\[
% \qquad\quad\ \
% \frac{A_1 {\stackrel{l}{\rightarrow}} A_1'}{A_1{|}A_2 {\stackrel{l}{\rightarrow}} A_1'{|}A_2} \qquad
% \frac{A_2 {\stackrel{l}{\rightarrow}} A_2'}{A_1{|}A_2 {\stackrel{l}{\rightarrow}} A_1{|}A_2'} \qquad
% \mbox{\sc(Tr-Par1)}
%\]
\hspace{3cm}
\begin{minipage}{4cm}
\infrule
{A_1 {\stackrel{l}{\rightarrow}} A_1'}
{A_1{|}A_2 {\stackrel{l}{\rightarrow}} A_1'{|}A_2}
\end{minipage} \quad
\begin{minipage}{4cm}
\infrule
{A_2 {\stackrel{l}{\rightarrow}} A_2'}
{A_1{|}A_2 {\stackrel{l}{\rightarrow}} A_1{|}A_2'}
\end{minipage}
\hfill\sc{(Tr-Par1)}
%{A_1 \TPAR A_2 \Tredwith{l} A_1' \TPAR A_2}
%\infrule[Tr-Par2]
%{A_2 \Tredwith{l} A_2'}
%{A_1 \TPAR A_2 \Tredwith{l} A_1 \TPAR A_2'}


% \infax[Tr-Com]{\Tin{x}{A_1}\TPAR \Tout{x}{A_2}\Tredsilent A_1\TPAR A_2}
%\infrule[Tr-Par3]
%{A_1 \Tredwith{a} A_1'  \andalso  A_2 \Tredwith{b} A_2'\andalso
%  \mbox{$a$ and $b$ have different polarities}}
%{A_1 \TPAR A_2 \Tredwith{\actcom{a}{b}} A_1' \TPAR A_2'}
%\infrule[Tr-Par3]
%
%
%%\[
% \qquad
% \frac{A_1 {\stackrel{x}{\rightarrow}} A_1' \ \   A_2 {\stackrel{\overline{y}}{\rightarrow}} A_2'}{A_1 {|} A_2 \Tredwith{\actcom{x}{\overline{y}}} A_1'{|}A_2'} \quad
% \frac{A_1 {\stackrel{\overline{y}}{\rightarrow}} A_1' \ \   A_2 {\stackrel{x}{\rightarrow}} A_2'}{A_1 {|} A_2 \Tredwith{\actcom{x}{\overline{y}}} A_1'{|}A_2'} \quad
% \mbox{\sc(Tr-Par2)}
%\]
\hspace{2.9cm}
\begin{minipage}{4cm}
\infrule
{A_1 {\stackrel{x}{\rightarrow}} A_1' \andalso A_2
{\stackrel{\overline{y}}{\rightarrow}} A_2'}
{A_1 {|} A_2 \Tredwith{\actcom{x}{\overline{y}}} A_1'{|}A_2'}
\end{minipage} \quad
\begin{minipage}{4cm}
\infrule
{A_1 {\stackrel{\overline{y}}{\rightarrow}} A_1' \andalso A_2
{\stackrel{x}{\rightarrow}} A_2'}
{A_1 {|} A_2 \Tredwith{\actcom{x}{\overline{y}}} A_1'{|}A_2'}
\end{minipage}
\hfill\sc{(Tr-Par2)}

\infrule[Tr-Com]
{A \Tredwith{\actcom{x}{\actout{x}}} A'}
{A \Tredsilent A'}

%\infrule[Tr-Or1]
%{A_1 \Tredwith{l} A_1'}
%{A_1 \TOR A_2 \Tredwith{l} A_1'}
%\infrule[Tr-Or2]
%{A_2 \Tredwith{l} A_2'}
%{A_1 \TOR A_2 \Tredwith{l} A_2'}
%%\[
% \qquad\qquad\quad\ \ \
% \frac{A_1 {\stackrel{l}{\rightarrow}} A_1'}{A_1{\oplus}A_2 {\stackrel{l}{\rightarrow}} A_1'} \qquad
% \frac{A_2 {\stackrel{l}{\rightarrow}} A_2'}{A_1{\oplus}A_2 {\stackrel{l}{\rightarrow}} A_2'} \qquad
% \mbox{\sc(Tr-Or)}
%\]
\hspace{2.9cm}
\begin{minipage}{4cm}
\infrule
{A_1 {\stackrel{l}{\rightarrow}} A_1'}
{A_1{\oplus}A_2 {\stackrel{l}{\rightarrow}} A_1'}
\end{minipage} \quad
\begin{minipage}{4cm}
\infrule
{A_2 {\stackrel{l}{\rightarrow}} A_2'}
{A_1{\oplus}A_2 {\stackrel{l}{\rightarrow}} A_2'}
\end{minipage}
\hfill\sc{(Tr-Or)}
\infrule[Tr-Rep]
{A\PAR \Trep{A} \Tredwith{l} A'}
{\Trep{A} \Tredwith{l} A'}

\infrule[Tr-Rec]
{\Tsubst{A}{\Tbvar}{\Trec{\Tbvar}{A}} \Tredwith{l} A'}
{\Trec{\Tbvar}{A} \Tredwith{l} A'}

\infrule[Tr-Rename]
{A \Tredwith{l} A'}
{\Tren{A}{\seq{x}}{\seq{y}} \Tredwith{\subst{\seq x}{\seq y}l} \Tren{A'}{\seq x}{\seq y}}

\infrule[Tr-Hiding]
{A \Tredwith{l} A'  \quad  \acctarget{l}{\cap}\{x\} = \emptyset}
{\nuexp{x}A \Tredwith{l} \nuexp{x}A'}

%% \infrule[TR-Hiding-In]
%% {A \Tredwith{y} A'  \andalso  x \ne y}
%% {\nuexp{x}A \Tredwith{y} \nuexp{x}A'}

%% \infrule[TR-Hiding-Out]
%% {A \Tredwith{\Toutatom{y}} A'  \andalso  x \ne y}
%% {\nuexp{x}A \Tredwith{\Toutatom{y}} \nuexp{x}A'}

%% \infrule[TR-Hiding-Silent]
%% {A \Tredsilent A'}
%% {\nuexp{x}A \Tredsilent \nuexp{x}A'}

%%%\infax[TR-Acc]{\Tacc{\acclab}{x}A_1 \Tredacc{x}{\acclab} A_1}

%% \infrule[TR-Context]{A_1\Tredwith{\Tredlab}A_2}{\Tevalcontxt[A_1]\Tredwith{\Tredlab} \Tevalcontxt[A_2]}

%\infrule[TR-Exclude1]
%{A \Tredwith{l} A'  \andalso  \acctarget{l} \subseteq S}
%{\exclude{A}{S}  \Tredsilent  \exclude{A'}{S}}
%\infrule[TR-Exclude2]
%{A \Tredwith{l} A'  \andalso  \acctarget{l} \cap S = \emptyset}
%{\exclude{A}{S}  \Tredwith{l}  \exclude{A'}{S}}

%% \[\begin{array}{c}
%%  \displaystyle\frac{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\subseteq}S}{\exclude{A}{S} {\stackrel{\tau}{\rightarrow}} \exclude{A'}{S}} \quad
%%  \displaystyle\frac{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\cap}S{=}\emptyset}{\exclude{A}{S} {\stackrel{l}{\rightarrow}} \exclude{A'}{S}} \quad \\
%%  \multicolumn{1}{r}{\mbox{\sc(Tr-Exclude)}\hspace{-2.1em}}
%% \end{array}\]

\hspace{2cm}
\begin{minipage}{4cm}
\infrule{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\subseteq}S}
        {\exclude{A}{S} {\stackrel{\tau}{\rightarrow}} \exclude{A'}{S}}
\end{minipage} \quad
\begin{minipage}{4cm}
 \infrule{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\cap}S{=}\emptyset}
         {\exclude{A}{S} {\stackrel{l}{\rightarrow}} \exclude{A'}{S}}
\end{minipage}
\hfill\sc{(Tr-Exclude)}

%\infrule[TR-Project1]
%{A \Tredwith{l} A'  \andalso  \acctarget{l} \subseteq S}
%{\project{A}{S}  \Tredwith{l}  \project{A'}{S}}
%\infrule[TR-Project2]
%{A \Tredwith{l} A'  \andalso  \acctarget{l} \cap S = \emptyset}
%{\project{A}{S}  \Tredsilent  \project{A'}{S}}

%% \[\begin{array}{c}
%%  \displaystyle\frac{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\subseteq}S}{\project{A}{S} {\stackrel{l}{\rightarrow}} \project{A'}{S}} \quad
%%  \displaystyle\frac{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\cap}S{=}\emptyset}{\project{A}{S} {\stackrel{\tau}{\rightarrow}} \project{A'}{S}} \quad \\
%%  \multicolumn{1}{r}{\mbox{\sc(Tr-Project)}\hspace{-2.1em}}
%% \end{array}\]
\hspace{2cm}
\begin{minipage}{4cm}
\infrule{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\subseteq}S}{\project{A}{S} {\stackrel{l}{\rightarrow}} \project{A'}{S}}
\end{minipage} \quad
\begin{minipage}{4cm}
\infrule{A {\stackrel{l}{\rightarrow}} A' \quad \acctarget{l}{\cap}S{=}\emptyset}{\project{A}{S} {\stackrel{\tau}{\rightarrow}} \project{A'}{S}} 
\end{minipage}
\hfill\sc{(Tr-Project)}

%% \infrule[TR-Cong]{A_1\TSPCONG A_1' \andalso A_1'\Tredwith{\Tredlab}A_2'\andalso
%%     A_2'\TSPCONG A_2}
%%   {A_1\Tredwith{\Tredlab} A_2}
\end{minipage}
}

\caption{Transition semantics of behavioral types}
\label{fig:red-behavioral-types}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi

\begin{rem}
\label{rm:nu-and-exclude}
\(\Thiding{x}{A}\) should not be confused with \(\exclude{A}{\set{x}}\).
\(\Thiding{x}{A}\) is the hiding operator of CCS, while
\(\exclude{A}{\set{x}}\) just replaces any actions on \(x\) with \(\tau\)~\cite{Kobayashi03TCS}.
For example,
\(\Thiding{x}{(\Tin{x}\Taccatom{\xi}{y})}\) cannot make any transition,
but \(\exclude{(\Tin{x}\Taccatom{\xi}{y})}{\set{x}}\Tredwith{\tau}\Tredwith{\redlabacc{\xi}{y}}
\exclude{\Tzero}{\set{x}}\).
\end{rem}

The set \(\traces{x}{A}\) defined below is the set of possible
access sequences on \(x\) described by \(A\).
\begin{defi}[traces]
\[
\traces{x}{A} =
  \set{\acclab_1\ldots\acclab_n \mid
   \project{A}{\set{x}} \Tredsacc{x}{\acclab_1}\cdots \Tredsacc{x}{\acclab_n}A'}
\]
\end{defi}
Note that \(\traces{x}{A}\) is prefix-closed (hence a trace set) by definition.
%%%We will usually use \(\traces{x}{A}\) when \(\FV(A)=\set{x}\) below.

We define the subtyping relation  \(A_1\newsubtype A_2\) below.
Intuitively, \(A_1\newsubtype A_2\) means that a process behaving according to \(A_1\)
can also be viewed as a process behaving according to \(A_2\).
To put in another way, \(A_1\newsubtype A_2\) means that \(A_2\) simulates \(A_1\).%
\iffull
\else
\footnote{Note that the subtyping relation defined here is the converse of the one
used in Igarashi and Kobayashi's generic type system~\cite{Kobayashi03TCS}.}
\fi
We define \(\newsubtype\) for only \emph{closed} types, i.e., those not containing
free type variables.

\begin{defi}[subtyping]
\label{def:subtype}
The subtyping relation \(\newsubtype\) on closed behavioral types is the largest
% precongruence
% preorder
relation such that \(A_1 \newsubtype A_2\) and \(A_1 \Tredwith{l} A_1'\)
implies \(A_2 \Tredswith{l} A_2'\) and \(A_1' \newsubtype A_2'\)
for some \(A_2'\).
%% such that the following conditions hold whenever \(A_1\subtype A_2\).
%% \begin{enumerate}
%% \item If \(A_2\Tredacc{x}{\acclab} A_2'\), then there exists \(A_1'\) such that
%%   \(A_1\Tredsacc{x}{\acclab}A_1'\) and \(A_1'\subtype A_2'\).
%% \item If \(A_2\Tredsilent^*\SPCONG A_2'\), then
%% there exists \(A_1'\) such that \(A_1\Tredsilent^*\SPCONG A_1'\) and \(A_1'\subtype A_2'\).
%% \end{enumerate}
\end{defi}
We often write \(A_1{\subtype} A_2\) for \(A_2{\newsubtype} A_1\),
and write \(A_1\eqtype A_2\) for \(A_1{\newsubtype} A_2\land A_2{\newsubtype} A_1\).

% \begin{defi}[subtyping]
% The subtyping relation \(\newsubtype\) on behavioral types is the largest precongruence
% such that the following conditions hold whenever \(A_1\newsubtype A_2\).
% \begin{enumerate}
% \item If \(A_1\Tredacc{x}{\acclab} A_1'\), then there exists \(A_2'\) such that
%   \(A_2\Tredsacc{x}{\acclab}A_2'\) and \(A_1'\subtype A_2'\).
% \item If \(A_1\Tredsilent^*\SPCONG A_1'\), then
% there exists \(A_2'\) such that \(A_2\Tredsilent^*\SPCONG A_2'\) and \(A_1'\subtype A_2'\).
% \end{enumerate}
% \end{defi}

\iffull
\begin{rem}
Note that the subtyping relation defined here is the converse of the one
used in Igarashi and Kobayashi's generic type system~\cite{Kobayashi03TCS}.
This is due to two different, dual views on behavioral types. Here, we think of
behavioral types as describing the behavior of processes. On the other hand,
Igarashi and Kobayashi~\cite{Kobayashi03TCS} think of behavioral types as
describing the assumption on the environment about what kind of process
is accepted by the environment. Because of this difference, they write
behavioral types on the lefthand side of \(\p\), and write \(A_1\& A_2\)
for non-deterministic choice instead of \(A_1\TOR A_2\).
\end{rem}
\fi
\begin{rem}
Depending on what property the type system should guarantee,
a finer subtyping relation may need to be chosen.
For example, the above definition allows\\
 \(
(\Tacc{W}{x}\Tzero) \TPAR (\Tacc{W}{x}\Tzero)  \newsubtype \Tacc{W}{x}\Tacc{W}{x}\Tzero\).
We may want to disallow this relation if we want to infer a property like
``no simultaneous writes on \(x\) can occur.''
\end{rem}

The following properties are satisfied by \(\newsubtype\). For proofs,
see Appendix~\ref{sec:app:subtyping}.
\begin{lem}\hfill
\label{le:subtyping-properties}
\begin{enumerate}
\item \(\newsubtype\) is a precongruence, i.e., \(\newsubtype\) is closed
under any behavioral type constructor.
\item If \(A_1\newsubtype A_2\), then \(\traces{x}{A_1}\subseteq \traces{x}{A_2}\)
for any \(x\).
\item \(B_1\TOR B_2\newsubtype A\)
if and only if \(B_1\newsubtype A\) and \(B_2\newsubtype A\) .
\item If \(\Tsubst{A}{\Tbvar}{B}\newsubtype B\), then
\(\Trec{\Tbvar}{A}\newsubtype B\).
\end{enumerate}
\end{lem}


\subsect{Typing}
\label{sec:typing-rules}

We consider two kinds of judgments, \(\Gamma\p v:\mvtype\) for
values, and \(\tjudge{\Gamma}{P}{A}\) for processes.
\(\Gamma\) is a mapping from a finite set of variables to value types.
In \(\tjudge{\Gamma}{P}{A}\),
 the type environment \(\Gamma\) describes the types of the variables,
and \(A\) describes the possible behaviors of \(P\).
For example, \(\tjudge{x\COL\Tchan{(b\COL\Tbool)\Tzero}}{P}{\Toutatom{x}\PAR\Toutatom{x}}\)
implies that \(P\) may send booleans along the channel \(x\) twice.
The judgment
\(\tjudge{y\COL\Tchan{(x\COL\Tchan{(b\COL\Tbool)\Tzero})\Toutatom{x}}}{Q}{\Tinatom{y}}\)
 means that \(Q\) may perform an input on \(y\) once, and then it may
send a boolean on the received value.
Note that in the judgment \(\tjudge{\Gamma}{P}{A}\),
the type \(A\) is an approximation of the behavior of \(P\) on free channels.
\(P\) may do less than what is specified by \(A\), but must not do more; for example,
\(\tjudge{x\COL\Tchan{(\,)\Tzero}}{\outatom{x}{\,}{}}{\Toutatom{x}\PAR\Toutatom{x}}\)
holds but
\(\tjudge{x\COL\Tchan{(\,)\Tzero}}{\outexp{x}{\,}{}\outatom{x}{\,}{}}{\Toutatom{x}}\)
does not. Because of this invariant, if \(A\) does not perform any invalid access, neither does \(P\).

We write \(\dom(\Gamma)\) for the domain of \(\Gamma\).
We write \(\emptyset\) for the empty type environment, and
write \(x_1\COL\tau_1,\ldots,x_n\COL\tau_n\) (where \(x_1,\ldots,x_n\) are distinct from
each other) for the type environment \(\Gamma\)
such that \(\dom(\Gamma) = \set{x_1,\ldots,x_n}\) and \(\Gamma(x_i) = \tau_i\) for each
\(i\in\set{1,\ldots,n}\).
When \(x\not\in \dom(\Gamma)\),  we write \(\Gamma,x\COL\tau\) for the type environment
\(\Delta\) such that \(\dom(\Delta) = \dom(\Gamma)\cup\set{x}\), \(\Delta(x)=\tau\),
and \(\Delta(y)=\Gamma(y)\) for \(y\in\dom(\Gamma)\). We define the \emph{value judgment}
relation $\Gamma\p v{:}\mvtype$ to be the least relation closed under
\[
 \Gamma,\, x{:}\mvtype \p x{:}\mvtype \qquad
 \Gamma \p \TRUE{:}\Tbool \qquad
 \Gamma \p \FALSE{:}\Tbool.
\]
We write \(\Gamma\p \seq{v}{:}\seq{\mvtype}\)
as an abbreviation for \((\Gamma\p v_1{:}\mvtype_1)\land \cdots \land (\Gamma\p v_n{:}\mvtype_n)\).


\begin{defi}
The type judgment relation \(\tjudge{\Gamma}{P}{A}\)
is the least relation closed under
the rules given in Figure~\ref{fig:typing}.
\end{defi}
We explain key rules below.

In rule \rname{T-Out}, the first premise \(\tjudge{\Gamma}{P}{A_2}\) implies that
the continuation of the output process behaves like \(A_2\), and
the second premise
    \({\Gamma} \p x\COL\Tchan{(\yy\COL\seq{\mvtype})A_1}\) implies that
 the tuple of values \(\seq{v}\) being sent may be used by an input process according to
\(\csubst{\seq{y}}{\seq{v}}A_1\).
Therefore, the whole behavior of the output process  is described by
\(\Tout{x}(\csubst{\yy}{\vv}A_1\PAR A_2)\). Here,
\(\csubstseq{v_1/x_1,\ldots,v_n/x_n}A\) stands for
\(\csubstseq{v_{i_1}/x_{i_1},\ldots,v_{i_k}/x_{i_k}}A\) where\\
\(\set{v_{i_1},\ldots,v_{i_k}} = \set{v_1,\ldots,v_n}\setdif\set{\TRUE,\FALSE}\).
For example,\(\csubstseq{\TRUE/x, y/z}A\) stands for \(\csubstseq{y/z}A\).
Note that, as in previous behavioral type systems~\cite{Kobayashi03TCS,Rehof02POPL},
the resource access and communications made on \(\seq{v}\) by the receiver of \(\seq{v}\)
are counted as the behavior of the output process (see Remark~\ref{rem:asymmetry-of-io}).

In rule \rname{T-In}, the first premise implies that the continuation of the input process
behaves like \(A_2\). Following previous behavioral type systems~\cite{Kobayashi03TCS,Rehof02POPL},
we split \(A_2\) into two parts: \(\project{A_2}{\set{\seq{y}}}\) and
\(\exclude{A_2}{\set{\seq{y}}}\).
The first part describes the behavior on the received values \(\seq{y}\) and is taken into
account in the channel type. The second part describes the resource access and communications
performed on other values, and is taken into account in
the behavioral type of the input process.
The condition \(\project{A_2}{\set{\yy}}\newsubtype A_1 \) requires that
the access and communication behavior on \(\seq{y}\) conforms to
\(A_1\), the channel arguments' behavior.

%In \rname{T-Par}, the premises imply that \(P_1\) and \(P_2\) behave like
% \(A_1\) and \(A_2\), so that \(P_1\PAR P_2\) behaves like \(A_1\TPAR A_2\).
%% Lucian -- this is obvious and not needed.


In  \rname{T-New}, the premise implies that \(P\) behaves like \(A\),
so that \(\nuexp{x}P\) behaves like \(\Thiding{x}{A}\).
Here, we only require that \(x\) is a channel, unlike in the previous
behavioral type systems for the \(\pi\)-calculus~\cite{Kobayashi03TCS,Kobayashi05ActInf}.
That is because we are only interested in the resource access behavior; the communication
behavior is used only for accurately inferring the resource access behavior.

In \rname{T-NewR}, we check that the process's behavior \(A\) conforms to the
resource usage specification \(\spec\).

Rule \rname{T-Sub} allows the type \(A'\) of a process to be replaced by
its approximation \(A\).

We remark that weakening of $\Gamma$ can be derived (Appendix~\ref{sec:app:subject-reduction},
Lemma~\ref{le:weakening}) and so is not needed as a rule.


\iftwocol
\begin{figure}
\else
\begin{figure}
\fi
\begin{center}
\fbox{\small
\iftwocol
\begin{minipage}{\hfigwidth} %[t]{8cm}
\else
\begin{minipage}{14.5 cm} %{17cm}
\fi
\typicallabel{T-Zero}

%\textbf{judgment for processes}
\infax[T-Zero]
            {\tjudge{\Gamma}{\zeroexp}{\Tzero}}

\rulesp{}

\infrule[T-Out]
%  {\tjudge{\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}{P}{A_2}\\
%%%     \Gamma \p v_i\COL{}\mvtype_i \mbox{ for each $i\in\{1,\ldots,n\}$}}
%   \Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1} \p \seq{v}\COL{}\seq{\mvtype}}
%  {\Gamma, x\COL{}\Tchan{(\seq{y}\COL{}\seq{\mvtype})A_1};
%    \Tout{x}(\csubst{\seq{y}}{\seq{v}}A_1\PAR A_2) \p
%     \outexp{x}{\seq{v}}{}P}
% LU: I removed the Gamma,x:t notation, and changed into Gamma\x notation like in the SD-rules.
   {\tjudge{\Gamma}{P}{A_2} \quad
    {\Gamma} \p x\COL\Tchan{(\yy\COL\seq{\mvtype})A_1} \quad
    \Gamma \p \vv\COL{}\seq{\mvtype}}
   {\tjudge{\Gamma}{\outexp{x}{\vv}{}P}{\Tout{x}(\csubst{\yy}{\vv}A_1\PAR A_2)}}

\rulesp{}

\infrule[T-In]
%   {\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1},
%    \seq{y}\COL\seq{\mvtype}; A_2 \p P\\
%    A_1 \subtype \project{A_2}{\set{\seq{y}}}
%%%    \andalso  \set{x_1,\ldots,x_n}\cap \FV(\Gamma) = \emptyset
%   }
%   {\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1};
%       \Tin{x}(\exclude{A_2}{\set{\seq{y}}})
%         \p \inexp{x}{\seq y}{}P}
%%%   {\InTE{x}{\typ{\seq y}{(\project{\Gamma}{\set{\seq y}})}}{\ev}
%%%       {(\exclude{\Gamma}{\set{\seq y}})}
%%%         \p \inexp{x}{\seq y}{\ev}P}
% LU: Again, I removed the Gamma,x notation
   {\tjudge{\Gamma, \yy\COL\seq{\mvtype}}{P}{A_2} \quad
    \Gamma \p x\COL{}\Tchan{(\yy\COL\seq{\mvtype})A_1} \quad
    \project{A_2}{\set{\yy}}\newsubtype A_1
    }
   {\tjudge{\Gamma}{\inexp{x}{\yy}{}P}{\Tin{x}(\exclude{A_2}{\set{\yy}})} }

\rulesp{}

\infrule[T-Par]
   {\tjudge{\Gamma}{P_1}{A_1}\andalso \tjudge{\Gamma}{P_2}{A_2}}
   {\tjudge{\Gamma}{P_1\PAR P_2}{A_1\TPAR{}A_2}}

\rulesp{}

\infrule[T-Rep]
   {\tjudge{\Gamma}{P}{A}}
   {\tjudge{\Gamma}{\repexp{P}}{\Trep{A}}}

\rulesp{}

\infrule[T-If]
  {\Gamma\p v\COL{}\Tbool\andalso \tjudge{\Gamma}{P}{A} \andalso \tjudge{\Gamma}{Q}{A}}
  {\tjudge{\Gamma}{\ifexp{v}{P}{Q}}{A}}

\rulesp{}

\infrule[T-New]
   {\tjudge{\Gamma, x\COL{}\Tchan{(\seq{y}\COL\seq{\mvtype})A_1}}{P}{A_2}
%%%    \andalso x\not\in \FV(\Gamma)
    }
%   {\tjudge{\Gamma}{\nuexp{x}P}{\Thiding{x}A_2}}
% LU: again I removed Gamma,x notation
%%%    {\Gamma; A_2 \p P \andalso
%%%     \Gamma \p x\COL{}\Tchan{(\yy\COL\seq{\mvtype})A_1}}
    {\tjudge{\Gamma}{\nuexp{x}P}{\Thiding{x}A_2}}

\rulesp{}

\infrule[T-Acc]
%  {\Gamma, x\COL\Tres; A \p P}
%  {\Gamma, x\COL\Tres; \Tacc{\acclab}{x}A \p \accexp{\acclab}{x}P}
% LU: again I removed Gamma,x notation
   {\tjudge{\Gamma}{P}{A}\andalso
    \Gamma \p x\COL\Tres}
   {\tjudge{\Gamma}{\accexp{\acclab}{x}P}{\Tacc{\acclab}{x}A} }

\rulesp{}

\infrule[T-NewR]
  {\tjudge{\Gamma, x\COL\Tres}{P}{A}\andalso \traces{x}{A} \subseteq {\spec}}
  {\tjudge{\Gamma}{\nurexp{x}{\spec}P}{\exclude{A}{\set{x}}}}

\rulesp{}

\infrule[T-Sub]
  {\tjudge{\Gamma}{P}{A'}\andalso A' \newsubtype A}
  {\tjudge{\Gamma}{P}{A}}

%\textbf{judgment for values}
%\infax[T-Var]{\Gamma, x\COL\mvtype \p x\COL{}\mvtype}
%\infrule[T-Bool]{b\in \set{\TRUE,\FALSE}}{\Gamma \p b\COL{} \Tbool}
%LU: I have moved these into the text
\end{minipage}
}
\caption{Typing Rules}
\label{fig:typing}
\end{center}
\iftwocol
\end{figure}
\else
\end{figure}
\fi

The following example shows how information about the usage of resources by an input process
is propagated to an output process.
\begin{exa}
Let us consider \(\nurexp{x}{\spec}P\), where 
\[
\begin{array}{l}
\spec=\prefixclos{R^*C}\\
P = \nuexp{y}(\outatom{y}{x,x}{}\PAR \inexp{y}{z_1,z_2}{}\Read(z_1).\Close(z_2)).
\end{array}
\]

Let \(\Gamma = y\COL \Tchan{(z_1,z_2)\Tacc{R}{z_1}\Taccatom{C}{z_2}}, x\COL\Tres\).
Then, the following judgment holds for the output and input processes.
\[
\begin{array}{l}
\tjudge{\Gamma }{\outatom{y}{x,x}{}}{\Tout{y}
   {\Tacc{R}{x}\Taccatom{C}{x}}}\\
\tjudge{\Gamma}{\inexp{y}{z_1,z_2}{}\Read(z_1).\Close(z_2)}{\Tin{y}\Tzero}
\end{array}
\]
Here, we have used subtyping relations
\(\csubstseq{x/z_1,x/z_2}\Tacc{R}{z_1}\Taccatom{C}{z_2}
\eqtype \Tacc{R}{x}\Taccatom{C}{x}\) and
\(\exclude{\Tacc{R}{z_1}\Taccatom{C}{z_2}}{\set{z_1,z_2}}\eqtype \Tzero\).
%
By using \rname{T-Par} and \rname{T-New}, we obtain
\[\tjudge{x\COL\Tres}{P}
  {\Thiding{y}(\Tout{y}{\Tacc{R}{x}\Taccatom{C}{x}}\TPAR \Tinatom{y})}\]
Using \rname{T-Sub} with $\Thiding{y}(\Tout{y}{\Tacc{R}{x}\Taccatom{C}{x}}\TPAR \Tinatom{y}) \eqtype \Tacc{R}{x}\Taccatom{C}{x}$ we get
\[\tjudge{x\COL\Tres}{P}{\Tacc{R}{x}\Taccatom{C}{x}}\]
%
Since \(\traces{x}{\Tacc{R}{x}\Taccatom{C}{x})} \subseteq \prefixclos{{R^*C}}\),
we obtain
\(\tjudge{\emptyset}{\nurexp{x}{\spec}P}{\Tzero}\)
by using \rname{T-NewR} and \rname{T-Sub}.
\eoe{}
\end{exa}

\begin{exa} \label{ex:typing-repeatread}
Recall Example~\ref{ex:repeatread}:
\begin{eqnarray*}
 P & \!\!=\!\! &  \nuexp{s}(\repexp\inexp{s}{n,x,r}{}P_1\ \PAR\ \nurexp{x}{\spec}P_2) \\
 P_1 & \!\!=\!\! & \IF\ n=0\ \THEN\ \outatom{r}{}{}\\
     &           &  \ELSE\ \nuexp{r'}(\outatom{\repread}{n-1,x,r'}{} \PAR \inexp{r'}{}{}\Read(x).\outatom{r}{}{}) \\
 P_2 & \!\!=\!\! & \nuexp{r}(\Init(x).\outatom{\repread}{100,x,r}{} \PAR \inexp{r}{}{}\Close(x) ) \\
 \spec & \!\!=\!\! & \prefixclos{IR^*C}
\end{eqnarray*}
Let $A_1 = \mu\alpha.(\Toutatom{r} \TOR \nuexp{r'}(\csubst{r}{r'}\alpha | \Tin{r'}\Tacc{R}{x}\Toutatom{r})$ and \\
let $\Gamma = s{:}\Tchan{(n{:}\textbf{int},\, x{:}\Tres,\, r{:}\Tchan{})\,A_1}$. Then
\begin{eqnarray*}
 & & \tjudge{\Gamma, n{:}\Tint, x{:}\Tres, r{:}\Tchan{}}{P_1}{A_1} \\
 & & \tjudge{\Gamma}{\repexp\inexp{s}{n,x,r}{}P_1}{\repexp\Tin{s}(\exclude{A_1}{\{n,x,r\}}) \eqtype \repexp\Tinatom{s}} \\
 & & \tjudge{\Gamma}{P_2}{\nuexp{r}(\Tacc{I}{x}A_1 | \Tin{r}\Taccatom{C}{x})}
\end{eqnarray*}
So long as $\traces{x}{\nuexp{r}(\Tacc{I}{x}A_1 | \Tin{r}\Taccatom{C}{x})} \subseteq \spec$, we obtain
$\tjudge{\emptyset}{P}{\textbf{0}}$. See Section~\ref{sec:constraint-solving} for the algorithm
that establishes $\traces{x}{\cdot} \subseteq \spec$.
\eoe{}
\end{exa}
\begin{rem}
\label{rem:combination-of-hiding-and-renaming}
The type \(A_1\) in the example above demonstrates how
recursion, hiding, and renaming are used together.
In general, in order to type a recursive process of the form
\(\repexp\inexp{s}{x}{}\nuexp{y}{(\cdots \outatom{s}{y}{}\cdots)}\),
we need to find a type that satisfies
\(\Thiding{y}{(\cdots \Tren{A}{x}{y}\cdots)}\newsubtype A\).
Moreover, for the type inference (in Section~\ref{sec:inference}),
we must find the \emph{least} such \(A\). Thanks to the type constructors for
recursion, hiding, and renaming, we can always do that: \(A\) can be
expressed by \(\Trec{\Tbvar}{\Thiding{y}{(\cdots\csubst{x}{y}\Tbvar\cdots)}}\)
(recall Lemma~\ref{le:subtyping-properties}.4).
\end{rem}

\begin{rem}
\label{rem:asymmetry-of-io}
A reader may wonder why the rules \rname{T-Out} and \rname{T-In} are asymmetric, in the sense
that information about the continuation of a receiver process is transferred to a sender process
but not vice versa. That design choice comes from the observation that a channel or resource
exchanged between a sender and a receiver are, in general, statically known only to the sender,
so that we have to put information about the behavior on the channel or resource
into the type of the sender.
For example, consider the process \((\nuexp{y}(\outatom{x}{y}{}\PAR \cdots)
\PAR \inexp{x}{z}{}\outatom{z}{\,}{}\).
Since the receiver \(\inexp{x}{z}{}\outatom{z}{\,}{}\) is not in the scope of \(y\),
we have to put the information that \(y\) will be used for output
into the type of the sender \(\outatom{x}{y}{}\)
(as \(\Tout{x}\Toutatom{y}\)).
It is still useful and possible to recover the symmetry in the treatment of senders and receivers
to some extent: see Section~8 of our previous paper~\cite{Kobayashi03TCS}.
\end{rem}



==> memo.tex <==
\section{Memorandum}

\subsection*{About Section~\protect\ref{sec:typing}}
\begin{memo}
If we defined \(\FV(\Gamma)\) as the set of *syntactically* free variables,
\(\exclude{\appty{\tau}{\seq x}}{\seq x}\) always contain
\(\seq x\), so \rname{T-New} cannot be applied.
(An alternative solution would be to introduce appropriate 
subtyping rules, so that if \(\Gamma\) contains no semantic
occurrence of a variable \(x\), \(\Gamma\) can be replaced by
some process type \(\Gamma'\) that contains no syntactic
occurrences of \(x\).
\end{memo}
\begin{memo}
The above definition does not work for non-semi-closed types:
Consider 
\(\tau = \recTE{\tv}{\absty{x}{(\InTE{x}{\,}{\ev}\InTE{y}{\tv}{\ev'}
             \appty{\tv}{x})}}\).
If we applied the above definition to non-semi-closed types,
we would get:
\(\project{\tau}{y} = \recTE{\tv}{\absty{x}{(\evTE{\ev}\InTE{y}{\tv}{\ev'}
             \appty{\tv}{x})}}\).
So, the type of a value received on \(y\) is changed.
We can relax a little the restriction (that the operations can be applied
only to semi-closed types) by memorizing which type variable is bound
by \(\mu\):
\begin{eqnarray*}
\project{\Gamma}{S} &=& \prjsub{\Gamma}{S}{\emptyset}\\
\prjsub{\zeroTE}{S}{V} &=& \zeroTE\\
\prjsub{(\InTE{x}{\tau}{\ev}\PrTy)}{S}{V} &=&
   \left\{
     \begin{array}{ll}
        \InTE{x}{\tau}{\ev}{(\prjsub{\PrTy}{S}{V})}
              & \mbox{if }x\in S\land V\cap \FV(\tau)=\emptyset\\
        \evTE{\ev}{(\prjsub{\PrTy}{S}{V})}
              & \mbox{if }x\not\in S
     \end{array}
   \right.\\
\prjsub{(\OutTE{x}{\tau}{\ev}\PrTy)}{S}{V} &=&
   \left\{
     \begin{array}{ll}
        \OutTE{x}{\tau}{\ev}{(\prjsub{\PrTy}{S}{V})}
              & \mbox{if }x\in S\land V\cap \FV(\tau)=\emptyset\\
        \evTE{\ev}{(\prjsub{\PrTy}{S}{V})}
              & \mbox{if }x\not\in S
     \end{array}
   \right.\\
\prjsub{(\evTE{\ev}{\PrTy})}{S}{V}
    &=& \evTE{\ev}{(\prjsub{\PrTy}{S}{V})}\\
\prjsub{(\GPrTy_1\TEOR\cdots\TEOR \GPrTy_n)}{S}{V}
    &=& (\prjsub{\GPrTy_1}{S}{V})\TEOR 
       \cdots\TEOR (\prjsub{\GPrTy_n}{S}{V})\\
\prjsub{(\PrTy_1\TEPAR\PrTy_2)}{S}{V} 
    &=& (\prjsub{\PrTy_1}{S}{V})\TEPAR (\prjsub{\PrTy_2}{S}{V})\\
\prjsub{(\PrTy_1\TEIOR\PrTy_2)}{S}{V} 
    &=& (\prjsub{\PrTy_1}{S}{V})\TEIOR (\prjsub{\PrTy_2}{S}{V})\\
\prjsub{(\appty{\tau}{\seq x})}{\{\seq y\}}{V} &=&
 \appty{(\prjsub{\tau}{S\cup S'}{V})}{\seq x}\\
 & &\mbox{ where }S' = \set{i | x_i \in S}\\
 & & \appty{\prjsub{\tau}{S}{V}}{\subst{\seq{y}}{\seq{\ig}}{\seq x}}
     \mbox{ is incorrect:}\\
 & & \mbox{We should not replace inner $x_i$ with    $\ig$}\\
\prjsub{\tv}{S}{V} &=& 
   \left\{\begin{array}{ll}
          \tv & \mbox{if $\tv\in\dom(V)$}\\
           \mbox{undefined} & \mbox{otherwise}
          \end{array}
    \right.\\
\prjsub{(\absty{\seq x}\Gamma)}{S}{V} &=&
    \absty{\seq x}{(\prjsub{\Gamma}{S'}{V})}\\
  & & \mbox{where }S' = (S\setdif\Nat)\cup \{x_i \mid i\in S\}\\
\prjsub{(\recTE{\tv}{\tau})}{S}{V}
    &=& \recTE{\tv}{(\prjsub{\tau}{S}{V\cup \set{\tv}})}\\
%%\ \\
\exclude{\PrTy}{S} &=& \project{\PrTy}{\VAR\setdif S}
\end{eqnarray*}

Anyway, the operations are partial even on semi-closed types:  
the projection is not defined for a recursive type
of the form \(\recty{\tv}{(...[\tv]...)}\).
We assume that before projections are applied, types are
transformed appropriately. For example, 
\(\recty{\tv}{(...[\tv]...)}\) should be transformed into
\(\recty{\tv}{(...[\recty{\tv}{(...[\tv]...)}]...)}\) beforehand.
To deal with a type like 
\(\recty{\tv}{(...[\tv]...\tv...)}\),
we need to refine subtyping rules. One candidate is:
\(\recTE{\tv}{\tau} = \recTE{\tv}{\tau'}\)
where \(\tau'\) is a type obtained by replacing *some* occurrences of
\(\tv\) in \(\tau\) with \(\recTE{\tv}{\tau}\).
%%%\begin{eqnarray*}
%%%\project{\Gamma}{S} &=& \prjsub{\Gamma}{S}{\nullfun}\\
%%%\prjsub{\zeroTE}{S}{\tmap} &=& \zeroTE\\
%%%\prjsub{(\InTE{x}{\tau}{\ev}\PrTy)}{S}{\tmap} &=&
%%%   \left\{
%%%     \begin{array}{ll}
%%%        \InTE{x}{\tmap\tau}{\ev}{(\prjsub{\PrTy}{S}{\tmap})}
%%%              & \mbox{if }x\in S\\
%%%        \evTE{\ev}{(\prjsub{\PrTy}{S}{\tmap})}
%%%              & \mbox{otherwise}
%%%     \end{array}
%%%   \right.\\
%%%\prjsub{(\OutTE{x}{\tau}{\ev}\PrTy)}{S}{\tmap} &=&
%%%   \left\{
%%%     \begin{array}{ll}
%%%        \OutTE{x}{\tmap\tau}{\ev}{(\prjsub{\PrTy}{S}{\tmap})}
%%%              & \mbox{if }x\in S\\
%%%        \evTE{\ev}{(\prjsub{\PrTy}{S}{\tmap})}
%%%              & \mbox{otherwise}
%%%     \end{array}
%%%   \right.\\
%%%\prjsub{(\evTE{\ev}{\PrTy})}{S}{\tmap}
%%%    &=& \evTE{\ev}{(\prjsub{\PrTy}{S}{\tmap})}\\
%%%\prjsub{(\GPrTy_1\TEOR\cdots\TEOR \GPrTy_n)}{S}{\tmap}
%%%    &=& (\prjsub{\GPrTy_1}{S}{\tmap})\TEOR 
%%%       \cdots\TEOR (\prjsub{\GPrTy_n}{S}{\tmap})\\
%%%\prjsub{(\PrTy_1\TEPAR\PrTy_2)}{S}{\tmap} 
%%%    &=& (\prjsub{\PrTy_1}{S}{\tmap})\TEPAR (\prjsub{\PrTy_2}{S}{\tmap})\\
%%%\prjsub{(\PrTy_1\TEIOR\PrTy_2)}{S}{\tmap} 
%%%    &=& (\prjsub{\PrTy_1}{S}{\tmap})\TEIOR (\prjsub{\PrTy_2}{S}{\tmap})\\
%%%\prjsub{(\appty{\tau}{\seq x})}{\{\seq y\}}{\tmap} &=&
%%% \appty{(\prjsub{\tau}{S\cup S'}{\tmap})}{\seq x}\\
%%% & &\mbox{ where }S' = \set{i | x_i \in S}\\
%%% & & \appty{\prjsub{\tau}{S}{\tmap}}{\subst{\seq{y}}{\seq{\ig}}{\seq x}}
%%%     \mbox{ is incorrect:}\\
%%% & & \mbox{We should not replace inner $x_i$ with    $\ig$}\\
%%%\prjsub{\tv}{S}{\tmap} &=& 
%%%   \left\{\begin{array}{ll}
%%%          \tv & \mbox{if $\tv\in\dom(\tmap)$}\\
%%%           \mbox{undefined} & \mbox{otherwise}
%%%          \end{array}
%%%    \right.\\
%%%\prjsub{(\absty{\seq x}\Gamma)}{S}{\tmap} &=&
%%%    \absty{\seq x}{(\prjsub{\Gamma}{S'}{\tmap})}\\
%%%  & & \mbox{where }S' = (S\setdif\Nat)\cup \{x_i \mid i\in S\}\\
%%%\prjsub{(\recTE{\tv}{\tau})}{S}{\tmap}
%%%    &=& \recTE{\tv}{(\prjsub{\tau}{S}{\subst{\tv}{\tau}\comp\tmap})}\\
%%%%%\ \\
%%%\exclude{\PrTy}{S} &=& \project{\PrTy}{\VAR\setdif S}
%%%\end{eqnarray*}
%%\]
\end{memo}

The following operation is probably not necessary.
\begin{defn}[combination of types]
The binary operation \(\Tcomb\) on semi-closed process and tuple
types is defined by:
\begin{eqnarray*}
\zeroTE \Tcomb \zeroTE &=& \zeroTE\\
\OutTE{x}{\tau}{\ev}\Gamma_1 \Tcomb \evTE{\ev}\Gamma_2
&=& \OutTE{x}{\tau}{\ev}{(\Gamma_1\Tcomb \Gamma_2)}\\
\evTE{\ev}\Gamma_1\Tcomb \OutTE{x}{\tau}{\ev}\Gamma_2
   &=& \OutTE{x}{\tau}{\ev}{(\Gamma_1\Tcomb \Gamma_2)}\\
\InTE{x}{\tau}{\ev}\Gamma_1 \Tcomb \evTE{\ev}\Gamma_2
&=& \InTE{x}{\tau}{\ev}{(\Gamma_1\Tcomb \Gamma_2)}\\
\evTE{\ev}\Gamma_1\Tcomb \InTE{x}{\tau'}{\ev}\Gamma_2
   &=& \InTE{x}{\tau}{\ev}{(\Gamma_1\Tcomb \Gamma_2)}\\
\evTE{\ev}{\Gamma_1}\Tcomb \evTE{\ev}{\Gamma_2} &=& 
   \evTE{\ev}{(\Gamma_1\Tcomb \Gamma_2)}\\
(\gamma_1\TEOR\cdots\TEOR\gamma_n)\Tcomb
  (\gamma_1'\TEOR\cdots\TEOR\gamma_n')
 &=& (\gamma_1\Tcomb\gamma_1')\TEOR\cdots \TEOR (\gamma_n\Tcomb\gamma_n')\\
(\Gamma_1\TEPAR\Gamma_2)\Tcomb(\Gamma_1'\TEPAR\Gamma_2')&=&
  (\Gamma_1\Tcomb\Gamma_1')\TEPAR(\Gamma_2\Tcomb\Gamma_2')\\
(\Gamma_1\TEIOR\Gamma_2)\Tcomb(\Gamma_1'\TEIOR\Gamma_2')&=&
  (\Gamma_1\Tcomb\Gamma_1')\TEIOR(\Gamma_2\Tcomb\Gamma_2')\\
(\appty{\tau_1}{\seq x})\Tcomb(\appty{\tau_2}{\seq x}) &=&
   \appty{(\tau_1\Tcomb\tau_2)}{\seq x}\\
\ \\
\tv\Tcomb \tv &=& \tv\\
(\absty{\seq x}\Gamma_1)\Tcomb(\absty{\seq x}\Gamma_2) &=&
   \absty{\seq x}{(\Gamma_1\Tcomb\Gamma_2)}\\
(\recTE{\tv}{\tau_1})\Tcomb (\recTE{\tv}{\tau_2}) &=&
  \recTE{\tv}{(\tau_1\Tcomb \tau_2)}
%%%\Gamma_1\Tcomb{}\Gamma_2 &=& \Gamma_1\Tcomb{\emptyset}\Gamma_2\\
%%%\zeroTE \Tcsub{V} \zeroTE &=& \zeroTE\\
%%%\OutTE{x}{\tau}{\ev}\Gamma_1 \Tcsub{V} \evTE{\ev}\Gamma_2
%%%&=& \OutTE{x}{\tau}{\ev}{(\Gamma_1\Tcsub{V} \Gamma_2)}\\
%%% & & \mbox{ if $V\cap \FV(\tau)=\emptyset$}\\
%%%\evTE{\ev}\Gamma_1\Tcsub{V} \OutTE{x}{\tau}{\ev}\Gamma_2
%%%   &=& \OutTE{x}{\tau}{\ev}{(\Gamma_1\Tcsub{V} \Gamma_2)}\\
%%% & & \mbox{ if $V\cap \FV(\tau)=\emptyset$}\\
%%%\InTE{x}{\tau}{\ev}\Gamma_1 \Tcsub{V} \evTE{\ev}\Gamma_2
%%%&=& \InTE{x}{\tau}{\ev}{(\Gamma_1\Tcsub{V} \Gamma_2)}\\
%%% & & \mbox{ if $V\cap \FV(\tau)=\emptyset$}\\
%%%\evTE{\ev}\Gamma_1\Tcsub{V} \InTE{x}{\tau'}{\ev}\Gamma_2
%%%   &=& \InTE{x}{\tau}{\ev}{(\Gamma_1\Tcsub{V} \Gamma_2)}\\
%%% & & \mbox{ if $V\cap \FV(\tau)=\emptyset$}\\
%%%\evTE{\ev}{\Gamma_1}\Tcsub{V} \evTE{\ev}{\Gamma_2} &=& 
%%%   \evTE{\ev}{(\Gamma_1\Tcsub{V} \Gamma_2)}\\
%%% & & \mbox{ if $V\cap \FV(\tau)=\emptyset$}\\
%%%(\gamma_1\TEOR\cdots\TEOR\gamma_n)\Tcsub{V}
%%%  (\gamma_1'\TEOR\cdots\TEOR\gamma_n')
%%% &=& (\gamma_1\Tcsub{V}\gamma_1')\TEOR\cdots \TEOR (\gamma_n\Tcsub{V}\gamma_n')\\
%%%(\Gamma_1\TEPAR\Gamma_2)\Tcsub{V}(\Gamma_1'\TEPAR\Gamma_2')&=&
%%%  (\Gamma_1\Tcsub{V}\Gamma_1')\TEPAR(\Gamma_2\Tcsub{V}\Gamma_2')\\
%%%(\Gamma_1\TEIOR\Gamma_2)\Tcsub{V}(\Gamma_1'\TEIOR\Gamma_2')&=&
%%%  (\Gamma_1\Tcsub{V}\Gamma_1')\TEIOR(\Gamma_2\Tcsub{V}\Gamma_2')\\
%%%(\appty{\tau_1}{\seq x})\Tcsub{V}(\appty{\tau_2}{\seq x}) &=&
%%%   \appty{(\tau_1\Tcsub{V}\tau_2)}{\seq x}\\
%%%\ \\
%%%\tv\Tcsub{V} \tv &=& 
%%%   \left\{\begin{array}{ll}
%%%          \tv & \mbox{if $\tv\in V$}\\
%%%           \mbox{undefined} & \mbox{otherwise}
%%%          \end{array}
%%%    \right.\\
%%%(\absty{\seq x}\Gamma_1)\Tcsub{V}(\absty{\seq x}\Gamma_2) &=&
%%%   \absty{\seq x}{(\Gamma_1\Tcsub{V}\Gamma_2)}\\
%%%(\recTE{\tv}{\tau_1})\Tcsub{V} (\recTE{\tv}{\tau_2}) &=&
%%%  \recTE{\tv}{(\tau_1\Tcsub{V\cup\set{\tv}} \tau_2)}
\end{eqnarray*}
\end{defn}
%%%The operation \(\TEcomb\) merges two types, by 
%%%matching the corresponding actions of \(\tau_1\) and \(\tau_2\).
%%%For example, if
%%%\(\tau_1=\evty{\ev}\outty{1}{\tau}{\ev'}{m}\zeroty\) and
%%%\(\tau_2=\inty{2}{\tau}{\ev}{m}\evty{\ev'}\zeroty\),
%%%\(\tau_1\TEcomb\tau_2\) is computed as
%%%\(\inty{2}{\tau}{\ev}{m}\outty{1}{\tau}{\ev'}{m}\zeroty\)
%%%by matching ``\(\evty{\ev}\)'' with ``\(\inty{2}{\tau}{\ev}{m}\)''
%%%and ``\(\outty{1}{\tau}{\ev'}{m}\)'' with ``\(\evty{\ev'}\)''.
%%%As this example shows,
%%%if \(\tau_1\TEcomb\tau_2=\tau_3\) holds, \(\tau_1\TPAR\tau_2\) 
%%%expresses a more liberal usage of values than \(\tau_3\). 
%%%That is why we define \(\tau_1\TPAR\tau_2\) to be a subtype of \(\tau_3\)
%%%below.
%%\(\exclude{\tau}{S}\) abstracts out the behavior on the channels
%%indexed by \(S\).
%%%As the above example shows,
%%%if \(\tau_1\TEcomb\tau_2=\tau_3\) holds, \(\tau_1\TPAR\tau_2\) 
%%%expresses a more liberal use than \(\tau_3\): In the above example,
%%%\(\tau_3\) indicates that the first element of a tuple can be used
%%%for output only after the second element is used for input, while
%%%\(\tau_1\TPAR\tau_2\) requires only that some action annotated with
%%%\(\ev\) (which may not be an input on the second element) must occur
%%%before the first element can be used for output. 


==> modal-logic.tex <==
\section{Modal logic}

\subsection{Syntax}
\[
\begin{array}{lcll}
A &::=& \PLTRUE \mid \PLsometr{\redlab}A \mid \PLout{x}{\ev}{n}\mid  \PLin{x}{\ev}{n}
       \mid (A\PAR B)\\
  & &  \mid \neg A \mid A\lor B \mid \eventual(A) \mid \exists x.A \mid
      \exists \ev.A \mid \exists i:C.A\\
%%%   & & \ERROR\\
%%%   & & \alpha\\
%%%   & & \neg A\\
%%%   & & \PLsometr{l}A\\
%%%   & & \PLout{x}{\ev}{n}\\
%%%   & & \PLin{x}{\ev}{n}\\
%%%   & & A\PAR B\\
%%%   & & (x)A & \mbox{For some local channel $x$, $A$ holds}\\
%%%   & & \nu\alpha.A   &\mbox{Greatest fixpoint}
\end{array}
\]

\paragraph{Abbreviations}
\begin{itemize}
\item \(\PLanytr{\redlab}A\equiv \neg\PLsometr{\redlab}\neg A\)
\item \(inv(A) \equiv  \neg \eventual(\neg A)\)
%%\item \(inv(A) \equiv \nu \alpha.([-]\alpha\land A)\)
%%\item \(\eventual(A) \equiv \mu \alpha.(\PLsometr{-}\alpha \lor A)\)
\item \(\PLsometr{-}A \equiv 
    \exists x.\exists \ev.\exists \ev'.(\PLsometr{x^{\ev,\ev'}}A \lor 
    \PLsometr{\epsilon^{\ev,\ev'}})\)
\item \(\ERROR \equiv \exists x.\exists \ev.\exists \ev'.
    \exists i.\exists j:i\neq j.(\PLout{x}{\ev}{m}\PAR \PLin{x}{\ev}{n})\)
\end{itemize}
\(\ERROR\) means that there is an immediate arity mismatch on free channels.

\paragraph{Properties}
\begin{itemize}
\item lack of arity mismatch\\
  \(\neg \eventual(\ERROR)\)
\item lack of race on \(\ev\)\\
  \(\neg ev (\exists x.\exists \ev'.\exists i,j.
    (\PLout{x}{\ev}{i} \PAR \PLout{x}{\ev'}{j}))\)
\item lack of deadlock\\
  \(\neg \eventual(\PLout{x}{\ev}{i}\land \neg\PLsometr{-}\TRUE))\)
\item garbage-channel collection\\
  \(\neg \eventual(\PLsometr{x^{\ev,\ev'}}\eventual(\PLout{x}{\ev}{i}\lor \PLin{x}{\ev}{j}))\) \\
\end{itemize}

\subsection{Semantics}
\begin{defn}[semantics of process logic]
The model \(\semPF{A}\) (the set of processes satisfying \(A\)) is defined by:
\[
\begin{array}{lcl}
\semPF{\TRUE} = \PSET\\
\semPF{\PLsometr{\redlab}A} = \set{P \mid P\redwith{\redlab}Q, Q\in \semPF{A}}\\
\semPF{\PLout{x}{\ev}{n}} = \set{P \mid 
    P\SCONG \nuexp{\seq{x_1}}\cdots \nuexp{\seq{x_n}}
   (\cdots+\outexp{x}{y_1,\ldots,y_n}{\ev}Q+\cdots\PAR R), 
    x\not\in\set{\seq{x_1},\ldots,\seq{x_n}}}\\
\semPF{\PLin{x}{\ev}{n}} = \set{P \mid 
    P\SCONG \nuexp{\seq{x_1}}\cdots \nuexp{\seq{x_n}}
   (\cdots+\inexp{x}{y_1,\ldots,y_n}{\ev}Q+\cdots \PAR
    R), x\not\in\set{\seq{x_1},\ldots,\seq{x_n}}}\\
\semPF{A\PAR B} = \set{P \mid P\SCONG \nuexp{\seq{x_1}}\cdots \nuexp{\seq{x_n}}(Q\PAR R), 
      Q\in\semPF{A}, R\in\semPF{B}, \{\seq{x_1},\ldots,\seq{x_n}\}\cap \FV(A\PAR B)
    = \emptyset}\\
\semPF{\neg A} = \PSET\setdif \semPF{A}\\
\semPF{A\lor B} = \semPF{A}\cup \semPF{B}\\
\semPF{\eventual(A)} = \set{P \mid P\red^* Q, Q\in \semPF{A}}\\
\semPF{\exists x.A} = \set{P \mid \exists x.(P \in \semPF{A})}\\
\semPF{\exists \ev.A} = \set{P \mid \exists \ev.(P \in \semPF{A})}
\end{array}
\]
We write \(P\models A\) if \(P\in \semPF{A}\).
\end{defn}

\begin{defn}[semantics of type logic]
The model \(\semTF{A}\) (the set of types satisfying \(A\)) is defined by:
\[
\begin{array}{lcl}
\semTF{\TRUE} = \TSET\\
\semTF{\PLsometr{\redlab}A} = \set{\Gamma \mid \Gamma\redwith{\labPtoT{\redlab}}Q, 
                                    Q\in \semTF{A}}\\
\semTF{\PLout{x}{\ev}{n}} = \set{P \mid 
    \Gamma\subTE \cdots+\outTE{x}{\tau}{\ev}{n}\Delta_1+\cdots\TEPAR \Delta_2}\\
\semTF{\PLin{x}{\ev}{n}} = \set{P \mid 
    \Gamma\subTE \cdots+\inTE{x}{\tau}{\ev}{n}\Delta_1+\cdots\TEPAR \Delta_2}\\
\semTF{A\PAR B} = \set{\Gamma \mid 
   \Gamma\subTE \Delta_1\TEPAR\Delta_2, \Delta_1\in \semTF{A}, \Delta_2\in \semTF{B}}\\
\semTF{\neg A} = \TSET\setdif \semTF{A}\\
\semTF{A\lor B} = \semTF{A}\cup \semTF{B}\\
\semTF{\eventual(A)} = \set{\Gamma \mid \Gamma\red^* \Delta, \Delta\in \semTF{A}}\\
\semTF{\exists x.A} = \set{\Gamma \mid \exists x.(\Gamma \in \semTF{A})}\\
\semTF{\exists \ev.A} = \set{\Gamma \mid \exists \ev.(\Gamma \in \semTF{A})}
\end{array}
\]
We write \(\Gamma\models A\) if \(\Gamma\in \semTF{A}\).
\end{defn}

\subsection{Connection between properties of processes and types}


\begin{defn}
The binary relations \(\TFtoPF\) and \(\PFtoTF\) are defined by:
\[
\begin{array}{lcl}
A \TFtoPF B \IFF \forall \Gamma, P.((\Gamma\p P \land \conTE(\Gamma))
    \imply (\Gamma \models A \imply P\models B))\\
A \PFtoTF B \IFF \forall \Gamma, P.((\Gamma\p P \land \conTE(\Gamma))
    \imply (P \models A \imply \Gamma\models B))
\end{array}
\]
\end{defn}

We can obtain the following inference rules on \(\TFtoPF\) and \(\PFtoTF\):

\paragraph{From the semantics ...}

\infrule{A\TFtoPF B}{\neg B\PFtoTF \neg A}
\infrule{A\PFtoTF B}{\neg B \TFtoPF \neg A}

and other rules from the usual logic, e.g.,
\infrule{A\PFtoTF B}{A \PFtoTF \exists y.[y/x]B}
\infrule{A\PFtoTF B \andalso x\not\in \FV(B)}
       {\exists x.A \PFtoTF B}

\infrule{A \PFtoTF B}{A \PFtoTF B\lor C}
\infrule{A \PFtoTF C}{A \PFtoTF B\lor C}
\infrule{A \PFtoTF C \andalso B\PFtoTF C}{A\lor B\PFtoTF C}
    
...

\paragraph{From the subject reduction theorem}
\infrule{A\PFtoTF B}{\PLsometr{l}A \PFtoTF \PLsometr{l}B}

\infrule{A\PFtoTF B}{\eventual(A) \PFtoTF \eventual(B)}

\paragraph{From Theorem~\ref{thm:normal-derivation}}

\infax{\PLout{x}{\ev}{n} \PFtoTF \PLout{x}{\ev}{n}}
\infax{\PLin{x}{\ev}{n} \PFtoTF \PLin{x}{\ev}{n}}
\infrule{A_1 \PFtoTF B_1\andalso A_2\PFtoTF B_2}
      {A_1\PAR A_2\PFtoTF B_1\PAR B_2}

\begin{defn}[positive/negative formulas]
The sets \(\PosF\) (\(\NegF\), resp.) of positive (negative, resp.) 
formulas are the least set 
satisfying the following rules:
\[
\begin{array}{lcl}
\PLout{x}{\ev}{n}, \PLin{x}{\ev}{n}\in \PosF\\
A \mbox{ does not contain a formula of the form }
  \PLout{x}{\ev}{n} \mbox{ or }\PLin{x}{\ev}{n} \imply {A \in \PosF\cap \NegF}\\
A, B\in \PosF \imply \PLsometr{\redlab}A, A\PAR B, A\lor B, \eventual(A),
   \exists x.A, \exists \ev.A, \exists i:C.A \in \PosF\\
A, B\in \NegF \imply \PLsometr{\redlab}A, A\PAR B, A\lor B, 
   \exists x.A, \exists \ev.A, \exists i:C.A \in \NegF\\
A \in \PosF \imply \neg A\in \NegF\\
A \in \NegF \imply \neg A\in \PosF
\end{array}
\]
\end{defn}

\begin{theorem}
If \(A\in \PosF\), then \(A\PFtoTF A\). If \(A\in \NegF\), then \(A\TFtoPF A\).
\end{theorem}
\proof %\begin{proof}
Induction on the structure of \(A\).\qed
%\end{proof}

\begin{corollary}
Let \(A\in \NegF\) and \(P\) be a closed formula.
Suppose that \(\reliable(\Gamma)\) implies \(\Gamma\p A\).
Suppose also that \(\Gamma\p P\) and \(\reliable(\Gamma)\).
Then, if \(P\red^* \nuexp{\seq{x_1}}\cdots\nuexp{\seq{x_n}}\nuexp{\seq{y}}Q\),
then \(\nuexp{\seq{x_1}}\cdots\nuexp{\seq{x_n}}Q\models A\).
\end{corollary}
\proof %\begin{proof}
From subject reduction, we have
\(\Gamma'\p \nuexp{\seq{x_1}}\cdots\nuexp{\seq{x_n}}\nuexp{\seq{y}}Q\) for
some \(\Gamma'\) such that \(\reliable(\Gamma')\) and \(\FV(\Gamma')=\emptyset\).
By the typing rules, we have
\(\Delta \p \nuexp{\seq{x_1}}\cdots\nuexp{\seq{x_n}}Q\) and \(\reliable(\Delta)\) for
some \(\Delta\). So, by the above theorem, we have 
\(\nuexp{\seq{x_1}}\cdots\nuexp{\seq{x_n}}Q \models A\).\qed
%\end{proof}
%%%\begin{itemize}
%%%\item lack of arity mismatch
%%%   \(\neg ev(\ERROR)\)
%%%\item lack of race
%%%   \(WF \land inv (\neg \exists x, \ev'.(x!^\ev.\TRUE | x!^{\ev'}.\TRUE))\)
%%%\item lack of deadlock\\
%%%  \(WF \land inv (\neg \exists x.(x!^\ev.\TRUE\land \neg \PLsometr{x^{\ev,\ev'}}\TRUE
%%%       \land \neg.\exists \ev'.(\ev'<\ev \land \PLsometr{\ev'}\TRUE)))\)
%%%\item garbage-channel collection\\
%%%  \(WF \land inv(\neg \exists x.\PLsometr{x^{\ev,\ev'}}ev(x!.\TRUE\lor x?.\TRUE))\).
%%%\end{itemize}

\subsection{Connecting process logic with type logic}

We write \({\cal A}\models A\) if \(\Gamma\p P\), \(\conTE(\Gamma)\),
and \(\Gamma\models {\cal A}\) imply \(P\models A\).

Conversely, we write \(A \models {\cal A}\) if
\(\Gamma\p P\), \(\conTE(\Gamma)\), and \(P\models A\) imply \(\Gamma\models {\cal A}\).

As corollaries, we have:
\begin{quote}
\(A \models {\cal A}\imply \neg {\cal A}  \models \neg A\)\\
\({\cal A} \models A\imply \neg A  \models \neg {\cal A}\)
\end{quote}


%%%We write \({\cal A}\models A\)
%%%if \(P\models A\)
%%% whenever (i)\(\Gamma\p P\), 
%%%(ii)\(\reliable(\Gamma)\imply \Gamma \models WF\land {\cal A}\),
%%%and (iii)\(\reliable(\Gamma)\).
%%%
%%%Conversely, we write \(A \models {\cal A}\) if
%%%
%%%\begin{quote}
%%% \(\Gamma\p P\)  and \(P\models A\) imply \(\Gamma \models {\cal A}\)
%%%\end{quote}
%%%\begin{quote}
%%%or, 
%%% \(\Gamma\p P\)  and \(P\models A\) imply 
%%%\(\Gamma\models {\cal A}\) and \(\Delta\models {\cal A}\) for any \(\Delta\)
%%%checked in the rule \rname{T-New}??
%%%\end{quote}
%%%
%%%$B!J8e<T$O$b$C$H87L)$KDj5A$G$-$J$$$+!)A0<T$b(B\({\cal A}\models A\)$B$H(B
%%%symmetric $B$G$J$$$N$G5$;}$,0-$$$7!$I=8=NO$KFq$"$j!%(B
%%%nu $B$G@8@.$5$l$k%A%c%M%k$K4X$9$k7?4D6-$r5-21$7$F$*$/$h$&$J(B
%%%\[\Gamma; S\p P\]$B$H$$$&(Btype judgment$B$rF3F~$9$l$P$h$$!)!)!K(B


Subject reduction theorem says ...

\[A \models {\cal A} \mbox{ implies } 
  \forall l.(\PLsometr{l}A \models \PLsometr{l}{\cal A})?\]

It implies

\[A \models {\cal A} \mbox{ implies } ev(A) \models ev({\cal A})\]

How to derive Theorem 3.6.2??

The following is a variant of Theorem 3.6.2: 
$B!J$?$@$7!$$3$l$ODjM}(B3.6.2$B$=$N$b$N$H$O0[$J$k!%DjM}(B3.6.2$B$G$O>r7o(Bok$B$K8@5Z$7$F$$$k$,(B
 $B2<$G$O(B\({\cal A}\)$B$H(Bok$B$OJLJ*$J$N$G!K(B
\begin{quote}
If \(inv({\cal A})\models A\), then 
\(inv({\cal A})\models inv(A)\).
$B!J(BIf \({\cal A} \models A\), then ...$B$G$b$h$$$H;W$o$l$k!K(B
\end{quote}
How to derive this?
\begin{quote}
It suffices to show \(ev(\neg A) \models ev(\neg inv({\cal A}))\).
For this to hold, it suffices to show \(\neg A \models \neg inv({\cal A})\),
which follows from \(inv({\cal A})\models A\)$B!%(B
\end{quote}

Theorem 3.6.3 says that the following inference rules are valid:
\infrule{A \models {\cal A} \andalso B \models {\cal B}}
     {A\PAR B \models {\cal A}\PAR {\cal B}}
\infax{x!.\TRUE \models x!.\TRUE}
 (\(\TRUE\)$B0J30$K$D$$$F$O!)!)(B)
\infax{x?.\TRUE \models x?.\TRUE}
 (\(\TRUE\)$B0J30$K$D$$$F$O!)!)(B)
   

Corollary 3.6.4 says:
\begin{quote}
(i)\(\Gamma \p P\) and \(P\models y?.\TRUE\) imply \(\Gamma\models y?.\TRUE\).\\
(ii)\(\Gamma \p P\) and 
\(P\models (y)y?.\TRUE\) imply \(\Gamma\models \PLsometr{\ev}\TRUE\).
\end{quote}

Theorem 3.6.5 says:
\begin{quote}
(i)\(\Gamma \p P\)  and \(\Gamma \models epsilon??^\ev.\TRUE\) imply
    \(P \models (y)y?.\TRUE\).
(ii)\(\Gamma\p P\) and \(\Gamma \models y??.\TRUE\) imply \(P\models y?.\TRUE\).\\
\end{quote}

==> revision.tex <==
\section*{$B2~Dj0F(B}

\begin{enumerate}
\item Recursive types $B$rF3F~!$<+M3JQ?t$r4^$s$@7?$K5v$9!J:Q$_!K(B
\item \rname{T-In}$B$r0lHL2=(B
\begin{verbatim}
  $B&#(B1 | $B&#(B2 |- P      $B&#(B2$B$O(By$B$r$U$/$^$J$$(B
  ---------------------------------------
   x?[(y)$B&#(B1].$B&#(B2 |- x?[y].P
\end{verbatim}
\rname{T-New}$B$O$H$j$"$($:$=$N$^$^(B
\item Sec. 3.6(subject reduction)$B$H(BSec. 6(General Type Soundness)$B$rM;9g(B
\item Type-checking/inference algorithm$B$rFHN)$N@a$K(B
\item Sec. 4(applications)$B$G!$(BGeneral type soundness$B$r$J$k$Y$/;H$&(B
\item Sec. 5(further applications)
     $B<+M3JQ?t$r4^$s$@7?$r5v$9$3$H$rMQ$$$F(BAbadi-Flangan$B$N7?%7%9%F%`$K$h$j6a$E$1$k(B
     $B!J$?$@$7(Btype soundness $B$O$3$3$^$G$N7k2L$+$i$O8@$($J$$$3$H$rCG$k!K(B
\item deadlock$B$N$?$a$N3HD%$O=|5n!J$^$H$^$C$F$$$J$$$N$G!K(B
\item Extension$B$H$7$F!$(Bnew $B$G:n$i$l$k%A%c%M%k$H$=$l0J30$N%A%c%M%k$N4X78$r%A%'%C%/$9$k(B
     $B$?$a$N3HD%$K$D$$$F!J:#$^$G$h$j>\$7$/!K8@5Z$9$k!%(B(todo$B$N(B7$B$r;2>H!K(B
     $B6qBNE*$K$O(B \(\nuexp{x:\Gamma}P\)$B$N$h$&$K!$(Bx$B$,B>$N%A%c%M%k$H$+$i$a$F$I$N$h$&$K;H$o$l$k$+$r(B
     $B@k8@2DG=$K$9$k!%(B
     $BNc$($P!$(B\(x\)$B$KAw?.$9$kA08e$K$O%m%C%/$r3MF@$9$k$N$G$"$l$P!$(B
\begin{verbatim}
    (nu x: (*l?[].x![].l![] | *x?[]))P
\end{verbatim} 
reply$B$,JV$C$F$+$i2rJ|$9$k$N$G$"$l$P(B
\begin{verbatim}
    (nu x: (*l?[].x![(r)r![()l![]]] | *x?[]))P
\end{verbatim} 
     reduction$B$O<!$N$h$&$KDj5A(B
\begin{verbatim}
              x                    x
         P  -----> Q    $B"O&$(B'.($B&#(B ----->$B&$(B' ==> $B&$(B<$B&$(B')
        ------------------------------------------------
         (nu x:$B&#(B)P ---> (nu x:$B&$(B)Q

              y^t                                       L
         P  -----> Q    $B"O&$(B'.$B"O(BL (\subseteq{y,t}).($B&#(B ----->$B&$(B' ==> $B&$(B<$B&$(B')
        --------------------------------------------------------------------
         (nu x:$B&#(B)P ---> (nu x:$B&$(B)Q

      $B$3$N>l9g!$&M$N5,B'$O<!$N$h$&$KJQ99(B

              $B&#(B |- P     ok($B&$(B, x)
            $B&$(B|$B&$(B'<$B&#(B     FV($B&$(B')\cap {x,y}=\emptyset $B!J?7$7$$4X78$H$7$F$^$H$a$k!)!K(B
         ------------------------------------------------------------------------
           $B&#",(Bx |- (nu x:<y,$B&$(B>)P
\end{verbatim}
\end{enumerate}




==> todo.tex <==
\begin{verbatim}
- Generic Type System$B$N%8%c!<%J%kHG(B

  $B3HD%0F(B

  A: $B85$N$b$N$=$N$^$^(B
  B: 1 + 3 + 6 + (10 + 11)
  C: B + 4
  D: C + 5
  E: D+7
  F: E+8

    1. free variables$B$K4X$9$k@)8B$NE15n(B:        done
        $BMxE@!'(BAbadi-Flanagan$B!$(BGordon-Jeffery
              $B$H$N4X78$,$h$jL@$i$+$K(B?

         5$B@a$N(Bobject $B$N(Bencoding$B$b$h$j<+A3$J(Bencoding$B$,;H$($k(B?
         Interface $B$N7?$r(B
           (l,m)*l?[].m![(s,r)(s:String|r![()l![]].l![])].l![]
         $B$H$9$l$P$h$$(B

    2. Petri net$B$X$N3HD%(B:                       $B8+Aw$j(B
       $B7?$r(BCCS$B$G$O$J$/(BPetri net$B$rMQ$$$FI=$9(B

    3. recursive type:                          done

    4. Table 1,2$B$N>r7o$N=q$-D>$7(B:               ??
       $BMxE@!'0lIt$N>r7o$,8+0W$/$J$k(B
       $B7gE@!'(Bdeadlock $B$N>r7o$r5-=R$9$k$?$a$K(B
             $B?7$7$$(Bformula$B$NF3F~$NI,MW$"$j!%(B
             $B%W%m%;%9$N@-<A$rI=$9<0$H(B
             $B7?$N@-<A$rI=$9<0$rJ,N%$9$kI,MW$"$j(B

    5. ok $B$H$7$FITJQ>r7o0J30$b5v$9(B              ??
       $B!u3F%A%c%M%k$4$H$K;H$o$lJ}$rJQ2=(B

       $B6qBNE*$K$O(B...

       - (nu x:A)P $B$N$h$&$K(Bannotation$B$rIU2C(B
       - reduction $B$r<!$N$h$&$KJQ99(B

              x           x
         P  -----> Q    A--->B
        ----------------------------
         (nu x:A)P ---> (nu x:B)Q
                l
       $B$?$@$7(B A------->B$B$O!$(B
       for all G, D, 
                     l
         G|=A /\  G---->D  ===> D|=B

       $B$^$?$O(B

       for all P, Q
                     l
         P|=A /\  P---->Q  ===> Q|=B

       $B$N$h$&$KDj5A$9$k!%(B
      $B!JN><T$OF1CM!)$@$H$7$?$i$I$&$d$C$F<($9!)!K(B

       $BMxE@!'ITJQ>r7o0J30$b07$($k$h$&$K$J$k(B
            $B!JNc!'(Bx!$B$NA0$K$OI,$:(By$B$K4X$9$kDL?.$,(B
                 $B$*$3$C$F$$$?!K(B

       $B7gE@!'(Bdeadlock$B$N>l9g$K$&$^$/E,MQ$G$-$J$$$N$G(B
             6$B@a$@$1$N$?$a$K(Breduction rule$B$*$h$S(B
             $B7?IU$15,B'$r:FDj5A$9$k$3$H$K$J$k!%(B

    6. modal logic $B$K(Bfixpoint operator$B$rF3F~(B:   to be done

    7. $B%A%c%M%k@8@.$N5,B'$N>r7o(Bok(G$B"-(Bx)$B$r(B:      ??
       G|=A $B$N7A$KJQ$($k(B

       5$B$N3HD%$OI,A3!J$=$&$G$J$$$H0UL#$,$J$$!K(B
       scope extrusion $B$,$"$k$?$a!$(B
       8$B$N3HD%$r$9$k$+!$(BA$B$N>r7o$H$7$F(B
       $B&#(B|=A /\ x\not\in FV($B&$(B) => $B&#(B|$B&$(B|=A
       $B!J8=>u$N(Bok$B$N(B3$BHVL\$N>r7o$KAjEv!K(B
       $B$rDI2C$9$kI,MQ$"$j(B
       $B!J$3$N>r7o$rDI2C$7$F$b0UL#$,$"$k!)!)(B
        ---> $B0UL#$,$"$k$3$H$O$"$k(B
         $B!V(Bx$B$KAw?.$,$*$3$kA0$K$OI,$:(By$B$K4X$9$kDL?.$,$*$3$C$F$$$k!W(B
         $B$OI=8=2DG=!K(B

       $BMxE@!'F1;~$K%A%c%M%k$r:n$i$J$/$F$b!$(B
             $B%A%c%M%k4V$N4X78$r%A%'%C%/$G$-$k(B

       $B$"$k$$$O!$(B

       - (nu x:$B&#(B)P $B$N$h$&$K(Bannotation$B$rIU2C(B
               ^^
       - reduction $B$r<!$N$h$&$KJQ99(B

              x                    x
         P  -----> Q    $B"O&$(B'.($B&#(B ----->$B&$(B' ==> $B&$(B<$B&$(B')
        ------------------------------------------------
         (nu x:$B&#(B)P ---> (nu x:$B&$(B)Q

              y^t                                       L
         P  -----> Q    $B"O&$(B'.$B"O(BL (\subseteq{y,t}).($B&#(B ----->$B&$(B' ==> $B&$(B<$B&$(B')
        --------------------------------------------------------------------
         (nu x:$B&#(B)P ---> (nu x:$B&$(B)Q


      $B$3$N>l9g!$&M$N5,B'$O<!$N$h$&$KJQ99(B

              $B&#(B |- P     ok($B&$(B, x)
            $B&$(B|$B&$(B'<$B&#(B     FV($B&$(B')\cap {x,y}=\emptyset $B!J?7$7$$4X78$H$7$F$^$H$a$k!)!K(B
         ------------------------------------------------------------------------
           $B&#",(Bx |- (nu x:<y,$B&$(B>)P

        $B>e$N5,B'$J$i(B $B&#(B |- (nu x:$B&$(B)P | Q ===>$B&#(B |- (nu x:$B&$(B)(P | Q)$B$O#O#K(B

           $B$$$:$l$K$7$F$b(B
               l?[].t.x![].l![]
           $B$H$J$C$?$H$-$K!$(Bl$B$,@5$7$/%m%C%/$5$l$F$$$kJ]>Z$,$J$$(B...$B!J(Bt$B$,(Bl![]$B$+$b$7$l$J$$$N$G!K(B
           $B&#(B1 * $B&#(B2 = $B&#(B $B$NJ,3d$O!$(B
           $B&#(B1$B",(BS * $B&#(B2$B"-(BS = $B&#(B $B$7$+5v$5$J$$$h$&$K$9$l$P$h$$!)(B
            l$B$,@5$7$/%m%C%/$H$7$FMQ$$$i$l$F$$$k$3$H$r8!::$9$l$P==J,!)(B
                 $B!JNc$($P(Bl?[].l![].x!.l?[].l![]$B$rJ,3d$9$k$H(Bl?[].t.x!.t.l![] | l![].l?[] $B$H$J$j!$(B
                   $B@5$7$$%m%C%/$N;HMQK!$K$J$i$J$$!K(B
       
    8. modal logic $B$K(Bspatial implication$B$rF3F~!'(B  ??

        $B&#(B -o A

       $B&#$rK~$?$9%W%m%;%9$HJB9T$KAv$l$P(BA$B$rK~$?$9!%(B
      (P |= $B&#(B -o A
       <=>
       $B"O(BQ.($B&#(B|-Q => P|Q |= A))

       (nu x:($B&#(B1|$B&#(B2) -o A)P | Q < (nu x:$B&#(B1 -o A)(P |Q)
           (if $B&#(B2|- Q)
     
           $B&#(B |- P    $B&$(B|$B&#"-(Bx |= A
          -----------------------------
           $B&#(B\x |- (nu x:$B&$(B-o A)P
          
       $B>e$N5,B'$G$O30B&$N%W%m%;%9$,&$$K$7$?$,$C$F$U$k$^$&(B
       $B$H$$$&J]>Z$,$J$$!%$=$3$G7?H=Dj$r(B

          $B&#(B |- P: $B&$(B
         
          $B&#$OJB9T$9$k%W%m%;%9$,&#$K$7$?$,$J$1$l$P$J$i$J$$$3$H$r(B 
          $B&$$O(BP$B<+?H$,&$$K$7$?$,$C$F$U$k$^$&$3$H$rI=$9(B

        $B$N$h$&$K3HD%$7(B

           $B&$(B |- P: $B&#(B    $B&$(B|$B&#"-(Bx |= A
          -----------------------------
           $B&$(B |- (nu x:$B&$(B-o A)P: $B&#(B\x

            $B&#(B|$B&$(B2 |- P1:$B&$(B1             $B&#(B|$B&$(B1 |- P2:$B&$(B2
          -------------------------------------------------
              $B&#(B |- P1|P2 : $B&$(B1|$B&$(B2

         $B$N$h$&$K7?IU$15,B'$rJQ99$7$?J}$,$h$$!)(B

      9. $B7?$H(Bmodal logic$B$N<0$rF10l;k$9$k(B:       ??

          A ::= $B&#(B | ...

         $B$N$h$&$KO@M}<0$K7?$rDI2C$7$F(B

          $B&#(B |= $B&$(B <=>  $B&$(B < $B&#(B
          P |= $B&$(B <=>  $B&$(B |- P

        $B$H$9$k$H(B
          $B&#(B |= $B&$(B /\ $B&#(B|- P => P |= $B&$(B
        $B$,@.$jN)$D!%(B
        
        $B5U$KO@M}<0$r7?$H$7$F07$&$H(B

           A|- P     B |- Q
         ---------------------
           A|B |- P|Q

         $B$N$h$&$J7?IU$15,B'$,$G$-$k!%(B
         $B&#"-(Bx, $B&#",(Bx $B$N$h$&$JA`:n$K$+$($F(B

          A$B"-(Bx B <=> $B"O&#(B.($B&#(B|=A => $B&#"-(Bx|= B)
        $B$N$h$&$KDj5A$9$k$3$H$K$9$k$H(B
           A |- P    A$B",(Bx B   A$B"-(Bx C
         ----------------------------
           B|= (nu x:C)P
        $B$N$h$&$J5,B'$,$G$-$k!)(B

     10. $BB?Aj7?$NF3F~(B:                  $B35MW$N$_=q$/(B

        $BB?Aj7?$rF3F~$9$k$H!$(BIf $B$r(Bchoice$B$r;H$o$J$$$G(Bencode $B$G$-$k(B

            Bool == ($B&A(B,$B&B(B;x, y)(x![$B&A(B].$B&A(B<> & y![$B&B(B].$B&B(B<>)

         $B$H$*$1$P(B
              true?[Bool] |- true?[x, y].x![]
              false?[Bool] |- true?[x, y].y![]

                 $B&#(B|- P         $B&$(B|- P
             ----------------------------------------------------------------------
             b![Bool].(x![()$B&#(B].$B&#(B&x![()$B&$(B].$B&$(B)|x?[()$B&#(B]|y?[()$B&$(B]|- b![x,y] | x?[].P | y?[].Q
             -------------------------------------------------------------------------------
             b![Bool].(t.$B&#(B& t.$B&$(B)| t | t |- (nu x, y)(b![x,y] | x?[].P | y?[].Q)

     11. first-class labels$B!'(B           $B=q$/$H$7$F$b35MW$N$_(B
         - new $B$G%A%c%M%k@8@.$@$1$G$J$/%i%Y%k@8@.$b$G$-$k$h$&$K$9$k(B
         - !, ?$B$N%i%Y%k$H$7$F(Bterm $B$r5v$9!%(B

         $BMxE@!'(BGordon-Jeffery$B$N(Bcorrespondence assertion$B$,$[$\D>@\I=8=$G$-$k(B

          begin{a,b,c}  ---> begin!^(a,b,c)[]

\end{verbatim}

